On Affinely Homogeneous Submanifolds: The Power Series Method of Equivalence

We determine all affinely homogeneous models for surfaces $S^2 \subset \mathbb{R}^4$, including the simply transitive models. We employ an improved power series method of equivalence, which captures invariants at the origin, creates branches, and infinitesimalizes calculations. We find several inequivalent terminal branches yielding each to some nonempty moduli space of homogeneous models, sometimes parametrized by a certain invariant algebraic variety. Three main features may be emphasized: 1) Iterated single-pointed jet bundles; 2) Cartan-enhanced power series method of equivalence; 3) Constant ping-pong between normal forms (nf) and vector fields (vf).

==> references.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{thebibliography}{XL}

{\scriptsize

{\bf\bibitem{Abdalla-Dillen-Vrancken-1997}
{\rm Abdalla}}, B.; {\rm Dillen}, F.; {\rm Vrancken}, L.:
{\em Affine homogeneous surfaces in $\R^3$ 
with vanishing Pick invariant},
Abh. Math. Sem. Univ. Hamburg {\bf 67} (1997), 105–115.

\smallskip

{\bf\bibitem{Arnaldsson-Valiquette-2020}
{\rm Arnaldsson}}, \"O; {\rm Valiquette}, F.:
{\em Invariants of surfaces in three-dimensional affine geometry},
{\tiny\sf arxiv.org/abs/2009.00670/},
Symmetry, Integrability and Geometry: 
Methods and Applications {\bf 17} (2021), 033, 25 pages.

\smallskip

{\bf\bibitem{Bluman-Kumei-1989}
{\rm Bluman}}, G.W.; {\em Kumei}, S.:
{\em Symmetries and differential equations},
Springer-Verlag, Berlin, 1989, xiv+412~pp.

\smallskip

{\bf\bibitem{Cartan-1937}
{\rm Cartan}}, \'E.:
{\em Les probl\`emes d'\'equivalence},
S\'eminaire de Math\'ematiques (Julia), 
tome 4 (1936--1937), 
exp. no.~4, pp.~1--40.

\smallskip

{\bf\bibitem{Chen-Merker-2019}
{\rm Chen}}, Z.; {\rm Merker}, J.:
{\em On differential invariants of parabolic surfaces},
Dissertationes Mathematic{\ae} {\bf 559}, 2021, 
doi: 10.4064/dm816-8-2020, 110 pages,
{\tiny\sf arxiv.org/abs/1908.07867/}

\smallskip

{\bf\bibitem{Chen-Merker-2020}
{\rm Chen}}, Z.; {\rm Merker}, J.:
{\em Affine homogeneous surfaces with Hessian rank 2
and algebras of differential invariants},
{\tiny\sf arxiv.org/abs/2010.02873/}, 20 pages.

\smallskip

{\bf\bibitem{Dieudonne-1964}
{\rm Dieudonn\'e}}, J.:
{\em Alg\`ebre lin\'eaire et g\'eom\'etrie \'el\'ementaire},
Hermann, Paris, 1964, 240~pp.

\smallskip

{\bf\bibitem{Doubrov-Govorov-2013}
{\rm Doubrov}}, B.; {\rm Govorov}, A.:
{\em Classification of generic 2-distributions
on 5-manifolds with transitive symmetry}, 
7 pages.

\smallskip

{\bf\bibitem{Doubrov-Komrakov-1998}
{\rm Doubrov}}, B.; {\rm Komrakov}, B.:
{\em Classification of homogeneous submanifolds 
in homogeneous spaces},
Towards 100 years after Sophus Lie (Kazan, 1998),
Lobachevskii J. Math. {\bf 3} (1999), 19--38.

\smallskip

{\bf\bibitem{Doubrov-Komrakov-Rabinovich-1996}
{\rm Doubrov}}, B.; {\rm Komrakov}, B.; {\rm Rabinovich}, M.: 
{\em Homogeneous surfaces in the three-dimensional affine geometry}. 
Geometry and topology of submanifolds, 
VIII (Brussels, 1995/Nordfjordeid, 1995), 
168--178, World Sci. Publ., River Edge, NJ, 1996.

\smallskip

{\bf\bibitem{Doubrov-Medvedev-The-2019} 
{\rm Doubrov}}, B.; {\rm Medvedev}, A.; {\rm The}, D.:
{\em Homogeneous integrable Legendrian contact structures 
in dimension five},
J. Geom. Analysis {\bf 30} (2020), no.~4, 3806--3858.

\smallskip

{\bf\bibitem{Doubrov-Medvedev-The-2020} 
{\rm Doubrov}}, B.; {\rm Medvedev}, A.; {\rm The}, D.:
{\em Homogeneous Levi non-degenerate hypersurfaces in $\C^3$}, 
Math. Z. {\bf 297} (2021), no.~1-2, 669--709.

\smallskip

{\bf\bibitem{Doubrov-Merker-The-2020} 
{\rm Doubrov}}, B.; {\rm Merker}, J.; The, D.:
{\em Classification of simply-transitive Levi non-degenerate 
hypersurfaces in $\C^3$},
Int. Math. Res. Not. IMRN 2022, no. 19, 15421--15473.

\smallskip

{\bf\bibitem{Eastwood-Ezhov-1999}
{\rm Eastwood}}, M.; {\rm Ezhov}, V.:
{\em On affine normal forms and a classification 
of homogeneous surfaces in affine three-space}, 
Geom. Dedicata {\bf 77} (1999), no.~1, 11--69.

\smallskip

{\bf\bibitem{Eastwood-Ezhov-2001-1} 
{\rm Eastwood}}, M.; {\rm Ezhov}, V.:
{\em Homogeneous hypersurfaces with isotropy in affine four-space},
Proc. Steklov Inst. Math. {\bf 235} (2001), no.~4, 49--63.

\smallskip

{\bf\bibitem{Eastwood-Ezhov-2001-2} 
{\rm Eastwood}}, M.; {\rm Ezhov}, V.:
{\em A classification of non-degenerate homogeneous 
equiaffine hypersurfaces in four complex dimensions}, 
Asian J. Math. {\bf 5} (2001), no. 4, 721--739.

\smallskip

{\bf \bibitem{Engel-Lie-Merker-2015}
{\rm Engel}}, F. and {\rm Lie}, S. (Authors), 
{\rm Merker}, J. (Editor):
{\em Theory of Transformation Groups I. 
General Properties of Continuous Transformation Groups. 
A Contemporary Approach and Translation.}
Springer-Verlag, Berlin, Heidelberg, 2015, xv+643~pp.

\smallskip

{\bf\bibitem{Engel-Lie-1893}
{\rm Engel}}, F., {\rm Lie}, S.:
{\em Theorie der transformationsgruppen. Dritter und
letzter Abschnitt.} 
Unter
Mitwirkung von Dr. Friedrich {\sf Engel}, bearbeitet von Sophus {\sf
Lie}, Verlag und Druck von B.G. Teubner, Leipzig und Berlin, 
xxix+836~pp. (1890). Reprinted by Chelsea Publishing Co., 
New York, N.Y. (1970)

\smallskip

{\bf\bibitem{Fels-Olver-1999}
{\rm Fels}}, M.; {\rm Olver}, P.J.:
{\em Moving coframes. II. Regularization and theoretical 
foundations}, Acta Appl. Math. {\bf 55} (1999), no.~2, 127--208.

\smallskip

{\bf\bibitem{Foo-Merker-2019}
{\rm Foo}}, W.G., {\rm Merker}, J.:
{\em Differential $\{e\}$-structures for equivalences
of $2$-nondegenerate Levi rank $1$ hypersurfaces $M^5 \subset \C^3$},
Constr. Math. Anal. {\bf 4} (2021), no.~3, 318--377.

\smallskip

{\bf\bibitem{Foo-Merker-Nurowski-Ta-2021} 
{\rm Foo}}, W.G.; {\rm Merker}, J.; {\rm Nurowski}, P.; 
{\rm Ta}, T.A.:
{\em Homogeneous $\mathfrak{C}_{2,1}$ models},
{\tiny\sf arxiv.org/abs/2104.09608/}, 13 pages.

\smallskip

{\bf\bibitem{Foo-Merker-Ta-2019}
{\rm Foo}}, W.G., {\rm Merker}, J., {\rm Ta}, T.-A.:
{\em Rigid equivalences of $5$-dimensional $2$-nondegenerate
rigid real hypersurfaces $M^{5}\subset\mathbb{C}^{3}$ 
of constant Levi rank $1$}, 
Michigan Mathematical Journal Advance Publication (Jan 2021), 
doi:10.1307/mmj/20205950.

\smallskip

{\bf\bibitem{Foo-Merker-Ta-2020}
{\rm Foo}}, W.G., {\rm Merker}, J., {\rm Ta}, T.-A.:
{\em On convergent Poincar\'e-Moser reduction
for Levi degenerate embedded $5$-dimensional CR manifolds},
New York J. Math. {\bf 28} (2022), 250--336.

\smallskip

{\bf\bibitem{Godlinski-2008} 
{\rm Godlinski}}, M.: 
{\em Geometry of third-order ordinary differential equations 
and its applications in General Relativity},
{\tiny\sf arxiv.org/abs/0810.2234/}, 2008, 80 pages.

\smallskip

{\bf\bibitem{Godlinski-Nurowski-2009} 
{\rm Godlinski}}, M.; Nurowski, P.: 
{\em Geometry of third order ODEs}
{\tiny\sf arxiv.org/abs/0902.4129/}, 2009, 45 pages.

\smallskip

{\bf\bibitem{Guggenheimer-1963}
{\rm Guggenheimer}}, H.W.:
{\em Differential Geometry}, 
Corrected reprint of the 1963 edition. 
Dover Books on Advanced Mathematics. 
Dover Publications, Inc., New York, 1977, x+378~pp.

\smallskip

{\bf\bibitem{Heyd-Merker-2023}
{\rm Heyd}}, J.; {\rm Merker}, J.: 
{\em Computation files}, 
{\tiny\sf www.imo.universite-paris-saclay.fr/$\sim$joel.merker/}, 
\href{https://www.imo.universite-paris-saclay.fr/~joel.merker/2-3-4-Hrank-1.zip}{{\tiny\sf 2-3-4-Hrank-1.zip}}, 
\href{https://www.imo.universite-paris-saclay.fr/~joel.merker/3S-R4.zip}{{\tiny\sf 3S-R4.zip}},
\href{https://www.imo.universite-paris-saclay.fr/~joel.merker/S2-R4.zip}{{\tiny\sf S2-R4.zip}}.

\smallskip

{\bf\bibitem{Hubert-Olver-2007}
{\rm Hubert}}, E.; {\rm Olver}, P.:
{\em Differential invariants of conformal and projective surfaces}, 
SIGMA Symmetry Integrability Geom. Methods Appl. {\bf 3} (2007), 
Paper 097, 15~pp.

\smallskip

{\bf\bibitem{Jensen-1977}
{\rm Jensen}}, G.:
{\em Higher order contact of submanifolds of homogeneous spaces}, 
Lecture Notes in Mathematics, Vol. 610. 
Springer-Verlag, Berlin-New York, 1977, xii+154~pp.

\smallskip

{\bf\bibitem{Kogan-2000}
{\rm Kogan}}, I.:
{\em Inductive construction of moving frames}, 
The geometrical study of differential equations 
(Washington, DC, 2000), 157--170, Contemp. Math., 285, 
Amer. Math. Soc., Providence, RI, 2001.

\smallskip

{\bf\bibitem{Kogan-2003}
{\rm Kogan}}, I.:
{\em Two algorithms for a moving frame construction},
Canad. J. Math. {\bf 55} (2003), no.~2, 266--291.

\smallskip

{\bf\bibitem{Lagrange-1797}
{\rm Lagrange}}, J.-L.:
{\em Théorie des fonctions analytiques, contenant les principes
du calcul différentiel}, 
Imprimerie de la république, 
Paris, Prairial An V, 1797, viii+276~pp.

\smallskip

{\bf\bibitem{Loboda-2020} 
{\rm Loboda}}, A.V.:
{\em Holomorphically Homogeneous Real Hypersurfaces in $\C^3$},
Trans. Moscow Math. Soc. {\bf 81} (2020), 169--228.

\smallskip

{\bf\bibitem{Merker-2008}
{\rm Merker}}, J.:
{\em Lie symmetries of partial differential equations 
and CR geometry}, 
Journal of Mathematical Sciences (N.Y.), {\bf 154} (2008), 817--922.

\smallskip

{\bf\bibitem{Merker-2020}
{\rm Merker}}, J.:
{\em A Lie-theoretic construction of Cartan-Moser chains},
J. Lie Theory {\bf 31} (2021) 1--34.

%%%\smallskip

%%%{\bf\bibitem{Merker-2021}
%%%{\rm Merker}}, J.:
%%%{\em Equivalences of PDE systems associated to 
%%%degenerate para-CR structures: foundational aspects},
%%%Partial Differ. Equ. Appl. {\bf 3} (2022), no.1, Paper No.~4, 57~pp.
%%%doi.org/10.1007/s42985-021-00138-z.

\smallskip

{\bf\bibitem{Merker-2022}
{\rm Merker}}, J.:
{\em Inexistence of non-product Hessian rank 1
affinely homogeneous hypersurfaces $H^n \subset \R^{n+1}$
in dimension $n \geqslant 5$},
Ufa Math. J. {\bf 15} (2023), no.~1, 56--121. 

\smallskip

{\bf\bibitem{Merker-Nurowski-2020-a}
{\rm Merker}}, J., {\rm Nurowski}, P.:
{\em On degenerate para-CR structures:
Cartan reduction and homogeneous models}, 
{\tiny\sf arxiv.org/abs/2003.08166/}, 37 pages,
Transformation Groups, 2023,
DOI: 10.1007/s00031-022-09746-4.

%%%\smallskip

%%%{\bf\bibitem{Merker-Nurowski-2020-b}
%%%{\rm Merker}}, J., {\rm Nurowski}, P.:
%%%{\em Five-dimensional para-CR manifolds and contact projective
%%%geometry in dimension three},
%%%Ann. Sc. Norm. Super. Pisa Cl. Sci. (5) {\bf 24} (2023), no.~1, 
%%%519--549.

\smallskip

{\bf\bibitem{Merker-Nurowski-2023}
{\rm Merker}}, J.; {\rm Nurowski}, P.:
{\em Homogeneous CR and para-CR structures in dimensions 5 and 3},
J. Geom. Anal. {\bf 34} (2023), Article No.~27, 50~pp.
DOI: 10.1007/s12220-023-01461-0

\smallskip

{\bf\bibitem{Merker-Pocchiola-2018}
{\rm Merker}}, J., {\rm Pocchiola}, S.:
Explicit absolute parallelism for $2$-nondegenerate real
hypersurfaces $M^5 \subset \C^3$ of constant Levi rank $1$.
Journal of Geometric Analysis, {\bf 30} (2020),
2689--2730, {\tiny\sf 10.1007/s12220-018-9988-3}.
Addendum: 3233--3242,
{\tiny\sf 10.1007/s12220-019-00195-2}.

\smallskip

{\bf\bibitem{Mozhei-2000}
{\rm Mozhei}}, N.P.:
{\em Homogeneous submanifolds 
in four-dimensional affine and projective
geometry}, 
Izv. Vyssh. Uchebn. Zaved. Mat. {\bf 7} (2000), 41--52.

\smallskip

{\bf\bibitem{Olver-1986}
{\rm Olver}}, P.J.:
{\em Applications of Lie groups to differential equations}, 
Graduate Texts in Mathematics, 107, 
Springer-Verlag, New York, 1986. xxvi+497~pp.

\smallskip

{\bf\bibitem{Olver-1995}
{\rm Olver}}, P.J.:
{\em Equivalence, Invariants, and Symmetry}, 
Cambridge, Cambridge University Press, 1995, xvi+525~pp.

\smallskip

{\bf\bibitem{Olver-1999}
{\rm Olver}}, P.J.:
{\em Classical invariant theory},
London Mathematical Society Student Texts, 44. 
Cambridge University Press, Cambridge, 1999. xxii+280~pp.

\smallskip

{\bf\bibitem{Olver-2007}
{\rm Olver}}, P.J.:
{\em Differential invariants of surfaces},
Differential Geom. Appl. {\bf 27} (2007), no.~2, 230--239. 

\smallskip

{\bf\bibitem{Olver-2007b}
{\rm Olver}}, P.J.:
{\em Generating differential invariants}, 
J. Math. Anal. Appl. {\bf 333} (2007), no.~1, 450–471.

\smallskip

{\bf\bibitem{Olver-2011}
{\rm Olver}}, P.J.:
{\em Recursive moving frames},
Results Math. {\bf 60} (2011), no.~1-4,423--452.

\smallskip

{\bf\bibitem{Olver-2018}
{\rm Olver}}, P.J.:
{\em Normal forms for submanifolds under group actions},
Symmetries, differential equations and applications, 1--25.
Springer Proc. Math. Stat. {\bf 266}, Springer, Cham, 2018.

\smallskip

{\bf\bibitem{Olver-Sabzevari-Valiquette-2023}
{\rm Olver}}, P.J.; {\rm Sabzevari}, M.; {\rm Valiquette}, F.:
{\em Normal forms, moving frames, and differential invariants
for nondegenerate hypersurfaces in $\C^2$},
J. Geom. Anal. {\bf 33} (2023), no.~6, 
Paper No.~192, 46~pp.

\smallskip

{\bf\bibitem{Olver-Valiquette-2018}
{\rm Olver}}, P.J.; {\rm Valiquette}, F.:
{\em Recursive moving frames for Lie pseudo-groups},
Results Math. {\bf 73} (2018), no.~2, Paper No.~57, 64~pp.

\smallskip

{\bf\bibitem{Snobl-Winternitz-2014}
{\rm Šnobl}}, L.; {\rm Winternitz}, P.:
{\em Classification and identification of Lie algebras},
CRM Monograph Series, 33, American Mathematical Society, 
Providence, RI, 2014. xii+306 pp.

\smallskip

{\bf\bibitem{The-2022}
{\rm The}}, D.:
{\em A Cartan-theoretic classification of multiply-transitive
(2,3,5)-distributions}, 
{\tiny\sf arxiv.org/abs/2205.03387/}, 28~pages.

\smallskip

{\bf\bibitem{Tresse-1893}
{\rm Tresse}}, A.:
{\em Sur les invariants différentiels des groupes continus 
de transformations},
Acta Math. {\bf 18} (1893), 1--88.

\smallskip

{\bf\bibitem{Valiquette-2013}
{\rm Valiquette}}, F.:
{\em Inductive moving frames},
Results Math. {\bf 64} (2013), no.~1-2, 37--58.

\smallskip

{\bf\bibitem{Wermann-2001}
{\rm Wermann}}, M.:
{\em Homogene Hyperfl\"achen im
vierdimensionalen \"aqui-affinen Raum},
Dortmund, Univ., Diss., 2001,
Shaker Verlag, Aachen, 2001.

}\end{thebibliography}


==> resultats.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\input preamble-resultats.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SectionHead{2b Models}
{2b-models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3a4a}\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\partial_x+2\,x\,\partial_u, &
e_2
\,:=\,
\partial_y, &
& 
\\
e_3
\,:=\,
x\,\partial_x+2\,u\,\partial_u, &
e_4
\,:=\,
x\,\partial_y, &
e_5
\,:=\,
y\,\partial_y, &
e_6
\,:=\,
v\,\partial_x,
\\
e_7
\,:=\,
u\,\partial_y, &
e_8
\,:=\,
v\,\partial_y, &
e_9
\,:=\,
v\,\partial_u, &
e_{10}
\,:=\,
v\,\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7 & e_8 & e_9 & e_{10}
\\
\hline
e_1 & 
0 & 0 & e_1 & e_2 & 0 & -\,2\,e_9 & 2\,e_4 & 0 & 0 & 0
\\
e_2 &
0 & 0 & 0 & 0 & e_2 & 0 & 0 & 0 & 0 & 0
\\
e_3 &
-\,e_1 & 0 & 0 & e_4 & 0 & -\,e_6 & 2\,e_7 & 0 & -\,2\,e_9 & 0
\\
e_4 &
-\,e_2 & 0 & -\,e_4 & 0 & e_4 & -\,e_8 & 0 & 0 & 0 & 0
\\
e_5 &
0 & -\,e_2 & 0 & -\,e_4 & 0 & 0 & -\,e_7 & -\,e_8 & 0 & 0
\\
e_6 &
2\,e_9 & 0 & e_6 & e_8 & 0 & 0 & 0 & 0 & 0 & -\,e_6
\\
e_7 &
-\,2\,e_4 & 0 & -\,2\,e_7 & 0 & e_7 & 0 & 0 & 0 & -\,e_8 & 0
\\
e_8 &
0 & 0 & 0 & 0 & e_8 & 0 & 0 & 0 & 0 & -\,e_8
\\
e_9 &
0 & 0 & 2\,e_9 & 0 & 0 & 0 & e_8 & 0 & 0 & -\,e_9
\\
e_{10} &
0 & 0 & 0 & 0 & 0 & e_6 & 0 & e_8 & e_9 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3a4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^4+F_{5,0}\,x^5
+
\big(
2+\tfrac{5}{4}\,F_{5,0}^2
\big)\,x^6
+
\big(
\tfrac{34}{7}\,F_{5,0}
+
\tfrac{25}{14}\,F_{5,0}^3
\big)\,x^7
+\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\big(1-\tfrac{5}{2}\,F_{5,0}\,x+2\,u\big)\,\partial_x
+
\big(2\,x-5\,F_{5,0}\,u\big)\,\partial_u, &
e_2
\,:=\,
\partial_y, & 
\\
e_3
\,:=\,
x\,\partial_y, &
e_4
\,:=\,
y\,\partial_y, &
e_5
\,:=\,
v\,\partial_x, &
e_6
\,:=\,
u\,\partial_y,
\\
e_7
\,:=\,
v\,\partial_y, &
e_8
\,:=\,
v\,\partial_u, &
e_9
\,:=\,
v\,\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\tiny
\def\arraystretch{1.25}
\begin{array}{c|ccccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7 & e_8 & e_9 
\\
\hline
e_1 & 
0 & 0 & e_2-\frac{5}{2}\,F_{5,0}\,e_3-2\,e_6 & 0 & 
\frac{5}{2}\,F_{5,0}\,e_5-2\,e_8 & 2\,e_3-5\,F_{5,0}\,e_6 &
0 & 2\,e_5+5\,F_{5,0}\,e_8 & 0
\\
e_2 &
0 & 0 & 0 & e_2 & 0 & 0 & 0 & 0 & 0 
\\
e_3 &
-\,e_2+\frac{5}{2}\,F_{5,0}\,e_3+2\,e_6 & 0 & 0 & e_3 & 
-\,e_7 & 0 & 0 & 0 & 0 
\\
e_4 &
0 & -\,e_2 & -\,e_3 & 0 & 0 & -\,e_6 & -\,e_7 & 0 & 0 
\\
e_5 &
-\,\frac{5}{2}\,F_{5,0}\,e_5+2\,e_8 & 0 & e_7 & 0 & 0 & 0 & 0 &
0 & -\,e_5
\\
e_6 &
-\,2\,e_3+5\,F_{5,0}\,e_6 & 0 & 0 & e_6 & 0 & 0 & 0 & -\,e_7 & 0
\\
e_7 &
0 & 0 & 0 & e_7 & 0 & 0 & 0 & 0 & -\,e_7
\\
e_8 &
-\,2\,e_5-5\,F_{5,0}\,e_8 & 0 & 0 & 0 & 0 & e_7 & 0 & 0 & -\,e_8
\\
e_9 &
0 & 0 & 0 & 0 & e_5 & 0 & e_7 & e_8 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3a4c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2-x^4+F_{5,0}\,x^5
+
\big(
2-\tfrac{5}{4}\,F_{5,0}^2
\big)\,x^6
+
\big(
-\,\tfrac{34}{7}\,F_{5,0}
+
\tfrac{25}{14}\,F_{5,0}^3
\big)\,x^7
+\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
for any value of $F_{5,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\big(1+\tfrac{5}{2}\,F_{5,0}\,x+2\,u\big)\,\partial_x
+
\big(2\,x+5\,F_{5,0}\,u\big)\,\partial_u, &
e_2
\,:=\,
\partial_y, & 
\\
e_3
\,:=\,
x\,\partial_y, &
e_4
\,:=\,
y\,\partial_y, &
e_5
\,:=\,
v\,\partial_x, &
e_6
\,:=\,
u\,\partial_y,
\\
e_7
\,:=\,
v\,\partial_y, &
e_8
\,:=\,
v\,\partial_u, &
e_9
\,:=\,
v\,\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\tiny
\def\arraystretch{1.25}
\begin{array}{c|ccccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7 & e_8 & e_9 
\\
\hline
e_1 & 
0 & 0 & e_2+\frac{5}{2}\,F_{5,0}\,e_3+2\,e_6 & 0 & 
-\,\frac{5}{2}\,F_{5,0}\,e_5-2\,e_8 & 2\,e_3+5\,F_{5,0}\,e_6 &
0 & -\,2\,e_5-5\,F_{5,0}\,e_8 & 0
\\
e_2 &
0 & 0 & 0 & e_2 & 0 & 0 & 0 & 0 & 0 
\\
e_3 &
-\,e_2-\frac{5}{2}\,F_{5,0}\,e_3-2\,e_6 & 0 & 0 & e_3 & 
-\,e_7 & 0 & 0 & 0 & 0 
\\
e_4 &
0 & -\,e_2 & -\,e_3 & 0 & 0 & -\,e_6 & -\,e_7 & 0 & 0 
\\
e_5 &
\frac{5}{2}\,F_{5,0}\,e_5+2\,e_8 & 0 & e_7 & 0 & 0 & 0 & 0 &
0 & -\,e_5
\\
e_6 &
-\,2\,e_3-5\,F_{5,0}\,e_6 & 0 & 0 & e_6 & 0 & 0 & 0 & -\,e_7 & 0
\\
e_7 &
0 & 0 & 0 & e_7 & 0 & 0 & 0 & 0 & -\,e_7
\\
e_8 &
2\,e_5+5\,F_{5,0}\,e_8 & 0 & 0 & 0 & 0 & e_7 & 0 & 0 & -\,e_8
\\
e_9 &
0 & 0 & 0 & 0 & e_5 & 0 & e_7 & e_8 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3b4a5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^2y^3+x^2y^4+x^2y^5+x^2y^6+\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
(1-y)\,\partial_x+2\,x\,\partial_u, &
e_2
\,:=\,
(1-y)\,\partial_y+u\,\partial_u, &
& 
\\
e_3
\,:=\,
x\,\partial_x+2\,u\,\partial_u, &
e_4
\,:=\,
-\,\frac{1}{2}\,u\,\partial_x+x\,\partial_y, &
e_5
\,:=\,
v\,\partial_x, &
e_6
\,:=\,
v\,\partial_y,
\\
e_7
\,:=\,
v\,\partial_u, &
e_8
\,:=\,
v\,\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7 & e_8 
\\
\hline
e_1 & 
0 & e_1 & e_1 & e_2 & -\,2\,e_7 & e_5 & 0 & 0
\\
e_2 &
-\,e_1 & 0 & 0 & e_4 & 0 & e_6 & -\,e_7 & 0
\\
e_3 &
-\,e_1 & 0 & 0 & e_4 & -\,e_5 & 0 & -\,2\,e_7 & 0
\\
e_4 &
-\,e_2 & -\,e_4 & -\,e_4 & 0 & -\,e_6 & 0 & \frac{1}{2}\,e_5 & 0
\\
e_5 &
2\,e_7 & 0 & e_5 & e_6 & 0 & 0 & 0 & -\,e_5
\\
e_6 &
-\,e_5 & -\,e_6 & 0 & 0 & 0 & 0 & 0 & -\,e_6
\\
e_7 &
0 & e_7 & 2\,e_7 & -\,\frac{1}{2}\,e_5 & 0 & 0 & 0 & -\,e_7
\\
e_8 &
0 & 0 & 0 & 0 & e_5 & e_6 & e_7 & 0
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3b4a5b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^2y^3+x^5+x^2y^4+4\,x^5y
\\
&
\ \ \ \ \
+x^2y^5+10\,x^5y^2+F_{7,0}\,x^7+\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
for any value of $F_{7,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\big(1-y+7\,F_{7,0}\,u\big)\,\partial_x
-\big(14\,F_{7,0}\,x+5\,u\big)\,\partial_y+2\,x\,\partial_u, &
e_2
\,:=\,
-\,x\,\partial_x+(1-y)\,\partial_y-u\,\partial_u, &
& 
\\
e_3
\,:=\,
v\,\partial_x, &
e_4
\,:=\,
v\,\partial_y, &
\\
e_5
\,:=\,
v\,\partial_u, &
e_6
\,:=\,
v\,\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 
0 & 0 & 14\,F_{7,0}\,e_4-2\,e_5 & e_3 & -\,7\,F_{7,0}\,e_3+5\,e_4 &
0
\\
e_2 &
0 & 0 & e_3 & e_4 & e_5 & 0
\\
e_3 &
-\,14\,F_{7,0}\,e_4+2\,e_5 & -\,e_3 & 0 & 0 & 0 & -\,e_3
\\
e_4 &
-\,e_3 & -\,e_4 & 0 & 0 & 0 & -\,e_4
\\
e_5 &
7\,F_{7,0}\,e_3-5\,e_4 & -\,e_5 & 0 & 0 & 0 & -\,e_5
\\
e_6 &
0 & 0 & e_3 & e_4 & e_5 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3b4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^3y+x^2y^3+3\,x^3y^2+x^5+x^2y^4+6\,x^3y^3
\\
&
\ \ \ \ \
+\tfrac{9}{4}\,x^4y^2+3\,x^5y+x^6
+\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\big(1+3\,x-y-5\,u\big)\,\partial_x
+\big(10\,x-3\,y-15\,u\big)\,\partial_y
+\big(2\,x+6\,u\big)\,\partial_u, &
\\
e_2
\,:=\,
\big(-\,2\,x+\tfrac{3}{2}\,u\big)\,\partial_x
+
\big(1-4\,x-y+4\,u\big)\,\partial_y
-\,3\,u\,\partial_u, &
& 
\\
e_3
\,:=\,
v\,\partial_x, &
e_4
\,:=\,
v\,\partial_y, &
\\
e_5
\,:=\,
v\,\partial_u, &
e_6
\,:=\,
v\,\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 
0 & -\,e_1-e_2 & -\,3\,e_3-10\,e_4-2\,e_5 & e_3+3\,e_4 & 
5\,e_3+15\,e_4-6\,e_5 & 0
\\
e_2 &
e_1+e_2 & 0 & 2\,e_3+4\,e_4 & e_4 &
-\frac{3}{2}\,e_3-4\,e_4+3\,e_5 & 0
\\
e_3 &
3\,e_3+10\,e_4+2\,e_5 & -2\,e_3-4\,e_4 & 0 & 0 & 0 & -\,e_3
\\
e_4 &
-\,e_3-3\,e_4 & -\,e_4 & 0 & 0 & 0 & -\,e_4
\\
e_5 &
-\,5\,e_3-15\,e_4+6\,e_5 & \frac{3}{2}\,e_3+4\,e_4-3\,e_5 & 0
& 0 & 0 & -\,e_5
\\
e_6 &
0 & 0 & e_3 & e_4 & e_5 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3c5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2,
\\
v
&
\,=\,
x^3,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\partial_x+2\,x\,\partial_u+3\,u\,\partial_v, &
e_2
\,:=\,
\partial_y, &
& 
\\
e_3
\,:=\,
x\,\partial_x+2\,u\,\partial_u+3\,v\,\partial_v, &
e_4
\,:=\,
x\,\partial_y, &
e_5
\,:=\,
y\,\partial_y, &
e_6
\,:=\,
u\,\partial_y,
\\
e_7
\,:=\,
v\,\partial_y,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7
\\
\hline
e_1 & 
0 & 0 & e_1 & e_2 & 0 & 2\,e_4 & 3\,e_6
\\
e_2 &
0 & 0 & 0 & 0 & e_2 & 0 & 0
\\
e_3 &
-\,e_1 & 0 & 0 & e_4 & 0 & 2\,e_6 & 3\,e_7
\\
e_4 &
-\,e_2 & 0 & -\,e_4 & 0 & e_4 & -\,e_6 & -\,e_7
\\
e_5 &
0 & -\,e_2 & 0 & -\,e_4 & 0 & -\,e_6 & -\,e_7
\\
e_6 &
-\,2\,e_4 & 0 & -\,2\,e_6 & 0 & e_6 & 0 & 0
\\
e_7 &
-\,3\,e_6 & 0 & -\,3\,e_7 & 0 & e_7 & 0 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3c5b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2-\tfrac{5}{9}\,x^6-\tfrac{10}{7}\,G_{6,0}\,x^7
+\big(-\,\tfrac{250}{189}-\tfrac{45}{14}\,G_{6,0}^2\big)\,x^8
+\cdots,
\\
v
&
\,=\,
x^3+x^5+G_{6,0}\,x^6
+\big(\tfrac{20}{21}+\tfrac{9}{7}\,G_{6,0}^2\big)\,x^7
+\big(\tfrac{15}{7}\,G_{6,0}+\tfrac{27}{14}\,G_{6,0}^3\big)\,x^8
+\cdots,
\endaligned\right.
\]
for any value of $G_{6,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\big(1-3\,G_{6,0}\,x-\tfrac{5}{3}\,u\big)\,\partial_x
+\big(2\,x-6\,G_{6,0}\,u-\tfrac{10}{3}\,v\big)\,\partial_u
+
\big(3\,u-9\,G_{6,0}\,v\big)\,\partial_v, &
e_2
\,:=\,
\partial_y, &
& 
\\
e_3
\,:=\,
x\,\partial_y, &
e_4
\,:=\,
y\,\partial_y, &
\\
e_5
\,:=\,
u\,\partial_y, &
e_6
\,:=\,
v\,\partial_y,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 
0 & 0 & e_2-3\,G_{6,0}\,e_3-\frac{5}{3}\,e_5 & 0 &
2\,e_3-6\,G_{6,0}\,e_5-\frac{10}{3}\,e_6 &
3\,e_5-9\,G_{6,0}\,e_6
\\
e_2 &
0 & 0 & 0 & e_2 & 0 & 0
\\
e_3 &
-\,e_2+3\,G_{6,0}\,e_3+\frac{5}{3}\,e_5 & 0 & 0 &
e_3 & 0 & 0
\\
e_4 &
0 & -\,e_2 & -\,e_3 & 0 & -\,e_5 & -\,e_6
\\
e_5 &
-\,2\,e_3+6\,G_{6,0}\,e_5+\frac{10}{3}\,e_6 & 0 & 0 &
e_5 & 0 & 0
\\
e_6 &
-\,3\,e_5+9\,G_{6,0}\,e_6 & 0 & 0 & e_6 & 0 & 0 
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3c5c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2-\tfrac{5}{9}\,x^6+\tfrac{10}{7}\,G_{6,0}\,x^7
+\big(\tfrac{250}{189}-\tfrac{45}{14}\,G_{6,0}^2\big)\,x^8
+\cdots,
\\
v
&
\,=\,
x^3-x^5+G_{6,0}\,x^6
+\big(\tfrac{20}{21}-\tfrac{9}{7}\,G_{6,0}^2\big)\,x^7
+\big(-\,\tfrac{15}{7}\,G_{6,0}+\tfrac{27}{14}\,G_{6,0}^3\big)\,x^8
+\cdots,
\endaligned\right.
\]
for any value of $G_{6,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\big(1+3\,G_{6,0}\,x+\tfrac{5}{3}\,u\big)\,\partial_x
+\big(2\,x+6\,G_{6,0}\,u+\tfrac{10}{3}\,v\big)\,\partial_u
+
\big(3\,u+9\,G_{6,0}\,v\big)\,\partial_v, &
e_2
\,:=\,
\partial_y, &
& 
\\
e_3
\,:=\,
x\,\partial_y, &
e_4
\,:=\,
y\,\partial_y, &
\\
e_5
\,:=\,
u\,\partial_y, &
e_6
\,:=\,
v\,\partial_y,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 
0 & 0 & e_2+3\,G_{6,0}\,e_3+\frac{5}{3}\,e_5 & 0 &
2\,e_3+6\,G_{6,0}\,e_5+\frac{10}{3}\,e_6 &
3\,e_5+9\,G_{6,0}\,e_6
\\
e_2 &
0 & 0 & 0 & e_2 & 0 & 0
\\
e_3 &
-\,e_2-3\,G_{6,0}\,e_3-\frac{5}{3}\,e_5 & 0 & 0 &
e_3 & 0 & 0
\\
e_4 &
0 & -\,e_2 & -\,e_3 & 0 & -\,e_5 & -\,e_6
\\
e_5 &
-\,2\,e_3-6\,G_{6,0}\,e_5-\frac{10}{3}\,e_6 & 0 & 0 &
e_5 & 0 & 0
\\
e_6 &
-\,3\,e_5-9\,G_{6,0}\,e_6 & 0 & 0 & e_6 & 0 & 0 
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3c5d}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^5+F_{6,0}\,x^6
+\big(\tfrac{65}{42}\,G_{5,0}+\tfrac{8}{7}\,F_{6,0}^2
+\tfrac{20}{63}\,F_{6,0}\,G_{5,0}^2
-\tfrac{100}{567}\,G_{5,0}^4\big)\,x^7
+\cdots,
\\
v
&
\,=\,
x^3+G_{5,0}\,x^5
+\big(\tfrac{7}{4}+\tfrac{2}{3}\,G_{5,0}\,F_{6,0}
+\tfrac{10}{27}\,G_{5,0}^3\big)\,x^6
\\
&
\ \ \ \ \
+\big(\tfrac{85}{42}\,G_{5,0}^2
+\tfrac{27}{14}\,F_{6,0}+\tfrac{4}{7}\,G_{5,0}\,F_{6,0}^2
+\tfrac{40}{63}\,G_{5,0}^3F_{6,0}+\tfrac{100}{567}\,G_{5,0}^5\big)\,x^7
+\cdots,
\endaligned\right.
\]
for any value of $G_{5,0},F_{6,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
\big(
1-2\,F_{6,0}\,x-\tfrac{10}{9}\,G_{5,0}^2\,x-\tfrac{5}{3}\,G_{5,0}\,u
-\tfrac{5}{2}\,v
\big)\,\partial_x
\\
&
\ \ \ \ \ 
+
\big(
2\,x-4\,F_{6,0}\,u-\tfrac{20}{9}\,G_{5,0}^2\,u
-\tfrac{10}{3}\,G_{5,0}\,v
\big)\,\partial_u
\\
&
\ \ \ \ \ 
+
\big(
3\,u-6\,F_{6,0}\,v-\tfrac{10}{3}\,G_{5,0}^2\,v
\big)\,\partial_v,
\\
\ \ \ \ \ 
e_2
&
\,:=\,
\partial_y,
\\
e_3
&
\,:=\,
x\,\partial_y,
\ \ \ \ \ 
e_4
\,:=\,
y\,\partial_y,
\ \ \ \ \ 
e_5
\,:=\,
u\,\partial_y,
\ \ \ \ \ 
e_6
\,:=\,
v\,\partial_y,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
{}
[e_1,e_3]
&
\,=\,
e_2
-
\big(\tfrac{10}{9}\,G_{5,0}^2+2\,F_{6,0}\big)\,e_3
-
\tfrac{5}{3}\,G_{5,0}\,e_5
-
\tfrac{5}{2}\,e_6,
\\
[e_1,e_5]
&
\,=\,
2\,e_3
-
\big(\tfrac{20}{9}\,G_{5,0}^2+4\,F_{6,0}\big)\,e_5
-
\tfrac{10}{3}\,G_{5,0}\,e_6,
\\
[e_1,e_6]
&
\,=\,
3\,e_5
-
\big(\tfrac{10}{3}\,G_{5,0}^2+6\,F_{6,0}\big)\,e_6,
\\
[e_4,e_5]
&
\,=\,
-\,e_5,
\\
[e_4,e_6]
&
\,=\,
-\,e_6.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3d4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^3y+x^2y^3+3x^3y^2+x^2y^4+
\\
&
\ \ \ \ \ 
+
6x^3y^3+\tfrac{9}{4}x^4y^2-\tfrac{27}{32}x^5y-\tfrac{135}{256}x^6
+
\cdots
,
\\
v
&
\,=\,
x^3+2x^3y+3x^3y^2+\tfrac{9}{4}x^4y+4x^3y^3
+9x^4y^2+\tfrac{27}{64}x^6
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(
3x+1-y-\tfrac{27}{4}u+\tfrac{81}{16}v
)\partial_x
+
(
\tfrac{81}{8}x-3y-\tfrac{81}{4}u+\tfrac{2997}{128}v
)\partial_y
+
\\
&
\ \ \ \ \ 
+
(
2x+6u-\tfrac{27}{8}v
)\partial_u
+
(
3u+9v
)\partial_v
,
\\
e_2
&
\,:=\,
(
-4x+\tfrac{9}{2}u-\tfrac{9}{4}v
)\partial_x
+
(
-9x+2-2y+\tfrac{27}{2}u-\tfrac{189}{16}v
)\partial_y
+
(
-6u+2v
)\partial_u
-8v\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & -2e_1-\tfrac{3}{2}e_2
\\
e_2 &
2e_1+\tfrac{3}{2}e_2 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3d4b6a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^2y^3+x^2y^4+x^2y^5+x^2y^6
+\cdots,
\\
v
&
\,=\,
x^3+2\,x^3y+3\,x^3y^2+4\,x^3y^3+5\,x^3y^4+6\,x^3y^5
+\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\big(1-y\big)\,\partial_x
+2\,x\,\partial_u+3\,u\,\partial_v, &
e_2
\,:=\,
\big(1-y\big)\,\partial_y+u\,\partial_u+2\,v\,\partial_v, &
& 
\\
e_3
\,:=\,
x\,\partial_x+2\,u\,\partial_u+3\,v\,\partial_v, &
e_4
\,:=\,
-\,\tfrac{2}{3}\,u\,\partial_x
+x\,\partial_y-\tfrac{1}{3}\,v\,\partial_u,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccc}
{} & e_1 & e_2 & e_3 & e_4
\\
\hline
e_1 & 
0 & e_1 & e_1 & e_2-\frac{1}{3}\,e_3
\\
e_2 &
-\,e_1 & 0 & 0 & e_4
\\
e_3 &
-\,e_1 & 0 & 0 & e_4
\\
e_4 &
-\,e_2+\frac{1}{3}\,e_3 & -\,e_4 & -\,e_4 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3d4b6b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^2y^3+x^2y^4+x^6+x^2y^5+5\,x^6y
\\
&
\ \ \ \ \ 
+x^2y^6+15\,x^6y^2+F_{8,0}\,x^8+x^2y^7+35\,x^6y^3+7\,F_{8,0}
+\cdots,
\\
v
&
\,=\,
x^3+2\,x^3y+3\,x^3y^2+4\,x^3y^3+5\,x^3y^4+\tfrac{15}{7}\,x^7
\\
&
\ \ \ \ \ 
+6\,x^3y^5+\tfrac{90}{7}\,x^7y+7\,x^3y^6+45\,x^7y^2
+\tfrac{7}{3}\,F_{8,0}\,x^9+\cdots,
\endaligned\right.
\]
for any value of $F_{8,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
\big(1-y+14\,F_{8,0}\,u\big)\,\partial_x
-\big(21\,F_{8,0}\,x+6\,v\big)\,\partial_y
+\big(2\,x+7\,F_{8,0}\,v\big)\,\partial_u
+3\,u\,\partial_v,
\\
e_2
&
\,:=\,
-\,x\,\partial_x
+\big(1-y\big)\,\partial_y
-u\,\partial_u-v\,\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & 0
\\
e_2 &
0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3d4b6c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^2y^3+x^2y^4-x^6+x^2y^5-5\,x^6y
\\
&
\ \ \ \ \ 
+x^2y^6-15\,x^6y^2+F_{8,0}\,x^8+x^2y^7-35\,x^6y^3
+7\,F_{8,0}\,x^8y
+\cdots,
\\
v
&
\,=\,
x^3+2\,x^3y+3\,x^3y^2+4\,x^3y^3+5\,x^3y^4-\tfrac{15}{7}\,x^7
\\
&
\ \ \ \ \ 
+6\,x^3y^5-\tfrac{90}{7}\,x^7y+7\,x^3y^6-45\,x^7y^2
+\tfrac{7}{3}\,F_{8,0}\,x^9+\cdots,
\endaligned\right.
\]
for any value of $F_{8,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
\big(1-y-14\,F_{8,0}\,u\big)\,\partial_x
+\big(21\,F_{8,0}\,x+6\,v\big)\,\partial_y
+\big(2\,x-7\,F_{8,0}\,v\big)\,\partial_u
+3\,u\,\partial_v,
\\
e_2
&
\,:=\,
-\,x\,\partial_x
+\big(1-y\big)\,\partial_y
-u\,\partial_u-v\,\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & 0
\\
e_2 &
0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2b3d4b6d}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+x^2y+x^2y^2+x^2y^3+x^2y^4+x^2y^5+F_{7,0}x^7+x^2y^6
+
\\
&
\ \ \ \ \ 
+
6F_{7,0}x^7y+(-\tfrac{3}{2}+\tfrac{7}{3}F_{7,0}G_{7,0})x^8
+
\cdots
,
\\
v
&
\,=\,
x^3+2x^3y+3x^3y^2+4x^3y^3+x^6+5x^3y^4+5x^6y+G_{7,0}x^7
+
\\
&
\ \ \ \ \ 
+
6x^3y^5+15x^6y^2+6G_{7,0}x^7y+(3F_{7,0}+\tfrac{7}{6}G_{7,0}^2)x^8
+
\cdots,
\endaligned\right.
\]
for any values of $F_{7,0}$, $G_{7,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
\big(
1-\tfrac{7}{3}G_{7,0}x-y+14F_{7,0}u+6v
\big)\partial_x
-
\big(
21F_{7,0}x+12u
\big)\partial_y
+
\big(
2x-\tfrac{14}{3}G_{7,0}u+7F_{7,0}v
\big)\partial_u
+
\\
&
\ \ \ \ \ 
-
\big(
7G_{7,0}v-3u
\big)\partial_v
,
\\
e_2
&
\,:=\,
-x\partial_x-(y-1)\partial_y-u\partial_u-v\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & 0
\\
e_2 &
0 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SectionHead{2c Models}
{2c-models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2c3a4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\partial_x+y\partial_u
, &
e_2
\,:=\,
\partial_y+x\partial_u
, &
e_3
\,:=\,
x\partial_x+u\partial_u
, &
e_4
\,:=\,
y\partial_y+u\partial_u
, 
\\
e_5
\,:=\,
v\partial_x
, &
e_6
\,:=\,
v\partial_y
, &
e_7
\,:=\,
v\partial_u
, &
e_8
\,:=\,
v\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7 & e_8 
\\
\hline
e_1 & 0 & 0 & e_1 & 0 & 0 & -e_7 & 0 & 0
\\
e_2 & 0 & 0 & 0 & e_2 & -e_7 & 0 & 0 & 0
\\
e_3 & -e_1 & 0 & 0 & 0 & -e_5 & 0 & -e_7 & 0
\\
e_4 & 0 & -e_2 & 0 & 0 & 0 & -e_6 & -e_7 & 0
\\
e_5 & 0 & e_7 & e_5 & 0 & 0 & 0 & 0 & -e_5
\\
e_6 & e_7 & 0 & 0 & e_6 & 0 & 0 & 0 & -e_6
\\
e_7 & 0 & 0 & e_7 & e_7 & 0 & 0 & 0 & -e_7
\\
e_8 & 0 & 0 & 0 & 0 & e_5 & e_ 6 & e_7 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2c3a4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^2y^2+2x^3y^3+5x^4y^4+14x^5y^5
+
\cdots
,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
-
(
2u-1
)\partial_x
+
y\partial_u
, &
e_2
\,:=\,
-
(
2u-1
)\partial_y
+
x\partial_u
, &
e_3
\,:=\,
x\partial_x-y\partial_y
,
\\
e_4
\,:=\,
v\partial_x
, &
e_5
\,:=\,
v\partial_y
, &
e_6
\,:=\,
v\partial_u
,
\\
e_7
\,:=\,
v\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7
\\
\hline
e_1 & 0 & 2e_3 & e_1 & 0 & -e_6 & 2e_4 & 0
\\
e_2 & -2e_3 & 0 & -e_2 & -e_6 & 0 & 2e_5 & 0
\\
e_3 & -e_1 & e_2 & 0 & -e_4 & e_5 & 0 & 0
\\
e_4 & 0 & e_6 & e_4 & 0 & 0 & 0 & -e_4
\\
e_5 & e_6 & 0 & -e_5 & 0 & 0 & 0 & -e_5
\\
e_6 & -2e_4 & -2e_5 & 0 & 0 & 0 & 0 & -e_6
\\
e_7 & 0 & 0 & 0 & e_4 & e_5 & e_6 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2c3b4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+y^3
,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\partial_x+y\partial_u
, &
e_2
\,:=\,
-3y\partial_x+\partial_y+x\partial_u
, &
e_3
\,:=\,
2x\partial_x+y\partial_y+3u\partial_u
,
\\
e_4
\,:=\,
v\partial_x
, &
e_5
\,:=\,
v\partial_y
, &
e_6
\,:=\,
v\partial_u
, &
e_7
\,:=\,
v\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7
\\
\hline
e_1 & 0 & 0 & 2e_1 & 0 & -e_6 & 0 & 0
\\
e_2 & 0 & 0 & e_2 & -e_6 & 3e_4 & 0 & 0
\\
e_3 & -2e_1 & -e_2 & 0 & -2e_4 & -e_5 & -3e_6 & 0
\\
e_4 & 0 & e_6 & 2e_4 & 0 & 0 & 0 & -e_4
\\
e_5 & e_6 & -3e_4 & e_5 & 0 & 0 & 0 & -e_5
\\
e_6 & 0 & 0 & 3e_6 & 0 & 0 & 0 & -e_6
\\
e_7 & 0 & 0 & 0 & e_4 & e_5 & e_6 & 0
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2c3b4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+y^3+xy^3+\tfrac{6}{5}y^5+\tfrac{6}{5}xy^5+\tfrac{51}{35}y^7+\tfrac{51}{35}xy^7+\tfrac{62}{35}y^9
+
\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{lll}
e_1
\,:=\,
(x+1)\partial_x
+
(u+y)\partial_u
, &
e_2
\,:=\,
-(3u+3y)\partial_x+\partial_y+x\partial_u
, &
e_3
\,:=\,
v\partial_x,
\\
e_4
\,:=\,
v\partial_y
, &
e_5
\,:=\,
v\partial_u
, &
e_6
\,:=\,
v\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 0 & 0 & -e_3 & -e_5 & -e_5 & 0
\\
e_2 & 0 & 0 & -e_5 & 3e_3 & 3e_3 & 0
\\
e_3 & e_3 & e_5 & 0 & 0 & 0 & -e_3
\\
e_4 & e_5 & -3e_3 & 0 & 0 & 0 & -e_4
\\
e_5 & e_5 & -3e_3 & 0 & 0 & 0 & -e_5
\\
e_6 & 0 & 0 & e_3 & e_4 & e_5 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2c3b4c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+y^3-xy^3-\tfrac{6}{5}y^5+\tfrac{6}{5}xy^5
+\tfrac{51}{35}y^7-\tfrac{51}{35}xy^7-\tfrac{62}{35}y^9
+
\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{lll}
e_1
\,:=\,
-(x-1)\partial_x-(u-y)\partial_u
, &
e_2
\,:=\,
(3u-3y)\partial_x+\partial_y+x\partial_u
, &
e_3
\,:=\,
v\partial_x
,
\\
e_4
\,:=\,
v\partial_y
, &
e_5
\,:=\,
v\partial_u
, &
e_6
\,:=\,
v\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 0 & 0 & e_3 & -e_5 & e_5 & 0
\\
e_2 & 0 & 0 & -e_5 & 3e_3 & -3e_3 & 0
\\
e_3 & -e_3 & e_5 & 0 & 0 & 0 & -e_3
\\
e_4 & e_5 & -3e_3 & 0 & 0 & 0 & -e_4
\\
e_5 & -e_5 & 3e_3 & 0 & 0 & 0 & -e_5
\\
e_6 & 0 & 0 & e_3 & e_4 & e_5 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2c3b4e}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+y^3+y^4+F_{1,3}xy^3+F_{0,5}y^5
+
(
\tfrac{5}{2}F_{0,5}F_{1,3}-3F_{1,3}^2-2F_{1,3}
)xy^4
+
\\
&
\ \ \ \ \ 
+
(
-3F_{1,3}^2+\tfrac{5}{2}F_{0,5}F_{1,3}^2-3F_{1,3}^3
)x^2y^3
+
\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in $\R^2 \ni F_{1,3},F_{0,5}$:
\[
\aligned
\B_1 & := F_{1,3}^2(5F_{0,5}-6F_{1,3}-6),
\\
\B_2 & := F_{1,3}(5F_{0,5}-8+6F_{1,3})(5F_{0,5}-6F_{1,3}-6),
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-
(
5F_{0,5}F_{1,3}x-6F_{1,3}^2x-7F_{1,3}x-1
)\partial_x
-
(
-3F_{1,3}y+\tfrac{5}{2}F_{0,5}F_{1,3}y-3F_{1,3}^2y
)\partial_y
+
\\
&
\ \ \ \ \ 
-
(
-y-10F_{1,3}u+\tfrac{15}{2}F_{0,5}F_{1,3}u-9F_{1,3}^3u
)\partial_u
,
\\
e_2
&
\,:=\,
-
(
10F_{0,5}x+3F_{1,3}u-12F_{1,3}x-12x+3y
)\partial_x
-
(
5F_{0,5}y-6F_{1,3}y-4y-1
)\partial_y
\\
&
\ \ \ \ \ 
-
(
15F_{0,5}u-18F_{1,3}u-16u-x
)\partial_u,
\end{array}
\]
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_3
\,:=\,
v\partial_x
, &
e_4
\,:=\,
v\partial_y
, &
e_5
\,:=\,
v\partial_u
, &
e_6
\,:=\,
v\partial_v,
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\tiny
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 0 &
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}} $(-10F_{0,5}+12F_{1,3}+12)e_1+(-3F_{1,3}+\tfrac{5}{2}F_{0,5}F_{1,3}-3F_{1,3}^2)e_2$
\end{tabular} 
}
& 
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$F_{1,3}(5F_{0,5}-6F_{1,3}-7)e_3$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
 $\tfrac{1}{2}F_{1,3}(-6+5F_{0,5}-6F_{1,3})e_4-e_5$
\end{tabular}
}
& 
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$\tfrac{1}{2}F_{1,3}(-20+15F_{0,5}-18F_{1,3})e_5$
\end{tabular}
}
& 0
\\
e_2 & 
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-(-10F_{0,5}+12F_{1,3}+12)e_1-(-3F_{1,3}+\tfrac{5}{2}F_{0,5}F_{1,3}-3F_{1,3}^2)e_2$
\end{tabular}
}
&
0
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$(-12+10F_{0,5}-12F_{1,3})e_3-e_5$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$3e_3+(5F_{0,5}-6F_{1,3}-4)e_4$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$3F_{1,3}e_3+(15F_{0,5}-18F_{1,3}-16)e_5$
\end{tabular}
}
& 0
\\
e_3 
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-F_{1,3}(5F_{0,5}-6F_{1,3}-7)e_3$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-(-12+10F_{0,5}-12F_{1,3})e_3+e_5$
\end{tabular}
}
& 0 & 0 & 0 & -e_3
\\
e_4 
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-\tfrac{1}{2}F_{1,3}(-6+5F_{0,5}-6F_{1,3})e_4+e_5$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-3e_3-(5F_{0,5}-6F_{1,3}-4)e_4$
\end{tabular}
}
& 0 & 0 & 0 & -e_4
\\
e_5 
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-\tfrac{1}{2}F_{1,3}(-20+15F_{0,5}-18F_{1,3})e_5$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-3F_{1,3}e_3-(15F_{0,5}-18F_{1,3}-16)e_5$
\end{tabular}
}
& 0 & 0 & 0 & -e_5
\\
e_6 & 0 & 0 & e_3 & e_4 & e_5 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2c3d}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+y^3+x^3+F_{4,0}y^4+F_{1,3}xy^3+
(
\tfrac{2}{9}F_{1,3}F_{0,4}-\tfrac{1}{9}F_{3,1}F_{1,3}+\tfrac{8}{9}F_{4,0}F_{0,4}
)x^2y^2
+
\\
&
\ \ \ \ \ 
+
F_{3,1}x^3y
+
F_{4,0}x^4
+
\cdots
,
\\
v
&
\,=\,
0,
\endaligned\right.
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^4 \ni F_{1,3},F_{3,1},F_{0,4},F_{4,0}$:
\[
\aligned
\B_1 & := F_{0,4}F_{1,3}-F_{3,1}F_{4,0},
\\
\B_2 & := -2F_{0,4}F_{3,1}^2+F_{1,3}^3+2F_{1,3}^2F_{4,0}-F_{3,1}^3,
\\
\B_3 & := 2F_{0,4}^2F_{3,1}+F_{0,4}F_{3,1}^2-F_{1,3}^2F_{4,0}-2F_{1,3}F_{4,0}^2,
\\
\B_4 & := -32F_{0,4}F_{4,0}^2+F_{1,3}^2F_{3,1}+2F_{1,3}F_{3,1}F_{4,0}-16F_{3,1}F_{4,0}^2+36
F_{0,4}F_{3,1}+18F_{3,1}^2+81F_{1,3}+162F_{4,0},
\\
\B_5 & :=  -32F_{0,4}^2F_{4,0}-16F_{0,4}F_{3,1}F_{4,0}+F_{1,3}F_{3,1}^2+2F_{3,1}^2F_{4,0}+18
F_{1,3}^2+36F_{1,3}F_{4,0}+162F_{0,4}+81F_{3,1},
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
&
\,:=\,
-
(
-1
+
\tfrac{1}{3}F_{1,3}x
+
\tfrac{8}{3}F_{4,0}x
-
9u
+
\tfrac{4}{9}F_{1,3}F_{0,4}u
-
\tfrac{2}{9}F_{3,1}F_{1,3}
+
\tfrac{16}{9}F_{4,0}F_{0,4}u
)\partial_x
-
(
3x
+
\tfrac{4}{3}F_{4,0}y
\\
&
\ \ \ \ \ 
+
\tfrac{2}{3}F_{1,3}y
+
3F_{3,1}u
)\partial_y
-
(
F_{1,3}u
+
4F_{4,0}u
-
y
)\partial_u
,
\\
e_2
&
\,:=\,
-
(
\tfrac{4}{3}F_{0,4}x
+
\tfrac{2}{3}F_{3,1}x
+
3y
+
3F_{1,3}u
)\partial_x
-
(
-1
+
\tfrac{1}{3}F_{3,1}y
+
\tfrac{8}{3}F_{0,4}y
-
9u
+
\tfrac{4}{9}F_{1,3}F_{0,4}u
+
\\
&
\ \ \ \ \ 
-
\tfrac{2}{9}F_{3,1}F_{1,3}u
+
\tfrac{16}{9}F_{4,0}F_{0,4}u
)\partial_y
-
(
4F_{0,4}u
+
F_{3,1}u
-
x
)\partial_u
, 
\\
e_3
&
\,:=\,
v\partial_x
,
\ \ \ \ \
e_4
\,:=\,
v\partial_y
,
\ \ \ \ \
e_5
\,:=\,
v\partial_u
,
\ \ \ \ \
e_6
\,:=\,
v\partial_v,
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 & 0 &
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}} $(-\tfrac{4}{3}F_{0,4}-\tfrac{2}{3}F_{3,1})e_1+(\tfrac{2}{3}F_{1,3}+\tfrac{4}{3}F_{4,0})e_2$
\end{tabular}
}
& 
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$(\tfrac{1}{3}F_{1,3}+\tfrac{8}{3}F_{4,0})e_3+3e_4$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$(\tfrac{2}{3}F_{1,3}+\tfrac{4}{3}F_{4,0})e_4-e_5$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$(\tfrac{4}{9}F_{1,3}F_{0,4}+\tfrac{16}{9}F_{4,0}F_{0,4}-\tfrac{2}{9}F_{3,1}F_{1,3}-9)e_3+3F_{3,1}e_4+(F_{1,3}+4F_{4,0})e_5$
\end{tabular}
}
& 0
\\
e_2 & \rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$(\tfrac{4}{3}F_{0,4}+\tfrac{2}{3}F_{3,1})e_1-(\tfrac{2}{3}F_{1,3}+\tfrac{4}{3}F_{4,0})e_2$
\end{tabular}
}
& 0 &
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$(\tfrac{4}{3}F_{0,4}+\tfrac{2}{3}F_{3,1})e_3-e_5$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$3e_3+(\tfrac{1}{3}F_{3,1}+\tfrac{8}{3}F_{0,4})e_4$
\end{tabular}
}
& 
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$3F_{1,3}e_3+(\tfrac{4}{9}F_{1,3}F_{0,4}+\tfrac{16}{9}F_{4,0}F_{0,4}-\tfrac{2}{9}F_{3,1}F_{1,3}-9)e_4+(4F_{0,4}+F_{3,1})e_5$
\end{tabular}
}
& 0
\\
e_3 
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-(\tfrac{1}{3}F_{1,3}+\tfrac{8}{3}F_{4,0})e_3-3e_4$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-(\tfrac{4}{3}F_{0,4}+\tfrac{2}{3}F_{3,1})e_3+e_5$
\end{tabular}
}
& 0 & 0 & 0 & -e_3
\\
e_4 & 
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-(\tfrac{2}{3}F_{1,3}+\tfrac{4}{3}F_{4,0})e_4+e_5$
\end{tabular}
}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-3e_3-(\tfrac{1}{3}F_{3,1}+\tfrac{8}{3}F_{0,4})e_4$
\end{tabular}
}
& 0 & 0 & 0 & - e_4
\\
e_5 
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-(\tfrac{4}{9}F_{1,3}F_{0,4}-\tfrac{2}{9}F_{3,1}F_{1,3}-9)e_3-3F_{3,1}e_4-(F_{1,3}+4F_{4,0})e_5$
\end{tabular}
}
& 
\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
$-3F_{1,3}e_3-(\tfrac{4}{9}F_{1,3}F_{0,4}+\tfrac{16}{9}F_{4,0}F_{0,4}-\tfrac{2}{9}F_{3,1}F_{1,3}-9)e_4-(4F_{0,4}+F_{3,1})e5$
\end{tabular}
}
& 0 & 0 & 0 & -e_5
\\
e_6 & 0 & 0 & e_3 & e_4 & e_5 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SectionHead{2d Models}
{2d-models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2d3a4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+y^2,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\partial_x
+
2x\partial_u
, &
e_2
\,:=\,
\partial_y
+
2y\partial_u
, &
e_3
\,:=\,
x\partial_x
+
y\partial_y
+
2u\partial_u
, &
e_4
\,:=\,
y\partial_x
-
x\partial_y
,
\\
e_5
\,:=\,
v\partial_x
, &
e_6
\,:=\,
v\partial_y
, &
e_7
\,:=\,
v\partial_u
, &
e_8
\,:=\,
v\partial_v,
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7 & e_8 
\\
\hline
e_1 & 0 & 0 & e_1 & -e_2 & -2e_7 & 0 & 0 & 0
\\
e_2 & 0 & 0 & e_2 & e_1 & 0 & -2e_7 & 0 & 0
\\
e_3 & -e_1 & -e_2 & 0 & 0 & -e_5 & -e_6 & -2e_7 & 0
\\
e_4 & e_2 & -e_1 & 0 & 0 & e_6 & -e_5 & 0 & 0
\\
e_5 & 2e_7 & 0 & e_5 & -e_6 & 0 & 0 & 0 & -e_5
\\
e_6 & 0 & 2e_7& e_6 & e_5 & 0 & 0 & 0 & -e_6
\\
e_7 & 0 & 0 & 2e_7 & 0 & 0 & 0 & 0 & -e_7
\\
e_8 & 0 & 0 & 0 & 0 & e_5 & e_6 & e_7 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2d3a4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+y^2
+
\tfrac{1}{2}y^4
+
x^2y^2
+
\tfrac{1}{2}x^4
+
\tfrac{1}{2}y^6
+
\tfrac{3}{2}x^2y^4
+
\tfrac{3}{2}x^4y^2
+
\tfrac{1}{6}x^6
+
\\
&
\ \ \ \ \ 
+
\tfrac{5}{8}y^8
+
\tfrac{5}{2}x^2y^6
+
\tfrac{15}{4}x^4y^4
+
\tfrac{5}{2}x^6y^2
+
\tfrac{5}{8}x^8
+
\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
(1-u)\partial_x
+
2x\partial_u
, &
e_2
\,:=\,
(1-u)\partial_y
+
2y\partial_u
, &
e_3
\,:=\,
y\partial_x
-
x\partial_y
, 
\\
e_4
\,:=\,
v\partial_x
, &
e_5
\,:=\,
v\partial_y
, &
e_6
\,:=\,
v\partial_u
, &
e_7
\,:=\,
v\partial_v,
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7
\\
\hline
e_1 & 0 & 2e_3 & -e_2 & -2e_6 & 0 & e_4 & 0
\\
e_2 & -2e_3 & 0 & e_1 & 0 & -2e_6 & e_5 & 0
\\
e_3 & e_2 & -e_1 & 0 & e_5 & -e_4 & 0 & 0
\\
e_4 & 2e_6 & 0 & -e_5 & 0 & 0 & 0 & -e_4
\\
e_5 & 0 & 2e_6 & e_4 & 0 & 0 & 0 & -e_5
\\
e_6 & -e_4 & -e_5 & 0 & 0 & 0 & 0 & -e_6
\\
e_7 & 0 & 0 & 0 & e_4 & e_5 & e_6 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2d3a4c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
x^2+y^2
-
\tfrac{1}{2}y^4
-
x^2y^2
-
\tfrac{1}{2}x^4
+
\tfrac{1}{2}y^6
+
\tfrac{3}{2}x^2y^4
+
\tfrac{3}{2}x^4y^2
+
\tfrac{1}{6}x^6
+
\\
&
\ \ \ \ \ 
-
\tfrac{5}{8}y^8
-
\tfrac{5}{2}x^2y^6
-
\tfrac{15}{4}x^4y^4
-
\tfrac{5}{2}x^6y^2
-
\tfrac{5}{8}x^8
+
\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
(1+u)\partial_x
+
2x\partial_u
, &
e_2
\,:=\,
(1+u)\partial_y
+
2y\partial_u
, &
e_3
\,:=\,
y\partial_x
-
x\partial_y
, 
\\
e_4
\,:=\,
v\partial_x
, &
e_5
\,:=\,
v\partial_y
, &
e_6
\,:=\,
v\partial_u
, &
e_7
\,:=\,
v\partial_v,
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 & e_7
\\
\hline
e_1 & 0 & -2e_3 & -e_2 & -2e_6 & 0 & -e_4 & 0
\\
e_2 & 2e_3 & 0 & e_1 & 0 & -2e_6 & -e_5 & 0
\\
e_3 & e_2 & -e_1 & 0 & e_5 & -e_4 & 0 & 0
\\
e_4 & 2e_6 & 0 & -e_5 & 0 & 0 & 0 & -e_4
\\
e_5 & 0 & 2e_6 & e_4 & 0 & 0 & 0 & -e_5
\\
e_6 & e_4 & e_5 & 0 & 0 & 0 & 0 & -e_6
\\
e_7 & 0 & 0 & 0 & e_4 & e_5 & e_6 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2d3b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
y^2
+
x^2
+
x^3
+
F_{0,4}y^4
+
F_{1,3}xy^3
+
F_{2,2}x^2y^2
+
F_{3,1}x^3y
+
F_{4,0}x^4
+
\cdots,
\\
v
&
\,=\,
0,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^5 \ni F_{0,4},F_{4,0},F_{1,3},F_{3,1},F_{2,2}$:
\[
\aligned
\B_1 
&
:= 
32F_{0,4}F_{3,1}
+
4F_{1,3}F_{2,2}
+
136F_{1,3}F_{4,0}
-
20F_{2,2}
F_{3,1}
+
24F_{3,1}F_{4,0}
-
174F_{1,3}
-
27F_{3,1},
\\
\B_2
&
:= -4F_{0,4}F_{2,2}
+
8F_{0,4}F_{4,0}
+
F_{1,3}^2
+
5F_{1,3}F_{3,1}
-
2F_{2,2}^2
+
4F_{2,2}F_{4,0}
-
6F_{0,4}
-
3F_{2,2},
\\
\B_3
& 
:= 8F_{0,4}F_{1,3}
-
24F_{0,4}F_{3,1}
+
88F_{1,3}F_{4,0}
-
16F_{2,2}F_{3,1}
+
24F_{3,1}F_{4,0}
-
111F_{1,3}
-
27F_{3,1},
\\
\B_4
&
:= 8F_{0,4}^2
-
12F_{0,4}F_{2,2}
+
8F_{0,4}F_{4,0}
+
32F_{1,3}F_{3,1}
-
12F_{2,2}^2
+
28F_{2,2}F_{4,0}+
12F_{0,4}
-
21F_{2,2},
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
(
2F_{2,2}x
-
4F_{4,0}x
+
3x
+
1
+
\tfrac{1}{3}yF_{1,3}
-
yF_{3,1}-uF_{2,2}
)\partial_x
-
(
\tfrac{1}{3}F_{1,3}x
-
xF_{3,1}
-
\tfrac{9}{2}y
-
2yF_{2,2}
+
\\
&
\ \ \ \ \ 
+
4yF_{4,0}
+
\tfrac{1}{2}uF_{1,3}
)\partial_y
+
(
4F_{2,2}u-8F_{4,0}u+9u+2x
)\partial_u
,
\\
e_2
&
\,:=\,
(
3F_{1,3}x
-
xF_{3,1}
+
\tfrac{4}{3}yF_{0,4}
-
\tfrac{2}{3}yF_{2,2}
-
\tfrac{3}{2}uF_{1,3}
)\partial_x
-
(
\tfrac{4}{3}xF_{0,4}
-
1
-
\tfrac{2}{3}F_{2,2}x
-
3yF_{1,3}
+
yF_{3,1}
+
\\
&
\ \ \ \ \ 
+
2uF_{0,4}
)\partial_y
+
(
6F_{1,3}u-2F_{3,1}u+2y
)\partial_u
, 
\\
e_3
&
\,:=\,
v\partial_x
,
\ \ \ \ \ 
e_4
\,:=\,
v\partial_y
,
\ \ \ \ \ 
e_5
\,:=\,
v\partial_u
, 
\ \ \ \ \ 
e_6
\,:=\,
v\partial_v,
\endaligned
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 & e_6 
\\
\hline
e_1 
&
0
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{4cm}}
$\tfrac{8}{3}F_{1,3}e_1
+
(
-
\tfrac{9}{2}
-
\tfrac{4}{3}F_{2,2}
+
4F_{4,0}
-
\tfrac{4}{3}F_{0,4}
)e_2$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
\begin{tabular}{p{4cm}}
$
(
-
2F_{2,2}
+
4F_{4,0}
-
3
)e_3
+
(
\tfrac{1}{3}F_{1,3}
-
F_{3,1}
)e_4
-
2e_5$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
(
-
\tfrac{1}{3}F_{1,3}
+
F_{3,1}
)e_3
+
(
-
2F_{2,2}
+
4F_{4,0}
-
\tfrac{9}{2}
)e_4$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
F_{2,2}e_3
+
\tfrac{1}{2}F_{1,3}e_4
+
(
-
4F_{2,2}
+
8F_{4,0}
-
9
)e_5$
\end{tabular}}
&
0
\\
e_2 &
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
-
\tfrac{8}{3}F_{1,3}e_1
-
(
-
\tfrac{9}{2}
-
\tfrac{4}{3}F_{2,2}
+
4F_{4,0}
-
\tfrac{4}{3}F_{0,4}
)e_2$
\end{tabular}}
&
0
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
(
-
3F_{1,3}
+
F_{3,1}
)e_3
+
(
\tfrac{4}{3}F_{0,4}
-
\tfrac{2}{3}F_{2,2}
)e_4$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
(
-
\tfrac{4}{3}F_{0,4}
+
\tfrac{2}{3}F_{2,2}
)e_3
+
(
-
3F_{1,3}
+
F_{3,1}
)e_4
-
2e_5$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
\tfrac{3}{2}F_{1,3}e_3
+
2F_{0,4}e_4
+
(
-
6F_{1,3}
+
2F_{3,1}
)e_5$
\end{tabular}}
&
0
\\
e_3 &
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
-
(
-
2F_{2,2}
+
4F_{4,0}
-
3
)e_3
-
(
\tfrac{1}{3}F_{1,3}
-
F_{3,1}
)e_4
+
2e_5$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
-
(
-
3F_{1,3}
+
F_{3,1}
)e_3
-
(
\tfrac{4}{3}F_{0,4}
-
\tfrac{2}{3}F_{2,2}
)e_4$
\end{tabular}}
&
0
&
0
&
0
&
-e_3
\\
e_4 &
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
-
(
-
\tfrac{1}{3}
F_{1,3}
+
F_{3,1}
)e_3
-
(
-
2F_{2,2}
+
4F_{4,0}
-
\tfrac{9}{2}
)e_4
$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
-
(
-
\tfrac{4}{3}F_{0,4}
+
\tfrac{2}{3}
F_{2,2}
)e_3
-
(
-
3F_{1,3}
+
F_{3,1}
)e_4
+
2e_5
$
\end{tabular}}
& 
0
&
0
&
0
&
-e_4
\\
e_5 &
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
-
F_{2,2}e_3
-
\tfrac{1}{2}F_{1,3}e_4
-
(
-
4F_{2,2}
+
8F_{4,0}
-
9
)e_5
$
\end{tabular}}
&
\rotatebox[origin=c]{90}{
	\begin{tabular}{p{4cm}}
$
-
\tfrac{3}{2}F_{1,3}e_3
-
2F_{0,4}e_4
-
(
-
6F_{1,3}
+
2F_{3,1}
)e_5
$
\end{tabular}}
&
0
&
0
&
0
&
-e_5
\\
e_6 & 0 & 0 & e_3 & e_4 & e_5 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SectionHead{2e Models}
{2e-models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
F_{0,4}y^4
+
F_{1,3}xy^3
+
F_{2,2}x^2y^2
+
F_{3,1}x^3y
+
x^4
+
\\
&
\ \ \ \ \ 
+
(
\tfrac{9}{10}F_{1,3}
-
\tfrac{9}{250}F_{0,4}F_{1,3}F_{3,1}
+
\tfrac{1}{25}F_{0,4}F_{1,3}G_{4,0}
+
\tfrac{32}{25}F_{0,4}^2
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{250}F_{0,4}G_{4,0}F_{3,1}G_{3,1}
+
\tfrac{2}{375}F_{0,4}G_{4,0}F_{3,1}F_{2,2}
+
\tfrac{1}{200}F_{0,4}G_{3,1}^2
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{75}F_{0,4}F_{2,2}^2
-
\tfrac{1}{60}F_{0,4}G_{3,1}F_{2,2}
+
\tfrac{1}{25}F_{0,4}F_{3,1}F_{5,0}
+
\tfrac{1}{250}F_{0,4}F_{3,1}^2G_{3,1}
+
\\
&
\ \ \ \ \ 
-
\tfrac{2}{375}F_{0,4}F_{3,1}^2F_{2,2})y^5
+
(
\tfrac{3}{4}G_{3,1}
+
F_{2,2}
+
\tfrac{1}{10}F_{0,4}F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \ 
-
\tfrac{2}{15}F_{0,4}F_{3,1}F_{2,2}
-
\tfrac{1}{10}F_{0,4}G_{4,0}G_{3,1}
+
\tfrac{2}{15}F_{0,4}G_{4,0}F_{2,2}
+
\tfrac{8}{5}F_{0,4}F_{1,3}
+
\\
&
\ \ \ \ \ 
+
F_{0,4}F_{5,0})xy^4
+
(
6F_{3,1}
-
4G_{4,0}
+
\tfrac{1}{10}G_{3,1}F_{1,3}F_{3,1}
-
\tfrac{2}{15}F_{2,2}F_{1,3}F_{3,1}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{10}G_{3,1}F_{1,3}G_{4,0}
+
\tfrac{2}{15}F_{2,2}F_{1,3}G_{4,0}
+
\tfrac{3}{5}F_{1,3}^2
+
F_{1,3}F_{5,0}
-
F_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{4}{3}F_{2,2}F_{0,4}
)x^2y^3
+
(
4
+
\tfrac{1}{10}G_{3,1}F_{3,1}F_{2,2}
-
\tfrac{1}{10}G_{3,1}G_{4,0}F_{2,2}
-
\tfrac{1}{2}G_{3,1}F_{1,3}
+
\\
&
\ \ \ \ \ 
+
\tfrac{14}{15}F_{2,2}F_{1,3}
+
F_{2,2}F_{5,0}
-
\tfrac{2}{15}F_{3,1}F_{2,2}^2
+
\tfrac{2}{15}G_{4,0}F_{2,2}^2)x^3y^2
+
\\
&
\ \ \ \ \ 
+
(
-
\tfrac{1}{10}G_{4,0}F_{3,1}G_{3,1}
+
\tfrac{2}{15}G_{4,0}F_{3,1}F_{2,2}
+
\tfrac{1}{8}G_{3,1}^2
+
\tfrac{1}{3}F_{2,2}^2
-
\tfrac{5}{12}G_{3,1}F_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{10}F_{3,1}F_{1,3}
+
F_{3,1}F_{5,0}
+
\tfrac{1}{10}F_{3,1}^2G_{3,1}
-
\tfrac{2}{15}F_{3,1}^2F_{2,2})x^4y
+
F_{5,0}x^5
+
\cdots
,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
+
G_{3,1}x^3y
+
G_{4,0}x^4
-
\tfrac{18}{5}F_{0,4}y^5
-
3F_{1,3}xy^4
+
\\
&
\ \ \ \ \ 
+
(
-
2F_{2,2}
+
3G_{3,1}
)x^2y^3
+
(
-
\tfrac{1}{10}G_{3,1}F_{3,1}F_{2,2}
+
\tfrac{1}{10}G_{3,1}G_{4,0}F_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{5}G_{3,1}F_{1,3}
+
\tfrac{3}{4}G_{3,1}F_{5,0}
+
\tfrac{3}{40}F_{3,1}G_{3,1}^2
-
\tfrac{3}{40}G_{4,0}G_{3,1}^2
)x^4y
+
\\
&
\ \ \ \ \ 
+
(
\tfrac{2}{25}G_{4,0}F_{3,1}G_{3,1}
-
\tfrac{8}{75}G_{4,0}F_{3,1}F_{2,2}
-
\tfrac{1}{10}G_{3,1}^2
+
\tfrac{2}{25}G_{4,0}F_{1,3}
+
\\
&
\ \ \ \ \ 
+
\tfrac{4}{5}G_{4,0}F_{5,0}
-
\tfrac{2}{25}G_{4,0}^2G_{3,1}
+
\tfrac{8}{75}G_{4,0}^2F_{2,2}
+
\tfrac{2}{15}G_{3,1}F_{2,2}
)x^5
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^7 \ni F_{0,4},F_{2,2},F_{1,3},F_{3,1},G_{3,1},G_{4,0},F_{5,0}$:
\[
\aligned
\B_1 
&
:= 16F_{0,4}^2F_{3,1}G_{3,1}
-
48F_{0,4}F_{3,1}^2
+
96F_{0,4}F_{3,1}G_{4,0}
+
12F_{1,3}F_{2,2}F_{3,1}
-
24F_{1,3}F_{2,2}G_{4,0}
+
\\
&
\ \ \ \ \ 
+
30F_{2,2}^2G_{3,1}
-
15F_{2,2}G_{3,1}^2
-
24F_{0,4}G_{3,1},
\\
\B_2
&
:= 180F_{0,4}F_{1,3}^2G_{3,1}
+
576F_{0,4}F_{2,2}F_{3,1}
+
864F_{0,4}F_{2,2}G_{4,0}
+
528F_{0,4}F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \ 
-
1448F_{0,4}G_{3,1}G_{4,0}
+
60F_{1,3}F_{2,2}^2
-
60F_{1,3}F_{2,2}G_{3,1}
+
375F_{1,3}G_{3,1}^2
-
432F_{0,4}F_{1,3}
+
\\
&
\ \ \ \ \ 
-
4320F_{0,4}F_{5,0}
-
2880F_{3,1}^2
+
9240F_{3,1}G_{4,0}
-
6960G_{4,0}^2
+
5040F_{2,2}
-
6840G_{3,1},
\\
\B_3
&
:= 
-
288F_{0,4}F_{2,2}F_{3,1}
+
1728F_{0,4}F_{2,2}G_{4,0}
+
996F_{0,4}F_{3,1}G_{3,1}
-
2216F_{0,4}G_{3,1}G_{4,0}
+
\\
&
\ \ \ \ \ 
+
540F_{1,3}^2F_{3,1}
-
1080F_{1,3}^2G_{4,0}
-
120F_{1,3}F_{2,2}^2
-
285F_{1,3}F_{2,2}G_{3,1}
+
465F_{1,3}G_{3,1}^2
+
\\
&
\ \ \ \ \ 
-
3024F_{0,4}F_{1,3}
+
2160F_{0,4}F_{5,0}
-
2340F_{3,1}^2
+
8520F_{3,1}G_{4,0}
-
7680G_{4,0}^2
-
10080F_{2,2}
+
1530G_{3,1},
\\
\B_4
&
:= 320F_{0,4}F_{1,3}G_{3,1}^2
+
480F_{1,3}^3G_{3,1}
+
1488F_{1,3}F_{2,2}F_{3,1}
+
1632F_{1,3}F_{2,2}G_{4,0}
-
2676F_{1,3}F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
696F_{1,3}G_{3,1}G_{4,0}
+
480F_{2,2}^3
+
1440F_{2,2}^2G_{3,1}
-
450F_{2,2}G_{3,1}^2
-
195G_{3,1}^3
-
1920F_{0,4}F_{2,2}
+
\\
&
\ \ \ \ \ 
+
1440F_{0,4}G_{3,1}
-
576F_{1,3}^2
-
12960F_{1,3}F_{5,0}
+
5040F_{3,1}
+
12960G_{4,0},
\\
\B_5
&
:= 240F_{0,4}^2F_{2,2}G_{3,1}
-
180F_{0,4}^2G_{3,1}^2
-
72F_{0,4}F_{2,2}F_{3,1}
+
432F_{0,4}F_{2,2}G_{4,0}
+
204F_{0,4}F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \ 
-
464F_{0,4}G_{3,1}G_{4,0}
+
60F_{1,3}F_{2,2}^2
+
525F_{1,3}F_{2,2}G_{3,1}
-
255F_{1,3}G_{3,1}^2
+
864F_{0,4}F_{1,3}
+
\\
&
\ \ \ \ \ 
-
2160F_{0,4}F_{5,0}
-
180F_{3,1}^2
+
240F_{3,1}G_{4,0}
+
240G_{4,0}^2
+
5040F_{2,2}
-
2790G_{3,1},
\\
\B_6 
&
:= 80F_{1,3}^2F_{2,2}G_{3,1}
-
360F_{1,3}F_{3,1}^2
+
1440F_{1,3}F_{3,1}G_{4,0}
-
1440F_{1,3}G_{4,0}^2
+
608F_{2,2}^2F_{3,1}
+
\\
&
\ \ \ \ \ 
-
208F_{2,2}^2G_{4,0}
-
4F_{2,2}F_{3,1}G_{3,1}
+
704F_{2,2}G_{3,1}G_{4,0}
-
159F_{3,1}G_{3,1}^2
-
291G_{3,1}^2G_{4,0}
+
\\
&
\ \ \ \ \ 
+
1440F_{0,4}F_{3,1}
-
2880F_{0,4}G_{4,0}
-
456F_{1,3}F_{2,2}
-
1344F_{1,3}G_{3,1}
-
2760F_{2,2}F_{5,0}
+
\\
&
\ \ \ \ \ 
+
1110F_{5,0}G_{3,1}
+
14400,
\\
\B_7 
&
:= 32F_{0,4}F_{1,3}F_{3,1}G_{3,1}
-
168F_{1,3}F_{3,1}^2
+
480F_{1,3}F_{3,1}G_{4,0}
-
288F_{1,3}G_{4,0}^2
+
96F_{2,2}^2F_{3,1}
+
\\
&
\ \ \ \ \ 
-
144F_{2,2}^2G_{4,0}
+
60F_{2,2}F_{3,1}G_{3,1}
+
192F_{2,2}G_{3,1}G_{4,0}
-
51F_{3,1}G_{3,1}^2
-
63G_{3,1}^2G_{4,0}
+
\\
&
\ \ \ \ \ 
+
288F_{0,4}F_{3,1}
-
576F_{0,4}G_{4,0}
+
24F_{1,3}F_{2,2}
-
288F_{1,3}G_{3,1}
-
360F_{2,2}F_{5,0}
+
270F_{5,0}G_{3,1}
+
2880,
\\
\B_8 
&
:= 2560F_{0,4}F_{1,3}F_{2,2}G_{4,0}
+
6840F_{1,3}F_{3,1}^2
-
15840F_{1,3}F_{3,1}G_{4,0}
+
4320F_{1,3}G_{4,0}^2
+
\\
&
\ \ \ \ \ 
-
288F_{2,2}^2F_{3,1}
+
25968F_{2,2}^2G_{4,0}
-
10836F_{2,2}F_{3,1}G_{3,1}
-
14784F_{2,2}G_{3,1}G_{4,0}
+
5229F_{3,1}G_{3,1}^2
+
\\
&
\ \ \ \ \ 
+
1161G_{3,1}^2G_{4,0}
-
27360F_{0,4}F_{3,1}
-
6720F_{0,4}G_{4,0}
+
216F_{1,3}F_{2,2}
+
6624F_{1,3}G_{3,1}
+
\\
&
\ \ \ \ \ 
-
3240F_{2,2}F_{5,0}
-
6210F_{5,0}G_{3,1}
-
43200,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
-
1
+
\tfrac{1}{5}F_{1,3}x
+
2xF_{5,0}
+
\tfrac{1}{5}xF_{3,1}G_{3,1}
-
\tfrac{4}{15}xF_{3,1}F_{2,2}
-
\tfrac{1}{5}xG_{4,0}G_{3,1}
+
\tfrac{4}{15}xG_{4,0}F_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{3}{2}G_{3,1}u
+
2vG_{4,0}
)\partial_x
-
(
4v
-
\tfrac{1}{2}xG_{3,1}
+
\tfrac{2}{3}xF_{2,2}
+
\tfrac{3}{5}yF_{1,3}
+
yF_{5,0}
-
2uG_{4,0}
+
3uF_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{10}yF_{3,1}G_{3,1}
-
\tfrac{2}{15}yF_{3,1}F_{2,2}
-
\tfrac{1}{10}yG_{4,0}G_{3,1}
+
\tfrac{2}{15}yG_{4,0}F_{2,2}
)\partial_y
-
(
-
y
+
\tfrac{4}{5}uF_{1,3}
+
3uF_{5,0}
+
\\
&
\ \ \ \ \ 
+
\tfrac{3}{10}uF_{3,1}G_{3,1}
-
\tfrac{2}{5}uF_{3,1}F_{2,2}
-
\tfrac{3}{10}uG_{4,0}G_{3,1}
+
\tfrac{2}{5}uG_{4,0}F_{2,2}
-
\tfrac{1}{2}vG_{3,1}
+
\tfrac{2}{3}vF_{2,2}
)\partial_u
+
\\
&
\ \ \ \ \ 
-
(
-
2x
+
\tfrac{2}{5}vF_{1,3}
+
4vF_{5,0}
+
\tfrac{2}{5}vF_{3,1}G_{3,1}
-
\tfrac{8}{15}vF_{3,1}F_{2,2}
-
\tfrac{2}{5}vG_{4,0}G_{3,1}
+
\tfrac{8}{15}vG_{4,0}F_{2,2}
)\partial_v
, 
\\
e_2
&
\,:=\,
-
(
\tfrac{4}{5}xF_{0,4}
-
\tfrac{9}{25}F_{1,3}xF_{3,1}
+
\tfrac{2}{5}F_{1,3}xG_{4,0}
-
\tfrac{1}{25}xG_{4,0}F_{3,1}G_{3,1}
+
\tfrac{4}{75}xG_{4,0}F_{3,1}F_{2,2}
+
\tfrac{1}{20}xG_{3,1}^2
+
\\
&
\ \ \ \ \ 
+
\tfrac{2}{15}xF_{2,2}^2
-
\tfrac{1}{6}xG_{3,1}F_{2,2}
+
\tfrac{2}{5}xF_{3,1}F_{5,0}
+
\tfrac{1}{25}xF_{3,1}^2G_{3,1}
-
\tfrac{4}{75}xF_{3,1}^2F_{2,2}
+
3y
+
\tfrac{1}{2}vG_{3,1}
)\partial_x
+
\\
&
\ \ \ \ \ 
-
(
F_{1,3}x
-
1
+
\tfrac{12}{5}yF_{0,4}
+
\tfrac{1}{40}yG_{3,1}^2
+
\tfrac{1}{15}yF_{2,2}^2
-
\tfrac{1}{2}G_{3,1}u
+
2uF_{2,2}
+
vF_{3,1}
-
\tfrac{1}{50}yG_{4,0}F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{2}{75}yG_{4,0}F_{3,1}F_{2,2}
-
\tfrac{9}{50}yF_{1,3}F_{3,1}
+
\tfrac{1}{5}yF_{1,3}G_{4,0}
-
\tfrac{1}{12}yG_{3,1}F_{2,2}
+
\tfrac{1}{5}yF_{3,1}F_{5,0}
+
\tfrac{1}{50}yF_{3,1}^2G_{3,1}
+
\\
&
\ \ \ \ \ 
-
\tfrac{2}{75}yF_{3,1}^2F_{2,2}
)\partial_y
-
(
-
x
+
\tfrac{16}{5}uF_{0,4}
-
\tfrac{27}{50}uF_{1,3}F_{3,1}
+
\tfrac{3}{5}uF_{1,3}G_{4,0}
-
\tfrac{3}{50}uG_{4,0}F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{2}{25}uG_{4,0}F_{3,1}F_{2,2}
+
\tfrac{3}{40}uG_{3,1}^2
+
\tfrac{1}{5}uF_{2,2}^2
-
\tfrac{1}{4}G_{3,1}uF_{2,2}
+
\tfrac{3}{5}uF_{3,1}F_{5,0}
+
\tfrac{3}{50}uF_{3,1}^2G_{3,1}
+
\\
&
\ \ \ \ \ 
-
\tfrac{2}{25}uF_{3,1}^2F_{2,2}
+
vF_{1,3}
)\partial_u
-
(
6u
+
\tfrac{8}{5}vF_{0,4}
-
\tfrac{18}{25}vF_{1,3}F_{3,1}
+
\tfrac{4}{5}vF_{1,3}G_{4,0}
-
\tfrac{2}{25}vG_{4,0}F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{8}{75}vG_{4,0}F_{3,1}F_{2,2}
+
\tfrac{1}{10}vG_{3,1}^2
+
\tfrac{4}{15}vF_{2,2}^2
-
\tfrac{1}{3}vG_{3,1}F_{2,2}
+
\tfrac{4}{5}vF_{3,1}F_{5,0}
+
\tfrac{2}{25}vF_{3,1}^2G_{3,1}
-
\tfrac{8}{75}vF_{3,1}^2F_{2,2}
)\partial_v,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
	\begin{tabular}{p{8cm}}
$(
-
\tfrac{4}{5}F_{0,4}
+
\tfrac{9}{25}F_{3,1}F_{1,3}
-
\tfrac{2}{5}G_{4,0}F_{1,3}
+
\tfrac{1}{25}G_{4,0}F_{3,1}G_{3,1}
-
\tfrac{4}{75}G_{4,0}F_{3,1}F_{2,2}
-
\tfrac{1}{20}G_{3,1}^2
-
\tfrac{2}{15}F_{2,2}^2
+
\tfrac{1}{6}G_{3,1}F_{2,2}
-
\tfrac{2}{5}F_{3,1}F_{5,0}
-
\tfrac{1}{25}F_{3,1}^2G_{3,1}
+
\tfrac{4}{75}F_{3,1}^2F_{2,2}
)e_1
+
(
\tfrac{1}{10}F_{3,1}G_{3,1}
-
\tfrac{2}{15}F_{3,1}F_{2,2}
-
\tfrac{1}{10}G_{4,0}G_{3,1}
+
\tfrac{2}{15}G_{4,0}F_{2,2}
-
\tfrac{2}{5}F_{1,3}
+
F_{5,0})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
	\begin{tabular}{p{8cm}}
$
-
(
-
\tfrac{4}{5}F_{0,4}
+
\tfrac{9}{25}F_{3,1}F_{1,3}
-
\tfrac{2}{5}G_{4,0}F_{1,3}
+
\tfrac{1}{25}G_{4,0}F_{3,1}G_{3,1}
-
\tfrac{4}{75}G_{4,0}F_{3,1}F_{2,2}
-
\tfrac{1}{20}G_{3,1}^2
-
\tfrac{2}{15}F_{2,2}^2
+
\tfrac{1}{6}G_{3,1}F_{2,2}
-
\tfrac{2}{5}F_{3,1}F_{5,0}
-
\tfrac{1}{25}F_{3,1}^2G_{3,1}
+
\tfrac{4}{75}F_{3,1}^2F_{2,2}
)e_1
-
(
\tfrac{1}{10}F_{3,1}G_{3,1}
-
\tfrac{2}{15}F_{3,1}F_{2,2}
-
\tfrac{1}{10}G_{4,0}G_{3,1}
+
\tfrac{2}{15}G_{4,0}F_{2,2}
-
\tfrac{2}{5}F_{1,3}
+
F_{5,0}
)e_2$
\end{tabular}}
&
0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4ba}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
F_{0,4}y^4
+
F_{1,3}xy^3
+
F_{2,2}x^2y^2
+
(
2
+
\tfrac{3}{256}G_{3,1}^4
-
\tfrac{7}{64}F_{1,3}G_{3,1}^2
+
\\
&
\ \ \ \ \ 
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)x^3y
+
(
\tfrac{9}{10}F_{1,3}
-
\tfrac{7}{160}F_{0,4}F_{1,3}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{6}{5}F_{0,4}^2
+
\tfrac{3}{64}G_{3,1}F_{0,4}G_{5,0}
+
\tfrac{3}{640}F_{0,4}G_{3,1}^3
-
\tfrac{1}{160}F_{0,4}G_{3,1}^2F_{2,2}
)y^5
+
(
\tfrac{3}{4}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{3}{2}F_{0,4}F_{1,3}
+
\tfrac{5}{4}F_{0,4}G_{5,0}
+
\tfrac{1}{8}F_{0,4}G_{3,1}^2
-
\tfrac{1}{6}G_{3,1}F_{0,4}F_{2,2}
+
F_{2,2}
)xy^4
+
\\
&
\ \ \ \ \ 
+
(
8
+
\tfrac{9}{128}G_{3,1}^4
-
\tfrac{17}{32}F_{1,3}G_{3,1}^2
+
\tfrac{45}{64}G_{3,1}^2G_{5,0}
-
\tfrac{3}{32}G_{3,1}^3F_{2,2}
+
G_{3,1}F_{0,4}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{6}F_{2,2}F_{1,3}G_{3,1}
+
\tfrac{1}{2}F_{1,3}^2
+
\tfrac{5}{4}F_{1,3}G_{5,0}
+
\tfrac{4}{3}F_{2,2}F_{0,4}
)x^2y^3
+
(
\tfrac{1}{8}G_{3,1}^2F_{2,2}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{2}F_{1,3}G_{3,1}
+
\tfrac{5}{4}F_{2,2}G_{5,0}
-
\tfrac{1}{6}G_{3,1}F_{2,2}^2
+
\tfrac{5}{6}F_{2,2}F_{1,3}
)x^3y^2
+
(
\tfrac{1}{8}G_{3,1}^2
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{6}
(
2
+
\tfrac{3}{256}G_{3,1}^4
-
\tfrac{7}{64}F_{1,3}G_{3,1}^2
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
G_{3,1}F_{2,2}
-
\tfrac{5}{12}G_{3,1}F_{2,2}
+
\tfrac{5}{4}
(
2
+
\tfrac{3}{256}G_{3,1}^4
-
\tfrac{7}{64}F_{1,3}G_{3,1}^2
+
\\
&
\ \ \ \ \ 
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
G_{5,0}
+
\tfrac{1}{8}
(
2
+
\tfrac{3}{256}G_{3,1}^4
+
\\
&
\ \ \ \ \ 
-
\tfrac{7}{64}F_{1,3}G_{3,1}^2
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
G_{3,1}^2
+
\tfrac{1}{3}F_{2,2}^2
)x^4y
+
\\
&
\ \ \ \ \ 
+
(
-
\tfrac{1}{10}
(
2
+
\tfrac{3}{256}G_{3,1}^4
-
\tfrac{7}{64}F_{1,3}G_{3,1}^2
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{3}G_{3,1}F_{0,4}
))
G_{3,1}
+
\tfrac{2}{15}
(
2
+
\tfrac{3}{256}G_{3,1}^4
-
\tfrac{7}{64}F_{1,3}G_{3,1}^2
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
F_{2,2}
+
\tfrac{1}{10}G_{3,1}
-
\tfrac{2}{15}F_{2,2})x^5
+
\cdots
,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
+
G_{3,1}x^3y
+
x^4
-
\tfrac{18}{5}F_{0,4}y^5
-
3F_{1,3}xy^4
+
(
-
2F_{2,2}
+
3G_{3,1}
)x^2y^3
+
\\
&
\ \ \ \ \ 
+
(
\tfrac{15}{16}G_{3,1}G_{5,0}
+
\tfrac{3}{32}G_{3,1}^3
-
\tfrac{1}{8}G_{3,1}^2F_{2,2}
+
\tfrac{1}{8}F_{1,3}G_{3,1})x^4y
+
G_{5,0}x^5
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^5 \ni F_{0,4},F_{1,3},F_{2,2},G_{3,1},G_{5,0}$:
\[
\aligned
\B_1 
&
:= 40F_{0,4}F_{1,3}F_{2,2}G_{3,1}
-
24F_{2,2}^3
-
98F_{2,2}^2G_{3,1}
+
119F_{2,2}G_{3,1}^2
+
63G_{3,1}^3
-
376F_{1,3}F_{2,2}
+
\\
&
\ \ \ \ \ 
+
1512F_{1,3}G_{3,1}
+
4020F_{2,2}G_{5,0}
+
840G_{3,1}G_{5,0},
\\
\B_2
&
:= 2560F_{0,4}^2F_{2,2}
-
1280F_{0,4}^2G_{3,1}
+
336F_{2,2}^3
-
1468F_{2,2}^2G_{3,1}
+
1514F_{2,2}G_{3,1}^2
-
297G_{3,1}^3
+
\\
&
\ \ \ \ \ 
+
8544F_{1,3}F_{2,2}
-
1668F_{1,3}G_{3,1}
+
12720F_{2,2}G_{5,0}
-
2310G_{3,1}G_{5,0},
\\
\B_3
&
:= 183840F_{2,2}^3G_{3,1}
-
1679176F_{1,3}F_{2,2}G_{3,1}
+
1714878F_{1,3}G_{3,1}^2
-
3867120F_{2,2}^2G_{5,0}
+
\\
&
\ \ \ \ \ 
+
5261580F_{2,2}G_{3,1}G_{5,0}
-
925695G_{3,1}^2G_{5,0}
-
2851328F_{0,4}F_{2,2}
+
1425664F_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \ 
+
2373288F_{1,3}^2
-
6520200F_{1,3}G_{5,0}
+
1467450G_{5,0}^2,
\\
\B_4
&
:= 245120F_{2,2}^4
-
5966248F_{1,3}F_{2,2}G_{3,1}
+
2145774F_{1,3}G_{3,1}^2
+
13260240F_{2,2}^2G_{5,0}
+
\\
&
\ \ \ \ \ 
-
10330260F_{2,2}G_{3,1}G_{5,0}
+
3681465G_{3,1}^2G_{5,0}
+
17645056F_{0,4}F_{2,2}
-
8822528F_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \ 
-
6649176F_{1,3}^2
+
161400F_{1,3}G_{5,0}
+
41153850G_{5,0}^2,
\\
\B_5
&
:= 
-
4802048F_{0,4}F_{2,2}G_{3,1}
+
7243008F_{0,4}G_{3,1}^2
+
10831752F_{1,3}^2F_{2,2}
-
3683292F_{1,3}^2G_{3,1}
+
\\
&
\ \ \ \ \ 
-
97567200F_{1,3}F_{2,2}G_{5,0}
+
15179940F_{1,3}G_{3,1}G_{5,0}
+
67614750F_{2,2}G_{5,0}^2
-
33807375G_{3,1}G_{5,0}^2
+
\\
&
\ \ \ \ \ 
-
58103808F_{0,4}F_{1,3}
+
145259520F_{0,4}G_{5,0}
-
164265600F_{2,2}
+
82132800G_{3,1},
\\
\B_6
&
:= 
-
9300648F_{0,4}F_{1,3}F_{2,2}
-
14461652F_{0,4}F_{1,3}G_{3,1}
-
37669380F_{0,4}F_{2,2}G_{5,0}
+
\\
&
\ \ \ \ \ 
+
18834690F_{0,4}G_{3,1}G_{5,0}
+
7055412F_{1,3}^3
-
11327820F_{1,3}^2G_{5,0}
-
15776775F_{1,3}G_{5,0}^2
+
\\
&
\ \ \ \ \ 
-
35143720F_{2,2}^2
-
38921092F_{2,2}G_{3,1}
+
26206992G_{3,1}^2
+
24473808F_{1,3}
-
61184520G_{5,0},
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
(
1
-
\tfrac{5}{2}xG_{5,0}
-
\tfrac{1}{4}xG_{3,1}^2
+
\tfrac{1}{3}xG_{3,1}F_{2,2}
-
\tfrac{3}{2}G_{3,1}u
-
2v
)\partial_x
-
(
4u
-
\tfrac{1}{2}xG_{3,1}
+
\tfrac{2}{3}xF_{2,2}
+
\tfrac{1}{2}yF_{1,3}
+
\\
&
\ \ \ \ \ 
+
\tfrac{5}{4}yG_{5,0}
+
\tfrac{1}{8}yG_{3,1}^2
+
\tfrac{9}{256}uG_{3,1}^4
-
\tfrac{1}{6}yG_{3,1}F_{2,2}
-
\tfrac{21}{64}uF_{1,3}G_{3,1}^2
+
\tfrac{45}{128}uG_{3,1}^2G_{5,0}
-
\tfrac{3}{64}uG_{3,1}^3F_{2,2}
+
\\
&
\ \ \ \ \ 
+
G_{3,1}uF_{0,4}
)\partial_y
-
(
-
y
+
\tfrac{15}{4}uG_{5,0}
+
\tfrac{3}{8}uG_{3,1}^2
-
\tfrac{1}{2}G_{3,1}uF_{2,2}
+
\tfrac{1}{2}uF_{1,3}
-
\tfrac{1}{2}vG_{3,1}
+
\tfrac{2}{3}vF_{2,2}
)\partial_u
+
\\
&
\ \ \ \ \ 
+
(
-
5vG_{5,0}
+
2x
-
\tfrac{1}{2}vG_{3,1}^2
+
\tfrac{2}{3}vG_{3,1}F_{2,2}
)\partial_v
,
\\
e_2
&
\,:=\,
(
\tfrac{7}{16}xF_{1,3}G_{3,1}
-
\tfrac{15}{32}xG_{3,1}G_{5,0}
-
\tfrac{3}{64}xG_{3,1}^3
+
\tfrac{1}{16}xG_{3,1}^2F_{2,2}
-
3y
-
\tfrac{1}{2}vG_{3,1}
)\partial_x
-
(
2yF_{0,4}
+
xF_{1,3}
+
\\
&
\ \ \ \ \ 
+
2v
-
1
+
\tfrac{3}{128}yG_{3,1}^3
-
\tfrac{1}{2}G_{3,1}u
+
2uF_{2,2}
+
\tfrac{3}{256}vG_{3,1}^4
-
\tfrac{7}{32}yF_{1,3}G_{3,1}
+
\tfrac{15}{64}yG_{3,1}G_{5,0}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{32}yG_{3,1}^2F_{2,2}
-
\tfrac{7}{64}vF_{1,3}G_{3,1}^2
+
\tfrac{15}{128}vG_{3,1}^2G_{5,0}
-
\tfrac{1}{64}vG_{3,1}^3F_{2,2}
+
\tfrac{1}{3}vG_{3,1}F_{0,4}
)\partial_y
+
\\
&
\ \ \ \ \ 
-
(
-
x
-
\tfrac{21}{32}uF_{1,3}G_{3,1}
+
\tfrac{45}{64}G_{3,1}uG_{5,0}
+
\tfrac{9}{128}uG_{3,1}^3
-
\tfrac{3}{32}uG_{3,1}^2F_{2,2}
+
2uF_{0,4}
+
vF_{1,3})\partial_u
+
\\
&
\ \ \ \ \ 
+
(
-
6u
+
\tfrac{7}{8}vF_{1,3}G_{3,1}
-
\tfrac{15}{16}vG_{3,1}G_{5,0}
-
\tfrac{3}{32}vG_{3,1}^3
+
\tfrac{1}{8}vG_{3,1}^2F_{2,2}
)\partial_v,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(
\tfrac{7}{16}F_{1,3}G_{3,1}
-
\tfrac{15}{32}G_{3,1}G_{5,0}
-
\tfrac{3}{64}G_{3,1}^3
+
\tfrac{1}{16}G_{3,1}^2F_{2,2})e_1
+
(
-
\tfrac{1}{6}G_{3,1}F_{2,2}
+
\tfrac{1}{8}G_{3,1}^2
-
\tfrac{1}{2}F_{1,3}
+
\tfrac{5}{4}G_{5,0}
)e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
	\begin{tabular}{p{7cm}}
$
-
(
\tfrac{7}{16}F_{1,3}G_{3,1}
-
\tfrac{15}{32}G_{3,1}G_{5,0}
-
\tfrac{3}{64}G_{3,1}^3
+
\tfrac{1}{16}G_{3,1}^2F_{2,2}
)e_1
-
(
-
\tfrac{1}{6}G_{3,1}F_{2,2}
+
\tfrac{1}{8}G_{3,1}^2
-
\tfrac{1}{2}F_{1,3}
+
\tfrac{5}{4}G_{5,0}
)e_2$
\end{tabular}}
&
0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4bb}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
F_{0,4}y^4
+
F_{1,3}xy^3
+
F_{2,2}x^2y^2
+
(
-
2
+
\tfrac{3}{256}G_{3,1}^4
+
\tfrac{7}{64}G_{3,1}^2F_{1,3}
+
\\
&
\ \ \ \ \ 
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4})x^3y
+
(
\tfrac{9}{10}F_{1,3}
+
\tfrac{6}{5}F_{0,4}^2
+
\\
&
\ \ \ \ \ 
+
\tfrac{7}{160}G_{3,1}F_{0,4}F_{1,3}
+
\tfrac{3}{64}G_{3,1}F_{0,4}G_{5,0}
+
\tfrac{3}{640}F_{0,4}G_{3,1}^3
-
\tfrac{1}{160}F_{0,4}G_{3,1}^2F_{2,2})y^5
+
\\
&
\ \ \ \ \ 
+
(
\tfrac{3}{4}G_{3,1}
+
\tfrac{3}{2}F_{0,4}F_{1,3}
-
\tfrac{5}{4}F_{0,4}G_{5,0}
-
\tfrac{1}{8}F_{0,4}G_{3,1}^2
+
\tfrac{1}{6}G_{3,1}F_{0,4}F_{2,2}
+
F_{2,2}
)xy^4
+
\\
&
\ \ \ \ \ 
+
(
-
8
+
\tfrac{9}{128}G_{3,1}^4
+
\tfrac{17}{32}G_{3,1}^2F_{1,3}
+
\tfrac{45}{64}G_{3,1}^2G_{5,0}
-
\tfrac{3}{32}G_{3,1}^3F_{2,2}
+
G_{3,1}F_{0,4}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{6}F_{2,2}G_{3,1}F_{1,3}
+
\tfrac{1}{2}F_{1,3}^2
-
\tfrac{5}{4}F_{1,3}G_{5,0}
+
\tfrac{4}{3}F_{2,2}F_{0,4}
)x^2y^3
+
(
-
\tfrac{1}{8}G_{3,1}^2F_{2,2}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{2}G_{3,1}F_{1,3}
-
\tfrac{5}{4}F_{2,2}G_{5,0}
+
\tfrac{1}{6}G_{3,1}F_{2,2}^2
+
\tfrac{5}{6}F_{2,2}F_{1,3}
)x^3y^2
+
(
\tfrac{1}{8}G_{3,1}^2
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{6}
(
-
2
+
\tfrac{3}{256}G_{3,1}^4
+
\tfrac{7}{64}G_{3,1}^2F_{1,3}
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
G_{3,1}F_{2,2}
-
\tfrac{5}{12}F_{2,2}G_{3,1}
-
(
\tfrac{5}{4}
(
-
2
+
\tfrac{3}{256}G_{3,1}^4
+
\tfrac{7}{64}G_{3,1}^2F_{1,3}
+
\\
&
\ \ \ \ \ 
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
G_{5,0}
-
(
\tfrac{1}{8}
(
-
2
+
\tfrac{3}{256}G_{3,1}^4
+
\\
&
\ \ \ \ \ 
+
\tfrac{7}{64}G_{3,1}^2F_{1,3}
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
G_{3,1}^2
+
\tfrac{1}{3}F_{2,2}^2
)x^4y
+
\\
&
\ \ \ \ \ 
+
(
-
(
\tfrac{1}{10}
(
-
2
+
\tfrac{3}{256}G_{3,1}^4
+
\tfrac{7}{64}G_{3,1}^2F_{1,3}
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
G_{3,1}
+
(
\tfrac{2}{15}
(
-
2
+
\tfrac{3}{256}G_{3,1}^4
+
\tfrac{7}{64}G_{3,1}^2F_{1,3}
+
\tfrac{15}{128}G_{3,1}^2G_{5,0}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{64}G_{3,1}^3F_{2,2}
+
\tfrac{1}{3}G_{3,1}F_{0,4}
)
)
F_{2,2}
-
\tfrac{1}{10}G_{3,1}
+
\tfrac{2}{15}F_{2,2}
)x^5
+\cdots
,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
+
G_{3,1}x^3y
-
x^4
-
\tfrac{18}{5}F_{0,4}y^5
-
3F_{1,3}xy^4
+
(
-
2F_{2,2}
+
3G_{3,1}
)x^2y^3
+
\\
&
\ \ \ \ \ 
+
(
-
\tfrac{15}{16}G_{3,1}G_{5,0}
-
\tfrac{3}{32}G_{3,1}^3
+
\tfrac{1}{8}G_{3,1}^2F_{2,2}
+
\tfrac{1}{8}G_{3,1}F_{1,3}
)x^4y
+
G_{5,0}x^5
+\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^5 \ni F_{0,4},F_{1,3},F_{2,2},G_{3,1},G_{5,0}$:
\[
\aligned
\B_1 
&
:= 1701000F_{1,3}F_{2,2}G_{5,0}^2+1354976F_{2,2}^3+8802232F_{2,2}^2G_{3,1}-1660396F_{2,2}G_{3,1}^2-5460477G_{3,1}^3
+
\\
&
\ \ \ \ \ -21058704F_{1,3}F_{2,2}+69200028F_{1,3}G_{3,1}-192961080F_{2,2}G_{5,0}-21141810G_{3,1}G_{5,0},
\\
\B_2 
&
:= 1575F_{1,3}^2G_{3,1}G_{5,0}-56F_{2,2}^3+1118F_{2,2}^2G_{3,1}+1501F_{2,2}G_{3,1}^2-1398G_{3,1}^3-1056F_{1,3}F_{2,2}
+
\\
&
\ \ \ \ \ +6732F_{1,3}G_{3,1}-28620F_{2,2}G_{5,0}+3060G_{3,1}G_{5,0},
\\
\B_3 
&
:= 1915G_{3,1}^4+14976F_{1,3}F_{2,2}G_{3,1}-26928F_{1,3}G_{3,1}^2-13920F_{2,2}^2G_{5,0}+62880F_{2,2}G_{3,1}G_{5,0}
+
\\
&
\ \ \ \ \ +29880G_{3,1}^2G_{5,0}+33792F_{0,4}F_{2,2}-16896F_{0,4}G_{3,1}-23472F_{1,3}^2-54000F_{1,3}G_{5,0}+11700G_{5,0}^2,
\\
\B_4 
&
:= 45960F_{0,4}F_{1,3}G_{3,1}G_{5,0}+27944F_{1,3}F_{2,2}G_{3,1}-9618F_{1,3}G_{3,1}^2-75960F_{2,2}^2G_{5,0}
+
\\
&
\ \ \ \ \ -108150F_{2,2}G_{3,1}G_{5,0}+61425G_{3,1}^2G_{5,0}+32256F_{0,4}F_{2,2}-16128F_{0,4}G_{3,1}+30240F_{1,3}^2
+
\\
&
\ \ \ \ \ 
-64080F_{1,3}G_{5,0}-349200G_{5,0}^2,
\\
\B_5 
&
:= -4802048F_{0,4}F_{2,2}G_{3,1}+7243008F_{0,4}G_{3,1}^2+10831752F_{1,3}^2F_{2,2}-3683292F_{1,3}^2G_{3,1}
+
\\
&
\ \ \ \ \ 
+97567200F_{1,3}F_{2,2}G_{5,0}-15179940F_{1,3}G_{3,1}G_{5,0}+67614750F_{2,2}G_{5,0}^2-33807375G_{3,1}G_{5,0}^2
+
\\
&
\ \ \ \ \ 
+58103808F_{0,4}F_{1,3}+145259520F_{0,4}G_{5,0}+164265600F_{2,2}-82132800G_{3,1},
\\
\B_6 
&
:= -9300648F_{0,4}F_{1,3}F_{2,2}-14461652F_{0,4}F_{1,3}G_{3,1}+37669380F_{0,4}F_{2,2}G_{5,0}
+
\\
&
\ \ \ \ \ 
-18834690F_{0,4}G_{3,1}G_{5,0}+7055412F_{1,3}^3+11327820F_{1,3}^2G_{5,0}-15776775F_{1,3}G_{5,0}^2
+
\\
&
\ \ \ \ \ 
-35143720F_{2,2}^2-38921092F_{2,2}G_{3,1}+26206992G_{3,1}^2-24473808F_{1,3}-61184520G_{5,0},
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
-
1
-
\tfrac{5}{2}xG_{5,0}
-
\tfrac{1}{4}xG_{3,1}^2
+
\tfrac{1}{3}xG_{3,1}F_{2,2}
+
\tfrac{3}{2}G_{3,1}u
-
2v
)\partial_x
-
(
-
4u
-
\tfrac{1}{2}xG_{3,1}
+
\tfrac{2}{3}xF_{2,2}
+
\\
&
\ \ \ \ \ 
+
\tfrac{1}{2}yF_{1,3}
-
\tfrac{5}{4}yG_{5,0}
-
\tfrac{1}{8}yG_{3,1}^2
+
\tfrac{9}{256}uG_{3,1}^4
+
\tfrac{1}{6}yG_{3,1}F_{2,2} 
+
\tfrac{21}{64}uF_{1,3}G_{3,1}^2
+
\tfrac{45}{128}uG_{3,1}^2G_{5,0}
+
\\
&
\ \ \ \ \ 
-
\tfrac{3}{64}uG_{3,1}^3F_{2,2}
+
uG_{3,1}F_{0,4}
)\partial_y
-
(
-
y
-
\tfrac{15}{4}uG_{5,0}
-
\tfrac{3}{8}uG_{3,1}^2
+
\tfrac{1}{2}uG_{3,1}F_{2,2}
+
\tfrac{1}{2}uF_{1,3}
-
\tfrac{1}{2}vG_{3,1}
+
\\
&
\ \ \ \ \ 
+
\tfrac{2}{3}vF_{2,2}
)\partial_u
-
(
-
2x
-
5vG_{5,0}
-
\tfrac{1}{2}vG_{3,1}^2
+
\tfrac{2}{3}vG_{3,1}F_{2,2}
)\partial_v
, 
\\
e_2
&
\,:=\,
-
(
\tfrac{7}{16}xG_{3,1}F_{1,3}
+
\tfrac{15}{32}xG_{3,1}G_{5,0}
+
\tfrac{3}{64}xG_{3,1}^3
-
\tfrac{1}{16}xG_{3,1}^2F_{2,2}
+
3y
+
\tfrac{1}{2}vG_{3,1}
)\partial_x
-
(
-
1
-
2v
+
\\
&
\ \ \ \ \ 
+
xF_{1,3}
+
2yF_{0,4}
+
\tfrac{3}{128}yG_{3,1}^3
-
\tfrac{1}{2}G_{3,1}u
+
2uF_{2,2}
+
\tfrac{3}{256}vG_{3,1}^4
+
\tfrac{7}{32}yG_{3,1}F_{1,3}
+
\tfrac{15}{64}yG_{3,1}G_{5,0}
+
\\
&
\ \ \ \ \ 
-
\tfrac{1}{32}yG_{3,1}^2F_{2,2}
+
\tfrac{7}{64}vG_{3,1}^2F_{1,3}
+
\tfrac{15}{128}vG_{3,1}^2G_{5,0}
-
\tfrac{1}{64}vG_{3,1}^3F_{2,2}
+
\tfrac{1}{3}vG_{3,1}F_{0,4}
)\partial_y
+
\\
&
\ \ \ \ \ 
-
(
-
x
+
\tfrac{21}{32}uG_{3,1}F_{1,3}
+
\tfrac{45}{64}uG_{3,1}G_{5,0}
+
\tfrac{9}{128}uG_{3,1}^3
-
\tfrac{3}{32}uG_{3,1}^2F_{2,2}
+
2uF_{0,4}
+
vF_{1,3}
)\partial_u
+
\\
&
\ \ \ \ \ 
-
(
6u
+
\tfrac{7}{8}vG_{3,1}F_{1,3}
+
\tfrac{15}{16}vG_{3,1}G_{5,0}
+
\tfrac{3}{32}vG_{3,1}^3
-
\tfrac{1}{8}vG_{3,1}^2F_{2,2}
)\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
	\begin{tabular}{p{7cm}}
$
(
-
\tfrac{7}{16}G_{3,1}F_{1,3}
-
\tfrac{15}{32}G_{3,1}G_{5,0}
-
\tfrac{3}{64}G_{3,1}^3
+
\tfrac{1}{16}G_{3,1}^2F_{2,2})e_1
+
(
\tfrac{1}{6}F_{2,2}G_{3,1}
-
\tfrac{1}{8}G_{3,1}^2
-
\tfrac{5}{4}G_{5,0}
-
\tfrac{1}{2}F_{1,3})e_2
$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
	\begin{tabular}{p{7cm}}
$
-
(
-
\tfrac{7}{16}G_{3,1}F_{1,3}
-
\tfrac{15}{32}G_{3,1}G_{5,0}
-
\tfrac{3}{64}G_{3,1}^3
+
\tfrac{1}{16}G_{3,1}^2F_{2,2}
)e_1
-
(
\tfrac{1}{6}F_{2,2}G_{3,1}
-
\tfrac{1}{8}G_{3,1}^2
-
\tfrac{5}{4}G_{5,0}
-
\tfrac{1}{2}F_{1,3})e_2
$
\end{tabular}}
&
0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4ca}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
F_{0,4}y^4
+
F_{2,2}x^2y^2+x^3y
+\cdots,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
+
2F_{2,2}x^3y
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^2 \ni F_{2,2},F_{0,4}$:
\[
\B_1 := 2F_{0,4}F_{2,2}-3,
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
3F_{2,2}u
-
1
)\partial_x
+
(
\tfrac{1}{3}F_{2,2}x
-
3u
)\partial_y
+
(
y
+
\tfrac{1}{3}F_{2,2}v
)\partial_u
+
2x\partial_v
,
\\
e_2
&
\,:=\,
-
(
F_{2,2}v
+
3y
)\partial_x
-
(
2F_{0,4}y
+
F_{2,2}u
+
v
-
1
)\partial_y
-
(
2F_{0,4}u
-
x
)\partial_u-6u\partial_v,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4cb}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
F_{0,4}y^4
+
F_{2,2}x^2y^2
-
x^3y
+
\cdots,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
+
2F_{2,2}x^3y
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^2 \ni F_{2,2},F_{0,4}$:
\[
\B_1= 2F_{0,4}F_{2,2}+3,
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
3F_{2,2}u
-
1
)\partial_x
+
(
\tfrac{1}{3}F_{2,2}x
+
3u
)\partial_y
+
(
y
+
\tfrac{1}{3}F_{2,2}v
)\partial_u
+
2x\partial_v,
\\
e_2
&
\,:=\,
-
(
F_{2,2}v
+
3y
)\partial_x
-
(
2F_{0,4}y
+
F_{2,2}u
-
v
-
1
)\partial_y
-
(
2F_{0,4}u
-
x
)\partial_u
-6u\partial_v,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4d}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
\tfrac{1}{2}x^2y^2
+
\tfrac{5}{4}xy^4
+
\tfrac{3}{4}y^6
+
\tfrac{7}{12}x^3y^3
-
\tfrac{1}{1080}x^6
+
\tfrac{9}{4}x^2y^5
+
\\
&
\ \ \ \ \
-
\tfrac{1}{60}x^5y^2
+
\cdots,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
+
x^3y
+
2x^2y^3
-
\tfrac{1}{30}x^5
+
\tfrac{5}{4}x^4y^2
-
\tfrac{15}{14}y^7
+
\tfrac{19}{4}x^3y^4
+
\\
&
\ \ \ \ \
-
\tfrac{1}{9}x^6y
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
-
1
+
\tfrac{3}{2}u
)\partial_x
+
\tfrac{1}{6}x\partial_y
+
(
y
+
\tfrac{1}{6}v
)\partial_u
+
2x\partial_v,
\\
e_2
&
\,:=\,
-
(
3y
+
\tfrac{1}{2}v
)\partial_x
-
(
-
1
+
\tfrac{1}{2}u
)\partial_y
+
x\partial_u
-
6u\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4fa}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
F_{0,4}y^4
+
xy^3
+
(
\tfrac{9}{10}
+
\tfrac{6}{5}F_{0,4}^2
)y^5
+
2F_{0,4}xy^4
+
x^2y^3
+\cdots,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
-
\tfrac{18}{5}F_{0,4}y^5
-
3xy^4
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
for any value of $F_{0,4}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
x
-
1
)\partial_x
-
y\partial_y
-
(
2u
-
y
)\partial_u
-
(
2v
-
2x
)\partial_v
,
\\
e_2
&
\,:=\,
-
3y\partial_x
-
(
2F_{0,4}y
+
x
-
1
)\partial_y
-
(2F_{0,4}u+v-x)\partial_u-6u\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0	
\\
e_2 & 0 & 0 
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4fb}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
F_{0,4}y^4
-
xy^3
+
(
\tfrac{-9}{10}
+
\tfrac{6}{5}F_{0,4}^2
)y^5
-
2F_{0,4}xy^4
+
x^2y^3
+
\\
&
\ \ \ \ \ 
+
(
-
\tfrac{14}{5}F_{0,4}
+
\tfrac{8}{5}F_{0,4}^3
)y^6
+
(
\tfrac{27}{10}
-
\tfrac{18}{5}F_{0,4}^2
)xy^5
+
3F_{0,4}x^2y^4
-
x^3y^3
+
\\
&
\ \ \ \ \ 
+
(
\tfrac{3}{2}
-
\tfrac{46}{7}F_{0,4}^2
+
\tfrac{16}{7}F_{0,4}^4
)y^7
+
(
\tfrac{56}{5}F_{0,4}
-
\tfrac{32}{5}F_{0,4}^3
)xy^6
+
\\
&
\ \ \ \ \ 
+
(
\tfrac{-27}{5}
+
\tfrac{36}{5}F_{0,4}^2
)x^2y^5
-
4F_{0,4}x^3y^4
+
x^4y^3
+
\cdots
,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
-
\tfrac{18}{5}F_{0,4}y^5
+
3xy^4
+
(
\tfrac{12}{5}
-
\tfrac{36}{5}F_{0,4}^2
)y^6
+
\tfrac{54}{5}F_{0,4}xy^5
+
\\
&
\ \ \ \ \ 
-
\tfrac{9}{2}x^2y^4
+
(
\tfrac{-96}{7}F_{0,4}^3
+
\tfrac{78}{7}F_{0,4}
)y^7
+
(
\tfrac{-48}{5}
+
\tfrac{144}{5}F_{0,4}^2
)xy^6
+
\\
&
\ \ \ \ \ 
-
\tfrac{108}{5}F_{0,4}x^2y^5
+
6x^3y^4
+
\cdots,
\endaligned\right.
\]
for any value of $F_{0,4}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
(x+1)\partial_x+y\partial_y+(2u+y)\partial_u+(2v+2x)\partial_v
,\\
e_2
&
\,:=\,
-3y\partial_x-(2F_{0,4}y-x-1)\partial_y-(2F_{0,4}u-v-x)\partial_u-6u\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3a4g}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
y^3
+
y^4
+
F_{0,5}y^5
+
(
\tfrac{5}{3}F_{0,5}^2
-
\tfrac{2}{3}F_{0,5}
)y^6
+
(
\tfrac{25}{7}F_{0,5}^3
-
\tfrac{10}{3}F_{0,5}^2
+
\\
&
\ \ \ \ \
+
\tfrac{16}{21}F_{0,5}
)y^7
+
\cdots
,
\\
v
&
\,=\,
x^2
-
\tfrac{3}{2}y^4
-
\tfrac{18}{5}y^5
+
(
-
4F_{0,5}
-
\tfrac{12}{5}y^6+
(
-
\tfrac{50}{7}F_{0,5}^2
-
\tfrac{20}{7}F_{0,5}
)y^7
+
\cdots,
\endaligned\right.
\]
for any value of $F_{0,5}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
y\partial_u+2x\partial_v+\partial_x
,
\\
e_2
&
\,:=\,
-(10F_{0,5}x-12x+3y)\partial_x-(5F_{0,5}y-4y-1)\partial_y-(15F_{0,5}u-16u-x)\partial_u
+
\\
&
\ \ \ \ \ 
-(20F_{0,5}v+6u-24v)\partial_v
,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & -(10F_{0,5}-12)e_1
\\
e_2 & (10F_{0,5}-12)e_1
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\[
\text{\bf Model 2e3a4h}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
y^3+xy
,
\\
v
&
\,=\,
x^2-\tfrac{3}{2}y^4
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{lll}
e_1
\,:=\,
y\partial_u+2x\partial_v+\partial_x
, &
e_2
\,:=\,
x\partial_u-6u\partial_v-3y\partial_x+\partial_y
,
& 
e_3
\,:=\,
3u\partial_u+4v\partial_v+2x\partial_x+y\partial_y
.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & 0 & 2e_1
\\
e_2 & 0 & 0 & e_2
\\
e_3 & -2e_1 & -e_2 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3b4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
xy^2
+
xy^3
+
x^2y^2
-
x^3y
+
\tfrac{3}{8}x^4
+
xy^4
+
3x^2y^3
-
3x^3y^2
+
\\
&
\ \ \ \ \
+
\tfrac{7}{8}x^4y
+
xy^5
+
6x^2y^4
-
4x^3y^3
-
\tfrac{21}{8}x^4y^2
+
\tfrac{9}{4}x^5y
-
\tfrac{3}{8}x^6
+
xy^6
+
\\
&
\ \ \ \ \
+
10x^2y^5
-
\tfrac{145}{8}x^4y^3
+
10x^5y^2
-
\tfrac{3}{2}x^6y
+
\cdots,
\\
v
&
\,=\,
x^2
-
x^2y^2
+
\tfrac{1}{4}x^4
-
2x^2y^3
-
2x^3y^2
+
\tfrac{3}{2}x^4y
-
\tfrac{1}{4}x^5
-
3x^2y^4
+
\\
&
\ \ \ \ \
-
8x^3y^3
+
\tfrac{7}{2}x^4y^2
-
\tfrac{1}{8}x^6
-
4x^2y^5
-
20x^3y^4
+
\tfrac{29}{4}x^5y^2
+
\\
&
\ \ \ \ \
-
3x^6y
+
\tfrac{3}{8}x^7
+\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
-
x
-
1
+
y
+
\tfrac{1}{2}v
)\partial_x
+
(
\tfrac{3}{2}x
-
2y
+
\tfrac{1}{2}u
-
\tfrac{3}{2}v
)\partial_y
-
(
-
y
+
u
-
\tfrac{3}{2}v
)\partial_u
+
\\
&
\ \ \ \ \
-
(
2u
-
2v
-
2x)\partial_v 
,
\\
e_2
&
\,:=\,
(
-
3x
+
u
)\partial_x
+
(
1
-
2x
-
2y
+
2u
+
v
)\partial_y
-
(
-
x
+
3u
+
2v
)\partial_u-6v\partial_v
.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & -2e_1
\\
e_2 & 2e_1 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3b4ba}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
xy^2
+
xy^3
+
x^3y
+
xy^4+
(
\tfrac{-8}{5}G_{4,0}
+
\tfrac{18}{5}x^3y^2
+
\tfrac{3}{25}
-
\tfrac{2}{5}G_{4,0}^2
+
\\
&
\ \ \ \ \
+
\tfrac{2}{5}G_{4,0}
(
\tfrac{4}{5}G_{4,0}
-
\tfrac{4}{5}+
\tfrac{7}{25}G_{4,0}
)x^5
+
\cdots,
\\
v
&
\,=\,
x^2
-
x^2y^2
+
G_{4,0}x^4
-
2x^2y^3
+
(
\tfrac{4}{5}G_{4,0}
-
\tfrac{4}{5}
)x^4y
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^1 \ni G_{4,0}$:
\[
\B_1 := (4G_{4,0}+1)(G_{4,0}-1),
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
2G_{4,0}v
+
y
-
1
)\partial_x
+
(
-
\tfrac{3}{5}x
-
\tfrac{2}{5}xG_{4,0}
-
\tfrac{9}{5}u
+
\tfrac{14}{5}uG_{4,0}
)\partial_y
-
(
-
y
+
\tfrac{3}{5}v
+
\tfrac{2}{5}G_{4,0}v
)\partial_u
+
\\
&
\ \ \ \ \
-
(
-
2x
+
2u
)\partial_v
,
\\
e_2
&
\,:=\,
(
\tfrac{8}{5}xG_{4,0}
-
\tfrac{8}{5}x
+
u
)\partial_x
-
(
-
1
+
2y
+
v
)\partial_y
+
(
x
+
\tfrac{8}{5}uG_{4,0}
-
\tfrac{8}{5}u
)\partial_u
+
(
\tfrac{16}{5}G_{4,0}v
-
\tfrac{16}{5}v
)\partial_v,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & (-\tfrac{3}{5}+\tfrac{8}{5}G_{4,0})e_1
\\
e_2 & -(-\tfrac{3}{5}+\tfrac{8}{5}G_{4,0})e_1 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3b4bb}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
xy^2
+
xy^3
-
x^3y
+
xy^4
+
(
-
\tfrac{8}{5}G_{4,0}
-
\tfrac{18}{5}
)x^3y^2
+
(
\tfrac{3}{25}
-
\tfrac{2}{5}G_{4,0}^2
+
\\
&
\ \ \ \ \
+
\tfrac{2}{5}G_{4,0}
(
\tfrac{4}{5}G_{4,0}
+
\tfrac{4}{5}
)
-
\tfrac{7}{25}G_{4,0}
)x^5
+
\cdots,
\\
v
&
\,=\,
x^2
-
x^2y^2
+
G_{4,0}x^4
-
2x^2y^3
+
(
\tfrac{4}{5}G_{4,0}
+
\tfrac{4}{5}
)x^4y
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^1 \ni G_{4,0}$:
\[
\B_1 := 4G_{4,0}^2+3G_{4,0}-1,
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
2G_{4,0}v
+
y
-
1
)\partial_x
+
(
\tfrac{3}{5}x
-
\tfrac{2}{5}xG_{4,0}
+
\tfrac{9}{5}u
+
\tfrac{14}{5}uG_{4,0}
)\partial_y
-
(
-
y
-
\tfrac{3}{5}v
+
\tfrac{2}{5}G_{4,0}v
)\partial_u
+
\\
&
\ \ \ \ \
-
(
-
2x
+
2u
)\partial_v
,
\\
e_2
&
\,:=\,
-
(
\tfrac{8}{5}xG_{4,0}
+
\tfrac{8}{5}x
-
u
)\partial_x
+
(
1
-
2y
+
v
)\partial_y
-
(
-
x
+
\tfrac{8}{5}uG_{4,0}
+
\tfrac{8}{5}u
)\partial_u
-
(
\tfrac{16}{5}G_{4,0}v
+
\tfrac{16}{5}v
)\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & (-\tfrac{3}{5}-\tfrac{8}{5}G_{4,0})e_1
\\
e_2 & -(-\tfrac{3}{5}-\tfrac{8}{5}G_{4,0})e_1 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3b4e}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy^6+xy^5+xy^4+xy^3+xy^2+xy
+\cdots
,
\\
v
&
\,=\,
-4x^2y^5-3x^2y^4-2x^2y^3-x^2y^2+x^2
+\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
\,:=\,
-(y-1)\partial_x+y\partial_u-(2u-2x)\partial_v
, &
e_2
\,:=\,
u\partial_x-(2y-1)\partial_y+x\partial_u
, 
\\
e_3
\,:=\,
\partial_uu+2\partial_vv+\partial_xx
.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & e_1 & e_1
\\
e_2 & -e_1 & 0 & 0
\\
e_3 & -e_1 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4aa}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
\tfrac{3}{4}x^2y^2
-
\tfrac{8}{9}x^4
+
\tfrac{1}{6}\sqrt{3}x^3y^2
+
\tfrac{2}{9}\sqrt{3}x^4y
+
\tfrac{9}{8}x^3y^3
+
\tfrac{1}{6}x^4y^2
-
\tfrac{8}{3}x^5y
+
\\
&
\ \ \ \ \
-
\tfrac{40}{27}x^6
+
\tfrac{5}{8}\sqrt{3}x^4y^3
+
\sqrt{3}x^5y^2
-
\tfrac{2}{9}\sqrt{3}x^6y
-
\tfrac{16}{27}\sqrt{3}x^7
+\cdots
,
\\
v
&
\,=\,
x^2
+
x^3y
+
x^4
+
\tfrac{1}{6}\sqrt{3}x^4y
+
\tfrac{2}{9}\sqrt{3}x^5
+
\tfrac{27}{16}x^4y^2
+
\tfrac{17}{6}x^5y
+
x^6
+
\tfrac{3}{4}\sqrt{3}x^5y^2
+
\\
&
\ \ \ \ \
+
\tfrac{5}{3}\sqrt{3}x^6y
+
\tfrac{8}{9}\sqrt{3}x^7 
+\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
-
\tfrac{1}{3}x\sqrt{3}
-
1
+
\tfrac{3}{2}u
+
2v
)\partial_x
+
(
-
\tfrac{16}{9}x\sqrt{3}
-
y\sqrt{3}
+
2u
+
\tfrac{32}{9}v
)\partial_y
+
\\
&
\ \ \ \ \
-
(
-
y
+
\tfrac{2}{3}\sqrt{3}u
+
\tfrac{16}{9}v\sqrt{3}
)\partial_u
+
(
2x
+
\tfrac{2}{3}v\sqrt{3}
)\partial_v
,
\\
e_2
&
\,:=\,
-(
-
\tfrac{1}{4}x\sqrt{3}
+
\tfrac{1}{2}v
)\partial_x
-
(
\tfrac{2}{3}x\sqrt{3}
-
1
+
\tfrac{1}{4}y\sqrt{3}
+
u
)\partial_y
-
(
-
x
+
\tfrac{2}{3}v\sqrt{3}
)\partial_u
+
\tfrac{1}{2}v\sqrt{3}\partial_v
.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & \tfrac{1}{4}\sqrt{3}e_1+\tfrac{1}{3}\sqrt{3}e_2
\\
e_2 & -\tfrac{1}{4}\sqrt{3}e_1-\tfrac{1}{3}\sqrt{3}e_2 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4d5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
x^3y
+
F_{4,1}x^4y
+
x^5
+
(
\tfrac{6}{5}F_{4,1}^2
+
\tfrac{2}{5}G_{4,0}^2
+
\tfrac{2}{5}G_{4,0}
+
\tfrac{6}{5}
)x^5y
+
\\
&
\ \ \ \ \
+
F_{6,0}x^6
+
(
\tfrac{13}{5}F_{4,1}
+
\tfrac{4}{5}G_{4,0}^2F_{4,1}
+
\tfrac{6}{5}F_{4,1}G_{4,0}
+
\tfrac{8}{5}F_{4,1}^3)x^6y
+
\\
&
\ \ \ \ \
+
F_{7,0}x^7
+
\cdots
,
\\
v
&
\,=\,
x^2
+
G_{4,0}x^4
+
\tfrac{4}{5}F_{4,1}G_{4,0}x^5
+
(
2G_{4,0}^2
+
\tfrac{4}{5}F_{4,1}^2G_{4,0}
)x^6
+
\\
&
\ \ \ \ \
+
(
\tfrac{136}{35}G_{4,0}^2F_{4,1}
+
\tfrac{32}{35}F_{4,1}^3G_{4,0}
)x^7
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
2F_{4,1}G_{4,0}x
+
2G_{4,0}^2v
-
2F_{4,1}x
-
2G_{4,0}v
-
G_{4,0}
+
1
)\partial_x
-
(
12F_{4,1}G_{4,0}y
-
6F_{6,0}G_{4,0}y
+
\\
&
\ \ \ \ \
-
2G_{4,0}^2u
-
13F_{4,1}y
+
6F_{6,0}y
+
5G_{4,0}u
-
3u
-
5x
)\partial_y
-
(
14F_{4,1}G_{4,0}u
-
6F_{6,0}G_{4,0}u
+
\\
&
\ \ \ \ \
-
15F_{4,1}u
+
6F_{6,0}u
-
G_{4,0}y
-
5v
+
y
)\partial_u
-
(
4F_{4,1}G_{4,0}v
-
4F_{4,1}v
-
2G_{4,0}x
+
2x
)\partial_v
,
\\
e_2
&
\,:=\,
(
F_{4,1}x
+
G_{4,0}
-
1
+
\tfrac{2}{5}F_{4,1}^2G_{4,0}y
+
\tfrac{2}{5}G_{4,0}^3y
-
\tfrac{1}{5}F_{4,1}^2y
-
G_{4,0}^2y
+
\tfrac{4}{5}G_{4,0}y
-
\tfrac{1}{5}y
-
G_{4,0}v
+
\\
&
\ \ \ \ \
+
v
)\partial_y
+
(
G_{4,0}x
-
x
+
\tfrac{2}{5}F_{4,1}^2G_{4,0}u
+
\tfrac{2}{5}G_{4,0}^3u
-
\tfrac{1}{5}F_{4,1}^2u
-
G_{4,0}^2u
+
\tfrac{4}{5}G_{4,0}u
-
\tfrac{1}{5}u
+
F_{4,1}v
)\partial_u,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^3 \ni G_{4,0},F_{4,1},F_{6,0}$:
\[
\B_1 := (2G_{4,0}-1)(G_{4,0}-1)(F_{4,1}^2+G_{4,0}^2-2G_{4,0}+1)(2F_{4,1}-F_{6,0}),
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & (6G_{4,0}-6)(2F_{4,1}-F_{6,0})e_2
\\
e_2 & -(6G_{4,0}-6)(2F_{4,1}-F_{6,0})e_2 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4d5b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
x^3y
+
F_{4,1}x^4y
+
(
\tfrac{6}{5}F_{4,1}^2
+
\tfrac{2}{5}G_{4,0}^2
+
\tfrac{2}{5}G_{4,0}
+
\tfrac{6}{5})x^5y
+
\\
&
\ \ \ \ \
+
(
\tfrac{4}{5}G_{4,0}^2F_{4,1}
+
\tfrac{6}{5}F_{4,1}G_{4,0}
+
\tfrac{8}{5}F_{4,1}^3
+
\tfrac{13}{5}F_{4,1}
)x^6y
+
\cdots,
\\
v
&
\,=\,
x^2
+
G_{4,0}x^4
+
\tfrac{4}{5}F_{4,1}G_{4,0}x^5
+
(
2G_{4,0}^2
+
\tfrac{4}{5}F_{4,1}^2G_{4,0}
)x^6
+
\\
&
\ \ \ \ \
+
(
\tfrac{136}{35}G_{4,0}^2F_{4,1}
+
\tfrac{32}{35}F_{4,1}^3G_{4,0}
)x^7
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-
(
2F_{4,1}x
+
2G_{4,0}v
-
1
)\partial_x
+
\tfrac{
(
2G_{4,0}^2u
-
5G_{4,0}u
+
3u
)
}{G_{4,0}-1}\partial_y
+
\tfrac{
(
-
2F_{4,1}G_{4,0}u
+
2F_{4,1}u
+
G_{4,0}y
-
y
)
}
{G_{4,0}-1}\partial_u
+
\\
&
\ \ \ \ \
-
(
4F_{4,1}v
-
2x
)\partial_v
,
\\
e_2
&
\,:=\,
\tfrac{
(
F_{4,1}x
-
G_{4,0}v
+
G_{4,0}
+
v
-
1
)
}
{G_{4,0}-1}\partial_y
+
\tfrac{(F_{4,1}v+G_{4,0}x-x)}{G_{4,0}-1}\partial_u
, 
\\
e_3
&
\,:=\,
\tfrac{(G_{4,0}y-y)}{G_{4,0}-1}\partial_y
+
\tfrac{(G_{4,0}u-u)}{G_{4,0}-1}\partial_u,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^2 \ni G_{4,0},F_{4,1}$:
\[
\B_1 := 2F_{4,1}^2G_{4,0}+2G_{4,0}^3-F_{4,1}^2-5G_{4,0}^2+4G_{4,0}-1,
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & \tfrac{F_{4,1}e_2}{G_{4,0}-1} & 0
\\
e_2 & -\tfrac{F_{4,1}e_2}{G_{4,0}-1} & 0 & e_2
\\
e_3 & -\tfrac{F_{4,1}e_2}{G_{4,0}-1} & 0 & e_2
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4e5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
-
x^3y
+
F_{4,1}x^4y
+
x^5
+
(
-
\tfrac{6}{5}F_{4,1}^2
+
\tfrac{2}{5}G_{4,0}^2
-
\tfrac{2}{5}G_{4,0}+\tfrac{6}{5}
)x^5y
+
\\
&
\ \ \ \ \
+
F_{6,0}x^6
+
(
-
\tfrac{13}{5}F_{4,1}
-
\tfrac{4}{5}G_{4,0}^2F_{4,1}
+
\tfrac{6}{5}F_{4,1}G_{4,0}
+
\tfrac{8}{5}F_{4,1}^3
)x^6y
+
F_{7,0}x^7
+
\\
&
\ \ \ \ \
+
\cdots
,
\\
v
&
\,=\,
x^2
+
G_{4,0}x^4
-
\tfrac{4}{5}F_{4,1}G_{4,0}x^5
+
(
2G_{4,0}^2
+
\tfrac{4}{5}F_{4,1}^2G_{4,0}
)x^6
+
\\
&
\ \ \ \ \
+
(
-
\tfrac{136}{35}G_{4,0}^2F_{4,1}
-
\tfrac{32}{35}F_{4,1}^3G_{4,0}
)x^7
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
(
2F_{4,1}x
-
2G_{4,0}v
+
1
)
\partial_x
+
\\
&
\ \ \ \ \
-
\tfrac{(-60F_{4,1}G_{4,0}y-30F_{6,0}G_{4,0}y-10G_{4,0}^2u-65F_{4,1}y-30F_{6,0}y-25G_{4,0}u-15u-25x)}{5G_{4,0}+5}\partial_y
+
\\
&
\ \ \ \ \
-
\tfrac{(-70F_{4,1}G_{4,0}u-30F_{6,0}G_{4,0}u-75F_{4,1}u-30F_{6,0}u-5G_{4,0}y-25v-5y)}{5G_{4,0}+5}\partial_u+(4F_{4,1}v+2x)\partial_v
,
\\
e_2
&
\,:=\,
-
\tfrac{(2F_{4,1}^2G_{4,0}y-2G_{4,0}^3y+F_{4,1}^2y-5G_{4,0}^2y-5F_{4,1}x-5G_{4,0}v-4G_{4,0}y-5G_{4,0}-5v-y-5)}{5G_{4,0}+5}\partial_y
+
\\
&
\ \ \ \ \
-
\tfrac{(2F_{4,1}^2G_{4,0}u-2G_{4,0}^3u+F_{4,1}^2u-5G_{4,0}^2u-5F_{4,1}v-4G_{4,0}u-5G_{4,0}x-u-5x)}{5G_{4,0}+5}\partial_u,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^3 \ni G_{4,0},F_{4,1},F_{6,0}$:
\[
\B_1 := -\tfrac{6}{5}(2G_{4,0}+1)(F_{4,1}+1+G_{4,0})(F_{4,1}-1-G_{4,0})(2F_{4,1}+F_{6,0}),
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & -\tfrac{(12F_{4,1}G_{4,0}+6F_{6,0}G_{4,0}+12F_{4,1}+6F_{6,0})}{G_{4,0}+1}e_2
\\
e_2 & \tfrac{(12F_{4,1}G_{4,0}+6F_{6,0}G_{4,0}+12F_{4,1}+6F_{6,0})}{G_{4,0}+1}e_2 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4e5b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
-
x^3y
+
F_{4,1}x^4y
+
(
-
\tfrac{6}{5}F_{4,1}^2
+
\tfrac{2}{5}G_{4,0}^2
-
\tfrac{2}{5}G_{4,0}
+
\tfrac{6}{5})x^5y
+
\\
&
\ \ \ \ \
+
(
-
\tfrac{4}{5}G_{4,0}^2F_{4,1}
+
\tfrac{6}{5}F_{4,1}G_{4,0}
+
\tfrac{8}{5}F_{4,1}^3
-
\tfrac{13}{5}F_{4,1}
)x^6y
+
\cdots
,
\\
v
&
\,=\,
x^2
+
G_{4,0}x^4
-
\tfrac{4}{5}F_{4,1}G_{4,0}x^5
+
(
2G_{4,0}^2
+
\tfrac{4}{5}F_{4,1}^2G_{4,0}
)x^6
+
\\
&
\ \ \ \ \
+
(
-
\tfrac{136}{35}G_{4,0}^2F_{4,1}
-
\tfrac{32}{35}F_{4,1}^3G_{4,0}
)x^7
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
2F_{4,1}u\partial_u
+
4F_{4,1}v\partial_v
+
2F_{4,1}x\partial_x
-
2G_{4,0}v\partial_x
+
2G_{4,0}u\partial_y
+
y\partial_u
+
2u\partial_v
+
3u\partial_y
+
\partial_x
, 
\\
e_2
&
\,:=\,
\tfrac{(F_{4,1}x+G_{4,0}v+G_{4,0}+v+1)}{G_{4,0}+1}\partial_y+
\tfrac{(F_{4,1}v+G_{4,0}x+x)}{G_{4,0}+1}\partial_u
, 
\\
e_3
&
\,:=\,
\tfrac{(G_{4,0}y+y)}{G_{4,0}+1}\partial_y+\tfrac{(G_{4,0}u+u)}{G_{4,0}+1}\partial_u,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Gr\"obner basis generator of 
moduli space core algebraic variety in 
$\R^2 \ni G_{4,0},F_{4,1}$:
\[
\B_1 := 2F_{4,1}^2G_{4,0}-2G_{4,0}^3+F_{4,1}^2-5G_{4,0}^2-4G_{4,0}-1,
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & \tfrac{F_{4,1}}{G_{4,0}+1}e_2
\\
e_2 & -\tfrac{F_{4,1}}{G_{4,0}+1}e_2 & 0 & e_2
\\
e_3 & -\tfrac{F_{4,1}}{G_{4,0}+1}e_2 & 0 & e_2
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4f5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
+
x^3y
+
x^4
+
\tfrac{5}{4}G_{5,0}x^4y
+
(
2
+
\tfrac{1}{8}G_{5,0}^2
)x^5y
+
(
-
\tfrac{5}{4}G_{5,0}^2
+
\tfrac{14}{5}
)x^6
\\
&
\ \ \ \ \
+
(
\tfrac{23}{4}G_{5,0}
+
\tfrac{25}{8}G_{5,0}^3
)x^6y
+
(
\tfrac{20}{7}(
-
\tfrac{5}{4}G_{5,0}^2
+
\tfrac{14}{5}
)G_{5,0}
-
\tfrac{67}{14}G_{5,0}
)x^7
+
\cdots
,
\\
v
&
\,=\,
x^2+x^4+G_{5,0}x^5+(2+(5}{4)G_{5,0}^2)x^6+((34}{7)G_{5,0}+(25}{14)G_{5,0}^3)x^7 
+
\cdots
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-(
\tfrac{5}{2}G_{5,0}x
+
2v
-
1
)\partial_x
+
\tfrac{1}{20}\tfrac{(600G_{5,0}^2x-150G_{5,0}^2y-20G_{5,0}u-80G_{5,0}v+16x)}{G_{5,0}}\partial_y
\\
&
-
\tfrac{1}{20}\tfrac{(200G_{5,0}^2u-600G_{5,0}^2v-20G_{5,0}y-16v)}{G_{5,0}}\partial_u
-
(5G_{5,0}v-2x)\partial_v
,
\\
e_2
&
\,:=\,
-
\tfrac{1}{4}(30G_{5,0}x-5G_{5,0}y+4v-4)\partial_y
+
\tfrac{1}{4}(5G_{5,0}u-30G_{5,0}v+4x)\partial_u 
.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4f5b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3y+x^4
+
F_{5,0}x^5
+
2x^5y
+
(
\tfrac{5}{6}F_{5,0}^2+\tfrac{17}{6}
)x^6
+
\\
&
\ \ \ \ \
+
(
\tfrac{151}{42}F_{5,0}
+
\tfrac{25}{42}F_{5,0}^3
)x^7
+
\cdots
,
\\
v
&
\,=\,
x^2+x^4+2x^6
+
\cdots
,
\endaligned\right.
\]
for any value of $F_{5,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-(2v-1)\partial_x+(5F_{5,0}y-u-4v)\partial_y+(5F_{5,0}u+y)\partial_u+2x\partial_v
,
\\
e_2
&
\,:=\,
-(v-1)\partial_y+x\partial_u
,
\\
e_3
&
\,:=\,
v\partial_u+x\partial_y
.
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & -5F_{5,0}e_2-e_3 & -5F_{5,0}e_3+e_2
\\
e_2 & 5F_{5,0}e_2+e_3 & 0 & 0
\\
e_3 & 5F_{5,0}e_2+e_3 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4g}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3y+2x^5y
+
\cdots
,
\\
v
&
\,=\,
2x^6+x^4+x^2 
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-(2v-1)\partial_x-u\partial_y+y\partial_u+2x\partial_v 
,
\ \ \ \ \
e_2
\,:=\,
-(v-1)\partial_y+x\partial_u
, 
\\
e_3
&
\,:=\,
v\partial_u+x\partial_y
,
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
e_4
\,:=\,
u\partial_u+y\partial_y,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccc}
{} & e_1 & e_2 & e_3 & e_4
\\
\hline
e_1 & 0 & -e_3 & e_2 & 0
\\
e_2 & e_3 & 0 & 0 & e_2
\\
e_3 & -e_2 & 0 & 0 & e_3
\\
e_4 & 0 & -e_2 & -e_3 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\[
\text{\bf Model 2e3c4h}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy-x^3y+x^4+F_{5,0}x^5+2x^5y
+
(
\tfrac{5}{6}F_{5,0}^2
-
\tfrac{17}{6}
)x^6
+
\\
&
\ \ \ \ \
+
(
-
\tfrac{151}{42}F_{5,0}
+
\tfrac{25}{42}F_{5,0}^3
)x^7
+
\cdots,
\\
v
&
\,=\,
x^2-x^4+2x^6\cdots
,
\endaligned\right.
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
(2v+1)\partial_x+(5F_{5,0}y+u-4v)\partial_y+(5F_{5,0}u+y)\partial_u+2x\partial_v
,
\\
e_2
&
\,:=\,
(v+1)\partial_y+x\partial_u
,
& 
\\
e_3
&
\,:=\,
v\partial_u+x\partial_y
,
\endaligned
\]
for any value of $F_{5,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & -5F_{5,0}e_2+e_3 & -5F_{5,0}e_3+e_2
\\
e_2 & 5F_{5,0}e_2-e_3 & 0 & 0
\\
e_3 & 5F_{5,0}e_3-e_2 & 0 & 0
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4j5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^5
+
\tfrac{2}{5}x^5y
+
F_{6,0}x^6
+
\tfrac{2}{5}F_{6,0}x^6y
+
(\tfrac{16}{7}+\tfrac{6}{7}F_{6,0}^2)x^7
+
\cdots
,
\\
v
&
\,=\,
x^2+x^4+\tfrac{2}{5}F_{6,0}x^5+(2+\tfrac{1}{5}F_{6,0}^2)x^6+(\tfrac{68}{35}F_{6,0}+\tfrac{4}{35}F_{6,0}^3)x^7
+\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-(F_{6,0}x+2v-1)\partial_x+(5x+2u)\partial_y-(F_{6,0}u-5v-y)\partial_u-(2F_{6,0}v-2x)\partial_v
, 
\\
e_2
&
\,:=\,
(1+\tfrac{2}{5}y)\partial_y+(x+\tfrac{2}{5}u)\partial_u,
\endaligned
\]
for any value of $F_{6,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4k5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^5+\tfrac{2}{5}x^5y+F_{6,0}x^6+\tfrac{2}{5}F_{6,0}x^6y+(-\tfrac{16}{7}+\tfrac{6}{7}F_{6,0}^2)x^7
+
\cdots
,
\\
v
&
\,=\,
x^2-x^4
-
\tfrac{2}{5}F_{6,0}x^5
+
(
2
-
\tfrac{1}{5}F_{6,0}^2
)x^6
+
(
\tfrac{68}{35}F_{6,0}
-
\tfrac{4}{35}F_{6,0}^3)x^7
+
\cdots
,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-(F_{6,0}x-2v-1)\partial_x-(5x+2u)\partial_y-(F_{6,0}u+5v-y)\partial_u-(2F_{6,0}v-2x)\partial_v 
, 
\\
e_2
&
\,:=\,
(1+\tfrac{2}{5}y)\partial_y+(x+\tfrac{2}{5}u)\partial_u
,
\endaligned
\]
for any value of $F_{6,0}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0 
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4l5a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^4+x^5+F_{6,0}x^6+(\tfrac{12}{7}F_{6,0}^2-\tfrac{5}{7}F_{6,0})x^7
+
\cdots
,
\\
v
&
\,=\,
x^2,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-(6F_{6,0}x-5x-1)\partial_x-(18F_{6,0}y+4v-20y)\partial_y-(24F_{6,0}u-25u-y)\partial_u
+
\\
&
\ \ \ \ \
-(12F_{6,0}v-10v-2x)\partial_v
,
\\
e_2
&
\,:=\,
x\partial_u+\partial_y, 
\\
e_3
&
\,:=\,
v\partial_u+x\partial_y,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & (18F_{6,0}-20)e_2 & e_2+(12F_{6,0}-15)e_3
\\
e_2 & -(18F_{6,0}-20)e_2 & 0 & 0 
\\
e_3 & -e_2+(12F_{6,0}-15)e_3 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2e3c4m}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
,
\\
v
&
\,=\,
x^2,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
y\partial_u+2x\partial_v+\partial_x
, &
e_2
\,:=\,
x\partial_u+\partial_y
, &
& 
\\
e_3
\,:=\,
u\partial_u+2v\partial_v+x\partial_x
, &
e_4
\,:=\,
v\partial_u+x\partial_y
, &
e_5
\,:=\,
u\partial_u+y\partial_y,
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccccc}
{} & e_1 & e_2 & e_3 & e_4 & e_5 
\\
\hline
e_1 & 0 & 0 & e_1 & e_2 & 0
\\
e_2 & 0 & 0 & 0 & 0 & e_2
\\
e_3 & -e_1 & 0 & 0 & e_4 & 0
\\
e_4 & -e_2 & 0 & -e_4 & 0 & e_4
\\
e_5 & 0 & -e_2 & 0 & -e_4 & 0
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SectionHead{2f Models}
{2f-models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+F_{0,3}y^3+(4-F_{0,3})x^3+F_{0,4}y^4+F_{1,3}xy^3+F_{2,2}x^2y^2+F_{3,1}x^3y
+
\\
&
\ \ \ \ \
+
F_{4,0}x^4
+
\cdots,
\\
v
&
\,=\,
y^2+x^2+(-8-G_{2,1})xy^2+G_{2,1}x^2y+G_{0,4}y^4+G_{1,3}xy^3
+
\cdots.
\endaligned\right.
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
\Big(
1-\tfrac{3}{8}uG_{2,1}F_{4,0}+\tfrac{3}{64}uG_{2,1}G_{1,3}+\tfrac{1}{16}vG_{2,1}F_{2,2}+\tfrac{15}{16}uF_{0,3}F_{3,1}-\tfrac{3}{2}vF_{3,1}-\tfrac{9}{32}xG_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{3}{64}xG_{2,1}^2+\tfrac{1}{16}vG_{2,1}G_{4,0}-3vG_{4,0}+\tfrac{27}{16}xF_{0,3}^2-\tfrac{9}{8}uG_{3,1}-\tfrac{3}{16}yF_{3,1}+\tfrac{1}{16}yG_{2,2}-\tfrac{3}{4}uG_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{3}{32}uG_{2,1}G_{2,2}-\tfrac{1}{8}vF_{0,3}F_{1,3}+\tfrac{57}{32}uF_{0,3}^2G_{2,1}+\tfrac{3}{8}vF_{0,3}F_{3,1}+\tfrac{5}{8}uF_{0,3}F_{2,2}+\tfrac{9}{32}uG_{2,1}F_{3,1}
+
\\
&
\ \ \ \ \
+17vG_{2,1}+21uF_{0,3}+42vF_{0,3}-\tfrac{21}{2}uG_{2,1}+\tfrac{3}{16}uG_{2,1}G_{4,0}+\tfrac{9}{16}xF_{3,1}-\tfrac{3}{16}xG_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{55}{8}vF_{0,3}G_{2,1}+\tfrac{5}{32}uF_{0,3}G_{1,3}+\tfrac{7}{8}uG_{1,3}+\tfrac{1}{64}vG_{2,1}G_{1,3}-\tfrac{1}{8}yF_{2,2}-\tfrac{7}{4}xF_{4,0}-\tfrac{1}{2}uF_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{51}{4}xF_{0,3}+\tfrac{9}{4}yF_{0,3}+\tfrac{7}{32}xG_{1,3}+\tfrac{7}{8}yG_{2,1}+\tfrac{1}{128}vG_{2,1}^3+\tfrac{1}{4}yF_{4,0}+\tfrac{1}{16}yF_{1,3}+\tfrac{1}{2}vG_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{1}{4}vG_{1,3}+\tfrac{3}{128}uG_{2,1}^3+\tfrac{45}{16}uF_{0,3}^3-12vF_{0,3}^2-\tfrac{1}{32}yG_{1,3}-\tfrac{1}{8}yG_{4,0}-\tfrac{33}{2}uF_{0,3}^2-\tfrac{1}{32}vG_{2,1}G_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{3}{16}vF_{0,3}G_{3,1}-\tfrac{7}{16}xF_{1,3}+\tfrac{9}{8}vF_{0,3}^3+\tfrac{3}{32}yG_{3,1}-\tfrac{1}{64}yG_{2,1}^2-\tfrac{9}{16}yF_{0,3}^2+\tfrac{5}{8}uF_{0,3}G_{4,0}+\tfrac{3}{4}vG_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{9}{16}vG_{2,1}^2+\tfrac{3}{32}vG_{2,1}F_{3,1}-\tfrac{1}{8}vF_{0,3}G_{2,2}+\tfrac{21}{32}vF_{0,3}^2G_{2,1}-\tfrac{5}{16}uF_{0,3}F_{1,3}+\tfrac{3}{16}uG_{2,1}F_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{37}{8}xG_{2,1}
-\tfrac{9}{64}uG_{2,1}G_{3,1}+\tfrac{1}{4}vF_{0,3}G_{4,0}-\tfrac{1}{32}vG_{2,1}F_{1,3}-3uF_{4,0}+\tfrac{1}{2}vF_{1,3}+\tfrac{1}{4}vF_{0,3}F_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{9}{8}uG_{2,1}^2-\tfrac{1}{8}vG_{2,1}F_{4,0}-\tfrac{3}{4}uF_{1,3}+\tfrac{7}{8}xG_{4,0}-vF_{2,2}+\tfrac{9}{4}uF_{3,1}-\tfrac{13}{2}uF_{0,3}G_{2,1}
+\tfrac{9}{16}xF_{0,3}G_{2,1}
+
\\
&
\ \ \ \ \
+\tfrac{1}{16}vF_{0,3}G_{1,3}+2vF_{4,0}-\tfrac{3}{16}yF_{0,3}G_{2,1}-\tfrac{3}{32}uG_{2,1}F_{1,3}+\tfrac{3}{8}xF_{2,2}-\tfrac{5}{4}uF_{0,3}F_{4,0}+\tfrac{23}{64}uF_{0,3}G_{2,1}^2
+
\\
&
\ \ \ \ \
+\tfrac{3}{2}uG_{4,0}+16x-\tfrac{3}{64}vG_{2,1}G_{3,1}-\tfrac{5}{16}uF_{0,3}G_{2,2}-\tfrac{1}{2}vF_{0,3}F_{4,0}+\tfrac{1}{8}vF_{0,3}G_{2,1}^2
+
\\
&
\ \ \ \ \
-\tfrac{15}{32}uF_{0,3}G_{3,1}-48v
\Big)\,\partial_x
-
\endaligned
\]
\[
\aligned
&
-
\Big(
-\tfrac{3}{8}uG_{2,1}F_{4,0}+\tfrac{3}{64}uG_{2,1}G_{1,3}+\tfrac{1}{16}vG_{2,1}F_{2,2}+\tfrac{15}{16}uF_{0,3}F_{3,1}+\tfrac{3}{4}vF_{3,1}-\tfrac{3}{32}xG_{3,1}+
\\
&
\ \ \ \ \
+\tfrac{1}{64}xG_{2,1}^2+\tfrac{1}{16}vG_{2,1}G_{4,0}+\tfrac{1}{2}vG_{4,0}+\tfrac{9}{16}xF_{0,3}^2+\tfrac{15}{8}uG_{3,1}-\tfrac{9}{16}yF_{3,1}+\tfrac{3}{16}yG_{2,2}+\tfrac{5}{4}uG_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{3}{32}uG_{2,1}G_{2,2}-\tfrac{1}{8}vF_{0,3}F_{1,3}+\tfrac{57}{32}uF_{0,3}^2G_{2,1}+\tfrac{3}{8}vF_{0,3}F_{3,1}+\tfrac{5}{8}uF_{0,3}F_{2,2}+\tfrac{9}{32}uG_{2,1}F_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{7}{2}vG_{2,1}+69uF_{0,3}+3vF_{0,3}+\tfrac{55}{2}uG_{2,1}+\tfrac{3}{16}uG_{2,1}G_{4,0}+\tfrac{3}{16}xF_{3,1}-\tfrac{1}{16}xG_{2,2}-\tfrac{25}{8}vF_{0,3}G_{2,1}
+
\\
&
\ \ \ \ \
+\tfrac{5}{32}uF_{0,3}G_{1,3}-\tfrac{5}{8}uG_{1,3}+\tfrac{1}{64}vG_{2,1}G_{1,3}-\tfrac{3}{8}yF_{2,2}-\tfrac{1}{4}xF_{4,0}-\tfrac{5}{2}uF_{2,2}-\tfrac{21}{4}xF_{0,3}
+
\\
&
\ \ \ \ \
+\tfrac{51}{4}yF_{0,3}+\tfrac{1}{32}xG_{1,3}+\tfrac{33}{8}yG_{2,1}+\tfrac{1}{128}vG_{2,1}^3+\tfrac{7}{4}yF_{4,0}+\tfrac{7}{16}yF_{1,3}-\tfrac{1}{4}vG_{2,2}+\tfrac{5}{8}vG_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{3}{128}uG_{2,1}^3+\tfrac{45}{16}uF_{0,3}^3-\tfrac{21}{4}vF_{0,3}^2-\tfrac{7}{32}yG_{1,3}-\tfrac{7}{8}yG_{4,0}-\tfrac{51}{2}uF_{0,3}^2-\tfrac{1}{32}vG_{2,1}G_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{3}{16}vF_{0,3}G_{3,1}-\tfrac{1}{16}xF_{1,3}+\tfrac{9}{8}vF_{0,3}^3+\tfrac{9}{32}yG_{3,1}-\tfrac{3}{64}yG_{2,1}^2-\tfrac{27}{16}yF_{0,3}^2+\tfrac{5}{8}uF_{0,3}G_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{3}{8}vG_{3,1}-\tfrac{3}{8}vG_{2,1}^2+\tfrac{3}{32}vG_{2,1}F_{3,1}-\tfrac{1}{8}vF_{0,3}G_{2,2}+\tfrac{21}{32}vF_{0,3}^2G_{2,1}-\tfrac{5}{16}uF_{0,3}F_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{3}{16}uG_{2,1}F_{2,2}-\tfrac{7}{8}xG_{2,1}-\tfrac{9}{64}uG_{2,1}G_{3,1}+\tfrac{1}{4}vF_{0,3}G_{4,0}-\tfrac{1}{32}vG_{2,1}F_{1,3}+5uF_{4,0}
-\tfrac{1}{4}vF_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{1}{4}vF_{0,3}F_{2,2}-\tfrac{13}{8}uG_{2,1}^2-\tfrac{1}{8}vG_{2,1}F_{4,0}+\tfrac{5}{4}uF_{1,3}+\tfrac{1}{8}xG_{4,0}+\tfrac{1}{2}vF_{2,2}-\tfrac{3}{4}uF_{3,1}
+
\\
&
\ \ \ \ \
-14uF_{0,3}G_{2,1}+\tfrac{3}{16}xF_{0,3}G_{2,1}+\tfrac{1}{16}vF_{0,3}G_{1,3}-vF_{4,0}-\tfrac{9}{16}yF_{0,3}G_{2,1}-\tfrac{3}{32}uG_{2,1}F_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{1}{8}xF_{2,2}-\tfrac{5}{4}uF_{0,3}F_{4,0}+\tfrac{23}{64}uF_{0,3}G_{2,1}^2-48u-\tfrac{9}{2}uG_{4,0}-20y+12x-\tfrac{3}{64}vG_{2,1}G_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{5}{16}uF_{0,3}G_{2,2}-\tfrac{1}{2}vF_{0,3}F_{4,0}+\tfrac{1}{8}vF_{0,3}G_{2,1}^2-\tfrac{15}{32}uF_{0,3}G_{3,1}
\Big)\partial_y
+
\endaligned
\]
\[
\aligned
&
+
\Big(
-\tfrac{7}{2}uF_{4,0}-\tfrac{7}{8}uF_{1,3}-\tfrac{35}{4}uG_{2,1}-\tfrac{9}{16}uG_{3,1}+\tfrac{3}{32}uG_{2,1}^2-\tfrac{1}{8}vF_{2,2}-\tfrac{51}{2}uF_{0,3}
+
\\
&
\ \ \ \ \
+\tfrac{9}{4}vF_{0,3}+\tfrac{7}{8}vG_{2,1}+\tfrac{3}{32}vG_{3,1}-\tfrac{1}{64}vG_{2,1}^2-\tfrac{9}{16}vF_{0,3}^2-\tfrac{3}{16}vF_{3,1}+\tfrac{1}{16}vG_{2,2}-\tfrac{1}{32}vG_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{1}{8}vG_{4,0}-\tfrac{3}{16}vF_{0,3}G_{2,1}+\tfrac{9}{8}uF_{0,3}G_{2,1}+\tfrac{7}{16}uG_{1,3}+\tfrac{7}{4}uG_{4,0}+\tfrac{27}{8}uF_{0,3}^2+\tfrac{9}{8}uF_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{3}{8}uG_{2,2}+36u+y+\tfrac{1}{4}vF_{4,0}+\tfrac{1}{16}vF_{1,3}+\tfrac{3}{4}uF_{2,2}
\Big)\partial_u
-
\endaligned
\]
\[
\aligned
&
-
\Big(
-uF_{4,0}-\tfrac{1}{4}uF_{1,3}-\tfrac{11}{2}uG_{2,1}-\tfrac{3}{8}uG_{3,1}+\tfrac{1}{16}uG_{2,1}^2-\tfrac{3}{4}vF_{2,2}-15uF_{0,3}+\tfrac{51}{2}vF_{0,3}
+
\\
&
\ \ \ \ \
+\tfrac{37}{4}vG_{2,1}+\tfrac{9}{16}vG_{3,1}-\tfrac{3}{32}vG_{2,1}^2-\tfrac{27}{8}vF_{0,3}^2
-\tfrac{9}{8}vF_{3,1}+\tfrac{3}{8}vG_{2,2}-\tfrac{7}{16}vG_{1,3}-\tfrac{7}{4}vG_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{9}{8}vF_{0,3}G_{2,1}+\tfrac{3}{4}uF_{0,3}G_{2,1}+\tfrac{1}{8}uG_{1,3}+\tfrac{1}{2}uG_{4,0}+\tfrac{9}{4}uF_{0,3}^2+\tfrac{3}{4}uF_{3,1}-\tfrac{1}{4}uG_{2,2}+24u
+
\\
&
\ \ \ \ \
-2x-32v+\tfrac{7}{2}vF_{4,0}+\tfrac{7}{8}vF_{1,3}+\tfrac{1}{2}uF_{2,2}
\Big)\partial_v
+
\endaligned
\]
\[
\aligned
\\
e_2
&
\,:=\,
\Big(
\tfrac{7}{2}uG_{0,4}-3uF_{0,4}-\tfrac{1}{8}yG_{0,4}+\tfrac{1}{4}yF_{0,4}+\tfrac{45}{16}uF_{0,3}^3-\tfrac{3}{16}yF_{1,3}+\tfrac{3}{128}uG_{2,1}^3+\tfrac{3}{32}yG_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{1}{16}yF_{3,1}+\tfrac{1}{16}yG_{2,2}-\tfrac{1}{64}yG_{2,1}^2-\tfrac{9}{16}yF_{0,3}^2-\tfrac{3}{4}uF_{1,3}-\tfrac{1}{32}yG_{3,1}-\tfrac{3}{32}uG_{2,1}F_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{1}{8}vF_{0,3}F_{3,1}+\tfrac{57}{32}uF_{0,3}^2G_{2,1}+\tfrac{5}{8}uF_{0,3}F_{2,2}+\tfrac{1}{8}vF_{0,3}G_{2,1}^2+\tfrac{5}{32}uF_{0,3}G_{3,1}-\tfrac{5}{16}uF_{0,3}F_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{1}{16}vG_{2,1}F_{2,2}-\tfrac{9}{64}uG_{2,1}G_{1,3}+2vF_{0,4}+\tfrac{7}{8}xG_{0,4}-\tfrac{7}{4}xF_{0,4}-vG_{0,4}-\tfrac{15}{32}uF_{0,3}G_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{3}{16}yF_{0,3}G_{2,1}+\tfrac{9}{32}uG_{2,1}F_{1,3}+\tfrac{9}{16}xF_{0,3}G_{2,1}-\tfrac{1}{32}vG_{2,1}F_{3,1}+\tfrac{3}{32}vG_{2,1}F_{1,3}+\tfrac{23}{64}uF_{0,3}G_{2,1}^2
+
\\
&
\ \ \ \ \
+\tfrac{15}{2}uG_{2,1}+\tfrac{3}{8}uG_{3,1}+\tfrac{3}{4}uG_{2,1}^2-vF_{2,2}-\tfrac{9}{32}xG_{1,3}-\tfrac{3}{8}yG_{2,1}+\tfrac{1}{128}vG_{2,1}^3+\tfrac{21}{32}vF_{0,3}^2G_{2,1}
+
\\
&
\ \ \ \ \
-\tfrac{1}{8}vF_{0,3}G_{2,2}+\tfrac{7}{32}xG_{3,1}+\tfrac{3}{64}xG_{2,1}^2+\tfrac{3}{16}uG_{2,1}F_{2,2}+\tfrac{3}{64}uG_{2,1}G_{3,1}+21uF_{0,3}+6vF_{0,3}
+
\\
&
\ \ \ \ \
-6vG_{2,1}-\tfrac{3}{4}vG_{3,1}+\tfrac{1}{16}vG_{2,1}^2-3vF_{0,3}^2+\tfrac{1}{2}vF_{3,1}+\tfrac{1}{2}vG_{2,2}+\tfrac{3}{4}vG_{1,3}-\tfrac{1}{8}vF_{0,3}G_{2,1}
+
\\
&
\ \ \ \ \
+\tfrac{11}{2}uF_{0,3}G_{2,1}+\tfrac{15}{16}uF_{0,3}F_{1,3}+\tfrac{15}{4}xF_{0,3}-\tfrac{9}{4}yF_{0,3}+\tfrac{3}{8}vF_{0,3}F_{1,3}-\tfrac{3}{32}uG_{2,1}G_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{9}{8}uG_{1,3}+\tfrac{1}{4}vF_{0,3}F_{2,2}+\tfrac{21}{8}xG_{2,1}-\tfrac{3}{16}xG_{2,2}+\tfrac{27}{16}xF_{0,3}^2+\tfrac{1}{4}vF_{0,3}G_{0,4}-\tfrac{1}{2}vF_{0,3}F_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{1}{16}vF_{0,3}G_{3,1}+\tfrac{1}{16}vG_{2,1}G_{0,4}
-\tfrac{5}{4}uF_{0,3}F_{0,4}-\tfrac{3}{8}uG_{2,1}F_{0,4}+\tfrac{5}{8}uF_{0,3}G_{0,4}-\tfrac{1}{8}vG_{2,1}F_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{1}{64}vG_{2,1}G_{3,1}-\tfrac{5}{16}uF_{0,3}G_{2,2}+\tfrac{3}{16}uG_{2,1}G_{0,4}-\tfrac{3}{16}vF_{0,3}G_{1,3}-\tfrac{7}{16}xF_{3,1}-\tfrac{3}{64}vG_{2,1}G_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{9}{8}vF_{0,3}^3+6uF_{0,3}^2-\tfrac{3}{4}uF_{3,1}-\tfrac{3}{4}uG_{2,2}-\tfrac{1}{32}vG_{2,1}G_{2,2}-\tfrac{1}{8}yF_{2,2}+\tfrac{9}{16}xF_{1,3}+24u
+
\\
&
\ \ \ \ \
-2y+14x-48v+\tfrac{3}{8}xF_{2,2}-\tfrac{3}{2}vF_{1,3}+\tfrac{3}{2}uF_{2,2}
\Big)\partial_x
-
\endaligned
\]
\[
\aligned
&
-
\Big(
-1-\tfrac{5}{2}uG_{0,4}+5uF_{0,4}-\tfrac{7}{8}yG_{0,4}+\tfrac{7}{4}yF_{0,4}+\tfrac{45}{16}uF_{0,3}^3-\tfrac{9}{16}yF_{1,3}+\tfrac{3}{128}uG_{2,1}^3
+
\\
&
\ \ \ \ \
+\tfrac{9}{32}yG_{1,3}+\tfrac{7}{16}yF_{3,1}+\tfrac{3}{16}yG_{2,2}-\tfrac{3}{64}yG_{2,1}^2-\tfrac{27}{16}yF_{0,3}^2-\tfrac{15}{4}uF_{1,3}-\tfrac{7}{32}yG_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{3}{32}uG_{2,1}F_{3,1}-\tfrac{1}{8}vF_{0,3}F_{3,1}+\tfrac{57}{32}uF_{0,3}^2G_{2,1}+\tfrac{5}{8}uF_{0,3}F_{2,2}+\tfrac{1}{8}vF_{0,3}G_{2,1}^2+\tfrac{5}{32}uF_{0,3}G_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{5}{16}uF_{0,3}F_{3,1}+\tfrac{1}{16}vG_{2,1}F_{2,2}-\tfrac{9}{64}uG_{2,1}G_{1,3}-vF_{0,4}+\tfrac{1}{8}xG_{0,4}-\tfrac{1}{4}xF_{0,4}+\tfrac{5}{2}vG_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{15}{32}uF_{0,3}G_{1,3}-\tfrac{9}{16}yF_{0,3}G_{2,1}+\tfrac{9}{32}uG_{2,1}F_{1,3}+\tfrac{3}{16}xF_{0,3}G_{2,1}-\tfrac{1}{32}vG_{2,1}F_{3,1}+\tfrac{3}{32}vG_{2,1}F_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{23}{64}uF_{0,3}G_{2,1}^2-\tfrac{17}{2}uG_{2,1}-\tfrac{9}{8}uG_{3,1}+\tfrac{1}{4}uG_{2,1}^2+\tfrac{1}{2}vF_{2,2}-\tfrac{3}{32}xG_{1,3}-\tfrac{25}{8}yG_{2,1}+\tfrac{1}{128}vG_{2,1}^3
+
\\
&
\ \ \ \ \
+\tfrac{21}{32}vF_{0,3}^2G_{2,1}-\tfrac{1}{8}vF_{0,3}G_{2,2}+\tfrac{1}{32}xG_{3,1}+\tfrac{1}{64}xG_{2,1}^2+\tfrac{3}{16}uG_{2,1}F_{2,2}+\tfrac{3}{64}uG_{2,1}G_{3,1}
+
\\
&
\ \ \ \ \
-15uF_{0,3}+21vF_{0,3}+\tfrac{5}{2}vG_{2,1}+\tfrac{1}{8}vG_{3,1}+\tfrac{1}{4}vG_{2,1}^2+\tfrac{15}{4}vF_{0,3}^2-\tfrac{1}{4}vF_{3,1}-\tfrac{1}{4}vG_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{3}{8}vG_{1,3}+\tfrac{29}{8}vF_{0,3}G_{2,1}-2uF_{0,3}G_{2,1}+\tfrac{15}{16}uF_{0,3}F_{1,3}-\tfrac{3}{4}xF_{0,3}-\tfrac{15}{4}yF_{0,3}+\tfrac{3}{8}vF_{0,3}F_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{3}{32}uG_{2,1}G_{2,2}+\tfrac{15}{8}uG_{1,3}+\tfrac{1}{4}vF_{0,3}F_{2,2}+\tfrac{3}{8}xG_{2,1}-\tfrac{1}{16}xG_{2,2}+\tfrac{9}{16}xF_{0,3}^2+\tfrac{1}{4}vF_{0,3}G_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{1}{2}vF_{0,3}F_{0,4}+\tfrac{1}{16}vF_{0,3}G_{3,1}+\tfrac{1}{16}vG_{2,1}G_{0,4}-\tfrac{5}{4}uF_{0,3}F_{0,4}-\tfrac{3}{8}uG_{2,1}F_{0,4}+\tfrac{5}{8}uF_{0,3}G_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{1}{8}vG_{2,1}F_{0,4}+\tfrac{1}{64}vG_{2,1}G_{3,1}-\tfrac{5}{16}uF_{0,3}G_{2,2}+\tfrac{3}{16}uG_{2,1}G_{0,4}-\tfrac{3}{16}vF_{0,3}G_{1,3}-\tfrac{1}{16}xF_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{3}{64}vG_{2,1}G_{1,3}+\tfrac{9}{8}vF_{0,3}^3-3uF_{0,3}^2+\tfrac{5}{4}uF_{3,1}+\tfrac{5}{4}uG_{2,2}-\tfrac{1}{32}vG_{2,1}G_{2,2}-\tfrac{3}{8}yF_{2,2}+\tfrac{3}{16}xF_{1,3}
+
\\
&
\ \ \ \ \
-72u-14y+2x+8v+\tfrac{1}{8}xF_{2,2}+\tfrac{3}{4}vF_{1,3}-\tfrac{1}{2}uF_{2,2}
\Big)\partial_y
+
\endaligned
\]
\[
\aligned
&
+
\Big(
\tfrac{7}{4}uG_{0,4}-\tfrac{7}{2}uF_{0,4}+\tfrac{9}{8}uF_{1,3}+\tfrac{1}{4}vF_{0,4}-\tfrac{1}{8}vG_{0,4}+\tfrac{23}{4}uG_{2,1}+\tfrac{7}{16}uG_{3,1}+\tfrac{3}{32}uG_{2,1}^2
+
\\
&
\ \ \ \ \
-\tfrac{1}{8}vF_{2,2}+\tfrac{15}{2}uF_{0,3}+\tfrac{3}{4}vF_{0,3}-\tfrac{3}{8}vG_{2,1}-\tfrac{1}{32}vG_{3,1}-\tfrac{1}{64}vG_{2,1}^2-\tfrac{9}{16}vF_{0,3}^2+\tfrac{1}{16}vF_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{1}{16}vG_{2,2}+\tfrac{3}{32}vG_{1,3}-\tfrac{3}{16}vF_{0,3}G_{2,1}+\tfrac{9}{8}uF_{0,3}G_{2,1}-\tfrac{9}{16}uG_{1,3}+\tfrac{27}{8}uF_{0,3}^2-\tfrac{7}{8}uF_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{3}{8}uG_{2,2}+28u+x-2v-\tfrac{3}{16}vF_{1,3}+\tfrac{3}{4}uF_{2,2}
\Big)\partial_u
+
\endaligned
\]
\[
\aligned
&
\ \ \ \ \
-
\Big(
\tfrac{1}{2}uG_{0,4}-uF_{0,4}+\tfrac{3}{4}uF_{1,3}+\tfrac{7}{2}vF_{0,4}-\tfrac{7}{4}vG_{0,4}+\tfrac{7}{2}uG_{2,1}+\tfrac{1}{8}uG_{3,1}+\tfrac{1}{16}uG_{2,1}^2
+
\\
&
\ \ \ \ \
-\tfrac{3}{4}vF_{2,2}+3uF_{0,3}-\tfrac{15}{2}vF_{0,3}-\tfrac{25}{4}vG_{2,1}-\tfrac{7}{16}vG_{3,1}-\tfrac{3}{32}vG_{2,1}^2-\tfrac{27}{8}vF_{0,3}^2+\tfrac{7}{8}vF_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{3}{8}vG_{2,2}+\tfrac{9}{16}vG_{1,3}-\tfrac{9}{8}vF_{0,3}G_{2,1}+\tfrac{3}{4}uF_{0,3}G_{2,1}-\tfrac{3}{8}uG_{1,3}+\tfrac{9}{4}uF_{0,3}^2
+
\\
&
\ \ \ \ \
-\tfrac{1}{4}uF_{3,1}-\tfrac{1}{4}uG_{2,2}+24u-2y-28v-\tfrac{9}{8}vF_{1,3}+\tfrac{1}{2}uF_{2,2}
\Big)\partial_v.
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
A Gr\"obner basis has a lot of generators to describe the
moduli space core algebraic variety in 
$\R^{12} \ni F_{0,3},G_{2,1},F_{0,4},G_{0,4},F_{4,0},G_{4,0},F_{1,3},G_{1,3},F_{3,1},G_{3,1},F_{2,2},G_{2,2}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 &
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(
14
+
\tfrac{3}{4}F_{0,3}G_{2,1}
+
\tfrac{1}{16}G_{2,1}^2
+
\tfrac{9}{4}F_{0,3}^2
+
\tfrac{1}{2}F_{1,3}
+
\tfrac{7}{4}G_{2,1}
-
\tfrac{1}{4}G_{2,2}
+
\tfrac{1}{2}F_{2,2}
+
\tfrac{3}{2}F_{0,3}
+
\tfrac{1}{8}G_{3,1}
-
\tfrac{1}{4}F_{3,1}
-
\tfrac{1}{4}G_{1,3}
+
\tfrac{7}{8}G_{0,4}
+
\tfrac{1}{8}G_{4,0}
-
\tfrac{1}{4}F_{4,0}
-
\tfrac{7}{4}F_{0,4}
)e_1
+
(
-
22
-
\tfrac{3}{4}F_{0,3}G_{2,1}
-
\tfrac{1}{16}G_{2,1}^2
-
\tfrac{9}{4}F_{0,3}^2
+
\tfrac{1}{4}F_{1,3}
+
\tfrac{15}{4}G_{2,1}
+
\tfrac{1}{4}G_{2,2}
-
\tfrac{1}{2}F_{2,2}
+
\tfrac{27}{2}F_{0,3}
+
\tfrac{1}{4}G_{3,1}
-
\tfrac{1}{2}F_{3,1}
-
\tfrac{1}{8}G_{1,3}
-
\tfrac{1}{8}G_{0,4}
-
\tfrac{7}{8}G_{4,0}
+
\tfrac{7}{4}F_{4,0}
+
\tfrac{1}{4}F_{0,4}
)e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
	\begin{tabular}{p{7cm}}
	$
	-
	(
	14
	+
	\tfrac{3}{4}F_{0,3}G_{2,1}
	+
	\tfrac{1}{16}G_{2,1}^2
	+
	\tfrac{9}{4}F_{0,3}^2
	+
	\tfrac{1}{2}F_{1,3}
	+
	\tfrac{7}{4}G_{2,1}
	-
	\tfrac{1}{4}G_{2,2}
	+
	\tfrac{1}{2}F_{2,2}
	+
	\tfrac{3}{2}F_{0,3}
	+
	\tfrac{1}{8}G_{3,1}
	-
	\tfrac{1}{4}F_{3,1}
	-
	\tfrac{1}{4}G_{1,3}
	+
	\tfrac{7}{8}G_{0,4}
	+
	\tfrac{1}{8}G_{4,0}
	-
	\tfrac{1}{4}F_{4,0}
	-
	\tfrac{7}{4}F_{0,4}
	)e_1
	+
	(
	-
	22
	-
	\tfrac{3}{4}F_{0,3}G_{2,1}
	-
	\tfrac{1}{16}G_{2,1}^2
	-
	\tfrac{9}{4}F_{0,3}^2
	+
	\tfrac{1}{4}F_{1,3}
	+
	\tfrac{15}{4}G_{2,1}
	+
	\tfrac{1}{4}G_{2,2}
	-
	\tfrac{1}{2}F_{2,2}
	+
	\tfrac{27}{2}F_{0,3}
	+
	\tfrac{1}{4}G_{3,1}
	-
	\tfrac{1}{2}F_{3,1}
	-
	\tfrac{1}{8}G_{1,3}
	-
	\tfrac{1}{8}G_{0,4}
	-
	\tfrac{7}{8}G_{4,0}
	+
	\tfrac{7}{4}F_{4,0}
	+
	\tfrac{1}{4}F_{0,4}
	)e_2$
	\end{tabular}}
& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
\text{A lot of terms at order 5}
,
\\
v
&
\,=\,
\text{A lot of terms at order 5},
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
\,:=\,
\text{A lot of terms}
, &
e_2
\,:=\,
\text{A lot of terms}.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
A Gr\"obner basis has many generators to describe the
moduli space core algebraic variety in 
$\R^{12} \ni F_{0,3},G_{2,1},G_{0,4},F_{0,4},
F_{4,0},G_{4,0},F_{1,3},G_{1,3},F_{3,1},G_{3,1},F_{2,2},G_{2,2}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 &
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(\tfrac{9}{8}F_{0,3}^2
+
\tfrac{1}{32}G_{2,1}^2
+
\tfrac{3}{8}F_{0,3}G_{2,1}
+
G_{0,4}
+
\tfrac{1}{4}G_{4,0}
+
\tfrac{1}{4}F_{1,3}
-
\tfrac{1}{8}G_{2,2}
+
\tfrac{1}{4}F_{2,2}
-
9F_{0,3}
+
\tfrac{1}{4}G_{3,1}
-
\tfrac{1}{2}F_{3,1}
-
\tfrac{1}{8}G_{1,3}
-
\tfrac{1}{2}F_{4,0}
-
2F_{0,4}
)e_1
+
(
-
8
-
\tfrac{9}{8}F_{0,3}^2
-
\tfrac{1}{32}G_{2,1}^2
-
\tfrac{3}{8}F_{0,3}G_{2,1}
-
\tfrac{1}{4}G_{0,4}
-
G_{4,0}
+
\tfrac{1}{2}F_{1,3}
+
G_{2,1}
+
\tfrac{1}{8}G_{2,2}
-
\tfrac{1}{4}F_{2,2}
-
3F_{0,3}
+
\tfrac{1}{8}G_{3,1}
-
\tfrac{1}{4}F_{3,1}
-
\tfrac{1}{4}G_{1,3}
+
2F_{4,0}
+
\tfrac{1}{2}F_{0,4})e_2
$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
-
(
\tfrac{9}{8}F_{0,3}^2
+
\tfrac{1}{32}G_{2,1}^2
+
\tfrac{3}{8}F_{0,3}G_{2,1}
+
G_{0,4}
+
\tfrac{1}{4}G_{4,0}
+
\tfrac{1}{4}F_{1,3}
-
\tfrac{1}{8}G_{2,2}
+
\tfrac{1}{4}F_{2,2}
-
9F_{0,3}
+
\tfrac{1}{4}G_{3,1}
-
\tfrac{1}{2}F_{3,1}
-
\tfrac{1}{8}G_{1,3}
-
\tfrac{1}{2}F_{4,0}
-
2F_{0,4}
)e_1
+
(
-
8
-
\tfrac{9}{8}F_{0,3}^2
-
\tfrac{1}{32}G_{2,1}^2
-
\tfrac{3}{8}F_{0,3}G_{2,1}
-
\tfrac{1}{4}G_{0,4}
-
G_{4,0}
+
\tfrac{1}{2}F_{1,3}
+
G_{2,1}
+
\tfrac{1}{8}G_{2,2}
-
\tfrac{1}{4}F_{2,2}
-
3F_{0,3}
+
\tfrac{1}{8}G_{3,1}
-
\tfrac{1}{4}F_{3,1}
-
\tfrac{1}{4}G_{1,3}
+
2F_{4,0}
+
\tfrac{1}{2}F_{0,4})e_2
$
\end{tabular}}
& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
\text{A lot of terms at order 5}
,
\\
v
&
\,=\,
\text{A lot of terms at order 5}
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
\,:=\,
\text{A lot of terms}
, &
e_2
\,:=\,
\text{A lot of terms}.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
A Gr\"obner basis has 92 generators to describe the
moduli space core algebraic variety in 
$\R^9 \ni _{0,3},F_{0,4},G_{0,4},
G_{4,0},F_{1,3},G_{1,3},G_{3,1},F_{2,2},G_{2,2}$.
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 &
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(
-
\tfrac{577}{36}
+
\tfrac{11}{432}F_{0,3}F_{2,2}
-
\tfrac{5}{24}F_{0,3}F_{0,4}
+
\tfrac{5}{192}F_{0,3}G_{3,1}
-
\tfrac{11}{576}F_{0,3}G_{1,3}
-
\tfrac{1}{72}F_{0,3}F_{1,3}
+
\tfrac{1}{216}F_{0,3}G_{2,2}
-
\tfrac{23}{48}F_{0,3}^3
+
\tfrac{175}{144}F_{0,3}^2
+
\tfrac{233}{54}F_{0,3}
+
\tfrac{1}{48}F_{1,3}
-
\tfrac{65}{144}F_{2,2}
+
\tfrac{73}{192}G_{1,3}
+
\tfrac{7}{144}G_{2,2}
-
\tfrac{71}{192}G_{3,1}
+
\tfrac{21}{8}F_{0,4}
-
\tfrac{1}{12}G_{0,4}
-
\tfrac{1}{4}G_{4,0}
)e_1
+
(
\tfrac{1097}{36}
-
\tfrac{187}{432}F_{0,3}F_{2,2}
+
\tfrac{85}{24}F_{0,3}F_{0,4}
-
\tfrac{85}{192}F_{0,3}G_{3,1}
+
\tfrac{187}{576}F_{0,3}G_{1,3}
+
\tfrac{17}{72}F_{0,3}F_{1,3}
-
\tfrac{17}{216}F_{0,3}G_{2,2}
+
\tfrac{391}{48}F_{0,3}^3
+
\tfrac{2209}{144}F_{0,3}^2
-
\tfrac{1369}{54}F_{0,3}
-
\tfrac{17}{48}F_{1,3}
+
\tfrac{97}{144}F_{2,2}
-
\tfrac{89}{192}G_{1,3}
-
\tfrac{47}{144}G_{2,2}
+
\tfrac{55}{192}G_{3,1}
-
\tfrac{21}{8}F_{0,4}
+
\tfrac{17}{12}G_{0,4}
+
\tfrac{5}{4}G_{4,0}
)e_2
$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
-
(
-
\tfrac{577}{36}
+
\tfrac{11}{432}F_{0,3}F_{2,2}
-
\tfrac{5}{24}F_{0,3}F_{0,4}
+
\tfrac{5}{192}F_{0,3}G_{3,1}
-
\tfrac{11}{576}F_{0,3}G_{1,3}
-
\tfrac{1}{72}F_{0,3}F_{1,3}
+
\tfrac{1}{216}F_{0,3}G_{2,2}
-
\tfrac{23}{48}F_{0,3}^3
+
\tfrac{175}{144}F_{0,3}^2
+
\tfrac{233}{54}F_{0,3}
+
\tfrac{1}{48}F_{1,3}
-
\tfrac{65}{144}F_{2,2}
+
\tfrac{73}{192}G_{1,3}
+
\tfrac{7}{144}G_{2,2}
-
\tfrac{71}{192}G_{3,1}
+
\tfrac{21}{8}F_{0,4}
-
\tfrac{1}{12}G_{0,4}
-
\tfrac{1}{4}G_{4,0}
)e_1
+
(
\tfrac{1097}{36}
-
\tfrac{187}{432}F_{0,3}F_{2,2}
+
\tfrac{85}{24}F_{0,3}F_{0,4}
-
\tfrac{85}{192}F_{0,3}G_{3,1}
+
\tfrac{187}{576}F_{0,3}G_{1,3}
+
\tfrac{17}{72}F_{0,3}F_{1,3}
-
\tfrac{17}{216}F_{0,3}G_{2,2}
+
\tfrac{391}{48}F_{0,3}^3
+
\tfrac{2209}{144}F_{0,3}^2
-
\tfrac{1369}{54}F_{0,3}
-
\tfrac{17}{48}F_{1,3}
+
\tfrac{97}{144}F_{2,2}
-
\tfrac{89}{192}G_{1,3}
-
\tfrac{47}{144}G_{2,2}
+
\tfrac{55}{192}G_{3,1}
-
\tfrac{21}{8}F_{0,4}
+
\tfrac{17}{12}G_{0,4}
+
\tfrac{5}{4}G_{4,0}
)e_2
$
\end{tabular}}
& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3d}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+2x^3+
(
-2+\tfrac{1}{2}F_{2,2}-\tfrac{1}{4}G_{3,1}-\tfrac{3}{4}G_{4,0}+\tfrac{1}{2}F_{3,1}-\tfrac{1}{4}G_{0,4}
)y^4
+
(
16
+
\\
&
\ \ \ \ \
-F_{2,2}+2F_{4,0}+\tfrac{1}{2}G_{3,1}+\tfrac{3}{2}G_{4,0}+\tfrac{1}{2}G_{0,4}
)xy^3
+
F_{2,2}x^2y^2+F_{3,1}x^3y
+
\\
&
\ \ \ \ \
+F_{4,0}x^4
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2+8xy^2-4x^2y+G_{0,4}y^4
+
(
G_{3,1}+2G_{4,0}-2G_{0,4}
)xy^3
+
\\
&
\ \ \ \ \
+
(
64+F_{2,2}+6F_{4,0}-\tfrac{3}{2}G_{3,1}-\tfrac{3}{2}G_{4,0}+\tfrac{3}{2}G_{0,4}+3F_{3,1}
)x^2y^2
+
\\
&
\ \ \ \ \
+
G_{3,1}x^3y+G_{4,0}x^4
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(
1+32u-16v+\tfrac{1}{3}xF_{2,2}-\tfrac{8}{3}xF_{4,0}-\tfrac{2}{3}xG_{0,4}+\tfrac{1}{12}xG_{3,1}+\tfrac{2}{3}xG_{4,0}+\tfrac{1}{6}yF_{2,2}-\tfrac{1}{3}yF_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{1}{12}yG_{0,4}-\tfrac{1}{12}yG_{3,1}+\tfrac{1}{12}yG_{4,0}+vF_{2,2}-2vF_{4,0}-\tfrac{1}{2}vG_{0,4}-\tfrac{1}{2}vG_{3,1}-\tfrac{3}{2}vG_{4,0}
+
\\
&
\ \ \ \ \
-4uF_{4,0}-2uG_{0,4}-\tfrac{1}{2}uG_{3,1}+2uG_{4,0}+\tfrac{8}{3}y+\tfrac{4}{3}x
)\partial_x
-
(
-\tfrac{4}{3}uG_{3,1}-\tfrac{2}{3}uG_{4,0}-\tfrac{1}{6}xF_{2,2}
+
\\
&
\ \ \ \ \
+\tfrac{1}{3}xF_{4,0}+\tfrac{1}{12}xG_{0,4}+\tfrac{1}{12}xG_{3,1}-\tfrac{1}{12}xG_{4,0}-\tfrac{1}{3}yF_{2,2}+\tfrac{8}{3}yF_{4,0}+\tfrac{2}{3}yG_{0,4}-\tfrac{1}{12}yG_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{2}{3}yG_{4,0}+\tfrac{2}{3}vF_{2,2}-\tfrac{4}{3}vF_{4,0}-\tfrac{4}{3}vG_{0,4}+\tfrac{1}{6}vG_{3,1}+\tfrac{4}{3}vG_{4,0}-\tfrac{16}{3}uF_{4,0}-\tfrac{4}{3}uG_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{8}{3}uF_{2,2}+3uF_{3,1}+\tfrac{32}{3}u+\tfrac{8}{3}y+\tfrac{10}{3}x+\tfrac{32}{3}v
)\partial_y
+
(
-\tfrac{4}{3}u+\tfrac{8}{3}v+\tfrac{1}{6}vF_{2,2}-\tfrac{1}{3}vF_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{1}{12}vG_{0,4}-\tfrac{1}{12}vG_{3,1}+\tfrac{1}{12}vG_{4,0}+\tfrac{2}{3}uF_{2,2}-\tfrac{16}{3}uF_{4,0}-\tfrac{4}{3}uG_{0,4}+\tfrac{1}{6}uG_{3,1}+\tfrac{4}{3}uG_{4,0}
+
\\
&
\ \ \ \ \
+y
)\partial_u
+
(
-\tfrac{28}{3}u+\tfrac{8}{3}v+\tfrac{2}{3}vF_{2,2}-\tfrac{16}{3}vF_{4,0}-\tfrac{4}{3}vG_{0,4}+\tfrac{1}{6}vG_{3,1}+\tfrac{4}{3}vG_{4,0}+\tfrac{2}{3}uF_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{4}{3}uF_{4,0}-\tfrac{1}{3}uG_{0,4}-\tfrac{1}{3}uG_{3,1}+\tfrac{1}{3}uG_{4,0}+2x
)\partial_v
,
\\
e_2
&
\,:=\,
-(
-\tfrac{3}{2}uG_{3,1}-\tfrac{3}{2}uG_{4,0}+\tfrac{2}{3}xF_{2,2}-\tfrac{4}{3}xG_{0,4}-\tfrac{1}{2}xG_{3,1}-xG_{4,0}+\tfrac{1}{3}yF_{2,2}-\tfrac{1}{6}yG_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{1}{4}yG_{3,1}-\tfrac{1}{2}yG_{4,0}+2vF_{2,2}-vG_{0,4}-vG_{3,1}-3vG_{4,0}+6uF_{4,0}-\tfrac{5}{2}uG_{0,4}+\tfrac{7}{6}xF_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{1}{3}yF_{3,1}+2vF_{3,1}+uF_{2,2}+4uF_{3,1}+64u+\tfrac{4}{3}y+\tfrac{14}{3}x-8v
)\partial_x
+
(
1-\tfrac{7}{2}uG_{3,1}
+
\\
&
\ \ \ \ \
-8uG_{4,0}-\tfrac{1}{3}xF_{2,2}+\tfrac{1}{6}xG_{0,4}+\tfrac{1}{4}xG_{3,1}+\tfrac{1}{2}xG_{4,0}-\tfrac{2}{3}yF_{2,2}+\tfrac{4}{3}yG_{0,4}+\tfrac{1}{2}yG_{3,1}
+
\\
&
\ \ \ \ \
+yG_{4,0}+\tfrac{4}{3}vF_{2,2}-\tfrac{8}{3}vG_{0,4}-vG_{3,1}-2vG_{4,0}-\tfrac{8}{3}uG_{0,4}-\tfrac{1}{3}xF_{3,1}-\tfrac{7}{6}yF_{3,1}+\tfrac{4}{3}vF_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{10}{3}uF_{2,2}+\tfrac{16}{3}uF_{3,1}+\tfrac{16}{3}u-\tfrac{20}{3}y-\tfrac{4}{3}x+\tfrac{16}{3}v
)\partial_y
+
\\
&
\ \ \ \ \
-
(
1-\tfrac{7}{2}uG_{3,1}-8uG_{4,0}-\tfrac{1}{3}xF_{2,2}+\tfrac{1}{6}xG_{0,4}+\tfrac{1}{4}xG_{3,1}+\tfrac{1}{2}xG_{4,0}-\tfrac{2}{3}yF_{2,2}+\tfrac{4}{3}yG_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{1}{2}yG_{3,1}+yG_{4,0}+\tfrac{4}{3}vF_{2,2}-\tfrac{8}{3}vG_{0,4}-vG_{3,1}-2vG_{4,0}-\tfrac{8}{3}uG_{0,4}-\tfrac{1}{3}xF_{3,1}-\tfrac{7}{6}yF_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{4}{3}vF_{3,1}+\tfrac{10}{3}uF_{2,2}+\tfrac{16}{3}uF_{3,1}+\tfrac{16}{3}u-\tfrac{20}{3}y-\tfrac{4}{3}x+\tfrac{16}{3}v
)\partial_u
+
\\
&
\ \ \ \ \
-
(
-\tfrac{32}{3}u+\tfrac{40}{3}v+\tfrac{7}{3}vF_{3,1}+\tfrac{4}{3}uF_{2,2}-uG_{3,1}-2uG_{4,0}-\tfrac{2}{3}uG_{0,4}+\tfrac{4}{3}uF_{3,1}+\tfrac{4}{3}vF_{2,2}
+
\\
&
\ \ \ \ \
-vG_{3,1}-2vG_{4,0}-\tfrac{8}{3}vG_{0,4}-2y
)\partial_v.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^6 \ni F_{2,2},F_{3,1},G_{3,1},G_{0,4},F_{4,0},G_{4,0}$:
\[
\aligned
\B_1 
&
:= 2F_{2,2}+8+2F_{3,1}-4F_{4,0}-3G_{0,4}-G_{3,1}-G_{4,0},
\\
\B_2 
&
:= -2F_{3,1}G_{3,1}+8F_{3,1}G_{4,0}-8F_{4,0}G_{3,1}+32F_{4,0}G_{4,0}+2G_{0,4}^2+G_{0,4}G_{3,1}-8G_{0,4}G_{4,0}
+
\\
&
\ \ \ \ \
+G_{3,1}^2-G_{3,1}G_{4,0}-10G_{4,0}^2+152F_{3,1}+608F_{4,0}-92G_{0,4}-84G_{3,1}-52G_{4,0}+2080,
\\
\B_3 
&
:= 2F_{3,1}G_{0,4}-2F_{3,1}G_{3,1}+6F_{3,1}G_{4,0}+8F_{4,0}G_{0,4}-8F_{4,0}G_{3,1}+24F_{4,0}G_{4,0}-8G_{0,4}G_{4,0}
+
\\
&
\ \ \ \ \
+G_{3,1}^2-8G_{4,0}^2+120F_{3,1}+480F_{4,0}-44G_{0,4}-76G_{3,1}-68G_{4,0}+1568,
\\
\B_4 
&
:= (8F_{4,0}+G_{3,1}-8G_{4,0}-104)(8F_{4,0}+2F_{3,1}-G_{0,4}-3G_{4,0}+24-G_{3,1}),
\\
\B_5 
&
:= 4F_{3,1}^2-8F_{3,1}G_{3,1}+16F_{3,1}G_{4,0}-64F_{4,0}^2+16F_{4,0}G_{0,4}-16F_{4,0}G_{3,1}+112F_{4,0}G_{4,0}
+
\\
&
\ \ \ \ \
+2G_{0,4}G_{3,1}-16G_{0,4}G_{4,0}+3G_{3,1}^2-2G_{3,1}G_{4,0}-32G_{4,0}^2+480F_{3,1}+1536F_{4,0}
+
\\
&
\ \ \ \ \
-200G_{0,4}-280G_{3,1}-344G_{4,0}+5312,
\\
\B_6 &
:= (G_{3,1}^2-8G_{3,1}G_{4,0}+16G_{4,0}^2-124G_{3,1}+560G_{4,0}+4512)
\\
&
\ \ \ \ \ \
(8F_{4,0}+2F_{3,1}-G_{0,4}-3G_{4,0}+24-G_{3,1}).
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(
-\tfrac{22}{3}-\tfrac{5}{6}F_{2,2}+\tfrac{7}{12}G_{3,1}+\tfrac{11}{12}G_{4,0}+\tfrac{17}{12}G_{0,4}-\tfrac{7}{6}F_{3,1}+\tfrac{1}{3}F_{4,0}
)e_1
+
(
\tfrac{4}{3}-\tfrac{2}{3}F_{2,2}+\tfrac{1}{6}G_{3,1}-\tfrac{1}{6}G_{4,0}+\tfrac{5}{6}G_{0,4}-\tfrac{1}{3}F_{3,1}+\tfrac{8}{3}F_{4,0}
)e_2
$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
-
(
-\tfrac{22}{3}-\tfrac{5}{6}F_{2,2}+\tfrac{7}{12}G_{3,1}+\tfrac{11}{12}G_{4,0}+\tfrac{17}{12}G_{0,4}-\tfrac{7}{6}F_{3,1}+\tfrac{1}{3}F_{4,0}
)e_1
-
(
\tfrac{4}{3}-\tfrac{2}{3}F_{2,2}+\tfrac{1}{6}G_{3,1}-\tfrac{1}{6}G_{4,0}+\tfrac{5}{6}G_{0,4}-\tfrac{1}{3}F_{3,1}+\tfrac{8}{3}F_{4,0}
)e_2
$
\end{tabular}}
& 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3e}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+2y^3
+
(
-8+\tfrac{1}{2}F_{3,1}-\tfrac{1}{4}G_{0,4}+\tfrac{1}{2}F_{2,2}-\tfrac{1}{4}G_{3,1}-\tfrac{3}{4}G_{4,0}
)y^4
+
\\
&
\ \ \ \ \
+
(
4+2F_{4,0}+\tfrac{1}{2}G_{0,4}+\tfrac{1}{2}G_{3,1}+\tfrac{3}{2}G_{4,0}-F_{2,2}
)xy^3
+
F_{2,2}x^2y^2
+
\\
&
\ \ \ \ \
+F_{3,1}x^3y+F_{4,0}x^4
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2-4xy^2+8x^2y+G_{0,4}y^4
+
(
-2G_{0,4}+G_{3,1}+2G_{4,0}
)xy^3
+
\\
&
\ \ \ \ \
+
(
28+6F_{4,0}+\tfrac{3}{2}G_{0,4}-\tfrac{3}{2}G_{3,1}-\tfrac{3}{2}G_{4,0}+F_{2,2}+3F_{3,1}
)x^2y^2
+
\\
&
\ \ \ \ \
+
G_{3,1}x^3y+G_{4,0}x^4
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1
&
\,:=\,
-(-1-\tfrac{80}{3}u-\tfrac{32}{3}v-\tfrac{1}{2}xF_{2,2}+\tfrac{1}{12}xG_{3,1}+\tfrac{7}{3}xF_{4,0}+\tfrac{7}{12}xG_{0,4}-\tfrac{7}{12}xG_{4,0}+\tfrac{2}{3}yF_{4,0}
+
\\
&
\ \ \ \ \
+\tfrac{1}{6}yG_{0,4}-\tfrac{1}{12}yG_{3,1}-\tfrac{1}{6}yG_{4,0}+2uF_{2,2}+\tfrac{5}{6}uG_{3,1}-\tfrac{32}{3}uF_{4,0}-\tfrac{5}{3}uG_{0,4}+\tfrac{5}{3}uG_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{8}{3}vF_{4,0}-\tfrac{2}{3}vG_{0,4}+\tfrac{1}{3}vG_{3,1}+\tfrac{8}{3}vG_{4,0}+\tfrac{8}{3}y+\tfrac{34}{3}x)\partial_x+(-32u+\tfrac{1}{2}yF_{2,2}-3uF_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{1}{12}xG_{3,1}-\tfrac{2}{3}xF_{4,0}-\tfrac{1}{6}xG_{0,4}+\tfrac{1}{6}xG_{4,0}-\tfrac{7}{3}yF_{4,0}-\tfrac{7}{12}yG_{0,4}-\tfrac{1}{12}yG_{3,1}+\tfrac{7}{12}yG_{4,0}
+
\\
&
\ \ \ \ \
+uG_{3,1}-8uF_{4,0}-2uG_{0,4}+4uG_{4,0}-4vF_{4,0}-\tfrac{28}{3}y-\tfrac{8}{3}x)\partial_y+(uF_{2,2}+y-\tfrac{1}{6}uG_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{14}{3}uF_{4,0}-\tfrac{62}{3}u-\tfrac{7}{6}uG_{0,4}+\tfrac{7}{6}uG_{4,0}-\tfrac{2}{3}vF_{4,0}-\tfrac{8}{3}v-\tfrac{1}{6}vG_{0,4}+\tfrac{1}{12}vG_{3,1}+\tfrac{1}{6}vG_{4,0})\partial_u
+
\\
&
\ \ \ \ \
+(2x+\tfrac{16}{3}u-\tfrac{8}{3}uF_{4,0}-\tfrac{2}{3}uG_{0,4}+\tfrac{1}{3}uG_{3,1}+\tfrac{2}{3}uG_{4,0}-\tfrac{68}{3}v+vF_{2,2}-\tfrac{1}{6}vG_{3,1}-\tfrac{14}{3}vF_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{7}{6}vG_{0,4}+\tfrac{7}{6}vG_{4,0})\partial_v
,
\\
e_2
&
\,:=\,
(-\tfrac{196}{3}u-\tfrac{64}{3}v+\tfrac{7}{6}xG_{0,4}+\tfrac{3}{4}xG_{3,1}+\tfrac{3}{2}xG_{4,0}-xF_{2,2}-\tfrac{4}{3}xF_{3,1}-\tfrac{1}{6}yF_{3,1}+\tfrac{1}{3}yG_{0,4}
+
\\
&
\ \ \ \ \
-6uF_{4,0}-\tfrac{1}{2}vG_{3,1}-\tfrac{29}{6}uG_{0,4}-\tfrac{3}{2}uG_{3,1}-\tfrac{9}{2}uG_{4,0}+3uF_{2,2}+\tfrac{8}{3}uF_{3,1}+\tfrac{2}{3}vF_{3,1}-\tfrac{4}{3}vG_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{56}{3}x-\tfrac{2}{3}y)\partial_x-(-64u-1-\tfrac{3}{4}yG_{3,1}-\tfrac{3}{2}yG_{4,0}+yF_{2,2}-\tfrac{1}{3}xG_{0,4}+\tfrac{1}{6}xF_{3,1}+\tfrac{4}{3}yF_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{7}{6}yG_{0,4}-4uG_{0,4}-\tfrac{1}{2}uG_{3,1}+2uF_{2,2}+2uF_{3,1}+vF_{3,1}-\tfrac{16}{3}x-\tfrac{68}{3}y)\partial_y-(-x-\tfrac{124}{3}u
+
\\
&
\ \ \ \ \
-\tfrac{7}{3}uG_{0,4}-\tfrac{3}{2}uG_{3,1}-3uG_{4,0}+2uF_{2,2}+\tfrac{8}{3}uF_{3,1}+\tfrac{1}{6}vF_{3,1}-\tfrac{1}{3}vG_{0,4}-\tfrac{16}{3}v)\partial_u-(-2y
+
\\
&
\ \ \ \ \
-\tfrac{4}{3}u+\tfrac{2}{3}uF_{3,1}-\tfrac{4}{3}uG_{0,4}-\tfrac{136}{3}v-\tfrac{7}{3}vG_{0,4}-\tfrac{3}{2}vG_{3,1}-3vG_{4,0}+2vF_{2,2}+\tfrac{8}{3}vF_{3,1})\partial_v
.
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^6 \ni F_{2,2},F_{3,1},F_{4,0},G_{0,4},G_{3,1},G_{4,0}$:
\[
\aligned
\B_1 & := 2F_{2,2}-48-3G_{0,4}-G_{4,0}+2F_{3,1}-4F_{4,0}-G_{3,1},
\\
\B_2 & := 2F_{3,1}G_{3,1}-8F_{3,1}G_{4,0}+8F_{4,0}G_{3,1}-32F_{4,0}G_{4,0}+4G_{0,4}^2+G_{0,4}G_{3,1}-12G_{0,4}G_{4,0}
+
\\
&
\ \ \ \ \
-G_{3,1}^2-G_{3,1}G_{4,0}+24G_{4,0}^2+40F_{3,1}+160F_{4,0}+116G_{0,4}+28G_{3,1}-132G_{4,0}+832,
\\
\B_3 & := 4F_{3,1}G_{0,4}-2F_{3,1}G_{3,1}+4F_{3,1}G_{4,0}+16F_{4,0}G_{0,4}-8F_{4,0}G_{3,1}+16F_{4,0}G_{4,0}-3G_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \
-4G_{0,4}G_{4,0}+G_{3,1}^2+3G_{3,1}G_{4,0}-12G_{4,0}^2+24F_{3,1}+96F_{4,0}-4G_{0,4}-44G_{3,1}
+
\\
&
\ \ \ \ \
-44G_{4,0}-64,
\\
\B_4 & := (16F_{4,0}-G_{3,1}-4G_{4,0}-12)(8F_{4,0}+2F_{3,1}+G_{0,4}-G_{3,1}-5G_{4,0}+16),
\\
\B_5 & := 4F_{3,1}^2-2F_{3,1}G_{3,1}-8F_{3,1}G_{4,0}-64F_{4,0}^2-16F_{4,0}G_{0,4}+8F_{4,0}G_{3,1}+48F_{4,0}G_{4,0}
+
\\
&
\ \ \ \ \
+G_{0,4}G_{3,1}+4G_{0,4}G_{4,0}-G_{3,1}G_{4,0}-4G_{4,0}^2+56F_{3,1}-32F_{4,0}+20G_{0,4}-4G_{3,1}
+
\\
&
\ \ \ \ \
-36G_{4,0}+320,
\\
\B_6 & := (G_{3,1}^2-8G_{3,1}G_{4,0}+16G_{4,0}^2+48G_{3,1}+64G_{4,0}-80)(8F_{4,0}+2F_{3,1}+G_{0,4}-G_{3,1}-5G_{4,0}+16).
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(
\tfrac{64}{3}+\tfrac{4}{3}G_{0,4}+\tfrac{2}{3}G_{3,1}+\tfrac{4}{3}G_{4,0}-F_{2,2}-\tfrac{4}{3}F_{3,1}+\tfrac{2}{3}F_{4,0}
)e_1
+
(
\tfrac{44}{3}+\tfrac{11}{12}G_{0,4}+\tfrac{1}{12}G_{3,1}-\tfrac{7}{12}G_{4,0}-\tfrac{1}{2}F_{2,2}-\tfrac{1}{6}F_{3,1}+\tfrac{7}{3}F_{4,0}
)e_2
$
\end{tabular}}
\\
e_2 & 
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
-(
\tfrac{64}{3}+\tfrac{4}{3}G_{0,4}+\tfrac{2}{3}G_{3,1}+\tfrac{4}{3}G_{4,0}-F_{2,2}-\tfrac{4}{3}F_{3,1}+\tfrac{2}{3}F_{4,0}
)e_1
+
-(
\tfrac{44}{3}+\tfrac{11}{12}G_{0,4}+\tfrac{1}{12}G_{3,1}-\tfrac{7}{12}G_{4,0}-\tfrac{1}{2}F_{2,2}-\tfrac{1}{6}F_{3,1}+\tfrac{7}{3}F_{4,0}
)e_2
$
\end{tabular}}
& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\[
\!\!\!\!\!
\text{\bf Model 2f3f4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3
+
(\tfrac{-3}{2}+\tfrac{1}{2}F_{2,2}-G_{4,0})x^4
+
(-4+F_{2,2}-G_{4,0})x^3y+F_{2,2}x^2y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(-4+F_{2,2}-G_{4,0})xy^3
+
(\tfrac{-3}{2}+\tfrac{1}{2}F_{2,2}-G_{4,0})y^4
+
(\tfrac{-29}{10}-\tfrac{3}{10}F_{2,2}+\tfrac{16}{5}G_{4,0}+
\\
&
\,\,\,\,\,\,\,\,
-F_{2,2}G_{4,0}
+\tfrac{1}{5}F_{2,2}^2+\tfrac{6}{5}G_{4,0}^2)x^5
+
(\tfrac{1}{2}F_{2,2}^2-2F_{2,2}G_{4,0}+\tfrac{3}{2}G_{4,0}^2-F_{2,2}+\tfrac{17}{2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,-\tfrac{1}{2})x^4y
+
(\tfrac{2}{3}F_{2,2}^2-2F_{2,2}G_{4,0}+\tfrac{7}{3}F_{2,2}-\tfrac{4}{3}G_{4,0}-17)x^3y^2
+
(F_{2,2}^2-4F_{2,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+3G_{4,0}^2+2F_{2,2}+G_{4,0}-19)x^2y^3
+
(\tfrac{-7}{2}-\tfrac{3}{2}F_{2,2}+12G_{4,0}-5F_{2,2}G_{4,0}+F_{2,2}^2
+
\\
&
\,\,\,\,\,\,\,\,
+6G_{4,0}^2)xy^4
+
(\tfrac{-29}{10}-\tfrac{3}{10}F_{2,2}+\tfrac{16}{5}G_{4,0}-F_{2,2}G_{4,0}+\tfrac{1}{5}F_{2,2}^2+\tfrac{6}{5}G_{4,0}^2)y^5
+
\cdots
,\\
v
& 
\,=\,
x^2+y^2+2x^2y+2xy^2+G_{4,0}x^4
+
(2F_{2,2}-4-2G_{4,0})x^3y
+
(-14+4F_{2,2}
+
\\
&
\,\,\,\,\,\,\,\,
-6G_{4,0})x^2y^2
+
(2F_{2,2}-4-2G_{4,0})xy^3
+
G_{4,0}y^4
+
(\tfrac{2}{5}F_{2,2}G_{4,0}-\tfrac{6}{5}G_{4,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{9}{5}F_{2,2}-\tfrac{12}{5}G_{4,0}-\tfrac{27}{5})x^5
+
(F_{2,2}^2-4F_{2,2}G_{4,0}+3G_{4,0}^2+4F_{2,2}-G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-27)x^4y
+
(\tfrac{8}{3}F_{2,2}^2-12F_{2,2}G_{4,0}+12G_{4,0}^2-\tfrac{14}{3}F_{2,2}+\tfrac{92}{3}G_{4,0}-14)x^3y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(2F_{2,2}^2-8F_{2,2}G_{4,0}+6G_{4,0}^2-4F_{2,2}+26G_{4,0}-10)x^2y^3
+
(2F_{2,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-6G_{4,0}^2+5F_{2,2}-8G_{4,0}-21)xy^4
+
(\tfrac{2}{5}F_{2,2}G_{4,0}-\tfrac{6}{5}G_{4,0}^2+\tfrac{9}{5}F_{2,2}-\tfrac{12}{5}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{27}{5})y^5
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := 
-
(F_{2,2}u+F_{2,2}x+G_{4,0}u+2G_{4,0}v-3G_{4,0}x-2u-5v-x-3y-1)\partial_x
-
(3F_{2,2}u
+
\\
&
\,\,\,\,\,\,\,\,
+F_{2,2}v+F_{2,2}y-5G_{4,0}u-G_{4,0}v-3G_{4,0}y-4u-4v)\partial_y
-
(2F_{2,2}u-6G_{4,0}u-u
+
\\
&
\,\,\,\,\,\,\,\,
-3v-y)\partial_u
-
(2F_{2,2}v-6G_{4,0}v-10u-2v-2x)\partial_v,\\
e_2 & := 
-
(3F_{2,2}u+F_{2,2}v+F_{2,2}x-5G_{4,0}u-G_{4,0}v-3G_{4,0}x-10u-v-3x+3y)\partial_x
+
\\
&
\,\,\,\,\,\,\,\,
-
(F_{2,2}u+F_{2,2}y+G_{4,0}u+2G_{4,0}v-3G_{4,0}y-8u-2v-4y-1)\partial_y
-
(2F_{2,2}u
+
\\
&
\,\,\,\,\,\,\,\,
-6G_{4,0}u-7u-x)\partial_u
-
(2F_{2,2}v-6G_{4,0}v+2u-8v-2y)\partial_v,\\
e_3 & := 
-
(2u-v+x-y)\partial_x
-
(2u-v-x+y)\partial_y
-
(2u-v)\partial_u
+
(4u-2v)\partial_v,
\endaligned
\]
with $F_{2,2},G_{4,0}$ satisfying:
\[
0 = F_{2,2}^2-6F_{2,2}G_{4,0}+9G_{4,0}^2-F_{2,2}+7G_{4,0}-6,
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 
0 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{6cm}}
$(-F_{2,2}+3G_{4,0})e_1+(F_{2,2}-3G_{4,0})e_2+(3F_{2,2}-9G_{4,0})e_3$
\end{tabular}}
&
-e_1+e_2+3e_3
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{6cm}}
$-(-F_{2,2}+3G_{4,0})e_1-(F_{2,2}-3G_{4,0})e_2-(3F_{2,2}-9G_{4,0})e_3$
\end{tabular}}
&
e_1-e_2-3e_3
\\
e_3 &
e_1-e_2-3e_3& -e_1+e_2+3e_3& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3f4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3
+
(-\tfrac{1}{40}G_{3,2}-\tfrac{1}{10}G_{4,0}+\tfrac{1}{4}G_{5,0})x^4
+
(\tfrac{-2}{3}-\tfrac{1}{20}G_{3,2}+\tfrac{4}{5}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{2}G_{5,0})x^3y
+
(\tfrac{7}{3}-\tfrac{1}{20}G_{3,2}+\tfrac{9}{5}G_{4,0}+\tfrac{1}{2}G_{5,0})x^2y^2
+
(\tfrac{-2}{3}-\tfrac{1}{20}G_{3,2}+\tfrac{4}{5}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{2}G_{5,0})xy^3
+
(-\tfrac{1}{40}G_{3,2}-\tfrac{1}{10}G_{4,0}+\tfrac{1}{4}G_{5,0})y^4
+
(\tfrac{-259}{135}-\tfrac{59}{450}G_{3,2}+\tfrac{63}{25}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{1200}G_{3,2}^2+\tfrac{1}{12}G_{5,0}^2+\tfrac{1}{50}G_{3,2}G_{4,0}-\tfrac{1}{60}G_{3,2}G_{5,0}-\tfrac{1}{5}G_{4,0}G_{5,0}+\tfrac{73}{90}G_{5,0})x^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(\tfrac{1}{3}+\tfrac{1}{4}G_{3,2}+2G_{4,0})x^4y
+
(\tfrac{-122}{27}-\tfrac{68}{45}G_{3,2}+\tfrac{42}{5}G_{4,0}+\tfrac{1}{120}G_{3,2}^2+\tfrac{5}{6}G_{5,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{5}G_{3,2}G_{4,0}-\tfrac{1}{6}G_{3,2}G_{5,0}-2G_{4,0}G_{5,0}+\tfrac{91}{9}G_{5,0})x^3y^2
+
(\tfrac{4}{3}+\tfrac{3}{10}G_{3,2}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{24}{5}G_{4,0}+2G_{5,0})x^2y^3
+
(-\tfrac{59}{90}G_{3,2}+\tfrac{43}{5}G_{4,0}+\tfrac{1}{240}G_{3,2}^2+\tfrac{5}{12}G_{5,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{10}G_{3,2}G_{4,0}-\tfrac{1}{12}G_{3,2}G_{5,0}-G_{4,0}G_{5,0}+\tfrac{73}{18}G_{5,0}-\tfrac{70}{27})xy^4
+
(\tfrac{-4}{3}+\tfrac{1}{20}G_{3,2}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{6}{5}G_{4,0})y^5
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2+2x^2y+2xy^2+G_{4,0}x^4
+
(\tfrac{4}{3}-\tfrac{1}{10}G_{3,2}+\tfrac{8}{5}G_{4,0}+G_{5,0})x^3y
+
\\
&
\,\,\,\,\,\,\,\,
+
(-\tfrac{2}{3}-\tfrac{1}{5}G_{3,2}+\tfrac{6}{5}G_{4,0}+2G_{5,0})x^2y^2
+
(\tfrac{4}{3}-\tfrac{1}{10}G_{3,2}+\tfrac{8}{5}G_{4,0}+G_{5,0})xy^3
+
\\
&
\,\,\,\,\,\,\,\,
+
G_{4,0}y^4+G_{5,0}x^5
+
(\tfrac{1}{120}G_{3,2}^2+\tfrac{5}{6}G_{5,0}^2+\tfrac{1}{5}G_{3,2}G_{4,0}-\tfrac{1}{6}G_{3,2}G_{5,0}-2G_{4,0}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{29}{18}G_{3,2}+\tfrac{100}{9}G_{5,0}-140}{27+10G_{4,0})x^4y
+
G_{3,2}x^3y^2
+
(\tfrac{-316}{27}-\tfrac{118}{45}G_{3,2}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{132}{5}G_{4,0}+\tfrac{1}{60}G_{3,2}^2+\tfrac{5}{3}G_{5,0}^2+\tfrac{2}{5}G_{3,2}G_{4,0}-\tfrac{1}{3}G_{3,2}G_{5,0}-4G_{4,0}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{146}{9}G_{5,0})x^2y^3
+
(\tfrac{2}{3}+\tfrac{1}{5}G_{3,2}-\tfrac{16}{5}G_{4,0}+3G_{5,0})xy^4
+
(\tfrac{-158}{135}-\tfrac{163}{450}G_{3,2}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{66}{25}G_{4,0}+\tfrac{1}{600}G_{3,2}^2+\tfrac{1}{6}G_{5,0}^2+\tfrac{1}{25}G_{3,2}G_{4,0}-\tfrac{1}{30}G_{3,2}G_{5,0}-\tfrac{2}{5}G_{4,0}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,+\tfrac{118}{45}G_{5,0})y^5
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1 & := 
(1-\tfrac{1}{5}uG_{3,2}G_{5,0}-\tfrac{1}{10}xG_{3,2}G_{5,0}+\tfrac{1}{10}vG_{3,2}G_{5,0}+\tfrac{1}{10}yG_{3,2}G_{5,0}-\tfrac{9}{100}yG_{3,2}G_{4,0}+\tfrac{9}{50}uG_{3,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{9}{10}vG_{4,0}G_{5,0}+\tfrac{9}{10}yG_{4,0}G_{5,0}-\tfrac{9}{5}uG_{4,0}G_{5,0}-\tfrac{9}{100}vG_{3,2}G_{4,0}+\tfrac{9}{100}xG_{3,2}G_{4,0}-\tfrac{9}{10}xG_{4,0}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{32}{9}u+\tfrac{43}{9}y-\tfrac{37}{9}x+\tfrac{61}{9}v+uG_{5,0}^2+\tfrac{149}{120}yG_{3,2}-\tfrac{59}{12}yG_{5,0}-\tfrac{107}{10}yG_{4,0}+\tfrac{18}{25}yG_{4,0}^2+\tfrac{1}{100}uG_{3,2}^2
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{73}{30}uG_{3,2}+\tfrac{28}{3}uG_{5,0}+\tfrac{93}{5}uG_{4,0}-\tfrac{36}{25}uG_{4,0}^2-\tfrac{1}{200}vG_{3,2}^2-\tfrac{1}{2}vG_{5,0}^2+\tfrac{149}{120}vG_{3,2}-\tfrac{59}{12}vG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{127}{10}vG_{4,0}+\tfrac{18}{25}vG_{4,0}^2-\tfrac{18}{25}xG_{4,0}^2+\tfrac{53}{12}xG_{5,0}+\tfrac{1}{200}xG_{3,2}^2-\tfrac{1}{200}yG_{3,2}^2-\tfrac{143}{120}xG_{3,2}-\tfrac{1}{2}yG_{5,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{119}{10}xG_{4,0}+\tfrac{1}{2}xG_{5,0}^2)\partial_x
+
(-\tfrac{1}{5}uG_{3,2}G_{5,0}+\tfrac{1}{10}xG_{3,2}G_{5,0}+\tfrac{1}{10}vG_{3,2}G_{5,0}-\tfrac{1}{10}yG_{3,2}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{9}{100}yG_{3,2}G_{4,0}+\tfrac{9}{50}uG_{3,2}G_{4,0}+\tfrac{9}{10}vG_{4,0}G_{5,0}-\tfrac{9}{10}yG_{4,0}G_{5,0}-\tfrac{9}{5}uG_{4,0}G_{5,0}-\tfrac{9}{100}vG_{3,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{9}{100}xG_{3,2}G_{4,0}+\tfrac{9}{10}xG_{4,0}G_{5,0}-\tfrac{86}{9}u-\tfrac{46}{9}y+\tfrac{16}{9}x+\tfrac{28}{9}v+uG_{5,0}^2-\tfrac{143}{120}yG_{3,2}+\tfrac{53}{12}yG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{119}{10}yG_{4,0}-\tfrac{18}{25}yG_{4,0}^2+\tfrac{1}{100}uG_{3,2}^2-\tfrac{7}{3}uG_{3,2}+\tfrac{25}{3}uG_{5,0}+21uG_{4,0}-\tfrac{36}{25}uG_{4,0}^2-\tfrac{1}{200}vG_{3,2}^2
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{1}{2}vG_{5,0}^2+\tfrac{31}{24}vG_{3,2}-\tfrac{65}{12}vG_{5,0}-\tfrac{23}{2}vG_{4,0}+\tfrac{18}{25}vG_{4,0}^2+\tfrac{18}{25}xG_{4,0}^2-\tfrac{59}{12}xG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{1}{200}xG_{3,2}^2+\tfrac{1}{200}yG_{3,2}^2+\tfrac{149}{120}xG_{3,2}+\tfrac{1}{2}yG_{5,0}^2-\tfrac{107}{10}xG_{4,0}-\tfrac{1}{2}xG_{5,0}^2)\partial_y
+
(-\tfrac{83}{9}u+\tfrac{43}{9}v
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{100}uG_{3,2}^2+uG_{5,0}^2-\tfrac{143}{60}uG_{3,2}+\tfrac{53}{6}uG_{5,0}+\tfrac{119}{5}uG_{4,0}-\tfrac{36}{25}uG_{4,0}^2-\tfrac{1}{200}vG_{3,2}^2-\tfrac{1}{2}vG_{5,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{149}{120}vG_{3,2}-\tfrac{59}{12}vG_{5,0}-\tfrac{107}{10}vG_{4,0}+\tfrac{18}{25}vG_{4,0}^2+\tfrac{9}{50}uG_{3,2}G_{4,0}-\tfrac{1}{5}uG_{3,2}G_{5,0}-\tfrac{9}{5}uG_{4,0}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{9}{100}vG_{3,2}G_{4,0}+\tfrac{1}{10}vG_{3,2}G_{5,0}+\tfrac{9}{10}vG_{4,0}G_{5,0}+y)\partial_u
-
(-\tfrac{154}{9}u+\tfrac{74}{9}v+\tfrac{1}{50}uG_{3,2}^2+2uG_{5,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{149}{30}uG_{3,2}+\tfrac{59}{3}uG_{5,0}+\tfrac{214}{5}uG_{4,0}-\tfrac{72}{25}uG_{4,0}^2-\tfrac{1}{100}vG_{3,2}^2-vG_{5,0}^2+\tfrac{143}{60}vG_{3,2}-\tfrac{53}{6}vG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{119}{5}vG_{4,0}+\tfrac{36}{25}vG_{4,0}^2+\tfrac{9}{25}uG_{3,2}G_{4,0}-\tfrac{2}{5}uG_{3,2}G_{5,0}-\tfrac{18}{5}uG_{4,0}G_{5,0}-\tfrac{9}{50}vG_{3,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{5}vG_{3,2}G_{5,0}+\tfrac{9}{5}vG_{4,0}G_{5,0}-2x)\partial_v,\\
e_2 & := 
-
(-\tfrac{3}{10}uG_{3,2}G_{5,0}-\tfrac{3}{20}xG_{3,2}G_{5,0}+\tfrac{3}{20}vG_{3,2}G_{5,0}+\tfrac{3}{20}yG_{3,2}G_{5,0}-\tfrac{21}{100}yG_{3,2}G_{4,0}+\tfrac{21}{50}uG_{3,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{21}{10}vG_{4,0}G_{5,0}+\tfrac{21}{10}yG_{4,0}G_{5,0}-\tfrac{21}{5}uG_{4,0}G_{5,0}-\tfrac{21}{100}vG_{3,2}G_{4,0}+\tfrac{21}{100}xG_{3,2}G_{4,0}-\tfrac{21}{10}xG_{4,0}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-8u+7y-\tfrac{11}{3}x+\tfrac{17}{3}v+\tfrac{3}{2}uG_{5,0}^2+\tfrac{59}{40}yG_{3,2}-\tfrac{29}{4}yG_{5,0}-\tfrac{91}{10}yG_{4,0}-\tfrac{18}{25}yG_{4,0}^2+\tfrac{3}{200}uG_{3,2}^2
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{31}{10}uG_{3,2}+16uG_{5,0}+\tfrac{93}{5}uG_{4,0}+\tfrac{36}{25}uG_{4,0}^2-\tfrac{3}{400}vG_{3,2}^2-\tfrac{3}{4}vG_{5,0}^2+\tfrac{57}{40}vG_{3,2}-\tfrac{27}{4}vG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{83}{10}vG_{4,0}-\tfrac{18}{25}vG_{4,0}^2+\tfrac{18}{25}xG_{4,0}^2+\tfrac{31}{4}xG_{5,0}+\tfrac{3}{400}xG_{3,2}^2-\tfrac{3}{400}yG_{3,2}^2-\tfrac{61}{40}xG_{3,2}-\tfrac{3}{4}yG_{5,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{79}{10}xG_{4,0}+\tfrac{3}{4}xG_{5,0}^2)\partial_x
-
(-1-\tfrac{3}{10}uG_{3,2}G_{5,0}+\tfrac{3}{20}xG_{3,2}G_{5,0}+\tfrac{3}{20}vG_{3,2}G_{5,0}-\tfrac{3}{20}yG_{3,2}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{21}{100}yG_{3,2}G_{4,0}+\tfrac{21}{50}uG_{3,2}G_{4,0}+\tfrac{21}{10}vG_{4,0}G_{5,0}-\tfrac{21}{10}yG_{4,0}G_{5,0}-\tfrac{21}{5}uG_{4,0}G_{5,0}-\tfrac{21}{100}vG_{3,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{21}{100}xG_{3,2}G_{4,0}+\tfrac{21}{10}xG_{4,0}G_{5,0}-14u-\tfrac{14}{3}y+4x+2v+\tfrac{3}{2}uG_{5,0}^2-\tfrac{61}{40}yG_{3,2}+\tfrac{31}{4}yG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{79}{10}yG_{4,0}+\tfrac{18}{25}yG_{4,0}^2+\tfrac{3}{200}uG_{3,2}^2-3uG_{3,2}+15uG_{5,0}+21uG_{4,0}+\tfrac{36}{25}uG_{4,0}^2-\tfrac{3}{400}vG_{3,2}^2
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{3}{4}vG_{5,0}^2+\tfrac{59}{40}vG_{3,2}-\tfrac{29}{4}vG_{5,0}-\tfrac{71}{10}vG_{4,0}-\tfrac{18}{25}vG_{4,0}^2-\tfrac{18}{25}xG_{4,0}^2-\tfrac{29}{4}xG_{5,0}-\tfrac{3}{400}xG_{3,2}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{3}{400}yG_{3,2}^2+\tfrac{59}{40}xG_{3,2}+\tfrac{3}{4}yG_{5,0}^2-\tfrac{91}{10}xG_{4,0}-\tfrac{3}{4}xG_{5,0}^2)\partial_y
-
(-\tfrac{25}{3}u+4v+\tfrac{3}{200}uG_{3,2}^2+\tfrac{3}{2}uG_{5,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{31}{2}uG_{5,0}-\tfrac{61}{20}uG_{3,2}+\tfrac{79}{5}uG_{4,0}+\tfrac{36}{25}uG_{4,0}^2-\tfrac{3}{400}vG_{3,2}^2-\tfrac{3}{4}vG_{5,0}^2-\tfrac{29}{4}vG_{5,0}+\tfrac{59}{40}vG_{3,2}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{91}{10}vG_{4,0}-\tfrac{18}{25}vG_{4,0}^2+\tfrac{21}{50}uG_{3,2}G_{4,0}-\tfrac{3}{10}uG_{3,2}G_{5,0}-\tfrac{21}{5}uG_{4,0}G_{5,0}-\tfrac{21}{100}vG_{3,2}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{3}{20}vG_{3,2}G_{5,0}+\tfrac{21}{10}vG_{4,0}G_{5,0}-x)\partial_u
+
(-18u+\tfrac{28}{3}v+\tfrac{3}{100}uG_{3,2}^2+3uG_{5,0}^2+29uG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{59}{10}uG_{3,2}+\tfrac{182}{5}uG_{4,0}+\tfrac{72}{25}uG_{4,0}^2-\tfrac{3}{200}vG_{3,2}^2-\tfrac{3}{2}vG_{5,0}^2-\tfrac{31}{2}vG_{5,0}+\tfrac{61}{20}vG_{3,2}-\tfrac{79}{5}vG_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{36}{25}vG_{4,0}^2+\tfrac{21}{25}uG_{3,2}G_{4,0}-\tfrac{3}{5}uG_{3,2}G_{5,0}-\tfrac{42}{5}uG_{4,0}G_{5,0}-\tfrac{21}{50}vG_{3,2}G_{4,0}+\tfrac{3}{10}vG_{3,2}G_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{21}{5}vG_{4,0}G_{5,0}+2y)\partial_v
\endaligned
\]
with $G_{3,2},G_{4,0},G_{5,0}$ satisfying:
\[
\aligned
0 & = 9G_{3,2}^2+432G_{3,2}G_{4,0}-180G_{3,2}G_{5,0}+5184G_{4,0}^2-4320G_{4,0}G_{5,0}+900G_{5,0}^2-1020G_{3,2}
+
\\
&
\,\,\,\,\,\,\,\,
-10080G_{4,0}+10200G_{5,0}+4000,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(\tfrac{-10}{9}-\tfrac{3}{25}G_{3,2}G_{4,0}+\tfrac{1}{20}G_{3,2}G_{5,0}+\tfrac{6}{5}G_{4,0}G_{5,0}-\tfrac{1}{400}G_{3,2}^2-\tfrac{1}{4}G_{5,0}^2-\tfrac{36}{25}G_{4,0}^2+\tfrac{17}{60}G_{3,2}+\tfrac{14}{5}G_{4,0}-\tfrac{17}{6}G_{5,0})e_1+(\tfrac{10}{9}+\tfrac{3}{25}G_{3,2}G_{4,0}-\tfrac{1}{20}G_{3,2}G_{5,0}-\tfrac{6}{5}G_{4,0}G_{5,0}+\tfrac{1}{400}G_{3,2}^2+\tfrac{1}{4}G_{5,0}^2+\tfrac{36}{25}G_{4,0}^2-\tfrac{17}{60}G_{3,2}-\tfrac{14}{5}G_{4,0}+\tfrac{17}{6}G_{5,0})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(\tfrac{-10}{9}-\tfrac{3}{25}G_{3,2}G_{4,0}+\tfrac{1}{20}G_{3,2}G_{5,0}+\tfrac{6}{5}G_{4,0}G_{5,0}-\tfrac{1}{400}G_{3,2}^2-\tfrac{1}{4}G_{5,0}^2-\tfrac{36}{25}G_{4,0}^2+\tfrac{17}{60}G_{3,2}+\tfrac{14}{5}G_{4,0}-\tfrac{17}{6}G_{5,0})e_1-(\tfrac{10}{9}+\tfrac{3}{25}G_{3,2}G_{4,0}-\tfrac{1}{20}G_{3,2}G_{5,0}-\tfrac{6}{5}G_{4,0}G_{5,0}+\tfrac{1}{400}G_{3,2}^2+\tfrac{1}{4}G_{5,0}^2+\tfrac{36}{25}G_{4,0}^2-\tfrac{17}{60}G_{3,2}-\tfrac{14}{5}G_{4,0}+\tfrac{17}{6}G_{5,0})e_2$
\end{tabular}}
&
0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\!\!\!\!\!
\text{\bf Model 2f3f4c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3
+
(\tfrac{2}{3}+\tfrac{1}{2}F_{3,1}-\tfrac{1}{2}G_{4,0})x^4
+
F_{3,1}x^3y
+
(5+F_{3,1}+G_{4,0})x^2y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
F_{3,1}xy^3
+
(\tfrac{2}{3}+\tfrac{1}{2}F_{3,1}-\tfrac{1}{2}G_{4,0})y^4
+
(\tfrac{11}{15}+\tfrac{34}{15}F_{3,1}+\tfrac{13}{15}G_{4,0}+\tfrac{1}{5}F_{3,1}^2
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{2}{5}F_{3,1}G_{4,0}-\tfrac{1}{2}G_{5,0})x^5
+
(-5-5F_{3,1}+6G_{4,0}+\tfrac{5}{2}G_{5,0})x^4y
+
(30+\tfrac{80}{3}F_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{34}{3}G_{4,0}+2F_{3,1}^2-4F_{3,1}G_{4,0}-5G_{5,0})x^3y^2
+
(-\tfrac{52}{3}-6F_{3,1}+5G_{5,0})x^2y^3
+
\\
&
\,\,\,\,\,\,\,\,
+
(\tfrac{56}{3}+\tfrac{34}{3}F_{3,1}+\tfrac{1}{3}G_{4,0}+F_{3,1}^2-2F_{3,1}G_{4,0}-\tfrac{5}{2}G_{5,0})xy^4
+
(-4-F_{3,1}+2G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{2}G_{5,0})y^5
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2+2x^2y+2xy^2+G_{4,0}x^4
+
(2F_{3,1}+\tfrac{16}{3})x^3y
+
(4F_{3,1}+2-2G_{4,0})x^2y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(2F_{3,1}+\tfrac{16}{3})xy^3
+
G_{4,0}y^4+G_{5,0}x^5
+
(\tfrac{88}{3}+\tfrac{86}{3}F_{3,1}-\tfrac{34}{3}G_{4,0}+2F_{3,1}^2
+
\\
&
\,\,\,\,\,\,\,\,
-4F_{3,1}G_{4,0}-5G_{5,0})x^4y
+
(-20F_{3,1}-\tfrac{104}{3}+16G_{4,0}+10G_{5,0})x^3y^2
+
(60
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{136}{3}F_{3,1}-\tfrac{20}{3}G_{4,0}+4F_{3,1}^2-8F_{3,1}G_{4,0}-10G_{5,0})x^2y^3
+
(-18-4F_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
+5G_{5,0})xy^4
+
(\tfrac{142}{15}+\tfrac{98}{15}F_{3,1}-\tfrac{34}{15}G_{4,0}+\tfrac{2}{5}F_{3,1}^2-\tfrac{4}{5}F_{3,1}G_{4,0}-G_{5,0})y^5
+
\cdots
,
\endaligned\right.
\]
for any value for $G_{5,0}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1 & := 
-
(-1-3vF_{3,1}G_{4,0}+3xF_{3,1}G_{4,0}+6F_{3,1}G_{4,0}u-3yF_{3,1}G_{4,0}+\tfrac{142}{3}u-25y+25x-27v
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{15}{2}yG_{4,0}-6xG_{4,0}^2-\tfrac{11}{2}vG_{4,0}+\tfrac{29}{2}xF_{3,1}-\tfrac{15}{2}xG_{5,0}+\tfrac{11}{2}xG_{4,0}+\tfrac{15}{2}vG_{5,0}+6vG_{4,0}^2-\tfrac{27}{2}yF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{15}{2}yG_{5,0}-12G_{4,0}^2u+28F_{3,1}u+17G_{4,0}u-15G_{5,0}u+6yG_{4,0}^2-\tfrac{27}{2}vF_{3,1})\partial_x
-
(\tfrac{11}{2}yG_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+6xG_{4,0}^2-\tfrac{15}{2}vG_{4,0}-\tfrac{27}{2}xF_{3,1}+\tfrac{15}{2}xG_{5,0}-\tfrac{15}{2}xG_{4,0}+\tfrac{15}{2}vG_{5,0}+6vG_{4,0}^2+\tfrac{29}{2}yF_{3,1}-\tfrac{15}{2}yG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-12G_{4,0}^2u+30F_{3,1}u+13G_{4,0}u-15G_{5,0}u-6yG_{4,0}^2-\tfrac{25}{2}vF_{3,1}+52u+26y-22x-\tfrac{64}{3}v
+
\\
&
\,\,\,\,\,\,\,\,
-3vF_{3,1}G_{4,0}+6F_{3,1}G_{4,0}u-3xF_{3,1}G_{4,0}+3yF_{3,1}G_{4,0})\partial_y
-
(-25v+51u-\tfrac{27}{2}vF_{3,1}-\tfrac{15}{2}vG_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{15}{2}vG_{5,0}+6vG_{4,0}^2-12G_{4,0}^2u+29F_{3,1}u+11G_{4,0}u-15G_{5,0}u-3vF_{3,1}G_{4,0}+6F_{3,1}G_{4,0}u
+
\\
&
\,\,\,\,\,\,\,\,
-y)\partial_u
+
(12F_{3,1}G_{4,0}u-6F_{3,1}G_{4,0}v-24G_{4,0}^2u+12G_{4,0}^2v+54F_{3,1}u-29F_{3,1}v+30G_{4,0}u
+
\\
&
\,\,\,\,\,\,\,\,
-11G_{4,0}v-30G_{5,0}u+15G_{5,0}v+98u-50v+2x)\partial_v,\\
e_2 & := 
(-3yF_{3,1}^2+3xF_{3,1}^2+6F_{3,1}^2u-3vF_{3,1}^2+9vF_{3,1}G_{4,0}-9xF_{3,1}G_{4,0}-18F_{3,1}G_{4,0}u+9yF_{3,1}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+90u-49y+45x-\tfrac{149}{3}v+\tfrac{49}{2}yG_{4,0}+6xG_{4,0}^2+\tfrac{49}{2}vG_{4,0}+\tfrac{69}{2}xF_{3,1}-\tfrac{15}{2}xG_{5,0}-\tfrac{45}{2}xG_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{15}{2}vG_{5,0}-6vG_{4,0}^2-\tfrac{71}{2}yF_{3,1}+\tfrac{15}{2}yG_{5,0}+12G_{4,0}^2u+68F_{3,1}u-47G_{4,0}u-15G_{5,0}u-6yG_{4,0}^2
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{73}{2}vF_{3,1})\partial_x
+
(1+3yF_{3,1}^2-3xF_{3,1}^2+6F_{3,1}^2u-3vF_{3,1}^2+9vF_{3,1}G_{4,0}+9xF_{3,1}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-18F_{3,1}G_{4,0}u-9yF_{3,1}G_{4,0}+\tfrac{284}{3}u+46y-46x-44v-\tfrac{45}{2}yG_{4,0}-6xG_{4,0}^2+\tfrac{45}{2}vG_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{71}{2}xF_{3,1}+\tfrac{15}{2}xG_{5,0}+\tfrac{49}{2}xG_{4,0}+\tfrac{15}{2}vG_{5,0}-6vG_{4,0}^2+\tfrac{69}{2}yF_{3,1}-\tfrac{15}{2}yG_{5,0}+12G_{4,0}^2u+70F_{3,1}u
+
\\
&
\,\,\,\,\,\,\,\,
-51G_{4,0}u-15G_{5,0}u+6yG_{4,0}^2-\tfrac{71}{2}vF_{3,1})\partial_y
+
(-46v+91u-\tfrac{71}{2}vF_{3,1}+\tfrac{49}{2}vG_{4,0}+\tfrac{15}{2}vG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-3vF_{3,1}^2-6vG_{4,0}^2+6F_{3,1}^2u+12G_{4,0}^2u+69F_{3,1}u-45G_{4,0}u-15G_{5,0}u+9vF_{3,1}G_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-18F_{3,1}G_{4,0}u+x)\partial_u
-
(12F_{3,1}^2u-6F_{3,1}^2v-36F_{3,1}G_{4,0}u+18F_{3,1}G_{4,0}v+24G_{4,0}^2u
+
\\
&
\,\,\,\,\,\,\,\,
-12G_{4,0}^2v+142F_{3,1}u-69F_{3,1}v-98G_{4,0}u+45G_{4,0}v-30G_{5,0}u+15G_{5,0}v+186u
+
\\
&
\,\,\,\,\,\,\,\,
-92v-2y)\partial_v,
\endaligned
\]
with $F_{3,1},G_{4,0}$ satisfying:
\[
\aligned
0 = 3F_{3,1}^2-12F_{3,1}G_{4,0}+12G_{4,0}^2+21F_{3,1}-30G_{4,0}+20,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 &
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(3F_{3,1}^2-12F_{3,1}G_{4,0}+12G_{4,0}^2+21F_{3,1}-30G_{4,0}+20)e_1+(-3F_{3,1}^2+12F_{3,1}G_{4,0}-12G_{4,0}^2-21F_{3,1}+30G_{4,0}-20)e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(3F_{3,1}^2-12F_{3,1}G_{4,0}+12G_{4,0}^2+21F_{3,1}-30G_{4,0}+20)e_1-(-3F_{3,1}^2+12F_{3,1}G_{4,0}-12G_{4,0}^2-21F_{3,1}+30G_{4,0}-20)e_2$
\end{tabular}}
&
0
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3f4da}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
yx+x^3+y^3-\tfrac{1}{16}x^4-\tfrac{1}{4}yx^3
+
\tfrac{41}{8}y^2x^2+\tfrac{3}{4}y^3x-\tfrac{9}{16}y^4-\tfrac{1}{8}x^5+8yx^4
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{11}{4}y^2x^3-5y^3x^2+\tfrac{43}{8}y^4x+3y^5+\tfrac{249}{64}x^6+\tfrac{89}{32}yx^5-\tfrac{921}{64}y^2x^4+\tfrac{495}{16}y^3x^3
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1879}{64}y^4x^2-\tfrac{167}{32}y^5x-\tfrac{343}{64}y^6
+
\cdots
,
\\
v
&
\,=\,x^2+y^2+2yx^2+2y^2x+\tfrac{9}{8}x^4+\tfrac{9}{2}yx^3-\tfrac{1}{4}y^2x^2+\tfrac{5}{2}y^3x+\tfrac{17}{8}y^4+\tfrac{5}{2}x^5
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{3}{4}yx^4+7y^2x^3+\tfrac{37}{2}y^3x^2+\tfrac{5}{2}y^4x-\tfrac{7}{4}y^5-\tfrac{17}{32}x^6+\tfrac{111}{16}yx^5+\tfrac{1505}{32}y^2x^4
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{89}{8}y^3x^3-\tfrac{287}{32}y^4x^2+\tfrac{271}{16}y^5x+\tfrac{367}{32}y^6
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1 & := 
(\tfrac{1}{2}y+\tfrac{1}{4}v+1+x)\partial_x
-
(7v\tfrac{1}{4}+5x\tfrac{1}{2})\partial_y
+
(y+u+\tfrac{1}{2}v)\partial_u
+
(2x+2v)\partial_v,\\
e_2 & := 
(u-7y\tfrac{1}{2}-15v\tfrac{1}{4}+4x)\partial_x
+
(1+3u+5y-11v\tfrac{1}{4}-\tfrac{1}{2}x)\partial_y
+
\\
&
\,\,\,\,\,\,\,\,
+
(x+9u-\tfrac{1}{2}v)\partial_u
-
(-2y+4u-10v)\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & \tfrac{7}{2}e_1-\tfrac{1}{2}e_2
\\
e_2 &
-\tfrac{7}{2}e_1+\tfrac{1}{2}e_2 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3f4db}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
yx+x^3+y^3+\tfrac{3}{32}x^4+\tfrac{1}{8}yx^3+\tfrac{65}{16}y^2x^2+\tfrac{9}{8}y^3x-\tfrac{13}{32}y^4-\tfrac{1}{16}x^5+\tfrac{37}{8}yx^4
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{37}{8}y^2x^3+y^3x^2+\tfrac{15}{16}y^4x+\tfrac{23}{8}y^5+\tfrac{99}{64}x^6+\tfrac{195}{32}yx^5+\tfrac{417}{64}y^2x^4+\tfrac{81}{16}y^3x^3
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{933}{64}y^4x^2+\tfrac{507}{32}y^5x-\tfrac{489}{64}y^6
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2+2yx^2+2y^2x+\tfrac{13}{16}x^4+\tfrac{15}{4}yx^3+\tfrac{15}{8}y^2x^2+\tfrac{7}{4}y^3x+\tfrac{29}{16}y^4+\tfrac{7}{4}x^5
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{31}{8}yx^4+6y^2x^3+\tfrac{37}{4}y^3x^2+\tfrac{37}{4}y^4x-\tfrac{17}{8}y^5+\tfrac{65}{32}x^6+\tfrac{105}{16}yx^5+\tfrac{515}{32}y^2x^4
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{315}{8}y^3x^3+\tfrac{615}{32}y^4x^2-\tfrac{223}{16}y^5x+\tfrac{469}{32}y^6
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := (y+\tfrac{11}{8}v+1-\tfrac{1}{2}x+\tfrac{3}{4}u)\partial_x-(\tfrac{3}{2}y+\tfrac{7}{8}v+2x+\tfrac{11}{4}u)\partial_y-(-y+2u-v)\partial_u+(2x+2u-v)\partial_v,\\
e_2 & := (\tfrac{1}{4}u-4y-\tfrac{31}{8}v+\tfrac{7}{2}x)\partial_x+(1+\tfrac{23}{4}u+\tfrac{9}{2}y-\tfrac{21}{8}v-x)\partial_y+(x+8u-v)\partial_u-(-2y+6u-9v)\partial_v.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 &
0 & \tfrac{5}{2}e_1+\tfrac{1}{2}e_2
\\
e_2 &
-\tfrac{5}{2}e_1-\tfrac{1}{2}e_2 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3f4ea}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
yx+x^3+y^3-\tfrac{9}{16}x^4+\tfrac{3}{4}yx^3+\tfrac{41}{8}y^2x^2-\tfrac{1}{4}y^3x-\tfrac{1}{16}y^4+3x^5+\tfrac{43}{8}yx^4
+
\\
&
\,\,\,\,\,\,\,\,
-5y^2x^3+\tfrac{11}{4}y^3x^2+8y^4x-\tfrac{1}{8}y^5-\tfrac{343}{64}x^6-\tfrac{167}{32}yx^5+\tfrac{1879}{64}y^2x^4+\tfrac{495}{16}y^3x^3
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{921}{64}y^4x^2+\tfrac{89}{32}y^5x+\tfrac{249}{64}y^6
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2+2yx^2+2y^2x+\tfrac{17}{8}x^4+\tfrac{5}{2}yx^3-\tfrac{1}{4}y^2x^2+\tfrac{9}{2}y^3x+\tfrac{9}{8}y^4-\tfrac{7}{4}x^5
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{5}{2}yx^4+\tfrac{37}{2}y^2x^3+7y^3x^2-\tfrac{3}{4}y^4x+\tfrac{5}{2}y^5+\tfrac{367}{32}x^6+\tfrac{271}{16}yx^5-\tfrac{287}{32}y^2x^4
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{89}{8}y^3x^3+\tfrac{1505}{32}y^4x^2+\tfrac{111}{16}y^5x-\tfrac{17}{32}y^6
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := (5x+1-\tfrac{1}{2}y+3u-11v\tfrac{1}{4})\partial_x+(-7x\tfrac{1}{2}+4y+u-15v\tfrac{1}{4})\partial_y+(y+9u-\tfrac{1}{2}v)\partial_u
+
\\
&
\,\,\,\,\,\,\,\,
-(-2x+4u-10v)\partial_v,\\
e_2 & := -(5y\tfrac{1}{2}+7v\tfrac{1}{4})\partial_x+(1+\tfrac{1}{2}x+y+\tfrac{1}{4}v)\partial_y+(x+u+\tfrac{1}{2}v)\partial_u+(2y+2v)\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & \tfrac{1}{2}e_1-\tfrac{7}{2}e_2
\\
e_2 &
-\tfrac{1}{2}e1+\tfrac{7}{2}e_2 & 0
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3f4eb}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
yx+x^3+y^3-\tfrac{13}{32}x^4+\tfrac{9}{8}yx^3+\tfrac{65}{16}y^2x^2+\tfrac{1}{8}y^3x+\tfrac{3}{32}y^4+\tfrac{23}{8}x^5+\tfrac{15}{16}yx^4
+
\\
&
\,\,\,\,\,\,\,\,
+y^2x^3+\tfrac{37}{8}y^3x^2+\tfrac{37}{8}y^4x-\tfrac{1}{16}y^5-\tfrac{489}{64}x^6+\tfrac{507}{32}yx^5+\tfrac{933}{64}y^2x^4+\tfrac{81}{16}y^3x^3
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{417}{64}y^4x^2+\tfrac{195}{32}y^5x+\tfrac{99}{64}y^6
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2+2yx^2+2y^2x+\tfrac{29}{16}x^4+\tfrac{7}{4}yx^3+\tfrac{15}{8}y^2x^2+\tfrac{15}{4}y^3x+\tfrac{13}{16}y^4-\tfrac{17}{8}x^5
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{37}{4}yx^4+\tfrac{37}{4}y^2x^3+6y^3x^2+\tfrac{31}{8}y^4x+\tfrac{7}{4}y^5+\tfrac{469}{32}x^6-\tfrac{223}{16}yx^5+\tfrac{615}{32}y^2x^4
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{315}{8}y^3x^3+\tfrac{515}{32}y^4x^2+\tfrac{105}{16}y^5x+\tfrac{65}{32}y^6
+
\cdot,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := (9x\tfrac{1}{2}+1-y+23u\tfrac{1}{4}-21v\tfrac{1}{8})\partial_x+(-4x+7y\tfrac{1}{2}+\tfrac{1}{4}u-31v\tfrac{1}{8})\partial_y+(y+8u-v)\partial_u
+
\\
&
\,\,\,\,\,\,\,\,-(-2x+6u-9v)\partial_v,\\
e_2 & := -(3x\tfrac{1}{2}+2y+11u\tfrac{1}{4}+7v\tfrac{1}{8})\partial_x+(1+x-\tfrac{1}{2}y+3u\tfrac{1}{4}+11v\tfrac{1}{8})\partial_y-(-x+2u-v)\partial_u
+
\\
&
\,\,\,\,\,\,\,\,+(2y+2u-v)\partial_v,
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & -\tfrac{1}{2}e_1-\tfrac{5}{2}e_2
\\
e_2 &
\tfrac{1}{2}e_1+\tfrac{5}{2}e_2 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3g}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+F_{0,3}y^3
+
(2-F_{0,3})x^3
+
F_{0,4}y^4
+
F_{1,3}xy^3
+
F_{2,2}x^2y^2
+
(\tfrac{26}{3}
+
\\
&
\ \ \ \ \
+\tfrac{41}{6}F_{0,3}^2+\tfrac{40}{9}F_{0,3}+\tfrac{1}{2}F_{1,3}+\tfrac{5}{6}F_{2,2}-\tfrac{5}{8}G_{1,3}-\tfrac{1}{6}G_{2,2}+\tfrac{3}{8}G_{3,1}-3F_{0,4}
+
\\
&
\ \ \ \ \
+2G_{0,4}+\tfrac{23}{2}F_{0,3}^3+\tfrac{1}{3}F_{0,3}F_{1,3}-\tfrac{11}{18}F_{0,3}F_{2,2}+\tfrac{11}{24}F_{0,3}G_{1,3}-\tfrac{1}{9}F_{0,3}G_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{5}{8}F_{0,3}G_{3,1}+5F_{0,3}F_{0,4})x^3y
+
(\tfrac{99}{8}-\tfrac{253}{96}F_{0,3}^4+\tfrac{14753}{864}F_{0,3}^2-\tfrac{187}{72}F_{0,3}^3
+
\\
&
\ \ \ \ \
+\tfrac{55}{192}F_{0,3}G_{1,3}-\tfrac{11}{24}F_{0,3}G_{0,4}-\tfrac{11}{144}F_{0,3}^2F_{1,3}+\tfrac{121}{864}F_{0,3}^2F_{2,2}-\tfrac{121}{1152}F_{0,3}^2G_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{11}{432}F_{0,3}^2G_{2,2}+\tfrac{55}{384}F_{0,3}^2G_{3,1}-\tfrac{55}{48}F_{0,3}^2F_{0,4}+\tfrac{29}{96}F_{0,3}F_{1,3}-\tfrac{47}{144}F_{0,3}F_{2,2}
+
\\
&
\ \ \ \ \
+\tfrac{9}{4}F_{0,3}F_{0,4}+\tfrac{23}{288}F_{0,3}G_{2,2}-\tfrac{31}{96}F_{0,3}G_{3,1}-\tfrac{5}{8}F_{0,3}G_{4,0}-\tfrac{1361}{72}F_{0,3}-\tfrac{15}{16}F_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{5}{32}G_{2,2}+\tfrac{7}{128}G_{3,1}-\tfrac{1}{32}F_{1,3}+\tfrac{11}{32}F_{2,2}+\tfrac{5}{8}G_{0,4}-\tfrac{9}{128}G_{1,3}+\tfrac{3}{8}G_{4,0})x^4
+
\cdots
,
\\
v
&
\,=\,
y^2
+
x^2
+
(-8-6F_{0,3})xy^2
+
(-4+6F_{0,3})x^2y
+
G_{0,4}y^4
+
G_{1,3}xy^3
+
\\
&
\ \ \ \ \
+
G_{2,2}x^2y^2
+
G_{3,1}x^3y
+
G_{4,0}x^4
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-(-1+3uG_{4,0}-\tfrac{1}{4}uG_{2,2}+\tfrac{11}{16}uG_{3,1}-\tfrac{233}{18}uF_{0,3}+\tfrac{7}{4}uF_{2,2}-\tfrac{221}{144}yF_{0,3}^2-\tfrac{1}{12}yG_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{23}{48}yF_{0,3}^3-\tfrac{13}{48}xF_{1,3}-\tfrac{85}{192}xG_{1,3}+\tfrac{1}{8}yF_{0,4}+\tfrac{43}{192}xG_{3,1}+\tfrac{5}{4}xG_{4,0}-\tfrac{17}{48}xG_{2,2}-\tfrac{1297}{54}xF_{0,3}
+
\\
&
\ \ \ \ \
+\tfrac{305}{54}yF_{0,3}+\tfrac{115}{48}vF_{0,3}^4+\tfrac{1}{48}yF_{2,2}+\tfrac{5}{48}yF_{1,3}-\tfrac{17}{8}xF_{0,4}+\tfrac{17}{12}xG_{0,4}+\tfrac{391}{48}xF_{0,3}^3+\tfrac{2461}{144}xF_{0,3}^2
+
\\
&
\ \ \ \ \
+\tfrac{31}{48}xF_{2,2}-\tfrac{1}{4}yG_{4,0}+uG_{0,4}-\tfrac{11}{192}yG_{3,1}-\tfrac{25}{192}vF_{0,3}^2G_{3,1}-\tfrac{11}{576}yF_{0,3}G_{1,3}-\tfrac{25}{72}uF_{0,3}G_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{43}{72}uF_{0,3}F_{2,2}+\tfrac{85}{24}xF_{0,3}F_{0,4}-\tfrac{85}{192}xF_{0,3}G_{3,1}-\tfrac{47}{192}vF_{0,3}G_{1,3}+\tfrac{3}{4}uF_{0,3}F_{0,4}+\tfrac{5}{192}yF_{0,3}G_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{17}{216}xF_{0,3}G_{2,2}+\tfrac{1}{216}yF_{0,3}G_{2,2}-\tfrac{29}{48}vF_{0,3}F_{1,3}-\tfrac{55}{432}vF_{0,3}^2F_{2,2}+\tfrac{25}{24}vF_{0,3}^2F_{0,4}+\tfrac{5}{4}vF_{0,3}G_{4,0}
+
\\
&
\ \ \ \ \
+\tfrac{7}{6}uF_{0,3}G_{0,4}+\tfrac{85}{192}vF_{0,3}G_{3,1}+\tfrac{187}{576}xF_{0,3}G_{1,3}+\tfrac{5}{12}vF_{0,3}G_{0,4}-\tfrac{1}{72}yF_{0,3}F_{1,3}-\tfrac{5}{24}yF_{0,3}F_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{161}{24}uF_{0,3}^4+\tfrac{5}{192}yG_{1,3}+\tfrac{1}{48}yG_{2,2}-\tfrac{4607}{108}uF_{0,3}^2+\tfrac{1961}{72}uF_{0,3}^3+\tfrac{7}{36}uF_{0,3}^2F_{1,3}+\tfrac{35}{12}uF_{0,3}^2F_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{35}{96}uF_{0,3}^2G_{3,1}+\tfrac{7}{2}uF_{0,3}G_{4,0}-\tfrac{3}{2}uF_{0,4}+\tfrac{5}{32}vG_{1,3}+\tfrac{5}{8}vF_{1,3}+\tfrac{1}{2}vG_{4,0}-\tfrac{11}{32}vG_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{77}{216}uF_{0,3}^2F_{2,2}-\tfrac{5}{216}vF_{0,3}^2G_{2,2}-\tfrac{7}{108}uF_{0,3}^2G_{2,2}+\tfrac{55}{576}vF_{0,3}^2G_{1,3}-\tfrac{187}{432}xF_{0,3}F_{2,2}
+
\\
&
\ \ \ \ \
+\tfrac{11}{432}yF_{0,3}F_{2,2}+\tfrac{47}{96}uF_{0,3}G_{3,1}-\tfrac{11}{144}vF_{0,3}G_{2,2}-\tfrac{31}{24}uF_{0,3}F_{1,3}-\tfrac{13}{96}uF_{0,3}G_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{7}{144}vF_{0,3}F_{2,2}+\tfrac{77}{288}uF_{0,3}^2G_{1,3}+\tfrac{5}{72}vF_{0,3}^2F_{1,3}+\tfrac{17}{72}xF_{0,3}F_{1,3}-\tfrac{15}{8}vF_{0,3}F_{0,4}+71u
+
\\
&
\ \ \ \ \
-\tfrac{71}{12}y+\tfrac{391}{12}x-\tfrac{7}{2}v-\tfrac{5}{4}uF_{1,3}-\tfrac{13}{16}uG_{1,3}+\tfrac{3}{4}vF_{0,4}-\tfrac{1}{2}vG_{0,4}+\tfrac{691}{144}vF_{0,3}^3-\tfrac{4201}{216}vF_{0,3}^2
+
\\
&
\ \ \ \ \
+\tfrac{413}{36}vF_{0,3}+\tfrac{1}{8}vF_{2,2}+\tfrac{1}{8}vG_{2,2})\partial_x
+
\\
&
\ \ \ \ \
+
(-2uG_{4,0}+\tfrac{5}{6}uG_{2,2}-\tfrac{49}{24}uG_{3,1}+\tfrac{5825}{54}uF_{0,3}-\tfrac{13}{6}uF_{2,2}-\tfrac{2461}{144}yF_{0,3}^2-\tfrac{17}{12}yG_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{391}{48}yF_{0,3}^3-\tfrac{5}{48}xF_{1,3}-\tfrac{5}{192}xG_{1,3}+\tfrac{17}{8}yF_{0,4}+\tfrac{11}{192}xG_{3,1}+\tfrac{1}{4}xG_{4,0}-\tfrac{1}{48}xG_{2,2}-\tfrac{143}{54}xF_{0,3}
+
\\
&
\ \ \ \ \
+\tfrac{1459}{54}yF_{0,3}+\tfrac{115}{48}vF_{0,3}^4-\tfrac{31}{48}yF_{2,2}+\tfrac{13}{48}yF_{1,3}-\tfrac{1}{8}xF_{0,4}+\tfrac{1}{12}xG_{0,4}+\tfrac{23}{48}xF_{0,3}^3+\tfrac{221}{144}xF_{0,3}^2
+
\\
&
\ \ \ \ \
-\tfrac{1}{48}xF_{2,2}-\tfrac{5}{4}yG_{4,0}-\tfrac{22}{3}uG_{0,4}-\tfrac{43}{192}yG_{3,1}-\tfrac{25}{192}vF_{0,3}^2G_{3,1}-\tfrac{187}{576}yF_{0,3}G_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{25}{216}uF_{0,3}G_{2,2}+\tfrac{421}{216}uF_{0,3}F_{2,2}+\tfrac{5}{24}xF_{0,3}F_{0,4}-\tfrac{5}{192}xF_{0,3}G_{3,1}-\tfrac{31}{576}vF_{0,3}G_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{241}{12}uF_{0,3}F_{0,4}+\tfrac{85}{192}yF_{0,3}G_{3,1}-\tfrac{1}{216}xF_{0,3}G_{2,2}+\tfrac{17}{216}yF_{0,3}G_{2,2}-\tfrac{67}{144}vF_{0,3}F_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{55}{432}vF_{0,3}^2F_{2,2}+\tfrac{25}{24}vF_{0,3}^2F_{0,4}+\tfrac{5}{4}vF_{0,3}G_{4,0}+\tfrac{7}{6}uF_{0,3}G_{0,4}+\tfrac{35}{192}vF_{0,3}G_{3,1}+\tfrac{11}{576}xF_{0,3}G_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{5}{12}vF_{0,3}G_{0,4}-\tfrac{17}{72}yF_{0,3}F_{1,3}-\tfrac{85}{24}yF_{0,3}F_{0,4}+\tfrac{161}{24}uF_{0,3}^4+\tfrac{85}{192}yG_{1,3}+\tfrac{17}{48}yG_{2,2}-\tfrac{5731}{54}uF_{0,3}^2
+
\end{array}
\]

\[
\def\arraystretch{1.25}
\begin{array}{ll}
&
\ \ \ \ \
-\tfrac{1489}{72}uF_{0,3}^3+\tfrac{7}{36}uF_{0,3}^2F_{1,3}+\tfrac{35}{12}uF_{0,3}^2F_{0,4}-\tfrac{35}{96}uF_{0,3}^2G_{3,1}+\tfrac{7}{2}uF_{0,3}G_{4,0}+11uF_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{29}{48}vG_{1,3}-\tfrac{5}{12}vF_{1,3}+vG_{4,0}+\tfrac{11}{48}vG_{3,1}-\tfrac{77}{216}uF_{0,3}^2F_{2,2}-\tfrac{5}{216}vF_{0,3}^2G_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{7}{108}uF_{0,3}^2G_{2,2}+\tfrac{55}{576}vF_{0,3}^2G_{1,3}-\tfrac{11}{432}xF_{0,3}F_{2,2}+\tfrac{187}{432}yF_{0,3}F_{2,2}+\tfrac{99}{32}uF_{0,3}G_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{53}{432}vF_{0,3}G_{2,2}-\tfrac{193}{72}uF_{0,3}F_{1,3}-\tfrac{589}{288}uF_{0,3}G_{1,3}-\tfrac{89}{432}vF_{0,3}F_{2,2}+\tfrac{77}{288}uF_{0,3}^2G_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{5}{72}vF_{0,3}^2F_{1,3}+\tfrac{1}{72}xF_{0,3}F_{1,3}+\tfrac{5}{24}vF_{0,3}F_{0,4}-\tfrac{266}{3}u-\tfrac{343}{12}y-\tfrac{1}{12}x+\tfrac{71}{3}v+\tfrac{1}{6}uF_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{55}{24}uG_{1,3}-\tfrac{1}{2}vF_{0,4}+\tfrac{1}{3}vG_{0,4}+\tfrac{1381}{144}vF_{0,3}^3-\tfrac{1415}{108}vF_{0,3}^2-\tfrac{325}{108}vF_{0,3}-\tfrac{1}{12}vF_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{1}{12}vG_{2,2})\partial_y
+
\\
&
\ \ \ \ \
-
(\tfrac{5}{2}uG_{4,0}-\tfrac{17}{24}uG_{2,2}+\tfrac{43}{96}uG_{3,1}-\tfrac{1378}{27}uF_{0,3}+\tfrac{31}{24}uF_{2,2}+\tfrac{17}{6}uG_{0,4}-\tfrac{17}{108}uF_{0,3}G_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{187}{216}uF_{0,3}F_{2,2}-\tfrac{11}{576}vF_{0,3}G_{1,3}+\tfrac{85}{12}uF_{0,3}F_{0,4}-\tfrac{1}{72}vF_{0,3}F_{1,3}+\tfrac{5}{192}vF_{0,3}G_{3,1}+\tfrac{2461}{72}uF_{0,3}^2
+
\\
&
\ \ \ \ \
+\tfrac{391}{24}uF_{0,3}^3-\tfrac{17}{4}uF_{0,4}+\tfrac{5}{192}vG_{1,3}+\tfrac{5}{48}vF_{1,3}-\tfrac{1}{4}vG_{4,0}-\tfrac{11}{192}vG_{3,1}-\tfrac{85}{96}uF_{0,3}G_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{1}{216}vF_{0,3}G_{2,2}+\tfrac{17}{36}uF_{0,3}F_{1,3}+\tfrac{187}{288}uF_{0,3}G_{1,3}+\tfrac{11}{432}vF_{0,3}F_{2,2}-\tfrac{5}{24}vF_{0,3}F_{0,4}+\tfrac{367}{6}u
+
\\
&
\ \ \ \ \
-y-\tfrac{71}{12}v-\tfrac{13}{24}uF_{1,3}-\tfrac{85}{96}uG_{1,3}+\tfrac{1}{8}vF_{0,4}-\tfrac{1}{12}vG_{0,4}-\tfrac{23}{48}vF_{0,3}^3-\tfrac{221}{144}vF_{0,3}^2+\tfrac{305}{54}vF_{0,3}
+
\\
&
\ \ \ \ \
+\tfrac{1}{48}vF_{2,2}+\tfrac{1}{48}vG_{2,2})\partial_u
+
(uG_{4,0}-\tfrac{1}{12}uG_{2,2}+\tfrac{11}{48}uG_{3,1}-\tfrac{124}{27}uF_{0,3}-\tfrac{1}{12}uF_{2,2}+\tfrac{1}{3}uG_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{1}{54}uF_{0,3}G_{2,2}-\tfrac{11}{108}uF_{0,3}F_{2,2}-\tfrac{187}{288}vF_{0,3}G_{1,3}+\tfrac{5}{6}uF_{0,3}F_{0,4}-\tfrac{17}{36}vF_{0,3}F_{1,3}+\tfrac{85}{96}vF_{0,3}G_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{221}{36}uF_{0,3}^2+\tfrac{23}{12}uF_{0,3}^3-\tfrac{1}{2}uF_{0,4}+\tfrac{85}{96}vG_{1,3}+\tfrac{13}{24}vF_{1,3}-\tfrac{5}{2}vG_{4,0}-\tfrac{43}{96}vG_{3,1}-\tfrac{5}{48}uF_{0,3}G_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{17}{108}vF_{0,3}G_{2,2}+\tfrac{1}{18}uF_{0,3}F_{1,3}+\tfrac{11}{144}uF_{0,3}G_{1,3}+\tfrac{187}{216}vF_{0,3}F_{2,2}-\tfrac{85}{12}vF_{0,3}F_{0,4}+\tfrac{11}{3}u+2x
+
\\
&
\ \ \ \ \
-\tfrac{391}{6}v-\tfrac{5}{12}uF_{1,3}-\tfrac{5}{48}uG_{1,3}+\tfrac{17}{4}vF_{0,4}-\tfrac{17}{6}vG_{0,4}-\tfrac{391}{24}vF_{0,3}^3-\tfrac{2461}{72}vF_{0,3}^2+\tfrac{1297}{27}vF_{0,3}
+
\\
&
\ \ \ \ \
-\tfrac{31}{24}vF_{2,2}+\tfrac{17}{24}vG_{2,2})\partial_v
,
\\
e_2
&
\,:=\,
(-\tfrac{1}{3}uG_{2,2}-\tfrac{3}{4}uG_{3,1}-\tfrac{238}{9}uF_{0,3}-\tfrac{1}{3}uF_{2,2}-\tfrac{7}{4}yF_{0,3}^2-\tfrac{1}{12}xF_{1,3}+\tfrac{17}{48}xG_{1,3}-\tfrac{1}{2}yF_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{5}{16}xG_{3,1}+\tfrac{1}{36}xG_{2,2}-\tfrac{4}{3}xF_{0,3}-\tfrac{4}{3}yF_{0,3}+\tfrac{1}{36}yF_{2,2}-\tfrac{1}{12}yF_{1,3}+\tfrac{5}{2}xF_{0,4}+\tfrac{11}{4}xF_{0,3}^2
+
\\
&
\ \ \ \ \
-\tfrac{17}{36}xF_{2,2}+2uG_{0,4}+\tfrac{1}{16}yG_{3,1}-\tfrac{7}{18}uF_{0,3}G_{2,2}-\tfrac{7}{18}uF_{0,3}F_{2,2}+\tfrac{5}{48}vF_{0,3}G_{1,3}
+
\\
&
\ \ \ \ \
+7uF_{0,3}F_{0,4}+\tfrac{5}{12}vF_{0,3}F_{1,3}-\tfrac{5}{16}vF_{0,3}G_{3,1}-\tfrac{1}{48}yG_{1,3}+\tfrac{1}{36}yG_{2,2}+\tfrac{47}{3}uF_{0,3}^2+\tfrac{49}{2}uF_{0,3}^3
+
\\
&
\ \ \ \ \
+6uF_{0,4}-\tfrac{1}{8}vG_{1,3}-\tfrac{1}{2}vF_{1,3}-\tfrac{1}{8}vG_{3,1}-\tfrac{7}{8}uF_{0,3}G_{3,1}-\tfrac{5}{36}vF_{0,3}G_{2,2}+\tfrac{7}{6}uF_{0,3}F_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{7}{24}uF_{0,3}G_{1,3}-\tfrac{5}{36}vF_{0,3}F_{2,2}+\tfrac{5}{2}vF_{0,3}F_{0,4}-\tfrac{68}{3}u+\tfrac{17}{9}y-\tfrac{91}{9}x-\tfrac{14}{3}v-2uF_{1,3}+\tfrac{1}{4}uG_{1,3}
+
\\
&
\ \ \ \ \
-3vF_{0,4}+\tfrac{35}{4}vF_{0,3}^3-\tfrac{59}{6}vF_{0,3}^2-\tfrac{85}{9}vF_{0,3}+\tfrac{1}{6}vF_{2,2}+\tfrac{1}{6}vG_{2,2})\partial_x
+
\\
&
\ \ \ \ \
-
(-1+\tfrac{4}{9}uG_{2,2}+\tfrac{1}{2}uG_{3,1}-\tfrac{250}{9}uF_{0,3}+\tfrac{22}{9}uF_{2,2}-\tfrac{11}{4}yF_{0,3}^2+\tfrac{1}{12}xF_{1,3}+\tfrac{1}{48}xG_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{5}{2}yF_{0,4}-\tfrac{1}{16}xG_{3,1}-\tfrac{1}{36}xG_{2,2}-\tfrac{5}{3}xF_{0,3}-\tfrac{5}{3}yF_{0,3}+\tfrac{17}{36}yF_{2,2}+\tfrac{1}{12}yF_{1,3}+\tfrac{1}{2}xF_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{7}{4}xF_{0,3}^2-\tfrac{1}{36}xF_{2,2}+\tfrac{5}{16}yG_{3,1}-\tfrac{7}{18}uF_{0,3}G_{2,2}-\tfrac{7}{18}uF_{0,3}F_{2,2}+\tfrac{5}{48}vF_{0,3}G_{1,3}+7uF_{0,3}F_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{5}{12}vF_{0,3}F_{1,3}-\tfrac{5}{16}vF_{0,3}G_{3,1}-\tfrac{17}{48}yG_{1,3}-\tfrac{1}{36}yG_{2,2}-\tfrac{100}{3}uF_{0,3}^2+\tfrac{49}{2}uF_{0,3}^3-8uF_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{1}{12}vG_{1,3}+\tfrac{1}{3}vF_{1,3}-\tfrac{1}{4}vG_{3,1}-\tfrac{7}{8}uF_{0,3}G_{3,1}-\tfrac{5}{36}vF_{0,3}G_{2,2}+\tfrac{7}{6}uF_{0,3}F_{1,3}+\tfrac{7}{24}uF_{0,3}G_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{5}{36}vF_{0,3}F_{2,2}+\tfrac{5}{2}vF_{0,3}F_{0,4}+\tfrac{128}{9}u+\tfrac{109}{9}y-\tfrac{17}{9}x-\tfrac{68}{9}v-\tfrac{4}{3}uF_{1,3}-\tfrac{1}{3}uG_{1,3}+2vF_{0,4}
+
\\
&
\ \ \ \ \
+2vG_{0,4}+\tfrac{35}{4}vF_{0,3}^3+\tfrac{50}{3}vF_{0,3}^2+\tfrac{35}{9}vF_{0,3}-\tfrac{1}{9}vF_{2,2}-\tfrac{1}{9}vG_{2,2})\partial_y
+
\\
&
\ \ \ \ \
+
(\tfrac{11}{2}uF_{0,3}^2+\tfrac{1}{3}uF_{0,3}-\tfrac{1}{6}uF_{1,3}-\tfrac{17}{18}uF_{2,2}+\tfrac{17}{24}uG_{1,3}+\tfrac{1}{18}uG_{2,2}-\tfrac{5}{8}uG_{3,1}+5uF_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{7}{4}vF_{0,3}^2+\tfrac{5}{3}vF_{0,3}-\tfrac{1}{12}vF_{1,3}+\tfrac{1}{36}vF_{2,2}-\tfrac{1}{48}vG_{1,3}+\tfrac{1}{36}vG_{2,2}+\tfrac{1}{16}vG_{3,1}-\tfrac{1}{2}vF_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{200}{9}u+\tfrac{17}{9}v+x)\partial_u
-
(7uF_{0,3}^2+\tfrac{34}{3}uF_{0,3}+\tfrac{1}{3}uF_{1,3}-\tfrac{1}{9}uF_{2,2}+\tfrac{1}{12}uG_{1,3}-\tfrac{1}{9}uG_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{1}{4}uG_{3,1}+2uF_{0,4}-\tfrac{11}{2}vF_{0,3}^2-\tfrac{10}{3}vF_{0,3}+\tfrac{1}{6}vF_{1,3}+\tfrac{17}{18}vF_{2,2}-\tfrac{17}{24}vG_{1,3}-\tfrac{1}{18}vG_{2,2}
+
\\
&
\ \ \ \ \
+\tfrac{5}{8}vG_{3,1}-5vF_{0,4}+\tfrac{76}{9}u+\tfrac{218}{9}v-2y)\partial_v.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
A Gr\"obner basis has 92 generators to describe the 
moduli space core algebraic variety in 
$\R^7 \ni F_{0,3},F_{0,4},G_{0,4},G_{1,3},
G_{2,2},G_{3,1},G_{4,0}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3h}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+2x^3
+
(\tfrac{1}{3}F_{2,2}-F_{4,0})y^4 
+
(36+F_{3,1}+G_{4,0}-G_{0,4})xy^3
+
F_{2,2}x^2y^2
+
\\
&
\ \ \ \ \
+
F_{3,1}x^3y
+
F_{4,0}x^4
+
\cdots,
\\
v
&
\,=\,
y^2+x^2-12x^2y
+
G_{0,4}y^4+G_{1,3}xy^3
+
(108+3G_{4,0}+3G_{0,4})x^2y^2
+
\\
&
\ \ \ \ \
+
(\tfrac{4}{3}F_{2,2}-8F_{4,0}+G_{1,3})x^3y
+
G_{4,0}x^4
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-(2xF_{4,0}-1-\tfrac{1}{4}G_{1,3}x+\tfrac{1}{10}yF_{3,1}-\tfrac{1}{10}yG_{0,4}-\tfrac{1}{10}yG_{4,0}-\tfrac{18}{5}y+2uF_{2,2}-\tfrac{1}{2}uG_{1,3}
+
\\
&
\ \ \ \ \
+36v+vF_{3,1}-vG_{0,4}+vG_{4,0})\partial_x
-(\tfrac{1}{10}xF_{3,1}-\tfrac{1}{10}xG_{0,4}-\tfrac{1}{10}xG_{4,0}+\tfrac{12}{5}x+2yF_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{1}{4}yG_{1,3}+\tfrac{1}{5}uF_{3,1}+\tfrac{14}{5}uG_{0,4}+\tfrac{4}{5}uG_{4,0}+\tfrac{144}{5}u+\tfrac{1}{2}vG_{1,3})\partial_y
-(4uF_{4,0}-y-\tfrac{1}{2}uG_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{1}{10}vF_{3,1}-\tfrac{1}{10}vG_{0,4}-\tfrac{1}{10}vG_{4,0}-\tfrac{18}{5}v)\partial_u
-(-2x+\tfrac{108}{5}u+\tfrac{2}{5}uF_{3,1}-\tfrac{2}{5}uG_{0,4}-\tfrac{2}{5}uG_{4,0}
+
\\
&
\ \ \ \ \
+4vF_{4,0}-\tfrac{1}{2}vG_{1,3})\partial_v
, 
\\
e_2
&
\,:=\,
-(\tfrac{1}{2}xF_{3,1}-xG_{0,4}+6x+\tfrac{1}{15}yF_{2,2}-\tfrac{1}{20}yG_{1,3}-5uG_{0,4}+3uF_{3,1}+3uG_{4,0}+108u
+
\\
&
\ \ \ \ \
+\tfrac{4}{3}vF_{2,2}-4vF_{4,0})\partial_x
+(1-\tfrac{1}{15}xF_{2,2}+\tfrac{1}{20}xG_{1,3}-12y-\tfrac{1}{2}yF_{3,1}+yG_{0,4}+\tfrac{8}{15}uF_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{9}{10}uG_{1,3}-4uF_{4,0}-2vG_{0,4})\partial_y
-(uF_{3,1}-2uG_{0,4}+18u-x+\tfrac{1}{15}vF_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{1}{20}vG_{1,3})\partial_u
-(-2y+\tfrac{4}{15}uF_{2,2}-\tfrac{1}{5}uG_{1,3}+24v+vF_{3,1}-2vG_{0,4})\partial_v
.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^6 \ni F_{3,1},F_{2,2},F_{4,0},G_{0,4},G_{1,3},G_{4,0}$:
\[
\aligned
\B_1 & := 96F_{2,2}G_{4,0}+216F_{4,0}G_{0,4}-792F_{4,0}G_{4,0}-63G_{0,4}G_{1,3}+63G_{1,3}G_{4,0}+1736F_{2,2}
+
\\
&
\ \ \ \ \
-14352F_{4,0}+708G_{1,3},
\\
\B_2 & := 36F_{2,2}G_{0,4}+204F_{2,2}G_{4,0}-1440F_{4,0}G_{4,0}-117G_{0,4}G_{1,3}+117G_{1,3}G_{4,0}+4304F_{2,2}
+
\\
&
\ \ \ \ \
-28320F_{4,0}+1392G_{1,3},
\\
\B_3 & := 56F_{2,2}G_{4,0}+24F_{3,1}F_{4,0}-432F_{4,0}G_{4,0}-27G_{0,4}G_{1,3}+33G_{1,3}G_{4,0}+1176F_{2,2}
+
\\
&
\ \ \ \ \
-7632F_{4,0}+468G_{1,3},
\\
\B_4 & := 5832F_{3,1}G_{4,0}-5832F_{4,0}G_{1,3}+1536G_{0,4}^2-10224G_{0,4}G_{4,0}+165G_{1,3}^2+6048G_{4,0}^2
+
\\
&
\ \ \ \ \
+147872F_{3,1}-227904G_{0,4}+394496G_{4,0}+6363648,
\\
\B_5 & := 10344F_{3,1}G_{4,0}+24576F_{4,0}^2-16488F_{4,0}G_{1,3}-11952G_{0,4}G_{4,0}+585G_{1,3}^2+8736G_{4,0}^2
+
\\
&
\ \ \ \ \
+287264F_{3,1}-282432G_{0,4}+680192G_{4,0}+13165056,
\\
\B_6 & := 1536F_{3,1}G_{0,4}+14616F_{3,1}G_{4,0}-16152F_{4,0}G_{1,3}-24144G_{0,4}G_{4,0}+615G_{1,3}^2
+
\\
&
\ \ \ \ \
+14304G_{4,0}^2+375776F_{3,1}-556224G_{0,4}+958208G_{4,0}+15957504,
\\
\B_7 & := 512F_{3,1}^2+14776F_{3,1}G_{4,0}-16824F_{4,0}G_{1,3}-21264G_{0,4}G_{4,0}+555G_{1,3}^2+14432G_{4,0}^2
+
\\
&
\ \ \ \ \
+409696F_{3,1}-537024G_{0,4}+987904G_{4,0}+16860672.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$ (\tfrac{-48}{5}-\tfrac{2}{5}F_{3,1}+\tfrac{9}{10}G_{0,4}-\tfrac{1}{10}G_{4,0})e_1+(2F_{4,0}-\tfrac{1}{5}G_{1,3}-\tfrac{1}{15}F_{2,2})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}} $
-(\tfrac{-48}{5}-\tfrac{2}{5}F_{3,1}+\tfrac{9}{10}G_{0,4}-\tfrac{1}{10}G_{4,0})e_1-(2F_{4,0}-\tfrac{1}{5}G_{1,3}-\tfrac{1}{15}F_{2,2})e_2$
\end{tabular}}
& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3i}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+2y^3
+
(\tfrac{1}{3}F_{2,2}-F_{4,0})y^4+(G_{4,0}+F_{3,1}-G_{0,4}-36)xy^3
+
F_{2,2}x^2y^2
+
\\
&
\ \ \ \ \
+F_{3,1}x^3y+F_{4,0}x^4
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2-12xy^2+G_{0,4}y^4+G_{1,3}xy^3
+
(3G_{4,0}+3G_{0,4}+108)x^2y^2
+
\\
&
\ \ \ \ \
+
(\tfrac{4}{3}F_{2,2}-8F_{4,0}+G_{1,3})x^3y
+G_{4,0}x^4
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-(-1+\tfrac{1}{2}xF_{3,1}-\tfrac{1}{2}xG_{0,4}-\tfrac{1}{2}xG_{4,0}-6x+\tfrac{2}{5}yF_{4,0}-\tfrac{1}{20}yG_{1,3}-\tfrac{56}{5}uF_{4,0}+\tfrac{9}{10}uG_{1,3}
+
\\
&
\ \ \ \ \
+2uF_{2,2}+2vG_{4,0})\partial_x
-(\tfrac{2}{5}xF_{4,0}-\tfrac{1}{20}G_{1,3}x-12y+\tfrac{1}{2}yF_{3,1}-\tfrac{1}{2}yG_{0,4}-\tfrac{1}{2}yG_{4,0}
+
\\
&
\ \ \ \ \
+3uF_{3,1}-2uG_{4,0}+4vF_{4,0})\partial_y
-(uF_{3,1}-uG_{0,4}-uG_{4,0}-18u-y+\tfrac{2}{5}vF_{4,0}
+
\\
&
\ \ \ \ \
-\tfrac{1}{20}vG_{1,3})\partial_u
-(-2x+\tfrac{8}{5}uF_{4,0}-\tfrac{1}{5}uG_{1,3}-12v+vF_{3,1}-vG_{0,4}-vG_{4,0})\partial_v 
,
\\
e_2
&
\,:=\,
-(\tfrac{1}{3}xF_{2,2}-\tfrac{1}{4}xG_{1,3}-\tfrac{6}{5}y+\tfrac{1}{10}yF_{3,1}-\tfrac{1}{5}yG_{0,4}+\tfrac{1}{5}uF_{3,1}+\tfrac{3}{5}uG_{0,4}+\tfrac{108}{5}u+3uG_{4,0}
+
\\
&
\ \ \ \ \
+\tfrac{2}{3}vF_{2,2}-4vF_{4,0}+\tfrac{1}{2}vG_{1,3})\partial_x
-(-1+\tfrac{1}{10}xF_{3,1}-\tfrac{1}{5}xG_{0,4}-\tfrac{36}{5}x+\tfrac{1}{3}yF_{2,2}-\tfrac{1}{4}yG_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{4}{3}uF_{2,2}+4uF_{4,0}-\tfrac{1}{2}uG_{1,3}+vF_{3,1})\partial_y
-(-x+\tfrac{2}{3}uF_{2,2}-\tfrac{1}{2}uG_{1,3}+\tfrac{1}{10}vF_{3,1}-\tfrac{1}{5}vG_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{36}{5}v)\partial_u
-(-2y+\tfrac{36}{5}u+\tfrac{2}{5}uF_{3,1}-\tfrac{4}{5}uG_{0,4}+\tfrac{2}{3}vF_{2,2}-\tfrac{1}{2}vG_{1,3})\partial_v.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^6 \ni F_{2,2},F_{3,1},F_{4,0},G_{0,4},G_{1,3},G_{4,0}$:
\[
\aligned
\B_1 & := 36F_{3,1}F_{4,0}-144F_{4,0}G_{4,0}-9G_{0,4}G_{1,3}+18G_{1,3}G_{4,0}+280F_{2,2}-1200F_{4,0}-24G_{1,3},
\\
\B_2 & := -240F_{2,2}G_{4,0}+216F_{4,0}G_{0,4}+1224F_{4,0}G_{4,0}+63G_{0,4}G_{1,3}-63G_{1,3}G_{4,0}-640F_{2,2}
+
\\
&
\ \ \ \ \
+11136F_{4,0}+888G_{1,3},
\\
\B_3 & := -120F_{2,2}G_{4,0}+27F_{3,1}G_{1,3}+288F_{4,0}G_{4,0}-9G_{0,4}G_{1,3}+9G_{1,3}G_{4,0}+280F_{2,2}
+
\\
&
\ \ \ \ \
-1200F_{4,0}-24G_{1,3},
\\
\B_4 & := -3672F_{3,1}G_{4,0}+3672F_{4,0}G_{1,3}+1200G_{0,4}^2+2304G_{0,4}G_{4,0}-129G_{1,3}^2-1440G_{4,0}^2
+
\\
&
\ \ \ \ \
-7360F_{3,1}+49920G_{0,4}+11744G_{4,0}+241920,
\\
\B_5 & := -192F_{3,1}G_{4,0}+192F_{4,0}^2+144F_{4,0}G_{1,3}+144G_{0,4}G_{4,0}+9G_{1,3}^2-240G_{4,0}^2+80F_{3,1}
+
\\
&
\ \ \ \ \
+240G_{0,4}-1456G_{4,0}+8640,
\\
\B_6 & := 300F_{3,1}G_{0,4}-756F_{3,1}G_{4,0}+456F_{4,0}G_{1,3}-408G_{0,4}G_{4,0}+33G_{1,3}^2-120G_{4,0}^2+7520F_{3,1}
+
\\
&
\ \ \ \ \
+960G_{0,4}-16288G_{4,0}+34560,
\\
\B_7 & := 200F_{3,1}^2-2168F_{3,1}G_{4,0}+1368F_{4,0}G_{1,3}+576G_{0,4}G_{4,0}+99G_{1,3}^2-1360G_{4,0}^2+8160F_{3,1}
+
\\
&
\ \ \ \ \
+2880G_{0,4}-20064G_{4,0}+103680.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(-\tfrac{1}{3}F_{2,2}+\tfrac{1}{5}G_{1,3}+\tfrac{2}{5}F_{4,0})e_1+(\tfrac{-24}{5}+\tfrac{2}{5}F_{3,1}-\tfrac{3}{10}G_{0,4}-\tfrac{1}{2}G_{4,0})e_2
$
\end{tabular}}
\\
e_2 & \rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$
(-\tfrac{1}{3}F_{2,2}+\tfrac{1}{5}G_{1,3}+\tfrac{2}{5}F_{4,0})e_1+(\tfrac{-24}{5}+\tfrac{2}{5}F_{3,1}-\tfrac{3}{10}G_{0,4}-\tfrac{1}{2}G_{4,0})e_2
$
\end{tabular}}
& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\[
\text{\bf Model 2f3j4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3+F_{4,0}x^4+F_{3,1}x^3y
+
(6F_{4,0}-\tfrac{21}{2})x^2y^2
+
(-1+F_{3,1})xy^3
+
\\
&
\,\,\,\,\,\,\,\,
+
(-\tfrac{1}{2}+F_{4,0})y^4
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2-6x^2y-6xy^2+G_{4,0}x^4
+
(8F_{4,0}-2F_{3,1}+4G_{4,0})x^3y
+
\\
&
\,\,\,\,\,\,\,\,
+
(57+6G_{4,0})x^2y^2
+
(8F_{4,0}+2-2F_{3,1}+4G_{4,0})xy^3
+
(G_{4,0}+1)y^4
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\aligned
e_1 & := 
(1-\tfrac{40}{3}xF_{4,0}+\tfrac{19}{6}xF_{3,1}+\tfrac{1}{3}xG_{4,0}+\tfrac{8}{3}yF_{4,0}-\tfrac{5}{6}yF_{3,1}+\tfrac{1}{3}yG_{4,0}+\tfrac{185}{2}u-\tfrac{147}{4}v+\tfrac{127}{4}x
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{136}{3}uF_{4,0}+\tfrac{32}{3}uF_{3,1}-\tfrac{8}{3}uG_{4,0}+\tfrac{40}{3}vF_{4,0}-\tfrac{25}{6}vF_{3,1}-\tfrac{1}{3}vG_{4,0}-\tfrac{15}{4}y)\partial_x
+
(\tfrac{8}{3}xF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{5}{6}xF_{3,1}+\tfrac{1}{3}xG_{4,0}-\tfrac{40}{3}yF_{4,0}+\tfrac{19}{6}yF_{3,1}+\tfrac{1}{3}yG_{4,0}+\tfrac{141}{2}u-\tfrac{115}{4}v-\tfrac{27}{4}x-\tfrac{112}{3}uF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{26}{3}uF_{3,1}-\tfrac{8}{3}uG_{4,0}+\tfrac{28}{3}vF_{4,0}-\tfrac{19}{6}vF_{3,1}-\tfrac{1}{3}vG_{4,0}+\tfrac{139}{4}y)\partial_y
+
(y-\tfrac{80}{3}uF_{4,0}+\tfrac{19}{3}uF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{2}{3}uG_{4,0}+\tfrac{133}{2}u+\tfrac{8}{3}vF_{4,0}-\tfrac{5}{6}vF_{3,1}+\tfrac{1}{3}vG_{4,0}-\tfrac{15}{4}v)\partial_u
-
(-2x-\tfrac{32}{3}uF_{4,0}+\tfrac{10}{3}uF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{4}{3}uG_{4,0}+33u+\tfrac{80}{3}vF_{4,0}-\tfrac{19}{3}vF_{3,1}-\tfrac{2}{3}vG_{4,0}-\tfrac{127}{2}v)\partial_v,\\
e_2 & := 
-
(\tfrac{7}{2}xF_{3,1}-\tfrac{1}{3}xG_{4,0}-\tfrac{40}{3}xF_{4,0}-\tfrac{1}{2}yF_{3,1}-\tfrac{1}{3}yG_{4,0}+\tfrac{8}{3}yF_{4,0}+\tfrac{213}{2}u-\tfrac{149}{4}v-\tfrac{25}{4}y
+
\\
&
\,\,\,\,\,\,\,\,
+10uF_{3,1}+\tfrac{8}{3}uG_{4,0}-\tfrac{112}{3}uF_{4,0}-\tfrac{7}{2}vF_{3,1}+\tfrac{1}{3}vG_{4,0}+\tfrac{52}{3}vF_{4,0}+\tfrac{117}{4}x)\partial_x
-
(-\tfrac{1}{2}xF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
-1-\tfrac{1}{3}xG_{4,0}+\tfrac{8}{3}xF_{4,0}+\tfrac{7}{2}yF_{3,1}-\tfrac{1}{3}yG_{4,0}-\tfrac{40}{3}yF_{4,0}+\tfrac{181}{2}u-\tfrac{105}{4}v+\tfrac{129}{4}y+8uF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{8}{3}uG_{4,0}-\tfrac{88}{3}uF_{4,0}-\tfrac{5}{2}vF_{3,1}+\tfrac{1}{3}vG_{4,0}+\tfrac{40}{3}vF_{4,0}-\tfrac{37}{4}x)\partial_y
-
(-x+\tfrac{123}{2}u+7uF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{2}{3}uG_{4,0}-\tfrac{80}{3}uF_{4,0}-\tfrac{37}{4}v-\tfrac{1}{2}vF_{3,1}-\tfrac{1}{3}vG_{4,0}+\tfrac{8}{3}vF_{4,0})\partial_u
+
(2y+19u+2uF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{4}{3}uG_{4,0}-\tfrac{32}{3}uF_{4,0}-\tfrac{129}{2}v-7vF_{3,1}+\tfrac{2}{3}vG_{4,0}+\tfrac{80}{3}vF_{4,0})\partial_v,
\endaligned
\]
with invariants $F_{3,1},F_{4,0},G_{4,0}$ satisfying:
\[
\aligned
0
\,=\,
\B_1 & := (2F_{3,1}+19+8F_{4,0})(153+16F_{3,1}-64F_{4,0}),
\\
0
\,=\,
\B_2 & := (2F_{4,0}+G_{4,0}+7)(153+16F_{3,1}-64F_{4,0}).
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(-\tfrac{51}{2}-\tfrac{8}{3}F_{3,1}+\tfrac{32}{3}F_{4,0})e_1+(-\tfrac{51}{2}-\tfrac{8}{3}F_{3,1}+\tfrac{32}{3}F_{4,0})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(-\tfrac{51}{2}-\tfrac{8}{3}F_{3,1}+\tfrac{32}{3}F_{4,0})e_1-(-\tfrac{51}{2}-\tfrac{8}{3}F_{3,1}+\tfrac{32}{3}F_{4,0})e_2$
\end{tabular}}
& 
0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3j4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3+F_{4,0}x^4+F_{3,1}x^3y
+
(6F_{4,0}-\tfrac{15}{2})x^2y^2
+
(1+F_{3,1})xy^3
+
\\
&
\,\,\,\,\,\,\,\,
+
(\tfrac{1}{2}+F_{4,0})y^4
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2-6x^2y-6xy^2+G_{4,0}x^4
+
(8F_{4,0}-2F_{3,1}+4G_{4,0})x^3y
+
\\
&
\,\,\,\,\,\,\,\,
+
(51+6G_{4,0})x^2y^2
+
(8F_{4,0}-2-2F_{3,1}+4G_{4,0})xy^3
+
(G_{4,0}-1)y^4
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := 
-
(-1+\tfrac{487}{6}u-\tfrac{269}{12}v+\tfrac{353}{12}x+\tfrac{8}{3}yF_{4,0}-\tfrac{1}{2}yF_{3,1}-\tfrac{1}{3}yG_{4,0}-\tfrac{40}{3}xF_{4,0}+\tfrac{7}{2}xF_{3,1}-\tfrac{1}{3}xG_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{40}{3}vF_{4,0}-\tfrac{5}{2}vF_{3,1}+\tfrac{1}{3}vG_{4,0}-\tfrac{88}{3}uF_{4,0}+8uF_{3,1}+\tfrac{8}{3}uG_{4,0}-\tfrac{97}{12}y)\partial_x
-
(\tfrac{571}{6}u-\tfrac{389}{12}v-\tfrac{61}{12}x
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{40}{3}yF_{4,0}+\tfrac{7}{2}yF_{3,1}-\tfrac{1}{3}yG_{4,0}+\tfrac{8}{3}xF_{4,0}-\tfrac{1}{2}xF_{3,1}-\tfrac{1}{3}xG_{4,0}+\tfrac{52}{3}vF_{4,0}-\tfrac{7}{2}vF_{3,1}+\tfrac{1}{3}vG_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{112}{3}uF_{4,0}+10uF_{3,1}+\tfrac{8}{3}uG_{4,0}+\tfrac{317}{12}y)\partial_y
-
(-y-\tfrac{80}{3}uF_{4,0}+7uF_{3,1}-\tfrac{2}{3}uG_{4,0}+\tfrac{335}{6}u
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{8}{3}vF_{4,0}-\tfrac{1}{2}vF_{3,1}-\tfrac{1}{3}vG_{4,0}-\tfrac{97}{12}v)\partial_u
+
(2x-\tfrac{32}{3}uF_{4,0}+2uF_{3,1}+\tfrac{4}{3}uG_{4,0}+\tfrac{43}{3}u+\tfrac{80}{3}vF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-7vF_{3,1}+\tfrac{2}{3}vG_{4,0}-\tfrac{353}{6}v)\partial_v,\\
e_2 & := 
(\tfrac{379}{6}u-\tfrac{323}{12}v-\tfrac{79}{12}y+\tfrac{1}{3}yG_{4,0}+\tfrac{8}{3}yF_{4,0}+\tfrac{19}{6}xF_{3,1}+\tfrac{1}{3}xG_{4,0}-\tfrac{40}{3}xF_{4,0}-\tfrac{5}{6}yF_{3,1}-\tfrac{19}{6}vF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{1}{3}vG_{4,0}+\tfrac{28}{3}vF_{4,0}+\tfrac{26}{3}uF_{3,1}-\tfrac{8}{3}uG_{4,0}-\tfrac{112}{3}uF_{4,0}+\tfrac{371}{12}x)\partial_x
+
(\tfrac{499}{6}u+1-\tfrac{407}{12}v+\tfrac{335}{12}y
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{1}{3}yG_{4,0}-\tfrac{40}{3}yF_{4,0}-\tfrac{5}{6}xF_{3,1}+\tfrac{1}{3}xG_{4,0}+\tfrac{8}{3}xF_{4,0}+\tfrac{19}{6}yF_{3,1}-\tfrac{25}{6}vF_{3,1}-\tfrac{1}{3}vG_{4,0}+\tfrac{40}{3}vF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{32}{3}uF_{3,1}-\tfrac{8}{3}uG_{4,0}-\tfrac{136}{3}uF_{4,0}-\tfrac{43}{12}x)\partial_y
+
(x+\tfrac{353}{6}u+\tfrac{19}{3}uF_{3,1}+\tfrac{2}{3}uG_{4,0}-\tfrac{80}{3}uF_{4,0}-\tfrac{43}{12}v
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{5}{6}vF_{3,1}+\tfrac{1}{3}vG_{4,0}+\tfrac{8}{3}vF_{4,0})\partial_u
-
(-2y+\tfrac{97}{3}u+\tfrac{10}{3}uF_{3,1}-\tfrac{4}{3}uG_{4,0}-\tfrac{32}{3}uF_{4,0}-\tfrac{335}{6}v-\tfrac{19}{3}vF_{3,1}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{2}{3}vG_{4,0}+\tfrac{80}{3}vF_{4,0})\partial_v,
\endaligned
\]
with invariants $F_{4,0},F_{3,1},G_{4,0}$ satisfying:
\[
\aligned
0
\,=\,
\B_1 & := (2F_{3,1}+25+8F_{4,0})(137-64F_{4,0}+16F_{3,1}),
\\
0
\,=\,
\B_2 & := (2F_{4,0}+G_{4,0}+7)(137-64F_{4,0}+16F_{3,1}),
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(\tfrac{137}{6}-\tfrac{32}{3}F_{4,0}+\tfrac{8}{3}F_{3,1})e_1+(\tfrac{137}{6}-\tfrac{32}{3}F_{4,0}+\tfrac{8}{3}F_{3,1})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(\tfrac{137}{6}-\tfrac{32}{3}F_{4,0}+\tfrac{8}{3}F_{3,1})e_1-^(\tfrac{137}{6}-\tfrac{32}{3}F_{4,0}+\tfrac{8}{3}F_{3,1})e_2$
\end{tabular}}
&
0
\end{array}
\]

\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
\end{tabular}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3j4c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3+F_{4,0}x^4
+
(4F_{4,0}-9)x^3y
+
(6F_{4,0}-9)x^2y^2
+
(4F_{4,0}-9)xy^3
+
\\
&
\,\,\,\,\,\,\,\,
+
F_{4,0}y^4+F_{5,0}x^5
+
(-24F_{4,0}+5F_{5,0}+27)x^4y
+
(108-72F_{4,0}+10F_{5,0})x^3y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(108-72F_{4,0}+10F_{5,0})x^2y^3
+
(-24F_{4,0}+5F_{5,0}+27)xy^4+F_{5,0}y^5
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2-6x^2y-6xy^2
+
(-2F_{4,0}-6)x^4
+
(-8F_{4,0}-6)x^3y
+
\\
&
\,\,\,\,\,\,\,\,
+
(18-12F_{4,0})x^2y^2
+
(-8F_{4,0}-6)xy^3
+
(-2F_{4,0}-6)y^4
+
G_{5,0}x^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(90+48F_{4,0}+5G_{5,0})x^4y
+
(108+144F_{4,0}+10G_{5,0})x^3y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(108+144F_{4,0}+10G_{5,0})x^2y^3
+
(90+48F_{4,0}+5G_{5,0})xy^4
+
G_{5,0}y^5
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := 
-
(-1+\tfrac{71}{2}xF_{4,0}+\tfrac{25}{4}xF_{5,0}+\tfrac{25}{8}xG_{5,0}-\tfrac{11}{2}yF_{4,0}-\tfrac{5}{4}yF_{5,0}-\tfrac{5}{8}yG_{5,0}+93uF_{4,0}+\tfrac{35}{2}uF_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{35}{4}uG_{5,0}-\tfrac{63}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}-12y+51x+135u-54v)\partial_x
-
(-\tfrac{11}{2}xF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{5}{4}xF_{5,0}-\tfrac{5}{8}xG_{5,0}+\tfrac{71}{2}yF_{4,0}+\tfrac{25}{4}yF_{5,0}+\tfrac{25}{8}yG_{5,0}+93uF_{4,0}+\tfrac{35}{2}uF_{5,0}+\tfrac{35}{4}uG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{63}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}+48y-9x+135u-54v)\partial_y
-
(71uF_{4,0}+99u-y+\tfrac{25}{2}uF_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{25}{4}uG_{5,0}-12v-\tfrac{11}{2}vF_{4,0}-\tfrac{5}{4}vF_{5,0}-\tfrac{5}{8}vG_{5,0})\partial_u
+
(2x+30u+22uF_{4,0}+5uF_{5,0}+\tfrac{5}{2}uG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-102v-71vF_{4,0}-\tfrac{25}{2}vF_{5,0}-\tfrac{25}{4}vG_{5,0})\partial_v,\\
e_2 & := 
-
(\tfrac{71}{2}xF_{4,0}+\tfrac{25}{4}xF_{5,0}+\tfrac{25}{8}xG_{5,0}-\tfrac{11}{2}yF_{4,0}-\tfrac{5}{4}yF_{5,0}-\tfrac{5}{8}yG_{5,0}+93uF_{4,0}+\tfrac{35}{2}uF_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{35}{4}uG_{5,0}-\tfrac{63}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}+48x-9y+135u-54v)\partial_x
-
(-\tfrac{11}{2}xF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{5}{4}xF_{5,0}-1-\tfrac{5}{8}xG_{5,0}+\tfrac{71}{2}yF_{4,0}+\tfrac{25}{4}yF_{5,0}+\tfrac{25}{8}yG_{5,0}+93uF_{4,0}+\tfrac{35}{2}uF_{5,0}+\tfrac{35}{4}uG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{63}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}-12x+51y+135u-54v)\partial_y
-
(71uF_{4,0}+99u-x
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{25}{2}uF_{5,0}+\tfrac{25}{4}uG_{5,0}-12v-\tfrac{11}{2}vF_{4,0}-\tfrac{5}{4}vF_{5,0}-\tfrac{5}{8}vG_{5,0})\partial_u
+
(2y+30u+22uF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+5uF_{5,0}+\tfrac{5}{2}uG_{5,0}-102v-71vF_{4,0}-\tfrac{25}{2}vF_{5,0}-\tfrac{25}{4}vG_{5,0})\partial_v,
\endaligned
\]
with invariants $F_{4,0},F_{5,0},G_{5,0}$ satisfying:
\[
0
\,=\,
\B_1
\,:=\,
152F_{4,0}^2+20F_{4,0}F_{5,0}+10F_{4,0}G_{5,0}
+240F_{4,0}-10F_{5,0}+5G_{5,0}-72,
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(-60-41F_{4,0}-\tfrac{15}{2}F_{5,0}-\tfrac{15}{4}G_{5,0})e_1+(60+41F_{4,0}+\tfrac{15}{2}F_{5,0}+\tfrac{15}{4}G_{5,0})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(-60-41F_{4,0}-\tfrac{15}{2}F_{5,0}-\tfrac{15}{4}G_{5,0})e_1-(60+41F_{4,0}+\tfrac{15}{2}F_{5,0}+\tfrac{15}{4}G_{5,0})e_2$
\end{tabular}}
&
0
\end{array}
\]

\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
\end{tabular}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3j4d}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3+F_{4,0}x^4
+
(4F_{4,0}-9)x^3y
+
(6F_{4,0}-9)x^2y^2
+
(4F_{4,0}-9)xy^3
+
\\
&
\,\,\,\,\,\,\,\,
+
F_{4,0}y^4+F_{5,0}x^5
+
(-24F_{4,0}+5F_{5,0}+27)x^4y
+
(108-72F_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+10F_{5,0})x^3y^2
+
(108-72F_{4,0}+10F_{5,0})x^2y^3
+
(-24F_{4,0}+5F_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+27)xy^4
+
F_{5,0}y^5
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2-6x^2y-6xy^2
+
(-2F_{4,0}-8)x^4
+
(-8F_{4,0}-14)x^3y
+
\\
&
\,\,\,\,\,\,\,\,
+
(6-12F_{4,0})x^2y^2
+
(-8F_{4,0}-14)xy^3
+
(-2F_{4,0}-8)y^4
+
G_{5,0}x^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(138+48F_{4,0}+5G_{5,0})x^4y
+
(252+144F_{4,0}+10G_{5,0})x^3y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(252+144F_{4,0}+10G_{5,0})x^2y^3
+
(138+48F_{4,0}+5G_{5,0})xy^4
+
G_{5,0}y^5
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := 
(-\tfrac{19}{2}yF_{4,0}-\tfrac{5}{4}yF_{5,0}+1-\tfrac{5}{8}yG_{5,0}+\tfrac{79}{2}xF_{4,0}+\tfrac{25}{4}xF_{5,0}+\tfrac{25}{8}xG_{5,0}+117uF_{4,0}+\tfrac{35}{2}uF_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{35}{4}uG_{5,0}-\tfrac{87}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}-\tfrac{33}{2}y+\tfrac{175}{2}x+260u-\tfrac{169}{2}v)\partial_x
+
(\tfrac{79}{2}yF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{25}{4}yF_{5,0}+\tfrac{25}{8}yG_{5,0}-\tfrac{19}{2}xF_{4,0}-\tfrac{5}{4}xF_{5,0}-\tfrac{5}{8}xG_{5,0}+117uF_{4,0}+\tfrac{35}{2}uF_{5,0}+\tfrac{35}{4}uG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{87}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}+\tfrac{181}{2}y-\tfrac{39}{2}x+260u-\tfrac{169}{2}v)\partial_y
+
(y+178u+79uF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{25}{2}uF_{5,0}+\tfrac{25}{4}uG_{5,0}-\tfrac{33}{2}v-\tfrac{19}{2}vF_{4,0}-\tfrac{5}{4}vF_{5,0}-\tfrac{5}{8}vG_{5,0})\partial_u
-
(38uF_{4,0}+5uF_{5,0}+84u
+
\\
&
\,\,\,\,\,\,\,\,
-2x+\tfrac{5}{2}uG_{5,0}-175v-79vF_{4,0}-\tfrac{25}{2}vF_{5,0}-\tfrac{25}{4}vG_{5,0})\partial_v,\\
e_2 & := 
(-\tfrac{5}{8}yG_{5,0}+\tfrac{79}{2}xF_{4,0}+\tfrac{25}{4}xF_{5,0}+\tfrac{25}{8}xG_{5,0}-\tfrac{19}{2}yF_{4,0}-\tfrac{5}{4}yF_{5,0}+117uF_{4,0}+\tfrac{35}{2}uF_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{35}{4}uG_{5,0}-\tfrac{87}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}+\tfrac{181}{2}x-\tfrac{39}{2}y+260u-\tfrac{169}{2}v)\partial_x
+
(1+\tfrac{25}{8}yG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{19}{2}xF_{4,0}-\tfrac{5}{4}xF_{5,0}-\tfrac{5}{8}xG_{5,0}+\tfrac{79}{2}yF_{4,0}+\tfrac{25}{4}yF_{5,0}+117uF_{4,0}+\tfrac{35}{2}uF_{5,0}+\tfrac{35}{4}uG_{5,0}
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{87}{2}vF_{4,0}-\tfrac{25}{4}vF_{5,0}-\tfrac{25}{8}vG_{5,0}-\tfrac{33}{2}x+\tfrac{175}{2}y+260u-\tfrac{169}{2}v)\partial_y
+
(x+178u+79uF_{4,0}
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{25}{2}uF_{5,0}
+\tfrac{25}{4}uG_{5,0}-\tfrac{33}{2}v-\tfrac{19}{2}vF_{4,0}-\tfrac{5}{4}vF_{5,0}-\tfrac{5}{8}vG_{5,0})\partial_u
-
(38uF_{4,0}+5uF_{5,0}+84u
+
\\
&
\,\,\,\,\,\,\,\,
-2y+\tfrac{5}{2}uG_{5,0}-175v-79vF_{4,0}-\tfrac{25}{2}vF_{5,0}-\tfrac{25}{4}vG_{5,0})\partial_v,
\endaligned
\]
with invariants $F_{4,0},F_{5,0},G_{5,0}$ satisfying:
\[
0
\,=\,
\B_1
\,:=\,
44F_{4,0}^2+10F_{4,0}F_{5,0}+5F_{4,0}G_{5,0}+114F_{4,0}+10F_{5,0}
+100,
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(107+49F_{4,0}+\tfrac{15}{2}F_{5,0}+\tfrac{15}{4}G_{5,0})e_1+(-107-49F_{4,0}-\tfrac{15}{2}F_{5,0}-\tfrac{15}{4}G_{5,0})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(107+49F_{4,0}+\tfrac{15}{2}F_{5,0}+\tfrac{15}{4}G_{5,0})e_1-(-107-49F_{4,0}-\tfrac{15}{2}F_{5,0}-\tfrac{15}{4}G_{5,0})e_2$
\end{tabular}} & 0
\end{array}
\]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3j4e}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3-\tfrac{1}{2}x^4-11x^3y-12x^2y^2-11xy^3-\tfrac{1}{2}y^4+F_{5,0}x^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(39+5F_{5,0})x^4y
+
(144+10F_{5,0})x^3y^2
+
(144+10F_{5,0})x^2y^3
+
\\
&
\,\,\,\,\,\,\,\,
+
(39+5F_{5,0})xy^4
+
F_{5,0}y^5
+
(-\tfrac{20}{3}F_{5,0}^2-\tfrac{373}{3}F_{5,0}-572)x^6
+
\\
&
\,\,\,\,\,\,\,\,
+
(-40F_{5,0}^2-776F_{5,0}-3549)x^5y
+
(-100F_{5,0}^2-1985F_{5,0}-9480)x^4y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(-\tfrac{400}{3}F_{5,0}^2-\tfrac{8000}{3}F_{5,0}-13060)x^3y^3
+
(-100F_{5,0}^2-1985F_{5,0}-9480)x^2y^4
+
\\
&
\,\,\,\,\,\,\,\,
+
(-40F_{5,0}^2-776F_{5,0}-3549)xy^5
+
(-\tfrac{20}{3}F_{5,0}^2-\tfrac{373}{3}F_{5,0}-572)y^6
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2-6x^2y-6xy^2-6x^4-6x^3y+18x^2y^2-6xy^3-6y^4
+
\\
&
\,\,\,\,\,\,\,\,
+
(-2F_{5,0}-16)x^5
+
(10-10F_{5,0})x^4y
+
(-52-20F_{5,0})x^3y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(-52-20F_{5,0})x^2y^3
+
(10-10F_{5,0})xy^4
+
(-2F_{5,0}-16)y^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(\tfrac{40}{3}F_{5,0}^2+\tfrac{710}{3}F_{5,0}+1120)x^6+(80F_{5,0}^2+1480F_{5,0}+6930)x^5y
+
\\
&
\,\,\,\,\,\,\,\,
+
(200F_{5,0}^2+3790F_{5,0}+17316)x^4y^2
+
(\tfrac{800}{3}F_{5,0}^2+\tfrac{15280}{3}F_{5,0}+23336)x^3y^3
+
\\
&
\,\,\,\,\,\,\,\,
+
(200F_{5,0}^2+3790F_{5,0}+17316)x^2y^4
+
(80F_{5,0}^2+1480F_{5,0}+6930)xy^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(\tfrac{40}{3}F_{5,0}^2+\tfrac{710}{3}F_{5,0}+1120)y^6
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := 
(1+\tfrac{467}{2}x+25xF_{5,0}-\tfrac{89}{2}y-5yF_{5,0}+70F_{5,0}u+662u-\tfrac{457}{2}v-25vF_{5,0})\partial_x
+
(-\tfrac{95}{2}x
+
\\
&
\,\,\,\,\,\,\,\,
-5xF_{5,0}+\tfrac{473}{2}y+25yF_{5,0}+70F_{5,0}u+662u-\tfrac{457}{2}v-25vF_{5,0})\partial_y
+
(y+50F_{5,0}u+470u
+
\\
&
\,\,\,\,\,\,\,\,
-\tfrac{89}{2}v-5vF_{5,0})\partial_u
-
(20F_{5,0}u-50F_{5,0}v+196u-467v-2x)\partial_v,\\
e_2 & := 
(\tfrac{473}{2}x+25xF_{5,0}-\tfrac{95}{2}y-5yF_{5,0}+70F_{5,0}u+662u-\tfrac{457}{2}v-25vF_{5,0})\partial_x
+
(-\tfrac{89}{2}x
+
\\
&
\,\,\,\,\,\,\,\,
-5xF_{5,0}+1+\tfrac{467}{2}y+25yF_{5,0}+70F_{5,0}u+662u-\tfrac{457}{2}v-25vF_{5,0})\partial_y
+
(x+50F_{5,0}u
+
\\
&
\,\,\,\,\,\,\,\,
+470u-\tfrac{89}{2}v-5vF_{5,0})\partial_u
-
(20F_{5,0}u-50F_{5,0}v+196u-467v-2y)\partial_v.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & (30F_{5,0}+281)e_1-(30F_{5,0}+281)e_2
\\
e_2 &
-(30F_{5,0}+281)e_1+(30F_{5,0}+281)e_2 & 0
\end{array}
\]

\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
\end{tabular}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3j4f}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3-9x^3y-9x^2y^2-9xy^3+F_{5,0}x^5
+
(27+5F_{5,0})x^4y
+
\\
&
\,\,\,\,\,\,\,\,
+
(108+10F_{5,0})x^3y^2
+
(108+10F_{5,0})x^2y^3
+
(27+5F_{5,0})xy^4
+
\\
&
\,\,\,\,\,\,\,\,
+
F_{5,0}y^5
+
(\tfrac{20}{3}F_{5,0}^2+\tfrac{365}{3}F_{5,0}+547)x^6
+
(40F_{5,0}^2+700F_{5,0}+3201)x^5y
+
\\
&
\,\,\,\,\,\,\,\,
+
(100F_{5,0}^2+1705F_{5,0}+7557)x^4y^2
+
(\tfrac{400}{3}F_{5,0}^2+\tfrac{6760}{3}F_{5,0}+9752)x^3y^3
+
\\
&
\,\,\,\,\,\,\,\,
+
(100F_{5,0}^2+1705F_{5,0}+7557)x^2y^4
+
(40F_{5,0}^2+700F_{5,0}+3201)xy^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(\tfrac{20}{3}F_{5,0}^2+\tfrac{365}{3}F_{5,0}+547)y^6
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2-6x^2y-6xy^2-7x^4-10x^3y+12x^2y^2-10xy^3-7y^4
+
\\
&
\,\,\,\,\,\,\,\,
+
(-2F_{5,0}-22)x^5
+
(4-10F_{5,0})x^4y
+
(-40-20F_{5,0})x^3y^2
+
\\
&
\,\,\,\,\,\,\,\,
+
(-40-20F_{5,0})x^2y^3
+
(4-10F_{5,0})xy^4
+
(-2F_{5,0}-22)y^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(-\tfrac{40}{3}F_{5,0}^2-\tfrac{766}{3}F_{5,0}-1136)x^6
+
(-80F_{5,0}^2-1472F_{5,0}-6498)x^5y
+
\\
&
\,\,\,\,\,\,\,\,
+
(-200F_{5,0}^2-3590F_{5,0}-16308)x^4y^2
+
(-\tfrac{800}{3}F_{5,0}^2-\tfrac{14240}{3}F_{5,0}-21568)x^3y^3
+
\\
&
\,\,\,\,\,\,\,\,
+
(-200F_{5,0}^2-3590F_{5,0}-16308)x^2y^4
+
(-80F_{5,0}^2-1472F_{5,0}-6498)xy^5
+
\\
&
\,\,\,\,\,\,\,\,
+
(-\tfrac{40}{3}F_{5,0}^2-\tfrac{766}{3}F_{5,0}-1136)y^6
+
\cdots,
\endaligned\right.
\]
for any value for $F_{5,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := 
-
(70F_{5,0}u-25F_{5,0}v+25F_{5,0}x-5F_{5,0}y+613u-226v+223x-46y-1)\partial_x
+
\\
&
\,\,\,\,\,\,\,\,
-
(70F_{5,0}u-25F_{5,0}v-5F_{5,0}x+25F_{5,0}y+613u-226v-43x+220y)\partial_y
+
\\
&
\,\,\,\,\,\,\,\,
-
(50F_{5,0}u-5F_{5,0}v+443u-46v-y)\partial_u
+
(20F_{5,0}u-50F_{5,0}v+166u-446v+2x)\partial_v,\\
e_2 & := 
-
(70F_{5,0}u-25F_{5,0}v+25F_{5,0}x-5F_{5,0}y+613u-226v+220x-43y)\partial_x
+
\\
&
\,\,\,\,\,\,\,\,
-
(70F_{5,0}u-25F_{5,0}v-5F_{5,0}x+25F_{5,0}y+613u-226v-46x+223y-1)\partial_y
+
\\
&
\,\,\,\,\,\,\,\,
-
(50F_{5,0}u-5F_{5,0}v+443u-46v-x)\partial_u
+
(20F_{5,0}u-50F_{5,0}v+166u-446v+2y)\partial_v.
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 
0 & -(30F_{5,0}+266)e_1+(30F_{5,0}+266)e_2
\\
e_2 &
(30F_{5,0}+266)e_1-(30F_{5,0}+266)e_2 & 0
\end{array}
\]

\rotatebox[origin=c]{90}{
\begin{tabular}{p{3cm}}
\end{tabular}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3j4g}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+y^3-\tfrac{1}{4}x^4-10x^3y-\tfrac{21}{2}x^2y^2-10xy^3-\tfrac{1}{4}y^4-\tfrac{37}{4}x^5-\tfrac{53}{4}x^4y
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{67}{2}x^3y^2+\tfrac{67}{2}x^2y^3-\tfrac{53}{4}xy^4-\tfrac{37}{4}y^5
+
\cdots
,
\\
v
&
\,=\,
x^2+y^2-6x^2y-6xy^2-\tfrac{13}{2}x^4-8x^3y+15x^2y^2-8xy^3-\tfrac{13}{2}y^4-\tfrac{1}{2}x^5
+
\\
&
\,\,\,\,\,\,\,\,
+\tfrac{199}{2}x^4y+139x^3y^2+139x^2y^3+\tfrac{199}{2}xy^4-\tfrac{1}{2}y^5
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\aligned
e_1 & := 
(1+\tfrac{9}{5}y+\tfrac{49}{5}u+4v)\partial_x
+
(-\tfrac{6}{5}x+3y+\tfrac{49}{5}u+4v)\partial_y
+
(y+3u+\tfrac{9}{5}v)\partial_u
-
(-2x+\tfrac{54}{5}u)\partial_v,\\
e_2 & := 
(-\tfrac{3}{5}y+\tfrac{7}{5}u+7v)\partial_x
+
(1+\tfrac{12}{5}x-3y+\tfrac{7}{5}u+7v)\partial_y
-
(-x+3u-\tfrac{12}{5}v)\partial_u
-
(-2y+\tfrac{42}{5}u+6v)\partial_v,\\
e_3 & := 
(x-\tfrac{1}{5}y+\tfrac{14}{5}u-v)\partial_x
+
(-\tfrac{1}{5}x+y+\tfrac{14}{5}u-v)\partial_y
+
(2u-\tfrac{1}{5}v)\partial_u
-
(\tfrac{4}{5}u-2v)\partial_v,
\endaligned
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 
0 
&
-\tfrac{9}{5}e_1-\tfrac{3}{5}e_2+\tfrac{3}{5}e_3
&
e_1-\tfrac{1}{5}e_2-\tfrac{7}{5}e_3
\\
e_2 &
\tfrac{9}{5}e_1+\tfrac{3}{5}e_2-\tfrac{3}{5}e_3 & 0
& 
-\tfrac{1}{5}e_1+e_2+\tfrac{11}{5}e_3
\\
e_3 &
-e_1+\tfrac{1}{5}e_2+\tfrac{7}{5}e_3
& 
\tfrac{1}{5}e_1-e_2-\tfrac{11}{5}e_3
& 
0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3k}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy-2y^3+2x^3
+
(-\tfrac{1}{4}F_{3,1}+\tfrac{1}{2}G_{0,4}+\tfrac{1}{8}G_{3,1})y^4
+
\\
&
\ \ \ \ \
+
(\tfrac{1}{2}G_{1,3}+F_{3,1}-\tfrac{1}{2}G_{3,1})xy^3
+
F_{2,2}x^2y^2+F_{3,1}x^3y+F_{4,0}x^4+\cdots
,
\\
v
&
\,=\,
y^2+x^2+4xy^2-4x^2y+G_{0,4}y^4+G_{1,3}xy^3
+
\\
&
\ \ \ \ \
+
(2F_{2,2}+3F_{3,1}-\tfrac{3}{2}G_{3,1}+64)x^2y^2
+
G_{3,1}x^3y
+
\\
&
\ \ \ \ \
+
(\tfrac{1}{2}F_{3,1}+2F_{4,0}-\tfrac{1}{4}G_{3,1})x^4
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(1+8u-8v+\tfrac{3}{4}xF_{2,2}-\tfrac{7}{2}xF_{4,0}+\tfrac{7}{16}G_{1,3}x-\tfrac{9}{16}xG_{3,1}+\tfrac{1}{4}yF_{2,2}-\tfrac{1}{2}yF_{4,0}+\tfrac{1}{16}yG_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{3}{16}yG_{3,1}-vF_{3,1}+2uF_{2,2}-8uF_{4,0}+\tfrac{3}{2}uG_{1,3}-3uG_{3,1}+\tfrac{3}{2}vF_{2,2}-7vF_{4,0}+\tfrac{3}{8}vG_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{5}{8}vG_{3,1}+4y)\partial_x
-
(2uF_{3,1}+32u+4v-\tfrac{1}{4}xF_{2,2}+\tfrac{1}{2}xF_{4,0}-\tfrac{1}{16}G_{1,3}x+\tfrac{3}{16}xG_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{3}{4}yF_{2,2}+\tfrac{7}{2}yF_{4,0}-\tfrac{7}{16}yG_{1,3}+\tfrac{9}{16}yG_{3,1}+4uF_{2,2}-12uF_{4,0}+uG_{1,3}-\tfrac{5}{2}uG_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{3}{2}vF_{2,2}-3vF_{4,0}+\tfrac{7}{8}vG_{1,3}-\tfrac{9}{8}vG_{3,1}+2y+2x)\partial_y
+
(y+\tfrac{3}{2}uF_{2,2}-7uF_{4,0}+\tfrac{7}{8}uG_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{9}{8}uG_{3,1}-2u+4v+\tfrac{1}{4}vF_{2,2}-\tfrac{1}{2}vF_{4,0}+\tfrac{1}{16}vG_{1,3}-\tfrac{3}{16}vG_{3,1})\partial_u
+
\\
&
\ \ \ \ \
+
(uF_{2,2}-2uF_{4,0}-4u+2x+\tfrac{1}{4}uG_{1,3}-\tfrac{3}{4}uG_{3,1}+\tfrac{3}{2}vF_{2,2}-7vF_{4,0}+\tfrac{7}{8}vG_{1,3}-\tfrac{9}{8}vG_{3,1})\partial_v
, 
\\
e_2
&
\,:=\,
-
(32u+4v-\tfrac{9}{16}xG_{1,3}+\tfrac{7}{8}xF_{3,1}-\tfrac{7}{4}xG_{0,4}+\tfrac{3}{4}xF_{2,2}-\tfrac{3}{16}yG_{1,3}+\tfrac{1}{8}yF_{3,1}-\tfrac{1}{4}yG_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{1}{4}yF_{2,2}-\tfrac{3}{2}uG_{3,1}+\tfrac{1}{2}vG_{3,1}-\tfrac{3}{2}uG_{1,3}+5uF_{3,1}-6uG_{0,4}+4uF_{2,2}-\tfrac{9}{8}vG_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{3}{4}vF_{3,1}-\tfrac{3}{2}vG_{0,4}+\tfrac{3}{2}vF_{2,2}-2x-2y)\partial_x
+
(8u+1-8v+\tfrac{3}{16}xG_{1,3}-\tfrac{1}{8}xF_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{1}{4}xG_{0,4}-\tfrac{1}{4}xF_{2,2}+\tfrac{9}{16}yG_{1,3}-\tfrac{7}{8}yF_{3,1}+\tfrac{7}{4}yG_{0,4}-\tfrac{3}{4}yF_{2,2}+\tfrac{1}{2}uG_{3,1}-3uG_{1,3}
+
\\
&
\ \ \ \ \
+2uF_{3,1}-4uG_{0,4}+2uF_{2,2}-\tfrac{9}{8}vG_{1,3}+\tfrac{3}{4}vF_{3,1}-\tfrac{7}{2}vG_{0,4}+\tfrac{3}{2}vF_{2,2}-4x)\partial_y
+
\\
&
\ \ \ \ \
-
(-x-\tfrac{9}{8}uG_{1,3}+\tfrac{7}{4}uF_{3,1}-\tfrac{7}{2}uG_{0,4}+\tfrac{3}{2}uF_{2,2}-2u-\tfrac{3}{16}vG_{1,3}+\tfrac{1}{8}vF_{3,1}-\tfrac{1}{4}vG_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{1}{4}vF_{2,2}+4v)\partial_u
-
(-2y-4u-\tfrac{3}{4}uG_{1,3}+\tfrac{1}{2}uF_{3,1}-uG_{0,4}+uF_{2,2}-\tfrac{9}{8}vG_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{7}{4}vF_{3,1}-\tfrac{7}{2}vG_{0,4}+\tfrac{3}{2}vF_{2,2})\partial_v,
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^6 \ni F_{2,2},F_{3,1},F_{4,0},G_{0,4},G_{1,3},G_{3,1}$:
\[
\aligned
\B_1 & := -16F_{2,2}G_{1,3}+16F_{2,2}G_{3,1}+4F_{3,1}^2-16F_{3,1}G_{0,4}-10F_{3,1}G_{1,3}+10F_{3,1}G_{3,1}-64F_{4,0}^2
+
\\
&
\ \ \ \ \
+56F_{4,0}G_{1,3}-40F_{4,0}G_{3,1}+16G_{0,4}^2+20G_{0,4}G_{1,3}-20G_{0,4}G_{3,1}+5G_{1,3}G_{3,1}-6G_{3,1}^2
+
\\
&
\ \ \ \ \
-32F_{3,1}-128F_{4,0}+64G_{0,4}+16G_{3,1};
\\
\B_2 & := 16F_{2,2}G_{1,3}-16F_{2,2}G_{3,1}+16F_{3,1}F_{4,0}+8F_{3,1}G_{0,4}+6F_{3,1}G_{1,3}-10F_{3,1}G_{3,1}+64F_{4,0}^2
+
\\
&
\ \ \ \ \
-56F_{4,0}G_{1,3}+32F_{4,0}G_{3,1}-16G_{0,4}^2-20G_{0,4}G_{1,3}+24G_{0,4}G_{3,1}-3G_{1,3}G_{3,1}+5G_{3,1}^2
+
\\
&
\ \ \ \ \
+128F_{3,1}+512F_{4,0}-256G_{0,4}-96G_{1,3}+32G_{3,1},
\\
\B_3 & := 128F_{2,2}F_{3,1}-1280F_{2,2}G_{0,4}+560F_{2,2}G_{1,3}-816F_{2,2}G_{3,1}+272F_{3,1}G_{0,4}+86F_{3,1}G_{1,3}
+
\\
&
\ \ \ \ \
-506F_{3,1}G_{3,1}+3072F_{4,0}^2+5184F_{4,0}G_{0,4}-2984F_{4,0}G_{1,3}+1944F_{4,0}G_{3,1}-544G_{0,4}^2
+
\\
&
\ \ \ \ \
-828G_{0,4}G_{1,3}+1788G_{0,4}G_{3,1}+160G_{1,3}^2-139G_{1,3}G_{3,1}+253G_{3,1}^2-10752F_{2,2}
+
\\
&
\ \ \ \ \
+6880F_{3,1}+71552F_{4,0}-19904G_{0,4}-11968G_{1,3}+8528G_{3,1}-40960,
\\
\B_4 & := 64F_{2,2}^2+1536F_{2,2}G_{0,4}-288F_{2,2}G_{1,3}+576F_{2,2}G_{3,1}-144F_{3,1}G_{0,4}+90F_{3,1}G_{1,3}
+
\\
&
\ \ \ \ \
+330F_{3,1}G_{3,1}-2304F_{4,0}^2-6720F_{4,0}G_{0,4}+2184F_{4,0}G_{1,3}-1464F_{4,0}G_{3,1}+288G_{0,4}^2
+
\\
&
\ \ \ \ \
+540G_{0,4}G_{1,3}-1692G_{0,4}G_{3,1}-192G_{1,3}^2+51G_{1,3}G_{3,1}-165G_{3,1}^2+15616F_{2,2}
+
\\
&
\ \ \ \ \
-5600F_{3,1}-86400F_{4,0}+19392G_{0,4}+13824G_{1,3}-11408G_{3,1}+55296,
\\
\B_5 & := 28128F_{2,2}G_{1,3}^2-19328F_{2,2}G_{1,3}G_{3,1}-8800F_{2,2}G_{3,1}^2-5522F_{3,1}G_{1,3}^2
+
\\
&
\ \ \ \ \
+29508F_{3,1}G_{1,3}G_{3,1}-23986F_{3,1}G_{3,1}^2+77312F_{4,0}^2G_{1,3}-77312F_{4,0}^2G_{3,1}
+
\\
&
\ \ \ \ \
-163592F_{4,0}G_{1,3}^2+234000F_{4,0}G_{1,3}G_{3,1}-70408F_{4,0}G_{3,1}^2+11044G_{0,4}G_{1,3}^2
+
\\
&
\ \ \ \ \
-59016G_{0,4}G_{1,3}G_{3,1}+47972G_{0,4}G_{3,1}^2+15164G_{1,3}^3-50755G_{1,3}^2G_{3,1}+38762G_{1,3}G_{3,1}^2
+
\\
&
\ \ \ \ \
-3171G_{3,1}^3-887296F_{2,2}G_{1,3}+887296F_{2,2}G_{3,1}-399136F_{3,1}G_{1,3}+642784F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \
+2107264F_{4,0}G_{1,3}-1132672F_{4,0}G_{3,1}+489024G_{0,4}G_{1,3}-976320G_{0,4}G_{3,1}-60960G_{1,3}^2
+
\\
&
\ \ \ \ \
+199568G_{1,3}G_{3,1}-260432G_{3,1}^2-3537408F_{3,1}-14149632F_{4,0}+7074816G_{0,4}
+
\\
&
\ \ \ \ \
+293888G_{1,3}+1474816G_{3,1},
\\
\B_6 & := 19328F_{2,2}G_{0,4}G_{1,3}-19328F_{2,2}G_{0,4}G_{3,1}+5232F_{2,2}G_{1,3}^2-5232F_{2,2}G_{3,1}^2+1410F_{3,1}G_{1,3}^2
+
\\
&
\ \ \ \ \
+4828F_{3,1}G_{1,3}G_{3,1}-6238F_{3,1}G_{3,1}^2-77312F_{4,0}G_{0,4}G_{1,3}+77312F_{4,0}G_{0,4}G_{3,1}+
\\
&
\ \ \ \ \
-15288F_{4,0}G_{1,3}^2+19312F_{4,0}G_{1,3}G_{3,1}-4024F_{4,0}G_{3,1}^2+4428G_{0,4}G_{1,3}^2
+
\\
&
\ \ \ \ \
-28984G_{0,4}G_{1,3}G_{3,1}+24556G_{0,4}G_{3,1}^2+552G_{1,3}^3-7393G_{1,3}^2G_{3,1}+6690G_{1,3}G_{3,1}^2
+
\\
&
\ \ \ \ \
+151G_{3,1}^3+29952F_{2,2}G_{1,3}-29952F_{2,2}G_{3,1}-116320F_{3,1}G_{1,3}+162976F_{3,1}G_{3,1}
+
\\
&
\ \ \ \ \
-585088F_{4,0}G_{1,3}+771712F_{4,0}G_{3,1}+271296G_{0,4}G_{1,3}-364608G_{0,4}G_{3,1}+138016G_{1,3}^2
+
\\
&
\ \ \ \ \
-251088G_{1,3}G_{3,1}+89744G_{3,1}^2-677376F_{3,1}-2709504F_{4,0}+1354752G_{0,4}
+
\\
&
\ \ \ \ \
+737280G_{1,3}-398592G_{3,1},
\\
\B_7 & := -7392F_{2,2}G_{1,3}^2+7248F_{2,2}G_{1,3}G_{3,1}+144F_{2,2}G_{3,1}^2+4832F_{3,1}G_{0,4}^2-2416F_{3,1}G_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \
-3588F_{3,1}G_{1,3}^2+3408F_{3,1}G_{1,3}G_{3,1}+482F_{3,1}G_{3,1}^2+19328F_{4,0}G_{0,4}^2-9664F_{4,0}G_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \
+15216F_{4,0}G_{1,3}^2-15360F_{4,0}G_{1,3}G_{3,1}+1352F_{4,0}G_{3,1}^2-9664G_{0,4}^3-4832G_{0,4}^2G_{1,3}
+
\endaligned
\]

\[
\aligned
&
\ \ \ \ \
+7248G_{0,4}^2G_{3,1}+7176G_{0,4}G_{1,3}^2-4400G_{0,4}G_{1,3}G_{3,1}-2172G_{0,4}G_{3,1}^2+816G_{1,3}^3
+
\\
&
\ \ \ \ \
+2136G_{1,3}^2G_{3,1}-3254G_{1,3}G_{3,1}^2+151G_{3,1}^3+109824F_{2,2}G_{1,3}-109824F_{2,2}G_{3,1}
+
\\
&
\ \ \ \ \
+135296F_{3,1}G_{0,4}+69176F_{3,1}G_{1,3}-93800F_{3,1}G_{3,1}+541184F_{4,0}G_{0,4}-162592F_{4,0}G_{1,3}
+
\\
&
\ \ \ \ \
+64096F_{4,0}G_{3,1}-270592G_{0,4}^2-273648G_{0,4}G_{1,3}+255248G_{0,4}G_{3,1}-42776G_{1,3}^2
+
\\
&
\ \ \ \ \
+33060G_{1,3}G_{3,1}+22028G_{3,1}^2+802048F_{3,1}+3208192F_{4,0}-1604096G_{0,4}
+
\\
&
\ \ \ \ \
-582400G_{1,3}+181376G_{3,1},
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & \rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(-2+\tfrac{1}{2}G_{1,3}-\tfrac{7}{8}F_{3,1}-F_{2,2}+\tfrac{1}{2}F_{4,0}+\tfrac{7}{4}G_{0,4}+\tfrac{3}{16}G_{3,1})e_1+(-2-\tfrac{1}{4}G_{1,3}-\tfrac{1}{8}F_{3,1}-F_{2,2}+\tfrac{7}{2}F_{4,0}+\tfrac{1}{4}G_{0,4}+\tfrac{9}{16}G_{3,1})e_2$
\end{tabular}}
\\
e_2 &
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(-2+\tfrac{1}{2}G_{1,3}-\tfrac{7}{8}F_{3,1}-F_{2,2}+\tfrac{1}{2}F_{4,0}+\tfrac{7}{4}G_{0,4}+\tfrac{3}{16}G_{3,1})e_1-(-2-\tfrac{1}{4}G_{1,3}-\tfrac{1}{8}F_{3,1}-F_{2,2}+\tfrac{7}{2}F_{4,0}+\tfrac{1}{4}G_{0,4}+\tfrac{9}{16}G_{3,1})e_2$
\end{tabular}}
& 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3n4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+4xy^3+4x^3y
+
\tfrac{1}{2}G_{5,0}y^5+5F_{5,0}xy^4+5G_{5,0}x^2y^3+10F_{5,0}x^3y^2
+
\\
&
\ \ \ \ \
+\tfrac{5}{2}G_{5,0}x^4y+F_{5,0}x^5+\tfrac{5}{4}F_{5,0}G_{5,0}y^6+(24+\tfrac{15}{8}G_{5,0}^2+\tfrac{15}{2}F_{5,0}^2)xy^5
+
\\
&
\ \ \ \ \
+\tfrac{75}{4}F_{5,0}G_{5,0}x^2y^4+(80+25F_{5,0}^2+\tfrac{25}{4}G_{5,0}^2)x^3y^3+\tfrac{75}{4}F_{5,0}G_{5,0}x^4y^2
+
\\
&
\ \ \ \ \
+(24+\tfrac{15}{8}G_{5,0}^2+\tfrac{15}{2}F_{5,0}^2)x^5y+\tfrac{5}{4}F_{5,0}G_{5,0}x^6+(\tfrac{34}{7}G_{5,0}+\tfrac{25}{112}G_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{75}{28}F_{5,0}^2G_{5,0})y^7+(68F_{5,0}+\tfrac{75}{8}F_{5,0}G_{5,0}^2+\tfrac{25}{2}F_{5,0}^3)xy^6+(102G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{75}{16}G_{5,0}^3+\tfrac{225}{4}F_{5,0}^2G_{5,0})x^2y^5+(340F_{5,0}+\tfrac{125}{2}F_{5,0}^3+\tfrac{375}{8}F_{5,0}G_{5,0}^2)x^3y^4
+
\\
&
\ \ \ \ \
+(170G_{5,0}+\tfrac{375}{4}F_{5,0}^2G_{5,0}+\tfrac{125}{16}G_{5,0}^3)x^4y^3+(204F_{5,0}+\tfrac{75}{2}F_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{225}{8}F_{5,0}G_{5,0}^2)x^5y^2+(34G_{5,0}+\tfrac{25}{16}G_{5,0}^3+\tfrac{75}{4}F_{5,0}^2G_{5,0})x^6y+(\tfrac{68}{7}F_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{75}{56}F_{5,0}G_{5,0}^2+\tfrac{25}{14}F_{5,0}^3)x^7
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2+2y^4+12x^2y^2+2x^4+2F_{5,0}y^5+5G_{5,0}xy^4+20F_{5,0}x^2y^3
+
\\
&
\ \ \ \ \
+10G_{5,0}x^3y^2+10F_{5,0}x^4y+G_{5,0}x^5+(8+\tfrac{5}{8}G_{5,0}^2+\tfrac{5}{2}F_{5,0}^2)y^6
+
\\
&
\ \ \ \ \
+15F_{5,0}G_{5,0}xy^5+(120+\tfrac{75}{8}G_{5,0}^2+\tfrac{75}{2}F_{5,0}^2)x^2y^4+50F_{5,0}G_{5,0}x^3y^3
+
\\
&
\ \ \ \ \
+(120+\tfrac{75}{8}G_{5,0}^2+\tfrac{75}{2}F_{5,0}^2)x^4y^2+15F_{5,0}G_{5,0}x^5y+(8+\tfrac{5}{8}G_{5,0}^2+\tfrac{5}{2}F_{5,0}^2)x^6
+
\\
&
\ \ \ \ \
+(\tfrac{136}{7}F_{5,0}+\tfrac{25}{7}F_{5,0}^3+\tfrac{75}{28}F_{5,0}G_{5,0}^2)y^7+(68G_{5,0}+\tfrac{25}{8}G_{5,0}^3+\tfrac{75}{2}F_{5,0}^2G_{5,0})xy^6
+
\\
&
\ \ \ \ \
+(408F_{5,0}+75F_{5,0}^3+\tfrac{225}{4}F_{5,0}G_{5,0}^2)x^2y^5+(340G_{5,0}+\tfrac{125}{8}G_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{375}{2}F_{5,0}^2G_{5,0})x^3y^4+(125F_{5,0}^3+\tfrac{375}{4}F_{5,0}G_{5,0}^2+680F_{5,0})x^4y^3
+
\\
&
\ \ \ \ \
+(204G_{5,0}+\tfrac{75}{8}G_{5,0}^3+\tfrac{225}{2}F_{5,0}^2G_{5,0})x^5y^2+(136F_{5,0}+25F_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{75}{4}F_{5,0}G_{5,0}^2)x^6y+(\tfrac{68}{7}G_{5,0}+\tfrac{25}{56}G_{5,0}^3+\tfrac{75}{14}F_{5,0}^2G_{5,0})x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-(-1+\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_x-(\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_y
+
\\
&
\ \ \ \ \
-(-y+\tfrac{5}{2}uG_{5,0}+\tfrac{5}{2}vF_{5,0})\partial_u-(-2x+10F_{5,0}u+\tfrac{5}{2}vG_{5,0})\partial_v
, 
\\
e_2
&
\,:=\,
-(\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_x-(-1+\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_y
+
\\
&
\ \ \ \ \
-(-x+5F_{5,0}u+\tfrac{5}{4}vG_{5,0})\partial_u-(5F_{5,0}v+5G_{5,0}u-2y)\partial_v
,
\end{array}
\]
for any value of $F_{5,0},G_{5,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3n4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+y^4+6x^2y^2+x^4+\tfrac{1}{2}G_{5,0}y^5+5F_{5,0}xy^4+5G_{5,0}x^2y^3+10F_{5,0}x^3y^2
+
\\
&
\ \ \ \ \
+\tfrac{5}{2}G_{5,0}x^4y+F_{5,0}x^5+(\tfrac{5}{4}F_{5,0}^2+\tfrac{5}{16}G_{5,0}^2)y^6+(24+\tfrac{15}{2}F_{5,0}G_{5,0})xy^5
+
\\
&
\ \ \ \ \
+(\tfrac{75}{4}F_{5,0}^2+\tfrac{75}{16}G_{5,0}^2)x^2y^4+(25F_{5,0}G_{5,0}+80)x^3y^3+(\tfrac{75}{4}F_{5,0}^2
+
\\
&
\ \ \ \ \
+\tfrac{75}{16}G_{5,0}^2)x^4y^2+(24+\tfrac{15}{2}F_{5,0}G_{5,0})x^5y+(\tfrac{5}{4}F_{5,0}^2+\tfrac{5}{16}G_{5,0}^2)x^6
+
\\
&
\ \ \ \ \
+(\tfrac{68}{7}F_{5,0}+\tfrac{75}{28}F_{5,0}^2G_{5,0}+\tfrac{25}{112}G_{5,0}^3)y^7+(\tfrac{25}{2}F_{5,0}^3+\tfrac{75}{8}G_{5,0}^2F_{5,0}
+
\\
&
\ \ \ \ \
+34G_{5,0})xy^6+(204F_{5,0}+\tfrac{225}{4}F_{5,0}^2G_{5,0}+\tfrac{75}{16}G_{5,0}^3)x^2y^5+(170G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{125}{2}F_{5,0}^3+\tfrac{375}{8}G_{5,0}^2F_{5,0})x^3y^4+(340F_{5,0}+\tfrac{375}{4}F_{5,0}^2G_{5,0}+\tfrac{125}{16}G_{5,0}^3)x^4y^3
+
\\
&
\ \ \ \ \
+(102G_{5,0}+\tfrac{75}{2}F_{5,0}^3+\tfrac{225}{8}G_{5,0}^2F_{5,0})x^5y^2+(68F_{5,0}+\tfrac{75}{4}F_{5,0}^2G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{25}{16}G_{5,0}^3)x^6y+(\tfrac{25}{14}F_{5,0}^3+\tfrac{75}{56}G_{5,0}^2F_{5,0}+\tfrac{34}{7}G_{5,0})x^7
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2+8xy^3+8x^3y+2F_{5,0}y^5+5G_{5,0}xy^4+20F_{5,0}x^2y^3
+
\\
&
\ \ \ \ \
+10G_{5,0}x^3y^2+10F_{5,0}x^4y+G_{5,0}x^5+(\tfrac{5}{2}F_{5,0}G_{5,0}+8)y^6+(15F_{5,0}^2
+
\\
&
\ \ \ \ \
+\tfrac{15}{4}G_{5,0}^2)xy^5+(120+\tfrac{75}{2}F_{5,0}G_{5,0})x^2y^4+(\tfrac{25}{2}G_{5,0}^2+50F_{5,0}^2)x^3y^3
+
\\
&
\ \ \ \ \
+(120+\tfrac{75}{2}F_{5,0}G_{5,0})x^4y^2+15F_{5,0}^2+\tfrac{15}{4}G_{5,0}^2)x^5y+(\tfrac{5}{2}F_{5,0}G_{5,0}
+
\\
&
\ \ \ \ \
+8)x^6+(\tfrac{68}{7}G_{5,0}+\tfrac{25}{7}F_{5,0}^3+\tfrac{75}{28}G_{5,0}^2F_{5,0})y^7+(136F_{5,0}+\tfrac{75}{2}F_{5,0}^2G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{25}{8}G_{5,0}^3)xy^6+(204G_{5,0}+75F_{5,0}^3+\tfrac{225}{4}G_{5,0}^2F_{5,0})x^2y^5+(680F_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{375}{2}F_{5,0}^2G_{5,0}+\tfrac{125}{8}G_{5,0}^3)x^3y^4+(125F_{5,0}^3+\tfrac{375}{4}G_{5,0}^2F_{5,0}+340G_{5,0})x^4y^3
+
\\
&
\ \ \ \ \
+(408F_{5,0}+\tfrac{225}{2}F_{5,0}^2G_{5,0}+\tfrac{75}{8}G_{5,0}^3)x^5y^2+(68G_{5,0}+25F_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{75}{4}G_{5,0}^2F_{5,0})x^6y+(\tfrac{136}{7}F_{5,0}+\tfrac{75}{14}F_{5,0}^2G_{5,0}+\tfrac{25}{56}G_{5,0}^3)x^7
+
\cdots.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-(-1+\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_x-(\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_y
+
\\
&
\ \ \ \ \
-(-y+5uF_{5,0}+\tfrac{5}{4}vG_{5,0})\partial_u-(5F_{5,0}v+5G_{5,0}u-2x)\partial_v 
,
\\
e_2
&
\,:=\,
-(\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_x-(-1+\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_y
+
\\
&
\ \ \ \ \
-(-x+\tfrac{5}{2}G_{5,0}u+\tfrac{5}{2}F_{5,0}v)\partial_u-(-2y+10uF_{5,0}+\tfrac{5}{2}vG_{5,0})\partial_v,
\end{array}
\]
for any value of $F_{5,0},G_{5,0}$,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\text{\bf Model 2f3n4c}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+\tfrac{1}{2}y^4+2xy^3+3x^2y^2+2x^3y+\tfrac{1}{2}x^4+F_{5,0}y^5+5F_{5,0}xy^4+10F_{5,0}x^2y^3
+
\\
&
\ \ \ \ \
+10F_{5,0}x^3y^2+5F_{5,0}x^4y+F_{5,0}x^5+(\tfrac{5}{2}F_{5,0}^2+2)y^6+(15F_{5,0}^2+12)xy^5
+
\\
&
\ \ \ \ \
+(\tfrac{75}{2}F_{5,0}^2+30)x^2y^4+(50F_{5,0}^2+40)x^3y^3+(\tfrac{75}{2}F_{5,0}^2+30)x^4y^2
+
\\
&
\ \ \ \ \
+(15F_{5,0}^2+12)x^5y+(\tfrac{5}{2}F_{5,0}^2+2)x^6+(\tfrac{50}{7}F_{5,0}^3+\tfrac{68}{7}F_{5,0})y^7+(50F_{5,0}^3
+
\\
&
\ \ \ \ \
+68F_{5,0})xy^6+(150F_{5,0}^3+204F_{5,0})x^2y^5+(250F_{5,0}^3+340F_{5,0})x^3y^4
+
\\
&
\ \ \ \ \
+(250F_{5,0}^3+340F_{5,0})x^4y^3+(150F_{5,0}^3+204F_{5,0})x^5y^2+(50F_{5,0}^3+68F_{5,0})x^6y
+
\\
&
\ \ \ \ \
+(\tfrac{50}{7}F_{5,0}^3+\tfrac{68}{7}F_{5,0})x^7
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2+y^4+4xy^3+6x^2y^2+4x^3y+x^4+2F_{5,0}y^5+10F_{5,0}xy^4+20F_{5,0}x^2y^3
+
\\
&
\ \ \ \ \
+20F_{5,0}x^3y^2+10F_{5,0}x^4y+2F_{5,0}x^5+(5F_{5,0}^2+4)y^6+(30F_{5,0}^2+24)xy^5
+
\\
&
\ \ \ \ \
+(75F_{5,0}^2+60)x^2y^4+(100F_{5,0}^2+80)x^3y^3+(75F_{5,0}^2+60)x^4y^2+(30F_{5,0}^2
+
\\
&
\ \ \ \ \
+24)x^5y+(5F_{5,0}^2+4)x^6+(\tfrac{100}{7}F_{5,0}^3+\tfrac{136}{7}F_{5,0})y^7+(100F_{5,0}^3+136F_{5,0})xy^6
+
\\
&
\ \ \ \ \
+(300F_{5,0}^3+408F_{5,0})x^2y^5+(500F_{5,0}^3+680F_{5,0})x^3y^4+(500F_{5,0}^3+680F_{5,0})x^4y^3
+
\\
&
\ \ \ \ \
+(300F_{5,0}^3+408F_{5,0})x^5y^2+(100F_{5,0}^3+136F_{5,0})x^6y+(\tfrac{100}{7}F_{5,0}^3+\tfrac{136}{7}F_{5,0})x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-(5F_{5,0}x+4u+2v-1)\partial_x-(5F_{5,0}y+4u+2v)\partial_y-(10F_{5,0}u-y)\partial_u-(10F_{5,0}v-2x)\partial_v
, 
\\
e_2
&
\,:=\,
-(5F_{5,0}x+4u+2v)\partial_x-(5F_{5,0}y+4u+2v-1)\partial_y-(10F_{5,0}u-x)\partial_u-(10F_{5,0}v-2y)\partial_v
, 
\\
e_3
&
\,:=\,
-(x-y)\partial_x+(x-y)\partial_y-(2u-v)\partial_u+(4u-2v)\partial_v
.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & -5F_{5,0}e_1+5F_{5,0}e_2 &-e_1+e_2
\\
e_2 & 5F_{5,0}e_1-5F_{5,0}e_2 & 0 & e_1-e_2
\\
e_3 & e_1-e_2 & -e_1+e_2 & 0
\end{array}
\]
for any value of $F_{5,0}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3n4d}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy-y^4-6x^2y^2-x^4+\tfrac{1}{2}G_{5,0}y^5+5F_{5,0}xy^4+5G_{5,0}x^2y^3+10F_{5,0}x^3y^2
+
\\
&
\ \ \ \ \
+\tfrac{5}{2}G_{5,0}x^4y+F_{5,0}x^5
+
(-\tfrac{5}{4}F_{5,0}^2-\tfrac{5}{16}G_{5,0}^2)y^6+(24-\tfrac{15}{2}F_{5,0}G_{5,0})xy^5
+
\\
&
\ \ \ \ \
+
(-\tfrac{75}{4}F_{5,0}^2-\tfrac{75}{16}G_{5,0}^2)x^2y^4
+
(-25F_{5,0}G_{5,0}+80)x^3y^3
+
(-\tfrac{75}{4}F_{5,0}^2
+
\\
&
\ \ \ \ \
-\tfrac{75}{16}G_{5,0}^2)x^4y^2
+
(24-\tfrac{15}{2}F_{5,0}G_{5,0})x^5y
+
(-\tfrac{5}{4}F_{5,0}^2-\tfrac{5}{16}G_{5,0}^2)x^6
+
\\
&
\ \ \ \ \
+
(-\tfrac{68}{7}F_{5,0}+\tfrac{75}{28}F_{5,0}^2G_{5,0}+\tfrac{25}{112}G_{5,0}^3)y^7
+
(\tfrac{25}{2}F_{5,0}^3+\tfrac{75}{8}G_{5,0}^2F_{5,0}
+
\\
&
\ \ \ \ \
-34G_{5,0})xy^6
+
(-204F_{5,0}+\tfrac{225}{4}F_{5,0}^2G_{5,0}+\tfrac{75}{16}G_{5,0}^3)x^2y^5
+
(-170G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{125}{2}F_{5,0}^3+\tfrac{375}{8}G_{5,0}^2F_{5,0})x^3y^4
+
(-340F_{5,0}+\tfrac{375}{4}F_{5,0}^2G_{5,0}+\tfrac{125}{16}G_{5,0}^3)x^4y^3
+
\\
&
\ \ \ \ \
+
(-102G_{5,0}+\tfrac{75}{2}F_{5,0}^3+\tfrac{225}{8}G_{5,0}^2F_{5,0})x^5y^2
+
(-68F_{5,0}+\tfrac{75}{4}F_{5,0}^2G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{25}{16}G_{5,0}^3)x^6y
+
(\tfrac{25}{14}F_{5,0}^3+\tfrac{75}{56}G_{5,0}^2F_{5,0}-\tfrac{34}{7}G_{5,0})x^7
+
\cdots
,
\endaligned\right.
\]

\[
\text{\bf Model 2f3n4d}
\ \ \ \ \
\left\{
\aligned
v
&
\,=\,
y^2+x^2-8xy^3-8x^3y+2F_{5,0}y^5+5G_{5,0}xy^4+20F_{5,0}x^2y^3+10G_{5,0}x^3y^2
+
\\
&
\ \ \ \ \
+10F_{5,0}x^4y+G_{5,0}x^5
+
(-\tfrac{5}{2}F_{5,0}G_{5,0}+8)y^6
+
(-15F_{5,0}^2-\tfrac{15}{4}G_{5,0}^2)xy^5
+
\\
&
\ \ \ \ \
+
(120-\tfrac{75}{2}F_{5,0}G_{5,0})x^2y^4
+
(-\tfrac{25}{2}G_{5,0}^2-50F_{5,0}^2)x^3y^3
+
(120
+
\\
&
\ \ \ \ \
-\tfrac{75}{2}F_{5,0}G_{5,0})x^4y^2
+
(-15F_{5,0}^2-\tfrac{15}{4}G_{5,0}^2)x^5y
+
(-\tfrac{5}{2}F_{5,0}G_{5,0}+8)x^6
+
\\
&
\ \ \ \ \
+
(-\tfrac{68}{7}G_{5,0}+\tfrac{25}{7}F_{5,0}^3+\tfrac{75}{28}G_{5,0}^2F_{5,0})y^7
+
(-136F_{5,0}+\tfrac{75}{2}F_{5,0}^2G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{25}{8}G_{5,0}^3)xy^6
+
(-204G_{5,0}+75F_{5,0}^3+\tfrac{225}{4}G_{5,0}^2F_{5,0})x^2y^5
+
(-680F_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{375}{2}F_{5,0}^2G_{5,0}+\tfrac{125}{8}G_{5,0}^3)x^3y^4
+
(125F_{5,0}^3+\tfrac{375}{4}G_{5,0}^2F_{5,0}-340G_{5,0})x^4y^3
+
\\
&
\ \ \ \ \
+
(-408F_{5,0}+\tfrac{225}{2}F_{5,0}^2G_{5,0}+\tfrac{75}{8}G_{5,0}^3)x^5y^2
+
(-68G_{5,0}+25F_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{75}{4}G_{5,0}^2F_{5,0})x^6y
+
(-\tfrac{136}{7}F_{5,0}+\tfrac{75}{14}F_{5,0}^2G_{5,0}+\tfrac{25}{56}G_{5,0}^3)x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(1+\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_x+(\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_y
+
\\
&
\ \ \ \ \
+(5uF_{5,0}+y+\tfrac{5}{4}vG_{5,0})\partial_u+(5F_{5,0}v+5G_{5,0}u+2x)\partial_v
, 
\\
e_2
&
\,:=\,
(\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_x+(1+\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_y
+
\\
&
\ \ \ \ \
+(x+\tfrac{5}{2}G_{5,0}u+\tfrac{5}{2}F_{5,0}v)\partial_u+(10uF_{5,0}+2y+\tfrac{5}{2}vG_{5,0})\partial_v
,
\end{array}
\]
for any value for $F_{5,0},G_{5,0}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3n4e}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy-4xy^3-4x^3y+\tfrac{1}{2}G_{5,0}y^5+5F_{5,0}xy^4+5G_{5,0}x^2y^3+10F_{5,0}x^3y^2
+
\\
&
\ \ \ \ \
+\tfrac{5}{2}G_{5,0}x^4y+F_{5,0}x^5-\tfrac{5}{4}F_{5,0}G_{5,0}y^6+(24-\tfrac{15}{8}G_{5,0}^2-\tfrac{15}{2}F_{5,0}^2)xy^5
+
\\
&
\ \ \ \ \
-\tfrac{75}{4}F_{5,0}G_{5,0}x^2y^4+(80-25F_{5,0}^2-\tfrac{25}{4}G_{5,0}^2)x^3y^3-\tfrac{75}{4}F_{5,0}G_{5,0}x^4y^2
+
\\
&
\ \ \ \ \
+(24-\tfrac{15}{8}G_{5,0}^2-\tfrac{15}{2}F_{5,0}^2)x^5y-\tfrac{5}{4}F_{5,0}G_{5,0}x^6+(-\tfrac{34}{7}G_{5,0}+\tfrac{25}{112}G_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{75}{28}F_{5,0}^2G_{5,0})y^7+(-68F_{5,0}+\tfrac{75}{8}F_{5,0}G_{5,0}^2+\tfrac{25}{2}F_{5,0}^3)xy^6+(-102G_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{75}{16}G_{5,0}^3+\tfrac{225}{4}F_{5,0}^2G_{5,0})x^2y^5+(-340F_{5,0}+\tfrac{125}{2}F_{5,0}^3+\tfrac{375}{8}F_{5,0}G_{5,0}^2)x^3y^4
+
\\
&
\ \ \ \ \
+(-170G_{5,0}+\tfrac{375}{4}F_{5,0}^2G_{5,0}+\tfrac{125}{16}G_{5,0}^3)x^4y^3+(-204F_{5,0}+\tfrac{75}{2}F_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{225}{8}F_{5,0}G_{5,0}^2)x^5y^2+(-34G_{5,0}+\tfrac{25}{16}G_{5,0}^3
+\tfrac{75}{4}F_{5,0}^2G_{5,0})x^6y+(-\tfrac{68}{7}F_{5,0}
+
\\
&
\ \ \ \ \
+\tfrac{75}{56}F_{5,0}G_{5,0}^2+\tfrac{25}{14}F_{5,0}^3)x^7
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2-2y^4-12x^2y^2-2x^4+2F_{5,0}y^5+5G_{5,0}xy^4+20F_{5,0}x^2y^3
+
\\
&
\ \ \ \ \
+10G_{5,0}x^3y^2+10F_{5,0}x^4y+G_{5,0}x^5+(8-\tfrac{5}{8}G_{5,0}^2-\tfrac{5}{2}F_{5,0}^2)y^6
+
\\
&
\ \ \ \ \
-15F_{5,0}G_{5,0}xy^5+(120-\tfrac{75}{8}G_{5,0}^2-\tfrac{75}{2}F_{5,0}^2)x^2y^4-50F_{5,0}G_{5,0}x^3y^3
+
\\
&
\ \ \ \ \
+(120-\tfrac{75}{8}G_{5,0}^2-\tfrac{75}{2}F_{5,0}^2)x^4y^2-15F_{5,0}G_{5,0}x^5y+(8-\tfrac{5}{8}G_{5,0}^2-\tfrac{5}{2}F_{5,0}^2)x^6
+
\\
&
\ \ \ \ \
+(-\tfrac{136}{7}F_{5,0}+\tfrac{25}{7}F_{5,0}^3+\tfrac{75}{28}F_{5,0}G_{5,0}^2)y^7+(-68G_{5,0}+\tfrac{25}{8}G_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{75}{2}F_{5,0}^2G_{5,0})xy^6+(-408F_{5,0}+75F_{5,0}^3+\tfrac{225}{4}F_{5,0}G_{5,0}^2)x^2y^5
+
\\
&
\ \ \ \ \
+(-340G_{5,0}+\tfrac{125}{8}G_{5,0}^3+\tfrac{375}{2}F_{5,0}^2G_{5,0})x^3y^4+(125F_{5,0}^3+\tfrac{375}{4}F_{5,0}G_{5,0}^2
+
\\
&
\ \ \ \ \
-680F_{5,0})x^4y^3+(-204G_{5,0}+\tfrac{75}{8}G_{5,0}^3+\tfrac{225}{2}F_{5,0}^2G_{5,0})x^5y^2+(-136F_{5,0}
+
\\
&
\ \ \ \ \
+25F_{5,0}^3+\tfrac{75}{4}F_{5,0}G_{5,0}^2)x^6y+(-\tfrac{68}{7}G_{5,0}+\tfrac{25}{56}G_{5,0}^3+\tfrac{75}{14}F_{5,0}^2G_{5,0})x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(1+\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_x+(\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_y+(y+\tfrac{5}{2}uG_{5,0}+\tfrac{5}{2}vF_{5,0})\partial_u
+
\\
&
\ \ \ \ \
+(2x+10F_{5,0}u+\tfrac{5}{2}vG_{5,0})\partial_v
,
\\
e_2
&
\,:=\,
(\tfrac{5}{2}xF_{5,0}+\tfrac{5}{4}yG_{5,0}+8u)\partial_x+(1+\tfrac{5}{4}xG_{5,0}+\tfrac{5}{2}yF_{5,0}+4v)\partial_y+(x+5F_{5,0}u+\tfrac{5}{4}vG_{5,0})\partial_u
+
\\
&
\ \ \ \ \
+(5F_{5,0}v+5G_{5,0}u+2y)\partial_v
,
\end{array}
\]
for any value of $F_{5,0},G_{5,0}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\!\!\!\!\!\!\!\!
\text{\bf Model 2f3n4f}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy-\tfrac{1}{2}y^4-2xy^3-3x^2y^2-2x^3y-\tfrac{1}{2}x^4+F_{5,0}y^5+5F_{5,0}xy^4+10F_{5,0}x^2y^3
+
\\
&
\ \ \ \ \
+10F_{5,0}x^3y^2+5F_{5,0}x^4y+F_{5,0}x^5+(-\tfrac{5}{2}F_{5,0}^2+2)y^6+(-15F_{5,0}^2+12)xy^5
+
\\
&
\ \ \ \ \
+(-\tfrac{75}{2}F_{5,0}^2+30)x^2y^4+(-50F_{5,0}^2+40)x^3y^3+(-\tfrac{75}{2}F_{5,0}^2+30)x^4y^2
+
\\
&
\ \ \ \ \
+(-15F_{5,0}^2+12)x^5y+(-\tfrac{5}{2}F_{5,0}^2+2)x^6+(\tfrac{50}{7}F_{5,0}^3-\tfrac{68}{7}F_{5,0})y^7+(50F_{5,0}^3
+
\\
&
\ \ \ \ \
-68F_{5,0})xy^6+(150F_{5,0}^3-204F_{5,0})x^2y^5+(250F_{5,0}^3-340F_{5,0})x^3y^4+(250F_{5,0}^3
+
\\
&
\ \ \ \ \
-340F_{5,0})x^4y^3+(150F_{5,0}^3-204F_{5,0})x^5y^2+(50F_{5,0}^3-68F_{5,0})x^6y+(\tfrac{50}{7}F_{5,0}^3
+
\\
&
\ \ \ \ \
-\tfrac{68}{7}F_{5,0})x^7
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2-y^4-4xy^3-6x^2y^2-4x^3y-x^4+2F_{5,0}y^5+10F_{5,0}xy^4
+
\\
&
\ \ \ \ \
+20F_{5,0}x^2y^3+20F_{5,0}x^3y^2
+10F_{5,0}x^4y+2F_{5,0}x^5+(-5F_{5,0}^2+4)y^6
+
\\
&
\ \ \ \ \
+(-30F_{5,0}^2+24)xy^5+(-75F_{5,0}^2+60)x^2y^4
+(-100F_{5,0}^2+80)x^3y^3
+
\\
&
\ \ \ \ \
+(-75F_{5,0}^2+60)x^4y^2
+(-30F_{5,0}^2+24)x^5y+(-5F_{5,0}^2+4)x^6
+(\tfrac{100}{7}F_{5,0}^3
+
\\
&
\ \ \ \ \
-\tfrac{136}{7}F_{5,0})y^7+(100F_{5,0}^3-136F_{5,0})xy^6+(300F_{5,0}^3
-408F_{5,0})x^2y^5+(500F_{5,0}^3
+
\\
&
\ \ \ \ \
-680F_{5,0})x^3y^4+(500F_{5,0}^3-680F_{5,0})x^4y^3+(300F_{5,0}^3
+
\\
&
\ \ \ \ \
-408F_{5,0})x^5y^2+(100F_{5,0}^3-136F_{5,0})x^6y+(\tfrac{100}{7}F_{5,0}^3-\tfrac{136}{7}F_{5,0})x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(5F_{5,0}x+4u+2v+1)\partial_x+(5F_{5,0}y+4u+2v)\partial_y+(10F_{5,0}u+y)\partial_u+(10F_{5,0}v+2x)\partial_v
,
\\
e_2
&
\,:=\,
(5F_{5,0}x+4u+2v)\partial_x+(5F_{5,0}y+4u+2v+1)\partial_y+(10F_{5,0}u+x)\partial_u+(10F_{5,0}v+2y)\partial_v
,
\\
e_3
&
\,:=\,
-(x-y)\partial_x+(x-y)\partial_y-(2u-v)\partial_u+(4u-2v)\partial_v
.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & 5F_{5,0}e_1-5F_{5,0}e_2 & -e_1+e_2
\\
e_2 & -5F_{5,0}e_1+5F_{5,0}e_2 & 0 & e_1-e_2
\\
e_3 & e_1-e_2 & -e_1+e_2 & 0
\end{array}
\]
for any value for $F_{5,0}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3n4g}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy-\tfrac{1}{2}y^4+2xy^3-3x^2y^2+2x^3y-\tfrac{1}{2}x^4-F_{5,0}y^5+5F_{5,0}xy^4
+
\\
&
\ \ \ \ \
-10F_{5,0}x^2y^3+10F_{5,0}x^3y^2-5F_{5,0}x^4y+F_{5,0}x^5+(-\tfrac{5}{2}F_{5,0}^2-2)y^6
+
\\
&
\ \ \ \ \
+(15F_{5,0}^2+12)xy^5+(-\tfrac{75}{2}F_{5,0}^2-30)x^2y^4+(50F_{5,0}^2+40)x^3y^3
+
\\
&
\ \ \ \ \
+(-\tfrac{75}{2}F_{5,0}^2-30)x^4y^2+(15F_{5,0}^2+12)x^5y+(-\tfrac{5}{2}F_{5,0}^2-2)x^6
+
\\
&
\ \ \ \ \
+(-\tfrac{50}{7}F_{5,0}^3-\tfrac{68}{7}F_{5,0})y^7+(50F_{5,0}^3+68F_{5,0})xy^6+(-150F_{5,0}^3
+
\\
&
\ \ \ \ \
-204F_{5,0})x^2y^5+(250F_{5,0}^3+340F_{5,0})x^3y^4+(-250F_{5,0}^3-340F_{5,0})x^4y^3
+
\\
&
\ \ \ \ \
+(150F_{5,0}^3+204F_{5,0})x^5y^2+(-50F_{5,0}^3-68F_{5,0})x^6y+(\tfrac{50}{7}F_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{68}{7}F_{5,0})x^7
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2+y^4-4xy^3+6x^2y^2-4x^3y+x^4+2F_{5,0}y^5-10F_{5,0}xy^4
+
\\
&
\ \ \ \ \
+20F_{5,0}x^2y^3
-20F_{5,0}x^3y^2+10F_{5,0}x^4y-2F_{5,0}x^5+(5F_{5,0}^2+4)y^6
+
\\
&
\ \ \ \ \
+(-30F_{5,0}^2-24)xy^5+(75F_{5,0}^2+60)x^2y^4+(-100F_{5,0}^2-80)x^3y^3
+
\\
&
\ \ \ \ \
+(75F_{5,0}^2+60)x^4y^2+(-30F_{5,0}^2-24)x^5y+(5F_{5,0}^2+4)x^6
+
\\
&
\ \ \ \ \
+(\tfrac{100}{7}F_{5,0}^3+\tfrac{136}{7}F_{5,0})y^7+(-100F_{5,0}^3
+
\\
&
\ \ \ \ \
-136F_{5,0})xy^6+(300F_{5,0}^3+408F_{5,0})x^2y^5+(-500F_{5,0}^3-680F_{5,0})x^3y^4
+
\\
&
\ \ \ \ \
v+(500F_{5,0}^3+680F_{5,0})x^4y^3+(-300F_{5,0}^3-408F_{5,0})x^5y^2+(100F_{5,0}^3
+
\\
&
\ \ \ \ \
+136F_{5,0})x^6y+(-\tfrac{100}{7}F_{5,0}^3-\tfrac{136}{7}F_{5,0})x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(5F_{5,0}x+4u-2v+1)\partial_x+(5F_{5,0}y-4u+2v)\partial_y+(10F_{5,0}u+y)\partial_u+(10F_{5,0}v+2x)\partial_v
,
\\
e_2
&
\,:=\,
-(5F_{5,0}x+4u-2v)\partial_x-(5F_{5,0}y-4u+2v-1)\partial_y-(10F_{5,0}u-x)\partial_u-(10F_{5,0}v-2y)\partial_v
, 
\\
e_3
&
\,:=\,
(x+y)\partial_x+(x+y)\partial_y+(2u+v)\partial_u+(4u+2v)\partial_v
.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & -5F_{5,0}e_1-5F_{5,0}e_2 & e_1+e_2
\\
e_2 & 5F_{5,0}e_1+5F_{5,0}e_2 & 0 & e_1+e_2
\\
e_3 & -e_1-e_2 & -e_1-e_2 & 0
\end{array}
\]
for any value for $F_{5,0}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3n4h}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+\tfrac{1}{2}y^4-2xy^3+3x^2y^2-2x^3y+\tfrac{1}{2}x^4-F_{5,0}y^5+5F_{5,0}xy^4
+
\\
&
\ \ \ \ \
-10F_{5,0}x^2y^3+10F_{5,0}x^3y^2-5F_{5,0}x^4y+F_{5,0}x^5+(\tfrac{5}{2}F_{5,0}^2-2)y^6+
\\
&
\ \ \ \ \
+(-15F_{5,0}^2+12)xy^5+(\tfrac{75}{2}F_{5,0}^2-30)x^2y^4+(-50F_{5,0}^2+40)x^3y^3
+
\\
&
\ \ \ \ \
+(\tfrac{75}{2}F_{5,0}^2-30)x^4y^2+(-15F_{5,0}^2+12)x^5y+(\tfrac{5}{2}F_{5,0}^2-2)x^6
+
\\
&
\ \ \ \ \
+(-\tfrac{50}{7}F_{5,0}^3+\tfrac{68}{7}F_{5,0})y^7+(50F_{5,0}^3-68F_{5,0})xy^6+(-150F_{5,0}^3
+
\\
&
\ \ \ \ \
+204F_{5,0})x^2y^5+(250F_{5,0}^3-340F_{5,0})x^3y^4+(-250F_{5,0}^3+340F_{5,0})x^4y^3
+
\\
&
\ \ \ \ \
+(150F_{5,0}^3-204F_{5,0})x^5y^2+(-50F_{5,0}^3+68F_{5,0})x^6y+(\tfrac{50}{7}F_{5,0}^3
+
\\
&
\ \ \ \ \
-\tfrac{68}{7}F_{5,0})x^7
+
\cdots
,
\\
v
&
\,=\,
y^2+x^2-y^4+4xy^3-6x^2y^2+4x^3y-x^4+2F_{5,0}y^5-10F_{5,0}xy^4
+
\\
&
\ \ \ \ \
+20F_{5,0}x^2y^3-20F_{5,0}x^3y^2+10F_{5,0}x^4y-2F_{5,0}x^5+(-5F_{5,0}^2+4)y^6
+
\\
&
\ \ \ \ \
+(30F_{5,0}^2-24)xy^5+(-75F_{5,0}^2+60)x^2y^4+(100F_{5,0}^2-80)x^3y^3
+
\\
&
\ \ \ \ \
+(-75F_{5,0}^2+60)x^4y^2+(30F_{5,0}^2-24)x^5y+(-5F_{5,0}^2+4)x^6
+
\\
&
\ \ \ \ \
+(\tfrac{100}{7}F_{5,0}^3-\tfrac{136}{7}F_{5,0})y^7+(-100F_{5,0}^3+136F_{5,0})xy^6+(300F_{5,0}^3
+
\\
&
\ \ \ \ \
-408F_{5,0})x^2y^5+(-500F_{5,0}^3+680F_{5,0})x^3y^4+(500F_{5,0}^3-680F_{5,0})x^4y^3
+
\\
&
\ \ \ \ \
+(-300F_{5,0}^3+408F_{5,0})x^5y^2+(100F_{5,0}^3-136F_{5,0})x^6y+(-\tfrac{100}{7}F_{5,0}^3
+
\\
&
\ \ \ \ \
+\tfrac{136}{7}F_{5,0})x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
-(5F_{5,0}x+4u-2v-1)\partial_x-(5F_{5,0}y-4u+2v)\partial_y-(10F_{5,0}u-y)\partial_u-(10F_{5,0}v-2x)\partial_v
,
\\
e_2
&
\,:=\,
(5F_{5,0}x+4u-2v)\partial_x+(5F_{5,0}y-4u+2v+1)\partial_y+(10F_{5,0}u+x)\partial_u+(10F_{5,0}v+2y)\partial_v
, 
\\
e_3
&
\,:=\,
(x+y)\partial_x+(x+y)\partial_y+(2u+v)\partial_u+(4u+2v)\partial_v
.
\end{array}
\]

\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|ccc}
{} & e_1 & e_2 & e_3
\\
\hline
e_1 & 0 & 5F_{5,0}e_1+5F_{5,0}e_2 & e_1+e_2
\\
e_2 & -5F_{5,0}e_1-5F_{5,0}e_2 & 0 & e_1+e_2
\\
e_3 & -e_1-e_2 & -e_1-e_2 & 0
\end{array}
\]
for any value for $F_{5,0}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2f3n4i}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
,
\\
v
&
\,=\,
x^2+y^2
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
y\partial_u+2x\partial_v+\partial_x
, &
e_2
\,:=\,
x\partial_u+2y\partial_v+\partial_y
, &
& 
\\
e_3
\,:=\,
2u\partial_u+2v\partial_v+x\partial_x+y\partial_y
, &
e_4
\,:=\,
v\partial_u+4u\partial_v+y\partial_x+x\partial_y
.
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccc}
{} & e_1 & e_2 & e_3 & e_4
\\
\hline
e_1 & 0 & 0 & e_1 & e_2 
\\
e_2 & 0 & 0 & e_2 & e_1
\\
e_3 & -e_1 & -e_2 & 0 & 0
\\
e_4 & -e_2 & -e_1 & 0 & 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SectionHead{2g Models}
{2g-models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\!\!\!\!\!\!
\text{\bf Model 2g3a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+F_{0,3}y^3+F_{3,0}x^3+F_{0,4}y^4+F_{1,3}xy^3+F_{2,2}x^2y^2+F_{3,1}x^3y+F_{4,0}x^4
+
\cdots,
\\
v
&
\,=\,
-y^2+x^2-6F_{0,3}xy^2+(6F_{3,0}-8)x^2y+G_{0,4}y^4+G_{1,3}xy^3+G_{2,2}x^2y^2
\\
&
\ \ \ \ \
+
G_{3,1}x^3y+G_{4,0}x^4
+
\cdots,
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(1-\tfrac{9}{2}xF_{0,3}F_{3,0}+\tfrac{15}{4}vF_{3,0}F_{3,1}+\tfrac{21}{2}uF_{0,3}F_{3,1}+\tfrac{15}{4}vF_{3,0}F_{1,3}+21uF_{0,3}G_{4,0}+\tfrac{5}{4}vF_{3,0}G_{2,2}
+
\\
&
\ \ \ \ \
+228uF_{0,3}F_{3,0}+\tfrac{15}{2}vF_{3,0}G_{4,0}+\tfrac{21}{2}uF_{0,3}F_{1,3}-189uF_{0,3}F_{3,0}^2+\tfrac{7}{2}uF_{0,3}G_{2,2}-8uF_{0,3}
+
\\
&
\ \ \ \ \
-80vF_{3,0}+9xF_{0,3}+\tfrac{3}{8}xG_{1,3}-\tfrac{1}{2}xF_{2,2}-3xF_{4,0}-\tfrac{135}{2}vF_{3,0}^3+\tfrac{1}{4}yG_{2,2}+\tfrac{3}{4}yF_{1,3}+\tfrac{3}{2}yG_{4,0}
+
\\
&
\ \ \ \ \
+\tfrac{3}{8}xG_{3,1}-\tfrac{27}{2}yF_{3,0}^2+\tfrac{3}{4}yF_{3,1}+15yF_{3,0}-2uF_{2,2}-\tfrac{1}{2}uG_{1,3}+147vF_{3,0}^2-3vF_{1,3}-3vF_{3,1}
+
\\
&
\ \ \ \ \
-8vG_{4,0}-vG_{2,2})\partial_x+(\tfrac{15}{4}vF_{0,3}F_{1,3}-\tfrac{21}{2}uF_{3,0}F_{3,1}-\tfrac{9}{2}yF_{0,3}F_{3,0}-\tfrac{135}{2}vF_{0,3}F_{3,0}^2
+
\\
&
\ \ \ \ \
+\tfrac{5}{4}vF_{0,3}G_{2,2}-\tfrac{21}{2}uF_{3,0}F_{1,3}-\tfrac{7}{2}uF_{3,0}G_{2,2}-21uF_{3,0}G_{4,0}+84vF_{0,3}F_{3,0}+\tfrac{15}{2}vF_{0,3}G_{4,0}
+
\\
&
\ \ \ \ \
+\tfrac{15}{4}vF_{0,3}F_{3,1}-\tfrac{3}{4}xF_{3,1}-\tfrac{1}{4}xG_{2,2}-\tfrac{3}{2}xG_{4,0}-\tfrac{1}{2}yF_{2,2}-3yF_{4,0}+\tfrac{3}{8}yG_{1,3}+\tfrac{3}{8}yG_{3,1}
+
\\
&
\ \ \ \ \
+189uF_{3,0}^3-\tfrac{1}{2}vG_{1,3}-390uF_{3,0}^2+9uF_{1,3}+6uF_{3,1}+3uG_{2,2}+20uG_{4,0}+\tfrac{27}{2}xF_{3,0}^2
+
\\
&
\ \ \ \ \
-\tfrac{3}{4}xF_{1,3}-18xF_{3,0}+6yF_{0,3}+200uF_{3,0}-8vF_{0,3})\partial_y-(uF_{2,2}+6uF_{4,0}-\tfrac{3}{4}uG_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{3}{4}uG_{3,1}+15vF_{3,0}-\tfrac{27}{2}vF_{3,0}^2+\tfrac{3}{4}vF_{1,3}+\tfrac{3}{4}vF_{3,1}+\tfrac{1}{4}vG_{2,2}+\tfrac{3}{2}vG_{4,0}-15uF_{0,3}
+
\\
&
\ \ \ \ \
+9uF_{0,3}F_{3,0}-y)\partial_u-(-18vF_{0,3}+vF_{2,2}+6vF_{4,0}-\tfrac{3}{4}vG_{1,3}-\tfrac{3}{4}vG_{3,1}+16u+54uF_{3,0}^2
+
\\
&
\ \ \ \ \
-3uF_{1,3}-78uF_{3,0}-3uF_{3,1}-uG_{2,2}-6uG_{4,0}+9vF_{0,3}F_{3,0}-2x)\partial_v 
, 
\\
e_2
&
\,:=\,
(-3yF_{0,3}-2vF_{2,2}-\tfrac{3}{4}xF_{3,1}+\tfrac{1}{4}xG_{2,2}+\tfrac{1}{2}yF_{2,2}+\tfrac{3}{8}yG_{1,3}+\tfrac{3}{8}yG_{3,1}-\tfrac{3}{2}vG_{1,3}-3uF_{1,3}
+
\\
&
\ \ \ \ \
+63uF_{3,0}F_{0,3}^2+\tfrac{15}{8}vF_{3,0}G_{3,1}+42uF_{0,3}F_{0,4}+\tfrac{21}{4}uF_{0,3}G_{1,3}+\tfrac{5}{2}vF_{3,0}F_{2,2}+15vF_{3,0}F_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{45}{2}vF_{0,3}F_{3,0}^2+\tfrac{15}{8}vF_{3,0}G_{1,3}+7uF_{0,3}F_{2,2}+\tfrac{21}{4}uF_{0,3}G_{3,1}+\tfrac{9}{2}yF_{0,3}F_{3,0}-27vF_{0,3}F_{3,0}
+
\\
&
\ \ \ \ \
-4x-\tfrac{3}{4}xF_{1,3}+3xF_{3,0}-2vG_{3,1}+3yF_{0,4}+\tfrac{27}{2}xF_{0,3}^2+\tfrac{3}{2}xG_{0,4}-2uG_{0,4}-12vF_{0,4}
+
\\
&
\ \ \ \ \
-18uF_{0,3}^2)\partial_x
+
(1+15vF_{0,3}F_{0,4}-42uF_{3,0}F_{0,4}-7uF_{3,0}F_{2,2}+\tfrac{15}{8}vF_{0,3}G_{3,1}+\tfrac{45}{2}vF_{3,0}F_{0,3}^2
+
\\
&
\ \ \ \ \
+\tfrac{5}{2}vF_{0,3}F_{2,2}+\tfrac{15}{8}vF_{0,3}G_{1,3}-63uF_{0,3}F_{3,0}^2-\tfrac{21}{4}uF_{3,0}G_{3,1}-\tfrac{21}{4}uF_{3,0}G_{1,3}+72uF_{0,3}F_{3,0}
+
\\
&
\ \ \ \ \
-\tfrac{9}{2}xF_{0,3}F_{3,0}-2vG_{0,4}+\tfrac{27}{2}yF_{0,3}^2+36uF_{0,4}-3xF_{0,4}-8y-\tfrac{3}{8}xG_{1,3}-\tfrac{1}{2}xF_{2,2}+\tfrac{1}{4}yG_{2,2}
+
\\
&
\ \ \ \ \
-\tfrac{3}{4}yF_{1,3}-\tfrac{3}{8}xG_{3,1}-\tfrac{3}{4}yF_{3,1}+6yF_{3,0}+4uF_{2,2}+\tfrac{9}{2}uG_{1,3}+5uG_{3,1}+\tfrac{3}{2}yG_{0,4}-18vF_{0,3}^2)\partial_y
+
\\
&
\ \ \ \ \
+
(-12u+9uF_{3,0}-\tfrac{3}{2}uF_{3,1}+3uG_{0,4}+\tfrac{1}{2}uG_{2,2}-3vF_{0,4}-\tfrac{1}{2}vF_{2,2}-\tfrac{3}{8}vG_{1,3}-\tfrac{3}{8}vG_{3,1}
+
\\
&
\ \ \ \ \
+27uF_{0,3}^2-\tfrac{3}{2}uF_{1,3}-\tfrac{9}{2}vF_{0,3}F_{3,0}+x)\partial_u
+
(27vF_{0,3}^2-\tfrac{3}{2}vF_{1,3}-\tfrac{3}{2}vF_{3,1}+3vG_{0,4}+\tfrac{1}{2}vG_{2,2}
+
\\
&
\ \ \ \ \
-16v+12uF_{0,4}+2uF_{2,2}+\tfrac{3}{2}uG_{1,3}+\tfrac{3}{2}uG_{3,1}-18uF_{0,3}+12vF_{3,0}+18uF_{0,3}F_{3,0}-2y)\partial_v.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
A Gr\"obner basis has 433 generators to describe the
moduli space core algebraic variety in 
$\R^{12} \ni F_{0,3},F_{0,4},F_{1,3},F_{2,2},F_{3,0},F_{3,1},F_{4,0},G_{0,4},G_{1,3},G_{2,2},G_{3,1},G_{4,0}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 
&
\rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(-4+\tfrac{27}{2}F_{3,0}^2+\tfrac{27}{2}F_{0,3}^2-12F_{3,0}-\tfrac{3}{2}F_{1,3}-\tfrac{3}{2}F_{3,1}+\tfrac{3}{2}G_{0,4}-\tfrac{3}{2}G_{4,0})e_1+(-6F_{0,3}+3F_{4,0}-\tfrac{3}{4}G_{1,3}-\tfrac{3}{4}G_{3,1}-3F_{0,4})e_2$
\end{tabular}}
\\
e_2 & \rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(-4+\tfrac{27}{2}F_{3,0}^2+\tfrac{27}{2}F_{0,3}^2-12F_{3,0}-\tfrac{3}{2}F_{1,3}-\tfrac{3}{2}F_{3,1}+\tfrac{3}{2}G_{0,4}-\tfrac{3}{2}G_{4,0})e_1-(-6F_{0,3}+3F_{4,0}-\tfrac{3}{4}G_{1,3}-\tfrac{3}{4}G_{3,1}-3F_{0,4})e_2$
\end{tabular}}
& 0
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2g3b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy+x^3+F_{0,4}y^4+F_{1,3}xy^3+F_{2,2}x^2y^2+(-F_{1,3}-G_{4,0}+9+G_{0,4})x^3y
+
\\
&
\ \ \ \ \
+(-\tfrac{1}{3}F_{2,2}-F_{0,4})x^4+(-\tfrac{1}{50}F_{1,3}G_{3,1}-\tfrac{14}{25}F_{0,4}F_{1,3}+\tfrac{3}{5}F_{0,4}-\tfrac{14}{25}F_{0,4}G_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{2}{5}F_{0,4}G_{4,0}-\tfrac{1}{50}G_{0,4}G_{3,1})y^5+(\tfrac{18}{5}F_{1,3}-\tfrac{1}{5}F_{1,3}^2-\tfrac{2}{5}F_{1,3}G_{4,0}-\tfrac{4}{3}F_{0,4}F_{2,2}
+
\\
&
\ \ \ \ \
+F_{0,4}G_{3,1}+\tfrac{18}{5}G_{0,4}-\tfrac{1}{5}G_{0,4}F_{1,3}-\tfrac{2}{5}G_{0,4}G_{4,0})xy^4+(\tfrac{6}{5}F_{2,2}-\tfrac{9}{5}G_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{78}{5}F_{0,4}-\tfrac{2}{15}F_{2,2}G_{4,0}+\tfrac{1}{5}G_{4,0}G_{3,1}+\tfrac{3}{5}F_{1,3}G_{3,1}-\tfrac{11}{15}F_{2,2}F_{1,3}+\tfrac{6}{5}F_{0,4}F_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{12}{5}F_{0,4}G_{4,0})x^2y^3+(\tfrac{324}{5}-\tfrac{44}{5}F_{1,3}-\tfrac{72}{5}G_{4,0}-\tfrac{4}{9}F_{2,2}^2+\tfrac{1}{3}F_{2,2}G_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{6}{5}F_{1,3}G_{4,0}+\tfrac{2}{5}F_{1,3}^2+\tfrac{4}{5}G_{4,0}^2)x^3y^2+(-\tfrac{25}{6}F_{2,2}+\tfrac{19}{10}G_{3,1}-\tfrac{68}{5}F_{0,4}
+
\\
&
\ \ \ \ \
+\tfrac{2}{3}F_{2,2}G_{4,0}-\tfrac{7}{20}G_{4,0}G_{3,1}-\tfrac{3}{10}F_{1,3}G_{3,1}+\tfrac{1}{2}F_{2,2}F_{1,3}+\tfrac{1}{5}F_{0,4}F_{1,3}
+
\\
&
\ \ \ \ \
+\tfrac{2}{5}F_{0,4}G_{4,0}-\tfrac{1}{3}F_{2,2}G_{0,4}+\tfrac{1}{4}G_{0,4}G_{3,1})x^4y+(\tfrac{-54}{25}-\tfrac{4}{25}F_{1,3}+\tfrac{42}{25}G_{4,0}
+
\\
&
\ \ \ \ \
+\tfrac{12}{25}G_{0,4}+\tfrac{4}{45}F_{2,2}^2-\tfrac{1}{15}F_{2,2}G_{3,1}+\tfrac{4}{15}F_{0,4}F_{2,2}-\tfrac{1}{5}F_{0,4}G_{3,1}-\tfrac{4}{25}F_{1,3}G_{4,0}
+
\\
&
\ \ \ \ \
+\tfrac{1}{25}G_{0,4}F_{1,3}+\tfrac{2}{25}G_{0,4}G_{4,0}-\tfrac{1}{25}F_{1,3}^2-\tfrac{4}{25}G_{4,0}^2)x^5
+
\cdots
,
\\
v
&
\,=\,
-y^2+x^2+6x^2y+G_{0,4}y^4+(-8F_{0,4}-\tfrac{4}{3}F_{2,2}-G_{3,1})xy^3+(-3G_{4,0}+27
+
\\
&
\ \ \ \ \
-3G_{0,4})x^2y^2+G_{3,1}x^3y+G_{4,0}x^4+(\tfrac{6}{5}G_{0,4}-\tfrac{2}{5}G_{0,4}G_{4,0}+\tfrac{2}{5}F_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{2}{75}F_{2,2}G_{3,1}+\tfrac{16}{75}F_{0,4}F_{2,2}-\tfrac{2}{5}G_{0,4}F_{1,3}+\tfrac{1}{50}G_{3,1}^2+\tfrac{48}{25}F_{0,4}^2-\tfrac{2}{5}G_{0,4}^2)y^5
+
\\
&
\ \ \ \ \
+(-\tfrac{24}{5}F_{2,2}-\tfrac{18}{5}G_{3,1}-\tfrac{126}{5}F_{0,4}+\tfrac{8}{15}F_{2,2}G_{4,0}+\tfrac{2}{5}G_{4,0}G_{3,1}+\tfrac{1}{5}F_{1,3}G_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{4}{15}F_{2,2}F_{1,3}+\tfrac{12}{5}F_{0,4}F_{1,3}+\tfrac{24}{5}F_{0,4}G_{4,0}-\tfrac{4}{3}F_{2,2}G_{0,4}+G_{0,4}G_{3,1})xy^4
+
\\
&
\ \ \ \ \
+(\tfrac{486}{5}+\tfrac{12}{5}F_{1,3}-\tfrac{108}{5}G_{4,0}-12G_{0,4}+\tfrac{8}{9}F_{2,2}^2+\tfrac{16}{3}F_{0,4}F_{2,2}-4F_{0,4}G_{3,1}
+
\\
&
\ \ \ \ \
+\tfrac{7}{5}F_{1,3}G_{4,0}+G_{0,4}F_{1,3}+2G_{0,4}G_{4,0}+\tfrac{2}{5}F_{1,3}^2+\tfrac{6}{5}G_{4,0}^2-\tfrac{1}{2}G_{3,1}^2)x^2y^3
+
\\
&
\ \ \ \ \
+(-\tfrac{2}{3}F_{2,2}+\tfrac{71}{5}G_{3,1}+\tfrac{64}{5}F_{0,4}+\tfrac{4}{3}F_{2,2}G_{4,0}-\tfrac{9}{5}G_{4,0}G_{3,1}-\tfrac{2}{5}F_{1,3}G_{3,1}
+
\\
&
\ \ \ \ \
-\tfrac{8}{5}F_{0,4}F_{1,3}-\tfrac{16}{5}F_{0,4}G_{4,0}+\tfrac{4}{3}F_{2,2}G_{0,4}-G_{0,4}G_{3,1})x^3y^2+(\tfrac{-27}{5}
+
\\
&
\ \ \ \ \
-\tfrac{13}{5}F_{1,3}+\tfrac{66}{5}G_{4,0}+\tfrac{24}{5}G_{0,4}-\tfrac{1}{3}F_{2,2}G_{3,1}-\tfrac{11}{10}F_{1,3}G_{4,0}-\tfrac{1}{10}G_{0,4}F_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{1}{5}G_{0,4}G_{4,0}-\tfrac{1}{5}F_{1,3}^2-\tfrac{7}{5}G_{4,0}^2+\tfrac{1}{4}G_{3,1}^2)x^4y+(-\tfrac{38}{75}F_{2,2}-\tfrac{23}{25}G_{3,1}-\tfrac{178}{25}F_{0,4}
+
\\
&
\ \ \ \ \
-\tfrac{28}{75}F_{2,2}G_{4,0}+\tfrac{7}{25}G_{4,0}G_{3,1}+\tfrac{1}{25}F_{1,3}G_{3,1}-\tfrac{4}{75}F_{2,2}F_{1,3}-\tfrac{4}{25}F_{0,4}F_{1,3}
+
\\
&
\ \ \ \ \
-\tfrac{8}{25}F_{0,4}G_{4,0})x^5
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(1+\tfrac{2}{3}xF_{2,2}-\tfrac{1}{2}xG_{3,1}-\tfrac{18}{5}y+\tfrac{1}{5}yF_{1,3}+\tfrac{2}{5}yG_{4,0}-\tfrac{4}{3}uF_{2,2}+4uF_{0,4}+\tfrac{1}{2}uG_{3,1}+vF_{1,3})\partial_x
+
\\
&
\ \ \ \ \
+(-\tfrac{1}{5}xF_{1,3}-\tfrac{2}{5}xG_{4,0}+\tfrac{3}{5}x+\tfrac{2}{3}yF_{2,2}-\tfrac{1}{2}yG_{3,1}+\tfrac{1}{5}uF_{1,3}-\tfrac{3}{5}uG_{4,0}+\tfrac{27}{5}u-3uG_{0,4}
+
\\
&
\ \ \ \ \
+4vF_{0,4}+\tfrac{2}{3}vF_{2,2}+\tfrac{1}{2}vG_{3,1})\partial_y-(-y-\tfrac{4}{3}uF_{2,2}+uG_{3,1}-\tfrac{18}{5}v+\tfrac{1}{5}vF_{1,3}+\tfrac{2}{5}vG_{4,0})\partial_u
+
\\
&
\ \ \ \ \
+(2x+\tfrac{18}{5}u+\tfrac{4}{5}uF_{1,3}+\tfrac{8}{5}uG_{4,0}+\tfrac{4}{3}vF_{2,2}-vG_{3,1})\partial_v
,
\\
e_2
&
\,:=\,
(xF_{1,3}+xG_{0,4}+xG_{4,0}-6x+\tfrac{1}{10}yG_{3,1}+\tfrac{4}{5}yF_{0,4}-2uG_{0,4}-3uF_{1,3}+4vF_{0,4})\partial_x
+
\\
&
\ \ \ \ \
-(-1+\tfrac{1}{10}xG_{3,1}+\tfrac{4}{5}xF_{0,4}+3y-yF_{1,3}-yG_{0,4}-yG_{4,0}+\tfrac{9}{10}uG_{3,1}+\tfrac{56}{5}uF_{0,4}+2uF_{2,2}
+
\\
&
\ \ \ \ \
+2vG_{0,4})\partial_y-(-x-2uF_{1,3}-2uG_{0,4}-2uG_{4,0}+9u+\tfrac{1}{10}vG_{3,1}+\tfrac{4}{5}vF_{0,4})\partial_u+(-2y
+
\\
&
\ \ \ \ \
+\tfrac{2}{5}uG_{3,1}+\tfrac{16}{5}uF_{0,4}-6v+2vF_{1,3}+2vG_{0,4}+2vG_{4,0})\partial_v.
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Gr\"obner basis generators of 
moduli space core algebraic variety in 
$\R^6 \ni F_{0,4},F_{1,3},F_{2,2},G_{0,4},G_{3,1},G_{4,0}$:
\[
\aligned
\B_1 & := 288F_{0,4}G_{4,0}+27F_{1,3}G_{3,1}+120F_{2,2}G_{4,0}+45G_{0,4}G_{3,1}-45G_{3,1}G_{4,0}-1212F_{0,4}-590F_{2,2}
+
\\
&
\ \ \ \ \
+120G_{3,1}; 
\\
\B_2 & := 1656F_{0,4}G_{3,1}+216F_{1,3}G_{4,0}+240F_{2,2}G_{3,1}+2160G_{0,4}G_{4,0}+177G_{3,1}^2+672G_{4,0}^2-2144F_{1,3}
+
\\
&
\ \ \ \ \
-13960G_{0,4}-7536G_{4,0}+13392; 
\\
\B_3 & := -1224F_{1,3}G_{4,0}+204F_{2,2}G_{3,1}+828G_{0,4}^2-2304G_{0,4}G_{4,0}-129G_{3,1}^2-588G_{4,0}^2+8776F_{1,3}
+
\\
&
\ \ \ \ \
+10076G_{0,4}+4524G_{4,0}+6912; 
\\
\B_4 & := -576F_{0,4}G_{4,0}+108F_{2,2}G_{0,4}-204F_{2,2}G_{4,0}-117G_{0,4}G_{3,1}+117G_{3,1}G_{4,0}+3684F_{0,4}
+
\\
&
\ \ \ \ \
+1186F_{2,2}-303G_{3,1};
\\
\B_5 & := 1242F_{1,3}G_{0,4}-882F_{1,3}G_{4,0}-60F_{2,2}G_{3,1}-2196G_{0,4}G_{4,0}-165G_{3,1}^2-444G_{4,0}^2+6148F_{1,3}
+
\\
&
\ \ \ \ \
+15404G_{0,4}+4092G_{4,0}-864;
\\
\B_6 & := 648F_{0,4}G_{0,4}+792F_{0,4}G_{4,0}+240F_{2,2}G_{4,0}+171G_{0,4}G_{3,1}-171G_{3,1}G_{4,0}-5808F_{0,4}
+
\\
&
\ \ \ \ \
-1480F_{2,2}+474G_{3,1};
\\
\B_7 & := 2466F_{1,3}G_{4,0}+276F_{2,2}^2-825F_{2,2}G_{3,1}+2718G_{0,4}G_{4,0}+474G_{3,1}^2+2382G_{4,0}^2-20759F_{1,3}
+
\\
&
\ \ \ \ \
-11617G_{0,4}-17841G_{4,0}-32373;
\\
\B_8 & := 504F_{0,4}G_{4,0}+18F_{1,3}F_{2,2}+156F_{2,2}G_{4,0}+45G_{0,4}G_{3,1}-72G_{3,1}G_{4,0}-2436F_{0,4}-674F_{2,2}
+
\\
&
\ \ \ \ \
+273G_{3,1}; 
\\
\B_9 & := 1104F_{0,4}F_{2,2}-3852F_{1,3}G_{4,0}+918F_{2,2}G_{3,1}-5400G_{0,4}G_{4,0}-615G_{3,1}^2-2784G_{4,0}^2
+
\\
&
\ \ \ \ \
+29878F_{1,3}+29150G_{0,4}+21462G_{4,0}+32346;
\\
\B_{10} & := 621F_{1,3}^2-2016F_{1,3}G_{4,0}+750F_{2,2}G_{3,1}-3600G_{0,4}G_{4,0}-525G_{3,1}^2-2316G_{4,0}^2+23269F_{1,3}
+
\\
&
\ \ \ \ \
+19280G_{0,4}+17988G_{4,0}+25704;
\\
\B_{11} & := 324F_{0,4}F_{1,3}-1584F_{0,4}G_{4,0}-480F_{2,2}G_{4,0}-180G_{0,4}G_{3,1}+261G_{3,1}G_{4,0}+8916F_{0,4}
+
\\
&
\ \ \ \ \
+2330F_{2,2}-894G_{3,1};
\\
\B_{12} & := 39744F_{0,4}^2+49104F_{1,3}G_{4,0}-9840F_{2,2}G_{3,1}+77040G_{0,4}G_{4,0}+7509G_{3,1}^2+33168G_{4,0}^2
+
\\
&
\ \ \ \ \
-372556F_{1,3}-438260G_{0,4}-263724G_{4,0}-313092; \\
\B_{13} & := -1944F_{1,3}G_{4,0}^2+324F_{2,2}G_{3,1}G_{4,0}-4536G_{0,4}G_{4,0}^2-351G_{3,1}^2G_{4,0}-1080G_{4,0}^3
+
\\
&
\ \ \ \ \
+27072F_{1,3}G_{4,0}-1986F_{2,2}G_{3,1}+53118G_{0,4}G_{4,0}+2094G_{3,1}^2+16530G_{4,0}^2-94388F_{1,3}
+
\\
&
\ \ \ \ \
-150154G_{0,4}-57450G_{4,0}-34560;
\\
\B_{14} & := 25920F_{0,4}G_{4,0}^2+4320F_{2,2}G_{4,0}^2+4860G_{0,4}G_{3,1}G_{4,0}+135G_{3,1}^3-2700G_{3,1}G_{4,0}^2
+
\\
&
\ \ \ \ \
-382320F_{0,4}G_{4,0}-70584F_{2,2}G_{4,0}-47376G_{0,4}G_{3,1}+49284G_{3,1}G_{4,0}+1298040F_{0,4}
+
\\
&
\ \ \ \ \
+251516F_{2,2}-146766G_{3,1};
\\
\B_{15} & := 6210G_{0,4}G_{3,1}^2-298080G_{0,4}G_{4,0}^2-22770G_{3,1}^2G_{4,0}+33120G_{4,0}^3-440376F_{1,3}G_{4,0}
+
\\
&
\ \ \ \ \
+141108F_{2,2}G_{3,1}+3240888G_{0,4}G_{4,0}+56847G_{3,1}^2-326472G_{4,0}^2+2925104F_{1,3}
+
\\
&
\ \ \ \ \
-8290352G_{0,4}-1614984G_{4,0}+16834608;
\\
\B_{16} & := 110160F_{0,4}G_{4,0}^2+405F_{2,2}G_{3,1}^2+24840F_{2,2}G_{4,0}^2+14175G_{0,4}G_{3,1}G_{4,0}-14175G_{3,1}G_{4,0}^2
+
\\
&
\ \ \ \ \
-1539900F_{0,4}G_{4,0}-364398F_{2,2}G_{4,0}-151317G_{0,4}G_{3,1}+213498G_{3,1}G_{4,0}
+
\\
&
\ \ \ \ \
+4969920F_{0,4}+1216192F_{2,2}-542742G_{3,1};
\\
\endaligned
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & \rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$(-\tfrac{12}{5}+\tfrac{4}{5}F_{1,3}+G_{0,4}+\tfrac{3}{5}G_{4,0})e_1+(-\tfrac{2}{3}F_{2,2}+\tfrac{2}{5}G_{3,1}-\tfrac{4}{5}F_{0,4})e_2$
\end{tabular}}
\\
e_2 & \rotatebox[origin=c]{0}{
\begin{tabular}{p{7cm}}
$-(-\tfrac{12}{5}+\tfrac{4}{5}F_{1,3}+G_{0,4}+\tfrac{3}{5}G_{4,0})e_1-(-\tfrac{2}{3}F_{2,2}+\tfrac{2}{5}G_{3,1}-\tfrac{4}{5}F_{0,4})e_2$
\end{tabular}} & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2g3c4a}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy-\tfrac{1}{6}y^4+x^2y^2-\tfrac{1}{6}x^4+F_{0,5}y^5-\tfrac{5}{2}G_{0,5}xy^4-10F_{0,5}x^2y^3+5G_{0,5}x^3y^2
+
\\
&
\ \ \ \ \
+5F_{0,5}x^4y-\tfrac{1}{2}G_{0,5}x^5+(\tfrac{15}{8}G_{0,5}^2-\tfrac{15}{2}F_{0,5}^2)y^6+(\tfrac{-2}{3}+45G_{0,5}F_{0,5})xy^5
+
\\
&
\ \ \ \ \
+(-\tfrac{225}{8}G_{0,5}^2+\tfrac{225}{2}F_{0,5}^2)x^2y^4+(\tfrac{20}{9}-150G_{0,5}F_{0,5})x^3y^3+(\tfrac{225}{8}G_{0,5}^2
+
\\
&
\ \ \ \ \
-\tfrac{225}{2}F_{0,5}^2)x^4y^2+(\tfrac{-2}{3}+45G_{0,5}F_{0,5})x^5y+(-\tfrac{15}{8}G_{0,5}^2+\tfrac{15}{2}F_{0,5}^2)x^6
+
\\
&
\ \ \ \ \
+(\tfrac{450}{7}F_{0,5}^3-\tfrac{675}{14}G_{0,5}^2F_{0,5}+\tfrac{17}{21}G_{0,5})y^7+(\tfrac{225}{4}G_{0,5}^3-675F_{0,5}^2G_{0,5}
+
\\
&
\ \ \ \ \
+\tfrac{34}{3}F_{0,5})xy^6+(-1350F_{0,5}^3+\tfrac{2025}{2}G_{0,5}^2F_{0,5}-17G_{0,5})x^2y^5+(-\tfrac{170}{3}F_{0,5}
+
\\
&
\ \ \ \ \
-\tfrac{1125}{4}G_{0,5}^3+3375F_{0,5}^2G_{0,5})x^3y^4+(\tfrac{85}{3}G_{0,5}-\tfrac{3375}{2}G_{0,5}^2F_{0,5}+2250F_{0,5}^3)x^4y^3
+
\\
&
\ \ \ \ \
+(34F_{0,5}+\tfrac{675}{4}G_{0,5}^3-2025F_{0,5}^2G_{0,5})x^5y^2+(-450F_{0,5}^3+\tfrac{675}{2}G_{0,5}^2F_{0,5}
+
\\
&
\ \ \ \ \
-\tfrac{17}{3}G_{0,5})x^6y+(-\tfrac{225}{28}G_{0,5}^3+\tfrac{675}{7}F_{0,5}^2G_{0,5}-\tfrac{34}{21}F_{0,5})x^7
+
\cdots
,
\\
v
&
\,=\,
-y^2+x^2-\tfrac{4}{3}xy^3+\tfrac{4}{3}x^3y+G_{0,5}y^5+10F_{0,5}xy^4-10G_{0,5}x^2y^3
+
\\
&
\ \ \ \ \
-20F_{0,5}x^3y^2+5G_{0,5}x^4y+2F_{0,5}x^5+(\tfrac{2}{9}-15G_{0,5}F_{0,5})y^6+(\tfrac{45}{2}G_{0,5}^2
+
\\
&
\ \ \ \ \
-90F_{0,5}^2)xy^5+(\tfrac{-10}{3}+225G_{0,5}F_{0,5})x^2y^4+(300F_{0,5}^2-75G_{0,5}^2)x^3y^3
+
\\
&
\ \ \ \ \
+(\tfrac{10}{3}-225G_{0,5}F_{0,5})x^4y^2+(\tfrac{45}{2}G_{0,5}^2-90F_{0,5}^2)x^5y+(\tfrac{-2}{9}+15G_{0,5}F_{0,5})x^6
+
\\
&
\ \ \ \ \
+(\tfrac{1350}{7}F_{0,5}^2G_{0,5}-\tfrac{225}{14}G_{0,5}^3-\tfrac{68}{21}F_{0,5})y^7+(\tfrac{34}{3}G_{0,5}-675G_{0,5}^2F_{0,5}
+
\\
&
\ \ \ \ \
+900F_{0,5}^3)xy^6+(-4050F_{0,5}^2G_{0,5}+\tfrac{675}{2}G_{0,5}^3+68F_{0,5})x^2y^5+(-4500F_{0,5}^3
+
\\
&
\ \ \ \ \
+3375G_{0,5}^2F_{0,5}-\tfrac{170}{3}G_{0,5})x^3y^4+(-\tfrac{340}{3}F_{0,5}+6750F_{0,5}^2G_{0,5}
+
\\
&
\ \ \ \ \
-\tfrac{1125}{2}G_{0,5}^3)x^4y^3+(2700F_{0,5}^3-2025G_{0,5}^2F_{0,5}+34G_{0,5})x^5y^2
+
\\
&
\ \ \ \ \
+(-1350F_{0,5}^2G_{0,5}+\tfrac{225}{2}G_{0,5}^3+\tfrac{68}{3}F_{0,5})x^6y+(-\tfrac{34}{21}G_{0,5}+\tfrac{675}{7}G_{0,5}^2F_{0,5}
+
\\
&
\ \ \ \ \
-\tfrac{900}{7}F_{0,5}^3)x^7
+
\cdots
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{ll}
e_1
&
\,:=\,
(1-\tfrac{15}{2}xG_{0,5}+15yF_{0,5}-\tfrac{4}{3}u)\partial_x-(15xF_{0,5}+\tfrac{15}{2}yG_{0,5}-\tfrac{2}{3}v)\partial_y+
\\
&
\ \ \ \ \
-(15F_{0,5}v+15G_{0,5}u-y)\partial_u+(60F_{0,5}u-15G_{0,5}v+2x)\partial_v
,\\
e_2
&
\,:=\,
(15xF_{0,5}+\tfrac{15}{2}yG_{0,5}-\tfrac{2}{3}v)\partial_x+(1-\tfrac{15}{2}xG_{0,5}+15yF_{0,5}-\tfrac{4}{3}u)\partial_y
+
\\
&
\ \ \ \ \
+(x+30F_{0,5}u-\tfrac{15}{2}G_{0,5}v)\partial_u+(30F_{0,5}v+30G_{0,5}u-2y)\partial_v
,
\end{array}
\]
for any value of $F_{0,5},G_{0,5}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cc}
{} & e_1 & e_2 
\\
\hline
e_1 & 0 & 0
\\
e_2 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[
\text{\bf Model 2g3c4b}
\ \ \ \ \
\left\{
\aligned
u
&
\,=\,
xy
,
\\
v
&
\,=\,
x^2-y^2
.
\endaligned\right.
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\def\arraystretch{1.25}
\begin{array}{llll}
e_1
\,:=\,
\partial_x+y\partial_u+2x\partial_v
, &
e_2
\,:=\,
\partial_y+x\partial_u-2y\partial_v
, &
& 
\\
e_3
\,:=\,
2u\partial_u+2v\partial_v+x\partial_x+y\partial_y
, &
e_4
\,:=\,
v\partial_u-4u\partial_v-y\partial_x+x\partial_y
.
\end{array}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\[
\footnotesize
\def\arraystretch{1.25}
\begin{array}{c|cccc}
{} & e_1 & e_2 & e_3 & e_4
\\
\hline
e_1 & 0 & 0 & e_1 & e_2
\\
e_2 & 0 & 0 & e_2 & e_1
\\
e_3 & -e_1 & -e_2 & 0 & 0
\\
e_4 & -e_2 & -e_1 & 0 & 0
\end{array}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\vfill\end{document}

